Differential Privacy with Multiple Selections

We consider the setting where a user with sensitive features wishes to obtain a recommendation from a server in a differentially private fashion. We propose a ``multi-selection'' architecture where the server can send back multiple recommendations and the user chooses one from these that matches best with their private features. When the user feature is one-dimensional -- on an infinite line -- and the accuracy measure is defined w.r.t some increasing function $\mathfrak{h}(.)$ of the distance on the line, we precisely characterize the optimal mechanism that satisfies differential privacy. The specification of the optimal mechanism includes both the distribution of the noise that the user adds to its private value, and the algorithm used by the server to determine the set of results to send back as a response and further show that Laplace is an optimal noise distribution. We further show that this optimal mechanism results in an error that is inversely proportional to the number of results returned when the function $\mathfrak{h}(.)$ is the identity function.

==> ashishproof.tex <==
\subsection{Optimal Ad Selection given Laplace Noise (Detailed Proof for odd $k$) }    
\label{sec-appendix:simres}
%\newcommand{\kk}{b}

\km{Does this correspond to a lemma from the main paper? If not, can we put a lemma in the main paper? Same for next section. Why is the odd case being discussed separately? Should we omit this section and only keep the next one?}

%In the last section, we know that users should report the location after adding Laplace noise. In this section, we calculate how the server respond, given a signal with Laplace noise.
We now show the optimal choice of $A$ to optimize cost function $\hat{f}(\mathbb{R},\epsilon,k)$ [in Equation \eqref{eq:hat_f_defn}] when $\mathfrak{h}(z)=z.$. To remove the assumptions in this section, please see Corollary \ref{cor:geofinal}.
%We first scale the problem so that $\epsilon = 1$. 
%For this simple case, the improvement does not depend on $\epsilon$, so we will assume that $\epsilon=1$ without loss of generality.
Specifically, we will assume that $\K=2\kk-1$ for some positive integer $\kk$.

Assuming the symmetry of $A$, let $A=\{-y_{\kk-1}, \ldots -y_1, 0, y_1, \ldots, y_{\kk-1}\}$, where $y_1,\ldots,y_{\kk-1}$ are positive numbers in increasing order. We will construct the set $y_1, \ldots, y_{\kk-1}$ inductively.%, and in the process, also obtain a bound on the expected distance of the result to the query. This analysis can be easily extended to show that this is the optimum response of the platform given that the user agent adds a Laplace noise. However, we will prove a more general result later in the paper and hence, for now, we will merely present a construction and a bound on its cost without showing that it is optimum. 
Let $x$ be a random variable drawn from Laplace distribution $\Lap$ with parameter $\epsilon$, and the goal is to minimize $D_{\kk}=\Exx{x\in \Lap}{\min_{a\in A}|x-a|}$. Since the density function of $\Lap$ satisfies $\rho_{\Lap}(x)=\rho_{\Lap}(-x)$, we have 
$$D_{\kk}=\Exx{x\sim \Lap}{\min_{a\in A}\mathfrak{h}(|x-a|) \bigg{|} x} >0,$$ 
i.e. the user has a positive private value. Under this conditioning, the variable $x$ is an exponential random variable of mean 1. In this case, the search result being used by the server will be one of $y_0, y_1$, \ldots, $y_{\kk-1}$. Clearly, $D_1 = 1$. To compute $D_{\kk+1}$, let $s = y_1$ and assume inductively (and consistent with the base case $k=1$) that $D_\kk = 1/\kk$. Then using the memorylessness property of exponential random variables, we get the recurrence
$$D_{\kk+1} = \int_{t=0}^s \min\{t, s-t\}e^{-t}dt +e^{-s}D_\kk.$$
Simplifying, we get
\begin{align*}
 D_{\kk+1} 
=& \int_{t=0}^{s/2} te^{-t}dt + s \int_{t=s/2}^{s} e^{-t}dt 
 -  \int_{t=s/2}^{s} t e^{-t}dt  +e^{-s}D_\kk\\
 =& \left(1 - (s/2) e^{-s/2} -  e^{-s/2}\right) + s \left(e^{-s/2}-e^{-s}\right) 
  - \left((s/2) e^{-s/2} +  e^{-s/2} - se^{-s} - e^{-s}\right) + e^{-s}D_\kk\\
 =& 1 - 2e^{-s/2} + e^{-s} + e^{-s}D_\kk \\
=& \left(1-e^{-s/2}\right)^2 + \left(e^{-s/2}\right)^2D_\kk
\end{align*}
Setting $\gamma = e^{-s/2}$, and minimizing by taking derivatives, we get $-2(1-\gamma) + 2\gamma D_\kk = 0$ which in turn gives 
$$\gamma = \frac{1}{D_\kk + 1} \qquad \mbox{and} \qquad D_{\kk+1} = \frac{D_\kk}{D_\kk+1}.$$ 
Plugging in the inductive hypothesis of $D_\kk = 1/\kk$, we get $D_{\kk+1} = 1/(\kk+1)$. Further, we get $s = 2\ln (1+1/\kk)$. Thus, by returning $\K=2\kk-1$ results, the expected ``cost of privacy" can be reduced by a factor of $\kk$. To obtain the actual positions $y_1, .., y_{\kk-1}$ we have to unroll the induction. For $i=1, \ldots, \kk-1$, the position  $y_i$ is given by:
$$y_i =  y_{i-1} + 2\ln (1 + 1/(\kk-i)).$$





==> costboundingproof.tex <==
\section{Proof of Theorem \ref{thm:upper-bound-relaxation}}
\label{sec:cost-boundinglemma}

\begin{theorem*}
    [Restatement of theorem \ref{thm:upper-bound-relaxation}]For any $\mathfrak{h}(.)$ satisfying property $\ref{item:first-propertyh}$, we have, $\funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)} \leq \funfnewgeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$.
\end{theorem*}

\begin{proof}

    Recall that
    \[  \funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
    \defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}\\ \Qname\in \Qrobs_{\text{unrestricted},\Signals}}} \sup_{\Dist \in \probm{U}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\left(\Disutility^{\mathfrak{h}(.)}(u,a)\right) },\]
    \[  \funfgeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
    \defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}\\ \Qname\in \Qrobs_{\text{restricted},\Signals}}} \sup_{\Dist \in \probm{\Users}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}\left(d_U(u,a)\right) }, \]
    and
    \[\Disutility^{\mathfrak{h}(.)}(u,m) := \inf\limits_{u': OPT(u')=m} \mathfrak{h}(d_U(u,u')).\]

    So we need to prove
    \begin{align*}
    & \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}\\ \Qname\in \Qrobs_{\text{unrestricted},\Signals}}} \sup_{\Dist \in \probm{U}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\left(\inf\limits_{u': OPT(u')=a} \mathfrak{h}(d_U(u,u'))\right) } \\
    \leq &
    \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}\\ \Qname\in \Qrobs_{\text{restricted},\Signals}}} \sup_{\Dist \in \probm{\Users}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}\left(d_U(u,a)\right) }
    \end{align*}

    It is sufficient to show, for any $\Signals$ and $\Pname\in \Probsgeo{\Signals}$, %and $\Dist \in \probm{U}$,
    
    \begin{align}
    & \inf_{\Qname\in \Qrobs_{\text{unrestricted},\Signals}}  \sup_{\Dist \in \probm{U}}\Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\left(\inf\limits_{u': OPT(u')=a} \mathfrak{h}(d_U(u,u'))\right) }  \nonumber \\
    \leq &
    \inf_{\Qname\in \Qrobs_{\text{restricted},\Signals}} \sup_{\Dist \in \probm{U}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}\left(d_U(u,a)\right) }  \label{sc:eq1} 
    \end{align}

    For $\Qname\in \Qrobs_{\text{restricted},\Signals}$, since $\Disutility^{\mathfrak{h}(.)}(u,m) := \inf\limits_{u': OPT(u')=m} \mathfrak{h}(d_U(u,u'))$, we have
    \begin{align}\label{sc:eq2}
     & \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}\left(d_U(u,a)\right) }   \geq  
    \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\Disutility^{\mathfrak{h}(.)}(u,\text{OPT}(a)) }.\nonumber\\
    &\hspace{-3 em}\implies \sup_{\Dist \in \probm{U}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}\left(d_U(u,a)\right) }   \geq  \sup_{\Dist \in \probm{U}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\Disutility^{\mathfrak{h}(.)}(u,\text{OPT}(a))}.
    \end{align}

    Given $\Qname\in \Qrobs_{\text{restricted},\Signals}$, we draw $A$ from $\Qname$, and let $B=[\text{OPT}(A_1), \text{OPT}(A_2), \ldots, \text{OPT}(A_k)]^T$. %If the size of $B$ is smaller than $k$, we add arbitrary elements in $M$ into $B$ so that $|B|=k$. 
    Suppose the distribution of $B$ is $\Qname'$, and we have
    \begin{align}\label{sc:eq3}
    \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}\left(d_U(u,OPT(a))\right) }
    =
    \Exxlimits{u\sim \Dist, s\sim \Pname_u, B\sim \Qname'_s}{ \min_{b\in \texttt{Set}(B)}\mathfrak{h}\left(d_U(u,b)\right) }.
    \end{align}

    Note that $\Qname' \in \Qrobs_{\text{unrestricted},\Signals}$, so combining Inequality \ref{sc:eq2} and Equality \ref{sc:eq3}, we have Equation \ref{sc:eq1}, which finishes the proof.
    

\end{proof}

==> gen-privacy-gensetup.tex <==
\subsection{An generalization of $\epsilon$-geographic differential privacy}{\label{sec:diff-privacy-gen}}

\km{Can we omit Appendix M and put that proof into this section? It's odd to have one Appendix point to another.}
\sss{Done}

Here we consider a slight generalization of $\epsilon$-geographic differential privacy and define $\mathfrak{g}(.)$-geographic differential privacy increasing convex function $\mathfrak{g}(.)$ satisfying Assumption \ref{assn:g_defn}.


\begin{assumption}{\label{assn:g_defn}}
    $\mathfrak{g}(.)$ is a convex function  satisfying $\mathfrak{g}(0)=0$ and $\mathfrak{g}(.)$ is differentiable at 0 with $\mathfrak{g}'(0)>0$
\end{assumption}

\begin{definition}[alternate definition of geo-DP]{\label{def:alt_geo_DP}}
        Let $\epsilon>0$ be a desired level of privacy and let $\mathcal{U}$ be a set of input data and $\mathcal{Y}$ be the set of all possible responses and $\Delta(\mathcal{Y})$ be the set of all probability distributions (over a sufficiently rich $\sigma$-algebra of $\mathcal{Y}$ given by $\sigma(\mathcal{Y})$). For any $\mathfrak{g}$ satisfying Assumption \ref{assn:g_defn} a mechanism $Q: u \rightarrow \Delta(\mathcal{Y})$ is $\mathfrak{g}(.)$-geographic differentially private if 

    $$ \mathbb{P}(Qu_1 \in S) \leq e^{\mathfrak{g}(|u_1-u_2|)} \mathbb{P}(Qu_2\in S)$$

    for all $S \in \sigma(\mathcal{Y})$ and $u_1,u_2 \in \mathcal{U}$.
\end{definition}

Observe that this definition captures cases where the privacy guarantees exist only when the distance between users is below some threshold. Similar to the notations setup in Section \ref{appendix-sec:formal-description}, the mechanism $\textbf{P}$ is $\mathfrak{g}(.)$-geographic differentially private iff ${P}_{u_1}(S) \leq e^{\mathfrak{g}(|u_1-u_2|)} {P}_{u_2}(S)$ for every measurable subset $S$ of $Z$ formally, $S \in \mathcal{F}_Z$ and any $\mathfrak{g}(.)$ satisfying Assumption \ref{assn:g_defn}. 






% We define a mechanism $\textbf{P}$ to be $\mathfrak{g}(.)$-geographic differentially private if ${P}_{u_1}(S) \leq e^{\mathfrak{g}(|u_1-u_2|)} {P}_{u_2}(S)$ for every measurable subset $S$ of $Z$. 
% \begin{assumption}{\label{assn:f_defn}}
%     $\mathfrak{g}(.)$ is a convex continuously increasing function thus ensuring that $\mathfrak{g}(0)=0$.
% \end{assumption}
%Note that in this part, we assume that $\mathfrak{g}(.)$ is a convex continuously increasing function thus ensuring that $\mathfrak{g}(0)=0$.

Under this notion of differential privacy, we may redefine cost function $f^{\text{alt},\mathfrak{h}(.)}(\epsilon,k)$ as follows. 

\[  \funfgeoalt{U}{\Ads}{\mathfrak{g}(.)}{\K}{\mathfrak{h}(.)}
\defeq \inf_{\Signals}\inf_{\Pname\in \Probsgeog{\Signals}} \inf_{\Qname\in \Qrobs_{ \Signals}} \sup_{u \in \real} \Exxlimits{s\sim \Pname_u}{ \Exxlimits{\vect{a} \sim \Qname_s}{ \min_{a\in \texttt{Set}(\vect{a})}\mathfrak{h}\left(|u-a|\right) }}, \]
% and for the case of local differential privacy is defined as
% \[  \funfloc{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
% \defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsloc{\Signals}\\ \Qname\in \Qrobs_{\Signals}}} \sup_{\Dist \in \probm{\Users}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\left(d_U(u,a)\right) }, \], 
where $\Probsgeog{\Signals}:=\{ \Pname | \forall u\in \real, \dsig{u}\text{~is a distribution on $\Signals$,} 
    \text{~and $\mathfrak{g}(.)$-geographic differential privacy is satisfied} \}$. 
The definition of $\Qrobs_{\Signals}$ are similar to that in Section \ref{sec:simmodel}.




% \begin{align}{\label{eqn:new_expr_f_alt}}
%     f^{\text{alt}}(U,\epsilon,k) & = \inf_{\textbf{P} \in \mathcal{P}^{\mathfrak{g}(.)}_{\mathbb{R}^k}} \underset{\mathcal{D} \in \mathbb{D}(U)}{\sup} \underset{u \sim \mathcal{D}(U);A \sim \textbf{P}_u}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h}(||u-a||_1) \right]\\
%     & = \inf_{\textbf{P} \in \mathcal{P}^{\mathfrak{g}(.)}_{\mathbb{R}^k}} \sup_{u \in \mathbb{R}} \underset{A \sim \textbf{P}_u}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h}(||u-a||_1) \right] %\label{infimization_expr}
% \end{align}

\begin{theorem} \label{thm:lap:sim-alt}
For $\mathfrak{g}(.)$-geographic differential privacy, adding Laplace noise, whose density function is $\rho(x)=\frac{\mathfrak{g}'(0)}{2} \cdot e^{- \mathfrak{g}'(0)\disrzero{x}} $, is one of the optimal choices of $\Probsgeog{\Signals}$ for users. Further, when $\mathfrak{h}(z)=z$, we have $\funfgeoalt{\real}{\Ads}{\mathfrak{g}(.)}{\K} {\mathfrak{h}(.)} = O\left(\frac{1}{\mathfrak{g}'(0) k}\right)$ and the optimal mechanism (choice of actions of users and server) itself can be computed in closed form.
\end{theorem}  


\begin{proof}
    The proof of this theorem follows identically to that of Theorem \ref{thm:lap:sim}. However, we require a slight modification of Lemma \ref{lemma:diff-privacy-condition} to prove it as stated and proven in Lemma \ref{lemma:diff-privacy-condition_gen}.
\end{proof}


\begin{lemma}{\label{lemma:diff-privacy-condition_gen}}
    Suppose, $P_u$ has a probability density function given by $g(u,.): \mathbb{R}^k \rightarrow \mathbb{R}$ for every $u \in \mathbb{R}$. Then, $P$ satisfies $\mathfrak{g}(.)$-geographic differential privacy iff $\max(|\overline{g}_u(u,\vect{x})|, |\underline{g}_u(u,\vect{x})|) \leq \mathfrak{g}'(0) g(u,\vect{x}) \text{ } \forall u \in \mathbb{R};\forall x \in \mathbb{R}^k$ \footnote{$\underline{g}_u(u,\vect{x})$, $\overline{g}_u(u,\vect{x})$ denote the lower and upper partial derivative w.r.t. $u$} whenever $\mathfrak{g}(.)$ satisfies Assumption \ref{assn:g_defn}.   
\end{lemma} 


The proof of this Lemma is very similar to that of Lemma \ref{lemma:diff-privacy-condition}.
%We prove this lemma in Section \ref{sec:diff-privacy-condition-gen-proof}.




\begin{proof}

\textbf{We first prove the only if statement.}

Assuming $\mathfrak{g}(.)$ geographic differential privacy we prove the desired constraint on $g(u,.)$. 

    Observe that since, $\{P_u\}_{u \in \mathbb{R}}$ satisfies $\mathfrak{g}(.)$ geographic-differential privacy, we must have $g(u_1, \vect{x}) \leq e^{\mathfrak{g}(|u_1-u_2|)} g(u_2, \vect{x})$.


  Thus, applying $\log$ on both sides we get, 

  \begin{align*}
      & \log g(u + \delta u, \vect{x}) - \log g(u, \vect{x}) \leq \mathfrak{g}(|\delta u|)\\
      \implies & \frac{\max(|\overline{g}_u(u,\vect{x})|, |\underline{g}_u(u,\vect{x})|)} {g(u,\vect{x})} \leq \mathfrak{g}'(0)
  \end{align*}
The last implication follows on limiting $\delta u$ towards zero and $\mathfrak{g}(0)=0$ thus, applying the lower and upper limits respectively and thus we prove the only if statement.

However, if $g(u,x) = 0$, we get the following 

\begin{align*}
      & g(u + \delta u, \vect{x}) - g(u,x)\leq 0\\
      \implies & {\max(|\overline{g}_u(u,\vect{x})|, |\underline{g}_u(u,\vect{x})|)} \leq 0
\end{align*}

The last inequality follows on applying $\delta u$ tending to 0 and applying upper and lower limits respectively.


\textbf{We now prove the if statement.}

Here assuming $\max(|\overline{g}_u(u,\vect{x})|, |\underline{g}_u(u,\vect{x})|) \leq \mathfrak{g}'(0) g(u,\vect{x})$, we prove $\mathfrak{g}(.)$-geographic differential privacy.

We first show that $g(u,\vect{x})$ is continuous in $u$. Observe that $\liminf\limits_{\delta u \to 0} g(u+\delta u) - g(u) = \lim\limits_{\delta u \to 0} \delta u\times \liminf\limits_{\delta u \to 0} \frac{ g(u+\delta u) - g(u)}{\delta u} = 0$ as $|\underline{g}_u (u,\vect{x})|= |\liminf\limits_{\delta u \to 0} \frac{ g(u+\delta u) - g(u)}{\delta u}| \leq \epsilon g(u,\vect{x})$. Similarly, using the bound on upper derivative, we show that $\limsup\limits_{\delta u \to 0} g(u+\delta u) - g(u) = 0$ and thus, we have continuity of $g(u,\vect{x})$ at $u$ for every $u \in \mathbb{R}^k$.

We first prove assuming $g(u,x) \neq 0 \forall u \in \mathbbm{R}$.
Now consider $u_1 >u_2$ for some $u_1,u_2 \in \mathbb{R}$.\\


\begin{align*}
    \log g(u_1,\vect{x}) - \log g(u_2, \vect{x}) \overset{(a)}{\leq} \int_{u = u_2}^{u_1} \frac{\overline{g}_u(u,\vect{x})}{g(u,\vect{x})} \leq & \mathfrak{g}'(0) (u_1 -u_2) \\
    & \overset{(b)}{\leq} \mathfrak{g}(u_1-u_2)
\end{align*}

The first inequality $(a)$ follows since we use an upper derivative and the inequality $(b)$ follows from the fact that $\mathfrak{g}(.)$ is a convex function and $\mathfrak{g}(0)=0$ as defined in Appendix \ref{sec:diff-privacy-gen}.

\begin{align*}
    \log g(u_1,\vect{x}) - \log g(u_2, \vect{x}) \geq \int_{u = u_2}^{u_1} \frac{\underline{g}_u(u,\vect{x})}{g(u,\vect{x})} \geq & -\mathfrak{g}'(0) (u_1 -u_2) \\
    & \overset{(c)}{\geq} - \mathfrak{g}(u_1-u_2)
\end{align*}


Inequality $(c)$ follows from the fact that $\mathfrak{g}(.)$ is a convex function. Thus, we get $g(u_1, \vect{x}) \leq e^{-\mathfrak{g}(|u_1-u_2|)} g(u_2,\vect{x})$ on taking exponent on both sides.
 
We now consider the other case that $g(u,\vect{x})=0$
for some $u \in \mathbbm{R}$. We now show that this implies $g(u,\vect{x})=0 \text{ } \forall u \in \mathbbm{R}$. Suppose not and there exists some $u_1$ s.t. $g(u_1,\vect{x})>0$ and consider the largest $u<u_1$ s.t. $g(u,\vect{x})=0$ (call it $u_0$)

Now, observe the following observe that we define the limits over extended reals i.e. $\mathbbm{R} \cup \{-\infty,\infty\}$. Observe that\\

\begin{align*}
    \lim\limits_{u \to u_1} g(u,\vect{x}) & = \lim\limits_{u \to u_0} g(u,\vect{x}) + \lim\limits_{\substack{d^l \to u_0\\d^u \to u_1}} (\log g(d^u,\vect{x}) - \log g(d^l,\vect{x}))\\
    & \leq \lim\limits_{u \to u_0} g(u,\vect{x}) + \int_{u = u_0}^{u_1} \frac{\overline{g}_u(u,\vect{x})}{g(u,\vect{x})}\\
    & {\leq} \lim\limits_{u \to u_0} g(u,\vect{x}) + \epsilon (u_1-u_0)\\
    & \overset{(a)}{=} -\infty + \epsilon(u_1-u_0) = -\infty
\end{align*}

$(a)$ follows from the fact that $g(u,\vect{x})$ is continuous in $u$ and $g(u_0,\vect{x})=0$.

Since, $g(u,\vect{x})$ is a continuous function, this implies that $g(u_1,\vect{x})=0$. Since we can make this argument for every $u_1 \in \mathbbm{R}$, we argue that $g(u,\vect{x})=0 \text{ }\forall u \in \mathbbm{R}$ and thus satisfy the condition of $\mathfrak{g}(.)$-geographic DP.





\end{proof}


==> geographic.tex <==
\section{Geographic differential privacy in $\real^{\Dim}$}

In this section, we consider the geographic differential privacy in $\real^{\Dim}$, so $\Users=\real^{\Dim}$, $\disg{x}{y}=\dis{x}{y}$, and $\defdis{u_1}{u_2}=\dis{u_1}{u_2}$.

\subsection{Optimality of symmetric mechanisms}



A little bit overloading $\C$, we define symmetric mechanism.

\begin{definition}[symmetric mechanism] \label{def:symmetric}

For $\Pname\in \Probs{\Kads}$, if for any $u\in \Users, \C\in \measure{\Kads}, c\in \rd$,
\begin{align*}
    \Pxx{u}{\C}=\Pxx{u+c}{\C+c},
\end{align*}
then we say $\Pname$ is a symmetric mechanism.

Let $\Psym$ be the set of symmetric mechanisms.

\end{definition}

In this subsection, we show it is sufficient to optimize over symmetric mechanisms. For any mechanism which has geographic differential privacy, by averaging the strategies of all the users, we get a symmetric mechanism which is as good as the original one.

\iffalse %%%%%%%%%%%

Before we show new lemmas, we define operations on sets.

\begin{definition}\label{def:setopt}

For any $A\in \Kads$, for any $v\in \rd, c\in \real$, define
\begin{align*}
A+v & \defeq \{ a+v | a\in A \}. \\
c\cdot A & \defeq \{ c\cdot a | a\in A \}.
\end{align*}

For any $\C\in \measure{\Kads}$, for any $v\in \rd, c\in \real$, define
\begin{align*}
\C+v & \defeq \{ A+v | A\in \C \}.\\
c\cdot \C & \defeq \{ c\cdot A | A\in \C \}.
\end{align*}

\end{definition}

\zhihao{already defined in notations}


\fi %%%%%%%%%%%%%%


The user set is $\rd$, so we cannot averaging the strategies of all the users, because there is not a uniform distribution over $\rd$. Instead, we average the users with a weight $\rho(x)\propto e^{-t \diszero{x}}$. If the original mechanism has $\epsilon$-geographic differential privacy, then the new symmetric one has $(\epsilon-t)$-geographic differential privacy. If $t$ goes to zero, the result is desired as long as $\funf{\Users}{\Ads}{\epsilon}{\K}$ is continuous with respect to $\epsilon$. We start with the continuity.



\begin{lemma}[corresponds to Claim \ref{cla:1}]  \label{lem:changeScale}

For any $\Users, \K$, for any $\epsilon>0$,
\begin{align}\label{limtChangeScale}
\limt{\epsilon'}{\epsilon^{-}}{ \funf{\Users}{\Ads}{\epsilon'}{\K}}  = \funf{\Users}{\Ads}{\epsilon}{\K}.
\end{align}



\end{lemma}

\begin{proof}

We first show that for any $\Users, \K$, for any $\epsilon_1,\epsilon_2>0$,
\begin{align}   \label{ineq:transeps}
    \funf{\Users}{\Ads}{\epsilon_1}{\K} \leq \frac{\epsilon_2}{\epsilon_1}\cdot  \funf{\Users}{\Ads}{\epsilon_2}{\K}.
\end{align}


  For any $\Pname\in \Probsx{\epsilon_2}{\Kads}$ and $\Dist\in \probm{\Users}$, we construct a new probability measure on $\Kads$. Let
  \begin{align*}
  \Ppxx{u}{\C}=\Pxx{\frac{\epsilon_1}{\epsilon_2}\cdot u}{\frac{\epsilon_1}{\epsilon_2}\cdot \C},
  \end{align*}
  for any $u\in \Users$ and $\C\in \measure{\Kads}$. Then for any $u_1,u_2\in \Users$, $\C\in \measure{\Kads}$
  \begin{align*}
  & \Ppxx{u_1}{\C}  \\
  =& \Pxx{\frac{\epsilon_1}{\epsilon_2}\cdot u_1}{\frac{\epsilon_1}{\epsilon_2}\cdot \C}  \\
  \leq &  e^{\epsilon_2 \cdot \dis{\frac{\epsilon_1}{\epsilon_2}\cdot u_1}{\frac{\epsilon_1}{\epsilon_2}\cdot u_2}} \Pxx{\frac{\epsilon_1}{\epsilon_2}\cdot u_2}{\frac{\epsilon_1}{\epsilon_2}\cdot \C}   \\
  = &  e^{\epsilon_1 \cdot \dis{ u_1}{u_2}} \Ppxx{u_2}{\C},
  \end{align*}
  which implies $\Ppname\in \Probsx{\epsilon_1}{\Kads}$. We also have
  \begin{align*}
  & \sup_{u\in \Users} \Exx{A\sim \Ppname_u}{ \min_{a\in A}\dis{u}{a} }   \\
  = & \sup_{u\in \Users} \Exx{A'\sim \Pname_{\frac{\epsilon_1}{\epsilon_2}u}}{ \min_{a\in \frac{\epsilon_2}{\epsilon_1}A'}\dis{u}{a} }   \\
  = & \sup_{u'\in \Users} \Exx{A'\sim \Pname_{u'}}{ \min_{a'\in A'}\dis{\frac{\epsilon_2}{\epsilon_1} u'}{\frac{\epsilon_2}{\epsilon_1}a'} }   \\
  = & \frac{\epsilon_2}{\epsilon_1}\cdot \sup_{u'\in \Users} \Exx{A'\sim \Pname_{u'}}{ \min_{a'\in A'}\dis{u'}{a'} }.
  \end{align*}

  Note that $\Pname$ is an arbitrary element in $\Probsx{\epsilon_2}{\Kads}$, so we have
  \begin{align*}
  \inf_{\Pname\in \Probsx{\epsilon_1}{\Kads}} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }
  \leq
  \frac{\epsilon_2}{\epsilon_1}\cdot \inf_{\Pname\in \Probsx{\epsilon_2}{\Kads}} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }.
  \end{align*}

  By Theorem \ref{thm:singpoint}, it is equivalent to Inequality \ref{ineq:transeps}.

  Note that we can swap the value of $\epsilon_1$ and $\epsilon_2$, so
  \begin{align*}
    \funf{\Users}{\Ads}{\epsilon_1}{\K} 
    \leq \frac{\epsilon_2}{\epsilon_1}\cdot  \funf{\Users}{\Ads}{\epsilon_2}{\K}
    \leq \frac{\epsilon_2}{\epsilon_1}\cdot \left(\frac{\epsilon_1}{\epsilon_2}\cdot  \funf{\Users}{\Ads}{\epsilon_1}{\K}\right),
  \end{align*}
  which means
  \begin{align*}
    \funf{\Users}{\Ads}{\epsilon_1}{\K} 
    = \frac{\epsilon_2}{\epsilon_1}\cdot  \funf{\Users}{\Ads}{\epsilon_2}{\K}.
  \end{align*}
  It implies this lemma.


\end{proof}




Based on this lemma of continuity, we show it is sufficient to consider symmetric mechanisms.


\begin{restatable}{theorem}{rstepb} \label{thm:symopt}

\iffalse%
\begin{align*}
\inf_{\Pname\in \Psym} \sup_{u\in \rd} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }
=
\inf_{\Pname\in \Probs{\Kads}} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }.
\end{align*}

According to Corollary \ref{lem:singpoint}, it implies
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }.
\end{align*}
\fi%


\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} },
\end{align*}
where $\Psym$ is the set of symmetric mechanisms.

\end{restatable}

%\rstepb*

\begin{proof}

For any $\epsilon'<\epsilon$ and $\Ppname\in \Probsx{\epsilon'}{\Kads}$, we define $\Pname$ as following. For any $u\in \Users$ and $\C\in \measure{\Kads}$,
\begin{align*}
    \Pxx{u}{\C}\defeq \int_{x\in \Users} \Ppxx{x}{x+\C-u} \nu(dx),
\end{align*}
where $\nu$ is a probability measure on $\Users$, with probability density
\begin{align*}
\rho_{\nu}(x) = \alpha \cdot e^{-(\epsilon-\epsilon')\|x\|_2},
\end{align*}
for any $x\in \Users$, where the constant $\alpha$ is the normalizer satisfying
\begin{align*}
\alpha = \left(\int_{x\in \Users}e^{-(\epsilon-\epsilon')\|x\|_2} dx \right)^{-1}.
\end{align*}

We first show $\Pname$ is symmetric. For any $u_1,u_2\in \Users$, $\C\in \measure{\Kads}$,
\begin{align}
& \Pxx{u_1}{\C} \\
%= & \int_{x\in \Users} \Ppxx{x}{x+\C-u_1} \nu(dx)   \\
= & \int_{x\in \Users} \Ppxx{x}{x+\C-u_1} \rho_{\nu}(x)dx   \\
\leq & e^{\epsilon' \dis{u_1}{u_2}}\cdot \int_{x\in \Users}  \Ppxx{x-u_1+u_2}{(x-u_1+u_2)+\C-u_2} \rho_{\nu}(x)dx   \\
\leq & e^{\epsilon' \dis{u_1}{u_2}}\cdot e^{(\epsilon-\epsilon') \dis{u_1}{u_2}} \cdot \int_{(x-u_1+u_2)\in \Users}  \Ppxx{x-u_1+u_2}{(x-u_1+u_2)+\C-u_2} \rho_{\nu}(x-u_1+u_2)dx   \label{ineq:intChange} \\
= & e^{\epsilon \dis{u_1}{u_2}} \cdot \int_{y\in \Users}  \Ppxx{y}{y+\C-u_2} \rho_{\nu}(y)dy  \\
\leq & e^{\epsilon \dis{u_1}{u_2}} \cdot \Pxx{u_2}{\C},  \\
\end{align}
Inequality \ref{ineq:intChange} holds since
\begin{align*}
    e^{(\epsilon-\epsilon') \dis{u_1}{u_2}}\rho_{\nu}(x-u_1+u_2)= e^{-(\epsilon-\epsilon')(\diszero{x-u_1+u_2}-\dis{u_1}{u_2})}\geq e^{-(\epsilon-\epsilon')\diszero{x}} = \rho_{\nu}(x)
\end{align*}
for any $x,u_1,u_2\in \Users$. Moreover, $\Pname_{u}$ should be normalized. For any $u\in \Users$, we have
\begin{align*}
 \Pxx{u}{\Kads}
=\int_{x\in \Users} \Ppxx{x}{\Kads} \nu(dx)
=\int_{x\in \Users} \nu(dx)
=1,
\end{align*}
so $\Pname_{u}$ is normalized, and thus $\Pname\in \Probs{\Kads}$.

%\zhihao{above, $\Pxx{u}{\Kads}$ is confusing}

Furthermore, for any $u\in \Users, \C\in \measure{\Kads}, c\in \rd$, we have
\begin{align*}
\Pxx{u+c}{\C+c}
= \int_{x\in \Users} \Ppxx{x}{x+(\C+c)-(u+c)} \nu(dx)
= \int_{x\in \Users} \Ppxx{x}{x+\C-u} \nu(dx)
=\Pxx{u}{\C},
\end{align*}
so $\Pname\in \Psym$.


We next bound the cost. For any $u\in \Users$,
\begin{align*}
& \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} } \\
=& \int_{A\in \Kads} \min_{a\in A}\dis{u}{a}\cdot  \int_{x\in \Users} \Ppxx{x}{x+dA-u} \nu(dx)   \\
=& \int_{x\in \Users} \nu(dx) \int_{A\in \Kads} \min_{a\in A}\dis{u}{a}\cdot   \Ppxx{x}{x+dA-u}    \\
=& \int_{x\in \Users} \nu(dx) \int_{A\in \Kads} \min_{a\in x+A-u}\dis{x}{a}\cdot   \Ppxx{x}{x+dA-u}    \\
=& \int_{x\in \Users} \nu(dx) \cdot \Exx{A'\sim \Ppname_{x}}{ \min_{a\in A'}\dis{x}{a} }    \\
\leq & \int_{x\in \Users} \nu(dx) \cdot \sup_{u'\in \Users} \Exx{A'\sim \Ppname_{u'}}{ \min_{a\in A'}\dis{u}{a} }    \\
= & \left( \sup_{u'\in \Users} \Exx{A'\sim \Ppname_{u'}}{ \min_{a\in A'}\dis{u}{a} } \right) \cdot \int_{x\in \Users} \nu(dx)   \\
= & \sup_{u'\in \Users} \Exx{A'\sim \Ppname_{u'}}{ \min_{a\in A'}\dis{u}{a} } ,
\end{align*}
which implies
\begin{align*}
\sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }
\leq
\sup_{u\in \Users} \Exx{A\sim \Ppname_{u}}{ \min_{a\in A}\dis{u}{a} }.
\end{align*}

Note that $\Ppname$ is an arbitrary element in $\Probsx{\epsilon'}{\Kads}$, so we have
\begin{align}\label{symAndChangeScale}
\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }
\leq
\inf_{\Ppname\in \Probsx{\epsilon'}{\Kads}} \sup_{u\in \Users} \Exx{A\sim \Ppname_{u}}{ \min_{a\in A}\dis{u}{a} }.
\end{align}

Combining Inequalities \ref{symAndChangeScale} and \ref{limtChangeScale}, we have
\begin{align}
\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }
\leq
\funf{\Users}{\Ads}{\epsilon}{\K}.
\end{align}

\iffalse%%%%%%
On the other hand, since $\Psym\subset \Probs{\Kads}$, we have
\begin{align}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname\in \Probs{\Kads}} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }
\leq
\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }.
\end{align}

\fi%%%%%%

On the other hand, we have $\funf{\Users}{\Ads}{\epsilon}{\K} \leq
\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }$, so
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }.
\end{align*}

\end{proof}

In symmetric mechanisms, all the users perform similarly. In fact, all the users have the same errors.

\begin{corollary}   \label{cor:symopt}

For any $u\in \Users$,
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
%=
%\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }
=
\inf_{\Pname\in \Psym} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }.
\end{align*}

\end{corollary}

\begin{proof}

For any $\Pname\in \Psym$, for any $u_1,u_2\in \Users$,
\begin{align*}
& \Exx{A\sim \Pname_{u_1}}{ \min_{a\in A}\dis{u_1}{a} }   \\
=& \Exx{A\sim \Pname_{u_1}}{ \min_{a\in A}\dis{u_2}{a+(u_1-u_2)} }   \\
=& \Exx{A\sim \Pname_{u_1}}{ \min_{a\in A+(u_2-u_1)}\dis{u_2}{a} }   \\
=& \Exx{A\sim \Pname_{u_2}}{ \min_{a\in A}\dis{u_2}{a} },
\end{align*}
which implies for any $\Pname\in \Psym$ and $u_0\in \Users$,
\begin{align*}
\sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\dis{u}{a} }
=
\Exx{A\sim \Pname_{u_0}}{ \min_{a\in A}\dis{u_0}{a} }.
\end{align*}

By Theorem \ref{thm:symopt}, this corollary holds.


\end{proof}


Since all the users have the same errors, we focus on a certain user, say, user 0. In this case, we write the equation in Corollary \ref{cor:symopt} in the following way.


\begin{lemma} [corresponds to Theorem \ref{thm:symopt:sim}]  \label{lem:symtor}

\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname\in \Psym} \Exx{A\sim \Pname_{\zero}}{ \min_{a\in A}\diszero{a} }
=
\inf_{\Rname \in \Rrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} },
\end{align*}
where $\zero$ is the zero vector, and
\begin{align*}
\Rrobs = \{ \Rname | \R{\cdot}\in \probm{\Kads}; \text{~and~} \forall \C\in \measure{\Kads}, \forall c\in \Ads, \R{\C}\leq e^{\epsilon\cdot \diszero{c}} \R{\C+c} \},
\end{align*}
where $\R{\C}$ means $\Prxx{A\sim \Rname}{A\in \C}$.

\end{lemma}

\begin{proof}

  The first equality follows directly from Corollary \ref{cor:symopt}.
  
  Then we show
      $ \{ \Pname_{\zero} | \Pname\in \Psym \} = \Rrobs $.
      
    For any $\Pname\in \Psym$, $\Pname_{\zero}\in \probm{\Kads}$, and for any $\C\in \measure{\Kads}, c\in \Ads$,
    \begin{align*}
        \Pname_{\zero}(\C)
        \leq e^{\epsilon\cdot \diszero{c}} \Pname_{-c}(\C)
        = e^{\epsilon\cdot \diszero{c}} \Pname_{\zero}(\C+c),
    \end{align*}
    where the last equality holds because $\Pname\in \Psym$. So we have $\{ \Pname_{\zero} | \Pname\in \Psym \} \subset \Rrobs$.
    
    For any $\Rname\in \Rrobs$, define $\Pname_{c}(\C)=\Rname(\C-c)$. Then we can verify that $\Pname\in \Psym$, so $\Rrobs \subset \{ \Pname_{\zero} | \Pname\in \Psym \}$.
    
    As a result, $ \{ \Pname_{\zero} | \Pname\in \Psym \} = \Rrobs $. Then we have
    \begin{align*}
    \inf_{\Pname\in \Psym} \Exx{A\sim \Pname_{\zero}}{ \min_{a\in A}\diszero{a} }
    =
    \inf_{\Rname \in \Rrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }.
    \end{align*}

\end{proof}



\begin{restatable}[corresponds to Theorem \ref{thm:symfinal:sim}]{theorem}{rstepc} \label{thm:symfinal}

\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} },
\end{align*}
where
\begin{align*}
\Srobs = \{ \Sname | \S{\cdot}\in \probm{\Ads}; \text{~and~} \forall x,y\in \Ads, \rho_{\Sname}(x)\leq e^{\epsilon \dis{x}{y}}\rho_{\Sname}(y) \} .
\end{align*}

%\begin{align*}
%\Srobs = \{ \Sname | \S{\cdot}\in \probm{\Ads}; \text{~and~} \forall \C\in \measure{\Ads}, \forall c\in \Ads, \S{\C}\leq e^{\epsilon\cdot \diszero{c}} \S{\C+c} \}.
%\end{align*}

\end{restatable}


%\rstepc*


\begin{proof}



%\newcommand{\rdk}{\left( \rd \right)^{\K}}

    Based on Lemma \ref{lem:symtor}, it is sufficient to show 
    \begin{align}\label{eq:symfinalsuf}
        \inf_{\Rname \in \Rrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }
        =
        \inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }.
    \end{align}
    
    It is easier to deal with probability measures on $\real^{n}$ for some $n\in \natr$, so we first convert the probability space from $\Kads$ to $\real^{n}$.
    \begin{align*}
        \inf_{\Rname \in \Rrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }
        =
        \inf_{\Rname \in \TRrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} },
    \end{align*}
    % \zhihao{need to prove the equality above?}
    
    where
    \begin{itemize}
        \item for $A=(a_1,\dots,a_{\K})\in \rdk$ where $a_1,\dots,a_{\K}\in \rd$, define
        \begin{align*}
            A+c \defeq \left\{  a_1+c, \dots, a_{\K}+c  \right\}.
        \end{align*}
        
        \item for $\C\in \measure{ \rdk }$ and $c\in \rd$, define
        \begin{align*}
            \C+c \defeq \left\{  A+c: A\in \C  \right\}.
        \end{align*}
        
        \item $
            \TRrobs \defeq \{ \Rname | \R{\cdot}\in \probm{ \rdk }; \text{~and~} \forall \C\in \measure{ \rdk }, \forall c\in \rd, \R{\C}\leq e^{\epsilon\cdot \diszero{c}} \R{\C+c} \}.
        $
    \end{itemize}
    
    

\newcommand{\rhovaname}{\rho_{V}}
\newcommand{\rhovbname}{\rho_{VB}}
\newcommand{\rhova}[1]{\rhovaname\left( #1 \right)}
\newcommand{\rhovb}[1]{\rhovaname\left( #1 \right)}
\newcommand{\Aball}[2]{\mathcal{B}_{#1,#2}}
\newcommand{\Aballsize}[2]{\left| \Aball{#1}{#2} \right|}
\newcommand{\ballsize}[1]{\left| \mathcal{B}_{#1} \right|}
    
    
    For $A=(a_1,\dots,a_{\K})\in \rdk$ where $a_1,\dots,a_{\K}\in \rd$, we can map it to $(a_1,\dots,a_{\K})\in \real^{d\times \K}$, so we can define Lebesgue measure on $\rdk$ by the corresponding Lebesgue measure on $\real^{d\times \K}$ (just to argue the integration is valid), and we define the 2-norm of $A$ to be
    \begin{align*}
        \|A\|_2 \defeq \sqrt{ \sum_{i=1}^{\K}\|a_i\|_2^2 },
    \end{align*}
    which is consistent to 2-norm on $\real^{d\times \K}$, and for $A,A'\in \rdk$ we define their distance to be $\|A-A'\|_2$.
    
    For $\eta >0$ and $A\in \rdk$, define the $\eta$-ball of $A$, denoted by $\Aball{A}{\eta}$, to be
    \begin{align*}
        \Aball{A}{\eta}\defeq \left\{ A'\in \rdk: \|A-A'\|_2<\eta \right\},
    \end{align*}
    and use $\Aballsize{A}{\eta}$ to denote the Lebesgue measure (corresponding to the volume) of $\Aball{A}{\eta}$. Note that there exists a real number, denoted by $\ballsize{\eta}\in \real$, satisfying $\Aballsize{A}{\eta}=\ballsize{\eta}$ for any $A\in \rdk$.
    
    
    Fix $\Rname \in \TRrobs$, note that $\Rname$ may not have density. We borrow the idea of \emph{mollifier} \cite{friedrichs1944identity} from the theory of partial differential equations, to construct a distribution with density which approximates $\Rname$. 
    
    Fix $\eta>0$, we define another probability measure $\Retaname \in \TRrobs$ which has density $\rhovaname(A)$ for all $A\in \rdk$.
    \begin{align*}
        \rhova{A}\defeq \frac{ \R{\Aball{A}{\eta}} }{\ballsize{\eta}}.
    \end{align*}
    
    $\rhovaname$ defines a valid probability measure because
    \begin{align*}
        \int_{\rdk} \rhova{A} dA
        =& \int_{\rdk} \frac{ \R{\Aball{A}{\eta}} }{\ballsize{\eta}} dA \\
        =& \frac{ 1 }{\ballsize{\eta}} \int_{A\in \rdk}\int_{B\in \Aball{A}{\eta}}  \R{dB}  dA \\
        =& \frac{ 1 }{\ballsize{\eta}} \int_{B\in \rdk} \R{dB} \int_{A\in \Aball{B}{\eta}}    dA \\
        =& \frac{ 1 }{\ballsize{\eta}} \int_{B\in \rdk} \R{dB} \ballsize{\eta} = 1.
    \end{align*}
    
    To show $\Retaname\in \TRrobs$, observe that for any $A\in \rdk$ and $c\in \rd$,
    \begin{align*}
        \rhovaname(A+c)  
        = \frac{ \R{\Aball{A+c}{\eta}} }{\ballsize{\eta}}    
        \leq  e^{\epsilon \diszero{c}} \frac{ \R{\Aball{A}{\eta}} }{\ballsize{\eta}}    
        \leq e^{\epsilon \diszero{c}}\rhovaname(A).
    \end{align*}
    
    It implies for any $\C\in \measure{\rdk}$ and $c\in \rd$,
    $
        \Reta{\C}
        = e^{\epsilon\cdot \diszero{c}} \Reta{\C+c},
    $
    so $\Retaname \in \TRrobs$.
    
    
    Next, we show the expected error of $\Retaname$ is close to that of $\Rname$. 
    \begin{align}
         \Exx{A\sim \Retaname}{ \min_{a\in A}\diszero{a} }
        =&
        \int_{A\in \rdk} \min_{a\in A}\diszero{a}\rhovaname(A) dA  \label{eq:costetabegin} \\
        =&
        \int_{A\in \rdk} \rhovaname(A) \min_{a\in A}\diszero{a} dA   \\
        =&
        \int_{A\in \rdk} \frac{ \R{\Aball{A}{\eta}} }{\ballsize{\eta}} \min_{a\in A}\diszero{a} dA   \\
        =&
        \frac{ 1 }{\ballsize{\eta}}  \int_{A\in \rdk}  \int_{B\in \Aball{A}{\eta}}  \R{dB}  \min_{a\in A}\diszero{a} dA   \\
        =&
        \frac{ 1 }{\ballsize{\eta}}  \int_{B\in \rdk}  \int_{A\in \Aball{B}{\eta}}    \min_{a\in A}\diszero{a} dA ~ \R{dB}  \\
        \leq&
        \frac{ 1 }{\ballsize{\eta}}  \int_{B\in \rdk}  \int_{A\in \Aball{B}{\eta}}    \left( \min_{a\in B}\diszero{a} + \eta \right) dA ~ \R{dB} \label{ineq:costaddeta} \\
        =&
          \int_{B\in \rdk}   \left( \min_{a\in B}\diszero{a} + \eta \right)  \R{dB}  \\
        =&
          \Exx{B\sim \Rname}{ \min_{a\in B}\diszero{a} }
        + \eta  \\
        =&
        \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }
        + \eta
        ,   \label{eq:costetaend}
    \end{align}
    where Inequality \ref{ineq:costaddeta} holds because for any $B\in \rdk$ and $A\in \Aball{B}{\eta}$, we have
    \begin{align*}
        \min_{a\in A}\diszero{a}
        \leq
        \min_{a\in B}\diszero{a} + \eta.
    \end{align*}
    
    We define an equivalence relation on $\rdk$. For $A,A'\in \rdk$, if $A=A'+c$ for a certain $c\in \rd$, we say they are in the same equivalence class. In each equivalence class, there exists a unique vector whose last entry is $0^{d}$, and We pick it as the representative of equivalence class. Let $G$ be the set of representatives from all equivalence classes. There is a natural bijection between $G$ and $\left(\rd\right)^{\K-1}$, which is $(a_1,a_2,\dots,a_{\K-1},0^{d})\leftrightarrow (a_1,a_2,\dots,a_{\K-1})$, so we define the Lebesgue measure on $G$ by the corresponding Lebesgue measure on $\left(\rd\right)^{\K-1}$. Then we have
    \begin{align*}
        &\Exx{A\sim \Retaname}{ \min_{a\in A}\diszero{a} }  \\
        =&
        \int_{A\in \rdk} \min_{a\in A}\diszero{a}\rhovaname(A) dA\\
        =&
        \int_{A\in G}\int_{c\in \rd} \min_{a\in A}\diszero{a-c}\rhovaname(A-c) ~dc~ dA \\
        =&
        \int_{A\in G} \left(\int_{x\in \rd}\rhovaname(A-x) dx\right)\left( \int_{c\in \rd} \min_{a\in A}\diszero{a-c}\frac{\rhovaname(A-c)}{\int_{x\in \rd}\rhovaname(A-x) dx} dc\right) dA \\
        \geq &
        \int_{A\in G} \left(\int_{x\in \rd}\rhovaname(A-x) dx\right)\left(  \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }\right) dA \\
        \geq & \inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }.
    \end{align*}
    
    Addition to Equations \ref{eq:costetabegin} to \ref{eq:costetaend}, we have
    \begin{align*}
         \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }
        \geq
        \Exx{A\sim \Retaname}{ \min_{a\in A}\diszero{a} } - \eta
        \geq
        \inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} } - \eta.
    \end{align*}
    
    Note that $\Rname$ and $\eta$ are arbitrary, so
    \begin{align}
        \inf_{\Rname \in \Rrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }
        \geq
        \inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }. \label{ineq:rsgre}
    \end{align}
    
    On the other hand, for any $A\in \Kads, \Sname \in \Srobs$, let $\Rname(\C)=\Exx{x\sim \Sname}{A-x\in \C}$ for any $\C\in \measure{\Kads}$. Then for any $\C\in \measure{\Kads}, c\in \Ads$,
    \begin{align*}
        \Rname(\C)
        =\Exx{x\sim \Sname}{A-x\in \C}
        \leq e^{\epsilon\cdot \diszero{c}}\Exx{x\sim (\Sname-c)}{A-x\in \C}
        = e^{\epsilon\cdot \diszero{c}}\Exx{x\sim \Sname}{A-x\in (\C+c)},
    \end{align*}
    which means $\Rname\in \Rrobs$, so
    \begin{align}
        \inf_{\Rname \in \Rrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }
        \leq
        \inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in (A-x)}\diszero{a} }
        =\inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }.\label{ineq:rsles}
    \end{align}
    
    Combining Inequalities \ref{ineq:rsgre} and \ref{ineq:rsles}, we have Equality \ref{eq:symfinalsuf}.
    
    
    
    


\iffalse %%%%%%%%%%%%%%%%

\zhihao{above, finished the proof. following is the previous proof}
    { \color{cyan}
    

    For any $A\in \Kads, \Sname \in \Srobs$, let $\Rname(\C)=\Exx{x\sim \Sname}{A-x\in \C}$ for any $\C\in \measure{\Kads}$. Then for any $\C\in \measure{\Kads}, c\in \Ads$,
    \begin{align*}
        \Rname(\C)
        =\Exx{x\sim \Sname}{A-x\in \C}
        \leq e^{\epsilon\cdot \diszero{c}}\Exx{x\sim (\Sname-c)}{A-x\in \C}
        = e^{\epsilon\cdot \diszero{c}}\Exx{x\sim \Sname}{A-x\in (\C+c)},
    \end{align*}
    which means $\Rname\in \Rrobs$, so
    \begin{align*}
        \inf_{\Rname \in \Rrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }
        \leq
        \inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in (A-x)}\diszero{a} }
        =\inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }.
    \end{align*}

    At the same time, we define an equivalence relation on $\Kads$. For $A,A'\in \Kads$, if $A=A'+c$ for a certain $c\in \Ads$, we say are in the same equivalence class. We can pick one representative for each equivalence class, and let $\tilde{\Kads}$ be the set of representatives from all equivalence classes, and we use $T(A)$ to denote the representative of the equivalence class that $A$ belongs to.
    
    For $\Rname\in \Rrobs$, we define a probability measure $\mu$ on $\tilde{\Kads}$, where for any $\C\in \measure{\tilde{\Kads}}$,
    \begin{align*}
        \mu(\C)\defeq \Rname(\{T(A)\in \C | A\in \Kads\}),
    \end{align*}
    and for each $\tilde{A}\in \tilde{\Kads}, \C\in\measure{\Ads}$, we define
    \begin{align*}
        \Sname_{\tilde{A}}(\C)\defeq 
        \Prxx{A\sim \Rrobs}{\exists c\in \C, \tilde{A}=A+c |T(A)\in\tilde{A}}.
    \end{align*}
    
    
    Then for any $\tilde{A}\in \tilde{\Kads}$, $\forall \C\in \measure{\Ads}, \forall c\in \Ads$,
    \begin{align*}
        \Sxx{\tilde{A}}{\C}
        \leq e^{\epsilon\cdot \diszero{c}} \Sxx{\tilde{A}}{\C+c}
    \end{align*}

    Then we have
    \begin{align*}
        \inf_{\Rname \in \Rrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }
        \geq \inf_{\mu \in \probm{\tilde{\Kads}}} \inf_{ \Sname_{\tilde{A}}\in \Srobs,~\text{for any}~\tilde{A}\in \tilde{\Kads} } \Exx{A\sim \Rname}{ \min_{a\in A}\diszero{a} }
    \end{align*}


    }
   
\fi %%%%%%%%%%%%% 
    

\end{proof}


{

\iffalse %%%%%%%

\begin{lemma}  \label{lem:densityexist}


For any $\Sname\in \Srobs$, probability density function $\rho_{\Sname}(x)$ exists for any $x\in \Ads$. Moreover, $\rho_{\Sname}(x)$ is continuous with respect to $x$.

\end{lemma}

\begin{corollary}   \label{cor:simplifysrobs}

\begin{align*}
\Srobs = \{ \Sname | \S{\cdot}\in \probm{\Ads}; \text{~and~} \forall x,y\in \Ads, \rho_{\Sname}(x)\leq e^{\epsilon \dis{x}{y}}\rho_{\Sname}(y) \} .
\end{align*}

\end{corollary}

\fi %%%%%%%

}




% \zhihao{ the proof is mixing up standard technicalities/formalism in real analysis with actual new/non-trivial ideas. From the perspective of verification, it will be helpful to separate them out.}




\subsection{Results for $\Dim=1$}

In this subsection, $\Dim=1$. That is, $\Users=\real$.

In this special case, adding Laplace noise is an optimal choice for users.




\begin{restatable}[corresponds to Theorem \ref{thm:lapopt:sim}]{theorem}{rstepd}     \label{thm:lapopt}


\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\disrzero{a-x} }
=
\inf_{A\in \Kads}  \Exx{x\sim \Lap}{ \min_{a\in A}\disrzero{a-x} },
\end{align*}
where $\Srobs$ is defined in Theorem \ref{thm:symfinal}, and $\Lap$ is the probability measure on $\Ads$ with density function
\begin{align*}
    \rho_{\Lap}(x)=e^{\epsilon \disrzero{x}}.
\end{align*}

\end{restatable}


%\rstepd*



We defer the proof for Theorem \ref{thm:lapopt} to Section \ref{sec:prooflapopt}. The rest of this subsection is a consequence of Theorem \ref{thm:lapopt}, which derives a closed form of the optimal mechanism. 

We have not argued whether an optimal mechanism exists, because it is possible that there is a sequence of mechanisms whose error goes to $\funf{\Users}{\Ads}{\epsilon}{\K}$, but none of them has error $\funf{\Users}{\Ads}{\epsilon}{\K}$. Next lemma is saying, the optimal mechanism exists.



\begin{lemma} [corresponds to Theorem \ref{thm:lap:sim}]  \label{lem:computefal}

\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\min_{A\in \Kads}  \Exx{x\sim \Lap}{ \min_{a\in A}\disrzero{a-x} },
\end{align*}
where $\Lap$ is the probability measure on $\Ads$ with density function
\begin{align*}
    \rho_{\Lap}(x)=e^{\epsilon \disrzero{x}}.
\end{align*}

\end{lemma}

\begin{proof}

    \newcommand{\diviate}{\emph{diverge}}
    \newcommand{\diviates}{\emph{diverges}}

  Let $v=(v_1,v_2,\dots,v_{\K})$ denote a vector in $\Ads^{\K}$, where $v_i\in \Ads$ (note that $\Ads=\real$ now) for $i\in [\K]$. Then we have
  \begin{align*}
      \funf{\Users}{\Ads}{\epsilon}{\K}
      =\inf_{A\in \Kads}  \Exx{x\sim \Lap}{ \min_{a\in A}\disrzero{a-x} }
      =\inf_{v\in \Ads^{\K}}  \Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{v_i-x} }
  \end{align*}
  where the first equality follows from Theorem \ref{thm:lapopt}. Then there exists a sequence $\{v^{(m)}\}_{m\in \natr}$, where $v^{(m)}\in \Ads^{\K}$ for any $m\in \natr$, so that
  \begin{align*}
      \limt{m}{+\infty}{\Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{v^{(m)}_i-x} }}
      =
      \funf{\Users}{\Ads}{\epsilon}{\K}.
  \end{align*}
  
  By Bolzano–Weierstrass theorem, there exists a sub-sequence $\{v^{(m_t)}\}_{t\in \natr}$, so that for any $i\in [\K]$,
  \begin{align*}
      \limt{t}{+\infty}{v^{(m_t)}_{i}}\in \real \cup \{\pm \infty\}.
  \end{align*}
  
  At the same time, we also have
  \begin{align*}
      \limt{t}{+\infty}{\Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{v^{(m_t)}_i-x} }}
      =
      \funf{\Users}{\Ads}{\epsilon}{\K}.
  \end{align*}
  
  For $i\in [\K]$, if $\limt{t}{+\infty}{v^{(m_t)}_{i}}\in \{\pm \infty\}$, we say $i$~\diviates.
  
  When $v=\zero$, $\Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{v_i-x} }=\Exx{x\sim \Lap}{\disrzero{x}}<\infty$, so $\funf{\Users}{\Ads}{\epsilon}{\K}<\infty$. Note that if all the elements in $[\K]$~\diviate, then $\limt{t}{+\infty}{\Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{v^{(m_t)}_i-x} }}=+\infty$, so at least one element in $[\K]$ does not~\diviate.
  
  If $j$~\diviates, for any $x\in \Ads$, there exists $t_0\in \natr$ so that for any $t>t_0$, $\min_{i\in [\K]\setminus\{j\}}\disrzero{v^{(m_t)}_i-x} = \min_{i\in [\K]}\disrzero{v^{(m_t)}_i-x}$, because at one element in $[\K]$ does not~\diviate. As a result, if we change $v^{(m_t)}_j$ to be $0$ for any $t\in \natr$, we still have $\limt{t}{+\infty}{\Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{v^{(m_t)}_i-x} }}=\funf{\Users}{\Ads}{\epsilon}{\K}$.
  
  After change $v^{(m_t)}_j$ for each $j$ that~\diviates, we have 
  \begin{align*}
      \limt{t}{+\infty}{v^{(m_t)}_{i}}\in \real,
  \end{align*}
  for any $i\in [\K]$, and we define $v^{(\infty)}_{i}\defeq \limt{t}{+\infty}{v^{(m_t)}_{i}}$. At the same time, we also have
  \begin{align*}
      \limt{t}{+\infty}{\Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{v^{(m_t)}_i-x} }}
      =
      \funf{\Users}{\Ads}{\epsilon}{\K}.
  \end{align*}
  
  Note that $\Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{v_i-x} }$ is continuous with respect to $v\in \Ads^{\K}$ (where $\Ads^{\K}=\real^{\K}$), so we have
  \begin{align*}
      \Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{v^{(\infty)}_i-x} }
      =
      \funf{\Users}{\Ads}{\epsilon}{\K},
  \end{align*}
  which implies the minimum point exists, so
  \begin{align*}
      \funf{\Users}{\Ads}{\epsilon}{\K}
        =
        \min_{A\in \Kads}  \Exx{x\sim \Lap}{ \min_{a\in A}\disrzero{a-x} },
  \end{align*}
  where the optimal $A$ is $\cup_{i\in [\K]}\{v^{(\infty)}_i\}$.

\end{proof}


%\zhihao{add some English for remaining lemmas}


\begin{lemma}   \label{lem:median}

If $\min_{A\in \Kads}  \Exx{x\sim \Lap}{ \min_{a\in A}\disrzero{a-x} }= \Exx{x\sim \Lap}{ \min_{a\in A^{*}}\disrzero{a-x} }$ and $A^{*}=\{x_1,x_2,\dots,x_{\K}\}$ where $x_1\leq x_2\leq \dots\leq x_{\K}$, we define $y_i\defeq (x_i+x_{i+1})/2$ for $i\in [\K -1]$, $y_0\defeq -\infty$, and $y_{\K}\defeq +\infty$. Then,
\begin{align} \label{eq:aveopt}
    \Prxx{z\sim \Lap}{  y_{i-1}<z<x_{i}} = \Prxx{z\sim \Lap}{  x_{i}<z<y_{i}}, \quad \forall~~i\in [\K].
\end{align}

\end{lemma}

\begin{proof}

Note that for any $i\in [\K]$, for any $z\in (y_{i-1},y_{i})$, $\min_{a\in A^{*}}\disrzero{a-x} = \disrzero{x_i-x}$. Then we have
\begin{align*}
    \Exx{x\sim \Lap}{ \min_{a\in A^{*}}\disrzero{a-x} }
    =
    \sum_{i=1}^{\K} \Prxx{z\sim \Lap}{y_{i-1}<z<y_{i}} \Exx{z\sim \Lap}{ \disrzero{x_i-z} | y_{i-1}<z<y_{i}}. 
\end{align*}
If $x_i\neq \Exx{z\sim \Lap}{ z | y_{i-1}<z<y_{i}}$ for a certain $i\in [\K]$, we can change the value of $x_i$ so that Equation \ref{eq:aveopt} holds, in which $x_i$ is somehow a median of $\Lap$ inside the interval $(y_{i-1},y_i)$, and then $\Exx{z\sim \Lap}{ \disrzero{x_i-z} | y_{i-1}<z<y_{i}}$ strictly decreases, which implies $\Exx{x\sim \Lap}{ \min_{a\in A^{*}}\disrzero{a-x} }$ decreases. However, $A^{*}$ is the optimal point, so it is a contradiction. As a result, for $i\in [\K]$, we have Equations \ref{eq:aveopt}.

\end{proof}

\begin{lemma}   \label{lem:aveadj}

Using the same definition of $x_i$ and $y_i$ as Lemma \ref{lem:median}, we have
\begin{enumerate}
    \item for $i\in [\K -1]$, if $y_i\leq 0$, we have $x_i=y_i-\frac{\log(1+1/i)}{\epsilon}$,
    \item for $i\in [\K]\setminus \{1\}$, if $y_{i-1}\geq 0$, we have $x_i=y_{i-1}+\frac{\log(1+1/(\K-i+1))}{\epsilon}$.
\end{enumerate}


\end{lemma}

\begin{proof}



We first show $x_i=y_i-\frac{\log(1+1/i)}{\epsilon}$ when $y_i\leq 0$. We prove it by induction. When $i=1$, by Equation \ref{eq:aveopt}, we have $\Prxx{z\sim \Lap}{  z<x_{1}} = \Prxx{z\sim \Lap}{  x_{1}<z<y_{1}}$. If $y_1\leq 0$, we have
\begin{align*}
    \int_{-\infty}^{x_{1}} e^{\epsilon z} dz = \int_{x_{1}}^{y_{1}} e^{\epsilon z} dz,
\end{align*}
which is equivalent to
\begin{align*}
    e^{\epsilon x_1} = e^{\epsilon y_1} - e^{\epsilon x_1},
\end{align*}
so $y_1=x_1+\log(2)/\epsilon$.

If $y_i\leq 0$, assuming $x_{i-1}=y_{i-1}-\frac{\log(1+1/(i-1))}{\epsilon}$, then $x_i=y_{i-1}+\frac{\log(1+1/(i-1))}{\epsilon}$. By Equation \ref{eq:aveopt}, we have
\begin{align*}
    \int_{y_{i-1}}^{x_i} e^{\epsilon z} dz = \int_{x_{i}}^{y_{i}} e^{\epsilon z} dz,
\end{align*}
which is equivalent to
\begin{align*}
    \exp{(\epsilon x_{i})} - \exp{\left(\epsilon x_{i} - \frac{\log(1+1/(i-1))}{\epsilon}\right)} = \exp{(\epsilon y_{i})} - \exp{(\epsilon x_{i})},
\end{align*}
so $y_i=x_i+\frac{\log(1+1/i)}{\epsilon}$.

As a result, for $i\in [\K -1]$, if $y_i\leq 0$, we have $x_i=y_i-\frac{\log(1+1/i)}{\epsilon}$.

By symmetry, using similar arguments, we know that for $i\in [\K]\setminus \{1\}$, if $y_{i-1}\geq 0$, then $x_i=y_{i-1}+\frac{\log(1+1/(\K-i+1))}{\epsilon}$.


\end{proof}


\begin{lemma}   \label{lem:geobalance}

Using the same definition of $x_i$ and $y_i$ as Lemma \ref{lem:median}, if $y_i\leq 0\leq y_{i+1}$ where $i\in [\K -2]$, then $|i-(\K-i)|\leq 1$.

\end{lemma}

\begin{proof}

By Lemma \ref{lem:aveadj}, we have
\begin{align*}
    \begin{cases}
    x_i=y_i-\frac{\log(1+1/i)}{\epsilon},    \\
    x_{i+2}=y_{i+1}+\frac{\log(1+1/(\K-i-1))}{\epsilon},
    \end{cases}
\end{align*}
which implies
\begin{align*}
    y_i+\frac{\log(1+1/i)}{\epsilon} = x_{i+1} = y_{i+1}-\frac{\log(1+1/(\K-i-1))}{\epsilon}.
\end{align*}

Since $y_i\leq 0\leq y_{i+1}$, we have $x_{i+1}\in \left[\beta_1,\beta_2 \right]$,
%\begin{align*}
%    x_{i+1}\in \left[\beta_1,\beta_2 \right].
%\end{align*}
where
\begin{align*}
    \beta_1 \defeq -\frac{\log(1+1/(\K-i-1))}{\epsilon},
    \quad
    \beta_2 \defeq \frac{\log(1+1/i)}{\epsilon}.
\end{align*}

Define 
\begin{align*}
    g_1(x)\defeq \int_{x-\frac{\log(1+1/i)}{\epsilon}}^{x} e^{-\epsilon |z|} dz,~~\text{and}~~
    g_2(x) \defeq  \int_{x}^{x+\frac{\log(1+1/(\K-i-1))}{\epsilon}} e^{-\epsilon |z|} dz,
\end{align*}
and define $h(x)\defeq g_1(x)/g_2(x)$. By Lemma \ref{lem:median}, we have $g_1(x_{i+1})=g_2(x_{i+1})$, which implies $h(x_{i+1})=1$.

For $\beta_1 \leq y_1<y_2\leq 0$, we have $g_1(y_1)= e^{y_1-y_2} g_1(y_2)$, and $g_2(y_1)> e^{y_1-y_2} g_2(y_2)$, so $h(y_1)< h(y_2)$. Similarly, for $0\leq y_1<y_2\leq \beta_2$, we have $g_1(y_1)< e^{y_2-y_1} g_1(y_2)$, and $g_2(y_1)= e^{y_2-y_1} g_2(y_2)$, so $h(y_1)< h(y_2)$. As a result, $h(x)$ is strictly increasing on $[\beta_1,\beta_2]$.

If $i>\K-i+1$, $h(\beta_2)<1$. If $i+1<\K-i$, $h(\beta_1)>1$. In both cases, for any $x\in [\beta_1,\beta_2]$, $h(x)\neq 1$. It contradicts to $h(x_{i+1})=1$ and $x_{i+1}\in [\beta_1,\beta_2]$. As a result, we have $|i-(\K -i)|\leq 1$.



\end{proof}

Combining Lemmas \ref{lem:aveadj} and \ref{lem:geobalance}, we have the following corollary.

\begin{corollary} [corresponds to Theorem \ref{thm:lap:sim}]  \label{cor:geofinal}

Using the same definition of $x_i$ and $y_i$ as Lemma \ref{lem:median},

\begin{enumerate}
    \item When $\K$ is odd, $x_{(\K+1)/2}=0$. For $i\in [(\K-1)/2]$, $x_i=-2\log((\K+3)/2-i)/\epsilon$. For $i\in [\K]\setminus [(\K+1)/2]$, $x_i=-x_{\K+1-i}$. That is, if $t\defeq (\K -1)/2$, then
    \begin{align*}
        \{x_1,\dots,x_{\K}\}=\left\{
        0, \pm \frac{2\log\left(\frac{t+1}{t}\right)}{\epsilon},
        \pm \frac{2\log\left(\frac{t+1}{t-1}\right)}{\epsilon},
        \dots,
        \pm \frac{2\log\left(\frac{t+1}{2}\right)}{\epsilon},
        \pm \frac{2\log\left(t+1\right)}{\epsilon}
        \right\}.
    \end{align*}
    \item When $\K$ is even, $x_{\K/2}=-\log(1+2/\K)/\epsilon$. For $i\in [\K/2-1]$, $x_i=x_{i+1}-(2\log(1+1/i))/\epsilon$. For $i\in [\K]\setminus [\K /2]$, $x_i=-x_{\K+1-i}$. That is, if $t\defeq \K /2$, then
    \begin{align*}
        \{x_1,\dots,x_{\K}\}=\left\{
         \pm \frac{\log\left(\frac{t+1}{t}\right)}{\epsilon},
        \pm \frac{\log\left(\frac{t(t+1)}{(t-1)^2}\right)}{\epsilon},
        \pm \frac{\log\left(\frac{t(t+1)}{(t-2)^2}\right)}{\epsilon},
        \dots,
        \pm \frac{\log\left(\frac{t(t+1)}{2^2}\right)}{\epsilon},
        \pm \frac{\log\left(t(t+1)\right)}{\epsilon}
        \right\}.
    \end{align*}
\end{enumerate}

Furthermore, by Lemma \ref{lem:computefal}, we have
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\Exx{x\sim \Lap}{ \min_{i\in [\K]}\disrzero{x_{i}-x} }
=
\begin{cases}
\frac{4}{\epsilon(\K +1)} , & \text{$\K$ is odd},  \\
\frac{2}{\epsilon} \log\left( 1+\frac{2}{\K} \right) , & \text{$\K$ is even},  \\
\end{cases}
\end{align*}
which implies $\funf{\Users}{\Ads}{\epsilon}{\K}$ is $O(1/(\epsilon \K))$.


\end{corollary}

Above, Theorem \ref{thm:main1} is proved.





\subsection{Proof for Theorem \ref{thm:lapopt}} \label{sec:prooflapopt}



  The first equation in Theorem \ref{thm:lapopt} is directly from Theorem \ref{thm:symfinal}. For any $A\in \Kads$, $x\in \real$, and $\Sname \in \Srobs$, we define
  \begin{align*}
    \fung{A}{x}\defeq \min_{a\in A}\disrzero{a-x} ,~~
    \fung{A}{\Sname}\defeq \Exx{x\sim \Sname}{ \fung{A}{x} }=\Exx{x\sim \Sname}{ \min_{a\in A}\disrzero{a-x} }.
  \end{align*}
  Then it is sufficient to show
  \begin{align} \label{eq:suff:lapopt}
    \inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \fung{A}{\Sname}=\inf_{A\in \Kads} \fung{A}{\Lap}.
  \end{align}




  To prove this equality, for any $(A,\Sname)$ where $A\in \Kads$ and $\Sname \in \Srobs$, we show that there exists $A'$ so that $\fung{A}{\Sname}\geq \fung{A'}{\Lap}$.
  
  In Section \ref{sec:convertexp}, we introduce an operation which converts any distribution in $\Srobs$ to a piece-wise exponential distribution (defined later). In Section \ref{sec:spaceremoval}, we show an operation that removes some space, which essentially concentrates the points in $A$ and the mass in $\Sname$ respectively. In Section \ref{sec:potential}, roughly speaking, we define a potential function based on i) the number of pieces in the piece-wise exponential distribution and ii) how concentrated $A$ and $\Sname$ are. We use the operations in Sections \ref{sec:convertexp} and \ref{sec:spaceremoval}, while the potential function decreases and $\fung{A}{\Sname}$ does not increase. The procedure stops some time because the potential function is discrete and bounded, and at that time, $\Sname$ becomes the Laplace distribution.
  
  
  \subsubsection{Conversion to piece-wise exponential distributions}    \label{sec:convertexp}
  
  
  \begin{definition}[\lar~interval, \sma~interval] \label{def:larsma}
  
  Fix $A\in \Kads$ and $\gamma\geq 0$. There exists a unique sequence of $-\infty=t_0<t_1<\dots<t_{2m+1}<+\infty$ where $m$ is a positive integer, so that $\min_{a\in A}\disrzero{a-t_i}=\gamma$ for any $0<i\leq 2m$. Moreover, for any $0\leq i\leq 2m$ and $x\in (t_i,t_{i+1})$, $\min_{a\in A}\disrzero{a-x}\leq \gamma$ if $i$ is odd, and $\min_{a\in A}\disrzero{a-x}\geq \gamma$ if $i$ is even.
  
  For each odd $i$, we call $[t_i,t_{i+1}]$ a~\sma~interval. For each even $i$, we call $(t_i,t_{i+1})$ a~\lar~interval. All the~\sma~intervals and~\lar~intervals form a partition of $\real$.
  
  Note that the number of~\sma~intervals is $m$, and the number of~\lar~intervals is $m+1$. We define $\funnum{A}{\gamma}$ to be $m$.
  
  \end{definition}
  
  \begin{observation} \label{obs:mcloseform}
  
  If $A=\{x_1,x_2,\dots,x_{\K}\}$ where $x_1\leq x_2\leq \dots\leq x_{\K}$, then
  \begin{align*}
      \funnum{A}{\gamma}=1+\sum_{i=1}^{\K -1}\I{x_{i+1}-x_{i}>2\gamma}.
  \end{align*}
  
  \end{observation}
  
  
  \begin{lemma} \label{lem:h}
  
  Fix $A\in \Kads$, $\gamma\geq 0$. For any $\Sname\in \Srobs$, there exists $\funextr{A}{\gamma}{\Sname}\in \Srobs$ that has the following properties.
  \begin{enumerate}
      
  
      \item If $\fung{A}{\Sname}\leq \gamma$, then $\fung{A}{ \funextr{A}{\gamma}{\Sname} }\leq \gamma$. \label{expr:item1}.
      
      
      \item For any~\sma~interval $[a,b]$, for any $x\in [a,b]$,
      
      $\rho_{\funextr{A}{\gamma}{\Sname}}(x)=\min \left\{ e^{\epsilon (x-a)}\rho_{\funextr{A}{\gamma}{\Sname}}(a), e^{\epsilon (b-x)}\rho_{\funextr{A}{\gamma}{\Sname}}(b) \right\}$. \label{expr:item2}
      
      \item For any~\lar~interval $(a,b)$ where $a,b\in \real$, for any $x\in [a,b]$,
      
      $\rho_{\funextr{A}{\gamma}{\Sname}}(x)= \max \left\{ e^{-\epsilon (x-a)}\rho_{\funextr{A}{\gamma}{\Sname}}(a), e^{-\epsilon (b-x)}\rho_{\funextr{A}{\gamma}{\Sname}}(b) \right\}$.
      
      \item For~\lar~interval $(a,+\infty)$, for any $x\in [a,+\infty)$, $\rho_{\funextr{A}{\gamma}{\Sname}}(x)=e^{-\epsilon (x-a)}\rho_{\funextr{A}{\gamma}{\Sname}}(a)$.
      
      \item For~\lar~interval $(-\infty,b)$, for any $x\in (-\infty,b]$, $\rho_{\funextr{A}{\gamma}{\Sname}}(x)=e^{-\epsilon (b-x)}\rho_{\funextr{A}{\gamma}{\Sname}}(b)$. \label{expr:item5}
      
  \end{enumerate}
  
  \end{lemma}


    Figure \ref{fig:pwexp} is an example of this lemma.

  
  \begin{proof}

  For $\Sname\in \Srobs$, we construct another probability measure $\Sxa$ on $\real$ as following.
  
  \begin{enumerate}
    
      
      \item For any~\sma~interval $[a,b]$, for any $x\in [a,b]$, let $\tilde{\rho}_{\Sxa}(x)=\min \left\{ e^{\epsilon (x-a)}\rho_{\Sname}(a), e^{\epsilon (b-x)}\rho_{\Sname}(b) \right\}$.
      
      \item For any~\lar~interval $(a,b)$ where $a,b\in \real$, for any $x\in (a,b)$, let $\tilde{\rho}_{\Sxa}(x)=\max \left\{ e^{-\epsilon (x-a)}\rho_{\Sname}(a), e^{-\epsilon (b-x)}\rho_{\Sname}(b) \right\}$.
      
      \item For~\lar~interval $(a,+\infty)$, for any $x\in (a,+\infty)$, let $\tilde{\rho}_{\Sxa}(x)=e^{-\epsilon (x-a)}\rho_{\Sname}(a)$.
      
      \item For~\lar~interval $(-\infty,b)$, for any $x\in (-\infty,b)$, let $\tilde{\rho}_{\Sxa}(x)=e^{-\epsilon (b-x)}\rho_{\Sname}(b)$.
      
  \end{enumerate}
  
    Note that these four items corresponds to Items \ref{expr:item2}-\ref{expr:item5} in the lemma.
  
  Since $\alpha\defeq \int_{\real}\tilde{\rho}_{\Sxa}(x)dx$ may not be 1, we should normalize it. If $(-\infty,b)$ and $(a,\infty)$ are two~\lar~intervals, then
  \begin{align*}
  & \int_{b}^{a}\tilde{\rho}_{\Sxa}(x)dx<+\infty,~~\text{since $\tilde{\rho}_{\Sxa}(x)$ is bounded on closed interval $[b,a]$,} \\
  & \int_{-\infty}^{b}\tilde{\rho}_{\Sxa}(x)dx = \rho_{\Sname}(b)\int_{-\infty}^{t_{1}}e^{-\epsilon \cdot(b-x)}dx < +\infty, \\
  & \int_{a}^{+\infty}\tilde{\rho}_{\Sxa}(x)dx = \rho_{\Sname}(a)\int_{a}^{+\infty}e^{-\epsilon \cdot (x-a)}dx < +\infty, \\
  \end{align*}
  so we have $\alpha<\infty$, and we can define
  \begin{align*}
  \rho_{\Sxa}(x)\defeq \frac{1}{\alpha} \tilde{\rho}_{\Sxa}(x).
  \end{align*}
  
  Let $\funextr{A}{\gamma}{\Sname}$ be $\Sxa$, then Items \ref{expr:item2}-\ref{expr:item5} holds.
  
  Next, we show Item $\ref{expr:item1}$ holds.
  
  If $x\in [a,b]$ where $[a,b]$ is a~\sma~interval, then $\rho_{\Sname}(x)\leq e^{\epsilon(x-a)}\rho_{\Sname}(a)$ and $\rho_{\Sname}(x)\leq e^{\epsilon(b-x)}\rho_{\Sname}(b)$, which implies
  \begin{align}\label{extr:tilde:c1}
      \tilde{\rho}_{\Sxa}(x)
      =\min\left\{e^{\epsilon(x-a)}\rho_{\Sname}(a), e^{\epsilon(b-x)}\rho_{\Sname}(b)\right\}
      \geq \rho_{\Sname}(x).
  \end{align}
  
  Similarly, if $x\in (a,b)$ where $(a,b)$ is a~\lar~interval and $a,b\in \real$, then $\rho_{\Sname}(x)\geq e^{-\epsilon(x-a)}\rho_{\Sname}(a)$ and $\rho_{\Sname}(x)\geq e^{-\epsilon(b-x)}\rho_{\Sname}(b)$, which implies
  \begin{align}\label{extr:tilde:c2}
      \tilde{\rho}_{\Sxa}(x)
      =\max\left\{e^{-\epsilon(x-a)}\rho_{\Sname}(a), e^{-\epsilon(b-x)}\rho_{\Sname}(b)\right\}
      \leq \rho_{\Sname}(x).
  \end{align}
  
  Using similar argument, when $x$ in~\lar~interval $(-\infty,b)$ or $(a,+\infty)$, we also have
  \begin{align} \label{extr:tilde:c3}
      \tilde{\rho}_{\Sxa}(x)
      \leq \rho_{\Sname}(x).
  \end{align}
  
  Combining the three cases (Inequality \ref{extr:tilde:c1}, \ref{extr:tilde:c2} and \ref{extr:tilde:c3}), for any $x\in \real$, we have
  \begin{align}\label{extr:tilde:c0}
      (\tilde{\rho}_{\Sxa}(x)-\rho_{\Sname}(x)) (\fung{A}{x}-\gamma)\leq 0,
  \end{align}
  because $\tilde{\rho}_{\Sxa}(x)\geq \rho_{\Sname}(x)$ in~\sma~intervals where $\fung{A}{x}\leq \gamma$, and $\tilde{\rho}_{\Sxa}(x)\leq \rho_{\Sname}(x)$ in~\lar~intervals where $\fung{A}{x}\geq \gamma$.



  If $\fung{A}{\Sname}\leq \gamma$, then
  \begin{align}
  & \fung{A}{\Sxa} - \gamma   \\
  = &  \int_{\real} \rho_{\Sxa}(x) (\fung{A}{x}-\gamma) dx   \\
  =&  \frac{1}{\alpha} \int_{\real} \tilde{\rho}_{\Sxa}(x) (\fung{A}{x}-\gamma) dx   \\
  \leq &  \frac{1}{\alpha} \int_{\real} (\tilde{\rho}_{\Sxa}(x)-\rho_{\Sname}(x)) (\fung{A}{x}-\gamma) dx \label{makeexp:addprevious}  \\
  \leq & 0,  \label{makeexp:leq}
  \end{align}
  where equality \ref{makeexp:addprevious} follows from $\int_{\real}\rho_{\Sname}(x)(\fung{A}{x}-\gamma)dx \leq 0$, and inequality \ref{makeexp:leq} follows from Inequality \ref{extr:tilde:c0}. Inequality \ref{makeexp:leq} is equivalent to Item $\ref{expr:item1}$.
  
  Finally, we need to show $\funextr{A}{\gamma}{\Sname}\in \Srobs$. For any $x,y\in \real$, if $x,y$ are in the same~\lar~or~\sma~interval, it is clear that $\rho_{\funextr{A}{\gamma}{\Sname}}(x)\leq e^{\epsilon\cdot \disr{x}{y}} \rho_{\funextr{A}{\gamma}{\Sname}}(y)$. If $x,y$ are not in the same~\lar~or~\sma~interval, assume $x,y$, and there exists $t_0<t_1<\dots<t_{\ell}$, where for any $0\leq i<\ell$, either $(t_i,t_{i+1})$ is a~\lar~interval or $[t_i,t_{i+1}]$ is a~\sma~interval, and $x\in (t_0,t_1)$, $y\in (t_{\ell-1},t_{\ell})$. Then we have
  \begin{align*}
      & \rho_{\funextr{A}{\gamma}{\Sname}}(x)\\
      \leq & e^{\epsilon (t_1-x)} \rho_{\funextr{A}{\gamma}{\Sname}}(t_1)\\
      \leq & e^{\epsilon (t_1-x)}e^{\epsilon (t_2-t_1)} \rho_{\funextr{A}{\gamma}{\Sname}}(t_2)\\
       & \dots\\
      \leq & e^{\epsilon (t_1-x)}e^{\epsilon (t_2-t_1)}\dots e^{\epsilon (t_{\ell-1}-t_{\ell-2})} \rho_{\funextr{A}{\gamma}{\Sname}}(t_{\ell-1})\\
      \leq & e^{\epsilon (t_1-x)}e^{\epsilon (t_2-t_1)}\dots e^{\epsilon (t_{\ell-1}-t_{\ell-2})}e^{\epsilon (y-t_{\ell-1})} \rho_{\funextr{A}{\gamma}{\Sname}}(y)\\
      =& e^{\epsilon (y-x)} \rho_{\funextr{A}{\gamma}{\Sname}}(y).
  \end{align*}
  
  Using similar arguments, when $x>y$, we also have
  $\rho_{\funextr{A}{\gamma}{\Sname}}(x) \leq e^{\epsilon (y-x)} \rho_{\funextr{A}{\gamma}{\Sname}}(y)$. As a result, $\funextr{A}{\gamma}{\Sname}\in \Srobs$.
  
  
  
  
  
  \iffalse%%%%%%
  For $0 \le i<|T|$, if $\fung{A}{x}\leq \fung{A}{\Sname}$ for any $x\in (t_i,t_{i+1})$, then $\tilde{\rho}_{\Sxa}(x)=\min\{ e^{\epsilon \disr{x}{t_i}}\rho_{\Sname}(t_i), e^{\epsilon \disr{x}{t_{i+1}}}\rho_{\Sname}(t_{i+1}) \}$. Note that as $x$ increasing in $(t_i,t_{i+1})$, $e^{\epsilon \disr{x}{t_i}}\rho_{\Sname}(t_i)$ is increasing and $e^{\epsilon \disr{x}{t_{i+1}}}\rho_{\Sname}(t_{i+1})$ is decreasing. Also, $e^{\epsilon \disr{x}{t_i}}\rho_{\Sname}(t_i) \leq e^{\epsilon \disr{x}{t_{i+1}}}\rho_{\Sname}(t_{i+1})$ when $x=t_i$, and $e^{\epsilon \disr{x}{t_i}}\rho_{\Sname}(t_i) \geq e^{\epsilon \disr{x}{t_{i+1}}}\rho_{\Sname}(t_{i+1})$ when $x=t_{i+1}$, both because $\Sname\in \Srobs$ which satisfies the privacy constraints. As a result, there exists $r\in [t_i,t_{i+1}]$, so that $\tilde{\rho}_{\Sxa}(x)= e^{\epsilon \disr{x}{t_i}}\rho_{\Sname}(t_i)$ for $x\in [t_i,r]$, and $\tilde{\rho}_{\Sxa}(x)= e^{\epsilon \disr{x}{t_{i+1}}}\rho_{\Sname}(t_{i+1})$ for $x\in [r,t_{i+1}]$. It implies that we can divide the interval $[t_i,t_{i+1}]$ into two small intervals, and inside each small interval, the value of $\tilde{\rho}_{\Sxa}(x)$ has form $a e^{\epsilon x}$ or $a e^{-\epsilon x}$, where $a>0$ is a fixed constant in each small interval, but $a$ can be different in different intervals. It also implies that $\tilde{\rho}_{\Sxa}(x)$ is continuous on $[t_i,t_{i+1}]$ with respect to $x$. Besides, note that $x$ is not a minimal point of $\tilde{\rho}_{\Sxa}(x)$ when $x\in (t_i,t_{i+1})$, which implies that $x$ is not a minimal point of $\tilde{\rho}_{\Sxa}(x)$ when $\fung{A}{x}<\fung{A}{\Sname}$. This property will be used later.

  Using the same argument, we can reach the same conclusion for each interval $(t_i,t_{i+1})$ where $0\leq i\leq |T|$. As a result, $\tilde{\rho}_{\Sxa}(x)$ is continuous on $\real$ with respect to $x$, and there exists $-\infty=s_0<s_1<\dots<s_m<s_{m+1}=+\infty$, so that $\tilde{\rho}_{\Sxa}(x) = a_i e^{b_i\epsilon x}$ for any $x\in (s_i,s_{i+1})$, where $0\leq i\leq m$, $a_i>0$ and $b_i\in \{-1,1\}$. Furthermore, if $b_i=b_{i+1}$, we can combine $(s_i,s_{i+1})$ and $s_{i+1},s_{i+2}$ into one interval. So, w.l.o.g., we assume $b_i=i~\text{mod}~2$, and $m$ is even.
  
  We define $\funextr{A}{\gamma}{\Sname}$ to be $\Sxa$.
  \fi%%%%%%%%%%%%
  
  \zhihaohalfcomment{Need a figure}
  
  \end{proof}
  
  
  
  \begin{definition} [monotone large/small, and \funmonname / \funmonsmaname]   \label{def:monlar}
  
  Fix $A\in \Kads, \Sname\in \Srobs$. For a~\lar~interval $(a,b)$ where $a,b\in \real\cup \{-\infty,+\infty\}$, if one of the following is true, we call $(a,b)$~\slar~interval.
  \begin{enumerate}
      \item $a\in \real$, and $\rho_{\Sname}(x)=e^{-\epsilon(x-a)}\rho_{\Sname}(a)$ for any $x\in (a,b)$.
      \item $b\in \real$, and $\rho_{\Sname}(x)=e^{-\epsilon(b-x)}\rho_{\Sname}(b)$ for any $x\in (a,b)$.
  \end{enumerate}
  
  We define $\funmon{A}{\gamma}{\Sname}$ to be the number of~\lar~intervals that are not~\slar~intervals.
  
  For a~\sma~interval $[a,b]$ where $a,b\in \real$, if one of the following is true, we call $[a,b]$~\ssma~interval.
  \begin{enumerate}
      \item $a\in \real$, and $\rho_{\Sname}(x)=e^{\epsilon(x-a)}\rho_{\Sname}(a)$ for any $x\in [a,b]$.
      \item $b\in \real$, and $\rho_{\Sname}(x)=e^{\epsilon(b-x)}\rho_{\Sname}(b)$ for any $x\in [a,b]$.
  \end{enumerate}
  
  We define $\funmonsma{A}{\gamma}{\Sname}$ to be the number of~\sma~intervals that are not~\ssma~intervals.

  See Figure \ref{fig:monvsreg} for an example.
  
  \end{definition}



    
  \begin{figure}
      \centering
        \begin{tikzpicture}
        \fill[cmlar] (0,0) rectangle (1,3.5);
        \fill[csma] (1,0) rectangle (3,3.5);
        \fill[clar] (3,0) rectangle (4.5,3.5);
        \fill[cmsma] (4.5,0) rectangle (6.5,3.5);
        \fill[cmlar] (6.5,0) rectangle (7.5,3.5);
        \coordinate (right) at (7.5,0);
        \coordinate (o) at (0,0);
        \coordinate (up) at (0,3.5);
        \coordinate (x0) at (4.5,0);
        \coordinate (s) at (2,0);
        \coordinate (t) at (5.5,0);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[<->](right)--(o)--(up);
        % here, eps=0.55
        \draw[blue,domain=0:2] plot(\x,{(1.5+0.5*cos((1-2)*1.5 r))*exp(0.55*(\x-1))} );
        \draw[blue,domain=2:3] plot(\x,{(1.5+0.5*cos((3-2)*1.5 r))*exp(-0.55*(\x-3))} );
        \draw[blue,domain=3:4.061681] plot(\x,{(1.5+0.5*cos((3-2)*1.5 r))*exp(-0.55*(\x-3))} );
        \draw[blue,domain=4.061681:4.5] plot(\x,{(1.5+0.5*cos((4.5-2)*1.5 r))*exp(0.55*(\x-4.5))} );
        \draw[blue,domain=4.5:6.5] plot(\x,{(1.5+0.5*cos((4.5-2)*1.5 r))*exp(0.55*(\x-4.5))} );
        \draw[blue,domain=6.5:7.5] plot(\x,{(1.5+0.5*cos((4.5-2)*1.5 r))*exp(0.55*(6.5-4.5))*exp(0.55*(6.5-\x))} );
        \fill (s) circle (2pt);
        \fill (t) circle (2pt);
        \draw[decorate,decoration={brace,raise=1pt,amplitude=3pt},purple] (x0) -- (t) node[black,midway,yshift=9pt] {$\gamma$};
        \end{tikzpicture}
      \caption{The lighter yellow part is a~\sma~interval but not a~\ssma~interval, while the darker yellow part is a~\ssma~interval. The lighter blue part is a~\lar~interval but not a~\slar~interval, while the darker blue parts are ~\slar~intervals.}    \label{fig:monvsreg}
  \end{figure}

  
  
  \begin{corollary}[corollary of Lemma \ref{lem:h}] \label{cor:extrexp}
  
  Fix $A\in \Kads$, $\gamma\geq 0$. For any $\Sname\in \Srobs$, for each~\sma~interval $[a,b]$ or~\lar~interval $(a,b)$, there exists $c\in [a,b]\setminus\{-\infty,+\infty\}$, so that $\rho_{\funextr{A}{\gamma}{\Sname}}(x)=\rho_{\funextr{A}{\gamma}{\Sname}}(c)e^{\epsilon \disr{x}{c}}$ for any $x\in (a,b)$. 
  
  Furthermore, for~\lar~interval $(a,b)$, it is a~\slar~interval if and only if $c\in \{a,b\}$. Similarly, for~\sma~interval $[a,b]$, there exists $c\in [a,b]$ so that $\rho_{\funextr{A}{\gamma}{\Sname}}(x)=\rho_{\funextr{A}{\gamma}{\Sname}}(c)e^{-\epsilon \disr{x}{c}}$ for any $x\in [a,b]$, and it is a~\ssma~interval if and only if $c\in \{a,b\}$.
  
  \end{corollary}
  
  
  
  \subsubsection{Space removal} \label{sec:spaceremoval}
  
  
  
  \begin{definition}[space removal]  \label{def:removal}
  
  For $\Sname\in \Srobs$, for $a,b\in \real$ where $a<b$, we can remove the space $[a,b)$ and splice $(-\infty,a)$ and $[b,+\infty)$ together. Formally, we define $\sr{a}{b}{\Srobs}$ to be the distribution with probability density
  \begin{align*}
      \rho_{\sr{a}{b}{\Srobs}}(x)\defeq
      \begin{cases}
        \alpha \rho_{\Srobs}(x), & x<a;    \\
        \alpha \rho_{\Srobs}(x+(b-a)), & x\geq a,
      \end{cases}
  \end{align*}
  where $\alpha = \left(1-\int_{a}^{b}\rho_{\Sname}(x)dx\right)^{-1}$ is the normalizer.
  
  Similarly, for $A\in \Kads$, we also define
  \begin{align*}
      \sra{a}{b}{A}\defeq \{ \srx{a}{b}{x} | x\in A \},
  \end{align*}
  where
  \begin{align*}
      \srx{a}{b}{x}\defeq
      \begin{cases}
        x, & x<a;    \\
        a, & a\leq x<b;    \\
        x-(b-a), & x\geq b.
      \end{cases}
  \end{align*}
  
  \end{definition}
  
  
  Recall that $\funnum{A}{\gamma}$ is the number of~\sma~intervals given $A$ and $\gamma$. Next, we show the number of~\sma~intervals cannot increase after space removal (Corollary \ref{cor:mvalremoval}). It is somehow obvious, but we still provide a proof, starting with Lemma \ref{lem:mvalremoval}.
  
  
  \begin{lemma} \label{lem:mvalremoval}
  
  For $A\in \Kads, \gamma\geq 0$, for $a,b\in \real$ where $a<b$, if $A=\{x_1,x_2,\dots,x_{\K}\}$ where $x_1\leq x_2\leq \dots\leq x_{\K}$, we have
  \begin{align*}
    \funnum{A}{\gamma} - \funnum{\sra{a}{b}{A}}{\gamma}=\sum_{i=1}^{\K -1}\I{\srx{a}{b}{x_{i+1}}-\srx{a}{b}{x_{i}}\leq 2\gamma \text{~and~} x_{i+1}-x_{i}>2\gamma}.
  \end{align*}
  
  \end{lemma}
  
  \begin{proof}
  
  According to the definition of $\srx{a}{b}{x}$ in Definition \ref{def:removal}, $\srx{a}{b}{x}\leq \srx{a}{b}{y}$ if $x\leq y$. If $A=\{x_1,x_2,\dots,x_{\K}\}$ where $x_1\leq x_2\leq \dots\leq x_{\K}$, then $\srx{a}{b}{x_1}\leq \srx{a}{b}{x_2}\leq \dots\leq \srx{a}{b}{x_{\K}}$. Note that $\sra{a}{b}{A}=\{\srx{a}{b}{x_1}, \srx{a}{b}{x_2}, \dots , \srx{a}{b}{x_{\K}}\}$, according to Observation \ref{obs:mcloseform}, we have
  \begin{align*}
      \funnum{\sra{a}{b}{A}}{\gamma}
      = 1+\sum_{i=1}^{\K -1}\I{\srx{a}{b}{x_{i+1}}-\srx{a}{b}{x_{i}}>2\gamma}.
  \end{align*}
  
  
  For $a,b\in \real$ where $a<b$, in the definition of $\srx{a}{b}{x}$ in Definition \ref{def:removal}, note that for any $x,y\in \real$, we have $\disr{\srx{a}{b}{x}}{\srx{a}{b}{y}} \leq \disr{x}{y}$, so $\I{\disr{\srx{a}{b}{x}}{\srx{a}{b}{y}}>2\gamma}\leq \I{\disr{x}{y}>2\gamma}$ for any $\gamma\geq 0$, so we have
  \begin{align*}
    \funnum{A}{\gamma} - \funnum{\sra{a}{b}{A}}{\gamma}
    =&\sum_{i=1}^{\K -1}\left( \I{x_{i+1}-x_{i}> 2\gamma} - \I{\sra{a}{b}{x_{i+1}}-\sra{a}{b}{x_{i}}> 2\gamma} \right)   \\
    =&\sum_{i=1}^{\K -1}\I{\sra{a}{b}{x_{i+1}}-\sra{a}{b}{x_{i}}\leq 2\gamma \text{~and~} x_{i+1}-x_{i}>2\gamma}.
  \end{align*}
  
  
  
  \end{proof}
  
  \begin{corollary} \label{cor:mvalremoval}
  
  
  For $A\in \Kads, \gamma\geq 0$, for $a,b\in \real$ where $a<b$, we have
  \begin{align*}
      \funnum{\sra{a}{b}{A}}{\gamma} \leq \funnum{A}{\gamma}.
  \end{align*}
  
  \end{corollary}
  

  Next lemma shows the mechanism can only become better after space removal.
  
  \begin{lemma} \label{lem:monotoneremoval}
  
  For $A\in \Kads, \gamma\geq 0, \Sname\in \Srobs$, for $a,b\in \real$ where $a<b$, if
  \begin{enumerate}
      \item $\rho_{\Sname}(a)=\rho_{\Sname}(b)$,
      \item $\fung{A}{\Sname}\leq \gamma$,
      \item $\int_{a}^{b}\fung{A}{x}\rho_{\Sname}(x)dx\geq \gamma \int_{a}^{b}\rho_{\Sname}(x)dx$,
  \end{enumerate}
  then
  \begin{enumerate}
      \item $\sr{a}{b}{\Sname}\in \Srobs$,
      \item $\fung{\sra{a}{b}{A}}{\sr{a}{b}{\Sname}}\leq \gamma$.
  \end{enumerate}
  
  \end{lemma}
  
  \begin{proof}
  
  Let $\alpha=\left(1-\int_{a}^{b}\rho_{\Sname}(x)dx\right)^{-1}$, which is the normalizer in Definition \ref{def:removal}.
  
  For $x,y\in \real$, we consider the following four cases.
  \begin{enumerate}
      \item $x,y\leq a$. $\rho_{\sr{a}{b}{\Sname}}(x)=\alpha\rho_{\Sname}(x)\leq e^{\epsilon\cdot \disr{x}{y}}\alpha\rho_{\Sname}(y)=\rho_{\sr{a}{b}{\Sname}}(y)$.
      \label{rmv:srobs:c1}
      
      \item $x,y\geq a$. $\rho_{\sr{a}{b}{\Sname}}(x)=\alpha\rho_{\Sname}(x+(b-a))\leq e^{\epsilon\cdot \disr{x}{y}}\alpha\rho_{\Sname}(y+(b-a))=\rho_{\sr{a}{b}{\Sname}}(y)$.
      \label{rmv:srobs:c2}
      
      \item $x<a$, $y\geq a$.
      $\rho_{\sr{a}{b}{\Sname}}(x)
      \leq  e^{\epsilon\cdot \disr{x}{a}}\rho_{\sr{a}{b}{\Sname}}(a)
      \leq e^{\epsilon\cdot \disr{x}{y}}\rho_{\sr{a}{b}{\Sname}}(y)$.
      \label{rmv:srobs:c3}
      
      \item $x\geq a$, $y< a$.
      $\rho_{\sr{a}{b}{\Sname}}(x)
      \leq  e^{\epsilon\cdot \disr{x}{a}}\rho_{\sr{a}{b}{\Sname}}(a)
      \leq e^{\epsilon\cdot \disr{x}{y}}\rho_{\sr{a}{b}{\Sname}}(y)$.
      \label{rmv:srobs:c4}
  \end{enumerate}
  Items \ref{rmv:srobs:c1} and \ref{rmv:srobs:c2} holds since $\Sname\in \Srobs$, and Items \ref{rmv:srobs:c3} and \ref{rmv:srobs:c4} follows from $\rho_{\Sname}(a)=\rho_{\Sname}(b)$ and Items \ref{rmv:srobs:c1} and \ref{rmv:srobs:c2}. The four cases imply $\sr{a}{b}{\Sname}\in \Srobs$.
  
  If $\fung{A}{\Sname}\leq \gamma$ and $\int_{a}^{b}\fung{A}{x}\rho_{\Sname}(x)dx\geq \gamma \int_{a}^{b}\rho_{\Sname}(x)dx$, we have
  \begin{align*}
      & \fung{\sra{a}{b}{A}}{\sr{a}{b}{\Sname}} \\
      = & \int_{-\infty}^{a}\fung{A}{x}\rho_{\sr{a}{b}{\Sname}}(x)dx + \int_{a}^{+\infty}\fung{A}{x}\rho_{\sr{a}{b}{\Sname}}(x)dx  \\
      = & \alpha \int_{-\infty}^{a}\fung{A}{x}\rho_{\Sname}(x)dx + \int_{a}^{+\infty}\fung{A}{x}\rho_{\Sname}(x+(b-a))dx  \\
      = & \alpha \left( \fung{A}{\Sname}-\int_{a}^{b}\fung{A}{x}\rho_{\Sname}(x)dx \right)  \\
      \leq & \alpha \left( \gamma - \gamma(1-\alpha^{-1}) \right) \\
      = & \gamma.
  \end{align*}
  
  
  \end{proof}
  
  
  \subsubsection{Proof using a potential function}  \label{sec:potential}
  
  
  \begin{lemma} \label{lem:tolaps1}
  
  For $A\in \Kads, \gamma\geq 0, \Sname\in \Srobs$, if $\fung{A}{\Sname}\leq \gamma$ and $\funmon{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}>0$, there exists $\Axa\in \Kads,\Sxa\in \Srobs$, so that
  \begin{enumerate}
      \item $\fung{\Axa}{\Sxa}\leq \gamma$.
      \item $\max \Axa-\min \Axa \leq \max A-\min A$.
      \item At least one of the following holds
      \begin{enumerate}
          \item $\funnum{\Axa}{\gamma}< \funnum{A}{\gamma}$
          \item All the the following holds.
          \begin{enumerate}
              \item $\funnum{\Axa}{\gamma}\leq \funnum{A}{\gamma}$.
              \item $\funmonsma{\Axa}{\gamma}{\funextr{\Axa}{\gamma}{\Sxa}}= \funmonsma{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}$.
              \item $\funmon{\Axa}{\gamma}{\funextr{\Axa}{\gamma}{\Sxa}}< \funmon{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}$.
          \end{enumerate} 
      \end{enumerate}
  \end{enumerate}
  
  \end{lemma}
  
  
  \begin{proof}

  Since $\funmon{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}>0$, by Corollary \ref{cor:extrexp}, there exists a~\lar~but not~\slar~interval $(a,b)$ and $c\in (a,b)$, so that $\rho_{\funextr{A}{\gamma}{\Sname}}(x)=\rho_{\funextr{A}{\gamma}{\Sname}}(c)e^{\epsilon \disr{x}{c}}$ for any $x\in (a,b)$.
  
  Let $\ell\defeq \sup\{x\geq 0 | (c-x,c+x)\subset (a,b)\}$, and we remove $[c-\ell,c+\ell)$. That is, let
  \begin{align*}
      \Axa = \sra{c-\ell}{c+\ell}{A},   \\
      \Sxa = \sr{c-\ell}{c+\ell}{\funextr{A}{\gamma}{\Sname}}.
  \end{align*}
  
  Then it is clearly that $\max \Axa-\min \Axa \leq \max A-\min A$.
  
  Since for any $x\in (a,b)$, $\fung{A}{x}\geq \gamma$, we have $\int_{c-\ell}^{c+\ell}\fung{A}{x}\rho_{\funextr{A}{\gamma}{\Sname}}(x)dx\geq \gamma \int_{c-\ell}^{c+\ell}\rho_{\funextr{A}{\gamma}{\Sname}}(x)dx$. Note that $\rho_{\funextr{A}{\gamma}{\Sname}}(c-\ell)=\rho_{\funextr{A}{\gamma}{\Sname}}(c+\ell)$ and $\fung{A}{\Sname}\leq \gamma$. According to Lemma \ref{lem:h} and Lemma \ref{lem:monotoneremoval}, we have $\Sxa\in \Srobs$ and $\fung{\Axa}{\Sxa}\leq \gamma$.
  
  Next, we consider some cases, and in each case, either $\funnum{\Axa}{\gamma}< \funnum{A}{\gamma}$, or $\funmon{\Axa}{\gamma}{\gamma}\leq \funmon{A}{\gamma}{\Sname}$ and $\funextr{\Axa}{\gamma}{\Sxa}=\Sxa$ are both satisfied.
  
  
  
  
  
  \paragraph{Case 1, $a=c-\ell$ and $b=c+\ell$.}
  
  Since there is a~\sma~interval with right endpoint $a$ and there is a~\sma~interval with left endpoint $b$, we can define $s\defeq \max\{x\in A| x\leq c\}$ and $t\defeq \min\{x\in A| x\geq c\}$. Since $c$ is in a~\lar~interval, $\fung{c}{A}>\gamma$, which implies $t-c>\gamma$ and $c-s>\gamma$, so $t-s>2\gamma$.
  
  Note that $\fung{A}{a}=\fung{A}{b}=\gamma$, so
  \begin{align*}
      \srx{c-\ell}{c+\ell}{t}-\srx{c-\ell}{c+\ell}{s}
      =\srx{a}{b}{t}-\srx{a}{b}{s}
      =(t+(a-b)) - s
      =(t-b)+(a-s)
      =2\gamma.
  \end{align*}
  
  If $A=\{x_1,x_2,\dots,x_{\K}\}$ where $x_1\leq x_2\leq \dots\leq x_{\K}$, then there exists $1\leq i_0<\K$ so that $x_{i_0}=s$ and $x_{i_0+1}=t$. By Lemma \ref{lem:mvalremoval}, we have
  \begin{align*}
      & \funnum{A}{\gamma} - \funnum{\Axa}{\gamma}  \\
      =& \funnum{A}{\gamma} - \funnum{\sra{a}{b}{A}}{\gamma} \\
      =& \sum_{i=1}^{\K -1}\I{\sra{a}{b}{x_{i+1}}-\sra{a}{b}{x_{i}}\leq 2\gamma \text{~and~} x_{i+1}-x_{i}>2\gamma} \\
      \geq & \I{\sra{a}{b}{x_{i_0+1}}-\sra{a}{b}{x_{i_0}}\leq 2\gamma \text{~and~} x_{i_0+1}-x_{i_0}>2\gamma} \\
      &=1,
  \end{align*}
  which implies $\funnum{\Axa}{\gamma}<\funnum{A}{\gamma}$.
  
  
  
  
  
  \paragraph{Case 2, $a=c-\ell$ and $b>c+\ell$.}
  
  According to Definition \ref{def:larsma}, for $A$, suppose $-\infty=w_0<w_1<\dots<w_{2m+1}<+\infty$ satisfies $(w_{2i},w_{2i+1})$ is a~\lar~interval for $0\leq i\leq m$, and $[w_{2i-1},w_{2i}]$ is a~\sma~interval for $1\leq i\leq m$. Then for $\Axa$, $(\srx{a}{c+\ell}{w_{2i}},\srx{a}{c+\ell}{w_{2i+1}})$ is a~\lar~interval for $0\leq i\leq m$, and $[\srx{a}{c+\ell}{w_{2i-1}},\srx{a}{c+\ell}{w_{2i}}]$ is a~\sma~interval for $1\leq i\leq m$.
  
  Suppose $w_{2i_0}=a$ and $w_{2 i_0 +1}=b$. Then $\srx{a}{c+\ell}{a}=a$ and $\srx{a}{c+\ell}{b}=b-2\ell$, and for any $x\in (a,b-2\ell)$, we have 
  \begin{align}
  & \rho_{\Sxa}(x)  \\
  =& \rho_{ \sr{a}{c+\ell}{\funextr{A}{\gamma}{\Sname}} }(x)  \\
  =& \alpha \rho_{\Sname}(x+(c+\ell-a)) \\
  =& e^{-\epsilon (b-x-c-\ell+a) } \alpha \rho_{\Sname}(b) \\
  =& e^{-\epsilon (b-x) } \rho_{ \sr{a}{c+\ell}{\funextr{A}{\gamma}{\Sname}} }(b+a-c-\ell) \\
  =& e^{-\epsilon ((b-2\ell)-x) } \rho_{\Sxa}(b-2\ell), \label{eq:removeslar}
  \end{align}
  where $\alpha=(1-\int_{a}^{c+\ell}\rho_{\Sname}(x)dx)^{-1}$, which is the same as the definition of $\alpha$ in the proof of Lemma \ref{lem:monotoneremoval}. It implies $(a,b-2\ell)$ is a~\slar~interval with respect to $\Axa$.
  
  Note that for $0\leq i\leq m$ and $i\neq i_0$, $(w_{2i},w_{2i+1})$ just shift by 0 or $2\ell$ after removing $[a,c+\ell)$, and the density of $\Sname$ just multiply by $\alpha$ inside the interval, that is, one of the following holds
  \begin{enumerate}
      \item For any $x\in (w_{2i},w_{2i+1})$,
      \begin{align}
          \srx{a}{c+\ell}{x}=x,~~\text{and}~~\rho_{\Sxa}(x)=\alpha\rho_{\funextr{A}{\gamma}{\Sname}}(x) \label{eq:remvshitc1}
      \end{align}
      \item For any $x\in (w_{2i},w_{2i+1})$,
      \begin{align}
          \srx{a}{c+\ell}{x}=x-2\ell,~~\text{and}~~\rho_{\Sxa}(x-2\ell)=\alpha\rho_{\funextr{A}{\gamma}{\Sname}}(x) \label{eq:remvshitc2}
      \end{align}
  \end{enumerate}
  
  As a result, when $i\neq i_0$, $(\srx{a}{c+\ell}{w_{2i}},\srx{a}{c+\ell}{w_{2i+1}})$ is a~\slar~interval with respect to $(\Axa,\funextr{\Axa}{\gamma}{\Sxa})$ if and only if $(w_{2i},w_{2i+1})$ is a~\slar~interval with respect to $(A,\funextr{A}{\gamma}{\Sname})$. As a result, $\funmon{\Axa}{\gamma}{\funextr{\Axa}{\gamma}{\Sxa}}< \funmon{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}$. 
  
  Similarly, for $1\leq i\leq m$, one of the following holds
  \begin{enumerate}
      \item For any $x\in [w_{2i-1},w_{2i}]$,
      \begin{align}
          \srx{a}{c+\ell}{x}=x,~~\text{and}~~\rho_{\Sxa}(x)=\alpha\rho_{\funextr{A}{\gamma}{\Sname}}(x) \label{eq:remvshitc3}
      \end{align}
      \item For any $x\in [w_{2i-1},w_{2i}]$,
      \begin{align}
          \srx{a}{c+\ell}{x}=x-2\ell,~~\text{and}~~\rho_{\Sxa}(x-2\ell)=\alpha\rho_{\funextr{A}{\gamma}{\Sname}}(x) \label{eq:remvshitc4}
      \end{align}
  \end{enumerate}
  
  So $[\srx{a}{c+\ell}{w_{2i-1}},\srx{a}{c+\ell}{w_{2i}}]$ is a~\ssma~interval with respect to $(\Axa,\funextr{\Axa}{\gamma}{\Sxa})$ if and only if $[w_{2i-1},w_{2i}]$ is a~\ssma~interval with respect to $(A,\funextr{A}{\gamma}{\Sname})$. As a result, $\funmonsma{\Axa}{\gamma}{\funextr{\Axa}{\gamma}{\Sxa}}= \funmonsma{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}$. 
  
  Finally, by Corollary \ref{cor:mvalremoval}, we also have $\funnum{\Axa}{\gamma}\leq \funnum{A}{\gamma}$.
  
  
  
  \paragraph{Case 3, $a<c-\ell$ and $b=c+\ell$.}
  
  Using the similar argument as the case when $a=c-\ell$ and $b>c+\ell$, we have $\funnum{\Axa}{\gamma}\leq \funnum{A}{\gamma}$, $\funmonsma{\Axa}{\gamma}{\Sxa}= \funmonsma{A}{\gamma}{\Sname}$,  $\funmon{\Axa}{\gamma}{\Sxa}< \funmon{A}{\gamma}{\Sname}$, and $\funextr{\Axa}{\gamma}{\Sxa}=\Sxa$.
  
  \end{proof}
  


  \begin{lemma}\label{lem:tolaps2}
  
  For $A\in \Kads, \gamma\geq 0, \Sname\in \Srobs$, if
  \begin{enumerate}
      \item $\fung{A}{\Sname}\leq \gamma$,
      \item $\funmon{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}=0$,
      \item $\rho_{\funextr{A}{\gamma}{\Sname}}(x)$ has a minimal point with respect to $x\in \real$,
  \end{enumerate}
  then there exists $\Axa\in \Kads,\Sxa\in \Sname$, so that
  \begin{enumerate}
      \item $\fung{\Axa}{\Sxa}\leq \gamma$.
      \item At least one of the following holds
      \begin{enumerate}
          \item $\max \Axa-\min \Axa \leq (\max A-\min A) - 2\gamma$
          \item $\max \Axa-\min \Axa \leq \max A-\min A$, and $\funnum{\Axa}{\gamma}< \funnum{A}{\Sname}$.
          \item All of the following holds.
          \begin{enumerate}
              \item $\max \Axa-\min \Axa \leq \max A-\min A$.
              \item $\funnum{\Axa}{\gamma}\leq \funnum{A}{\gamma}$.
              \item $\funmonsma{\Axa}{\gamma}{\funextr{A}{\gamma}{\Sxa}}< \funmonsma{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}$.
          \end{enumerate} 
      \end{enumerate}
  \end{enumerate}
  
  \end{lemma}
  
  
  \begin{proof}

  Suppose $x_0$ is a minimal point of $\rho_{\funextr{A}{\gamma}{\Sname}}$ with respect to $x\in \real$. By Corollary \ref{cor:extrexp}, $x_0$ does not belong to the interior of a~\sma~interval. Since $\funmon{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}=0$, according to Definition \ref{def:monlar}, $x_0$ does not belong to the interior of a~\lar~interval. As a result, $x_0$ is at the boundary of a~\sma~interval.
  
  W.l.o.g., we assume there is a~\sma~interval $[x_0,b]$. (Otherwise, the~\sma~interval is $[a,x_0]$, and the proof will be similar.) Then there is also a~\slar~interval $(a,x_0)$. If $a=-\infty$, by Corollary \ref{cor:extrexp}, $x_0$ is not a minimal point, so $a\in \real$. As a result, we can define $s\defeq \max\{x\in A| x\leq x_0\}$ and $t\defeq \min\{x\in A| x\geq x_0\}$. We also define $y\defeq \sup\{ x<x_0 | \rho_{\funextr{A}{\gamma}{\Sname}}(x)\neq e^{\epsilon(x_0-x)}\rho_{\funextr{A}{\gamma}{\Sname}}(x_0) \}$, $z\defeq \inf\{ x>x_0 | \rho_{\funextr{A}{\gamma}{\Sname}}(x)\neq e^{\epsilon(x-x_0)}\rho_{\funextr{A}{\gamma}{\Sname}}(x_0) \}$, $\ell=\min\{x_0-y,z-x_0\}$, and $w=x_0-(s+t)/2$.
  
  For any $\zeta\leq \min\{\gamma,w\}$, $\fung{A}{x_0-\zeta}=\gamma+\zeta$ and $\fung{A}{x_0+\zeta}=\gamma-\zeta$. We define $v\defeq \min\{\ell, \gamma, w\}$, and then for any $\zeta\leq v$, we have
  \begin{align} \label{eq:rmsym}
  \begin{cases}
  \rho_{\funextr{A}{\gamma}{\Sname}}(x_0-\zeta) = \rho_{\funextr{A}{\gamma}{\Sname}}(x_0+\zeta)\\
  \int_{x_0-\zeta}^{x_0+\zeta}\fung{A}{x}\rho_{\funextr{A}{\gamma}{\Sname}}(x)dx = \gamma \int_{x_0-\zeta}^{x_0+\zeta}\rho_{\funextr{A}{\gamma}{\Sname}}(x)dx 
  \end{cases}
  \end{align}
  
  \iffalse
  \begin{figure}
      \centering
        \begin{tikzpicture}
        \draw[<->](3.2,0)--(0,0)--(0,3.2);
        \draw(0,0)--(-1,0);
        \draw[red,domain=-0.2:0.8] plot(\x,4*\x) node at (0.8,3.5){$y=4x$};
        \draw[blue,domain=-1:1] plot(\x,2*\x*\x) node at (1.1,2.2){$y=x^2$};
        \draw[cyan,domain=-1:2,smooth] plot(\x,{0.3*sin(4*\x r)}) node at (2.3,0.6){$y=0.3sin(4x)$};
        \end{tikzpicture}
      \caption{template}
  \end{figure}
  \fi
  
  \begin{figure}
      \centering
        \begin{tikzpicture}
        \coordinate (right) at (10,0);
        \coordinate (o) at (0,0);
        \coordinate (up) at (0,5);
        \coordinate (y) at (3,0);
        \coordinate (z) at (6.5,0);
        \coordinate (x0) at (5,0);
        \coordinate (s) at (2.6,0);
        \coordinate (t) at (6,0);
        \coordinate (ast) at (4.3,0);
        \draw node at ([yshift=-0.3cm]y) {$y$};
        \draw node at ([yshift=-0.3cm]z) {$z$};
        \draw node at ([yshift=-0.3cm]x0) {$x_0$};
        \draw node at ([yshift=-0.3cm]s) {$s$};
        \draw node at ([yshift=-0.3cm]t) {$t$};
        \draw node at ([yshift=-0.3cm]ast) {$\frac{s+t}{2}$};
        \draw[<->](right)--(o)--(up);
        \draw[blue,domain=0.5:1.5] plot(\x,{0.2*exp(3)*exp(-\x)} );
        \draw[blue,domain=1.5:3] plot(\x,{0.2*exp(\x)} );
        \draw[red,dashed](y)--(3,{0.2*exp(3)});
        \draw[blue,domain=3:5] plot(\x,{0.2*exp(3)*exp(-(\x-3))} );
        \draw[blue,domain=5:6.5] plot(\x,{0.2*exp(1)*exp((\x-5))} );
        \draw[red,dashed](z)--(6.5,{0.2*exp(1)*exp((6.5-5))});
        \draw[blue,domain=6.5:9.5] plot(\x,{0.2*exp(2.5)*exp(-(\x-6.5))} );
        \draw[red,dashed](x0)--(5,{0.2*exp(1)});
        \fill (0.5,0) circle (2pt);
        \fill (s) circle (2pt);
        \fill (t) circle (2pt);
        \fill (9,0) circle (2pt);
        \draw[densely dotted] (4.3,-1)--(4.3,4.5)--(5.7,4.5)--(5.7,-1)--cycle;
        \draw node at (6,4.8) {\small maximum scope of $(x_0-\zeta,x_0+\zeta)$};
        \draw[decorate,decoration={brace,raise=1pt,amplitude=3pt},purple] (x0) -- (t) node[black,midway,yshift=9pt] {$\gamma$};
        \draw[decorate,decoration={brace,raise=1pt,amplitude=3pt},purple] (ast) -- (x0) node[black,midway,yshift=9pt] {$w$};
        \draw[decorate,decoration={brace,raise=10pt,amplitude=9pt},purple] (x0) -- (z) node[black,midway,yshift=25pt] {$\ell$};
        \end{tikzpicture}
      \caption{Example for Equation \ref{eq:rmsym}}
  \end{figure}
  
  
  
  
  Let
  \begin{align*}
  \Axa&=\sra{x_0-v}{x_0+v}{A},\\
  \Sxa&=\sr{x_0-v}{x_0+v}{\Sname}.
  \end{align*}
  
  Then $\max \Axa-\min \Axa \leq \max A-\min A$. Since $\fung{A}{\Sname}\leq \gamma$, by Lemma \ref{lem:h}, $\fung{A}{\funextr{A}{\gamma}{\Sname}}\leq \gamma$. Then by Equations \ref{eq:rmsym} and Lemma \ref{lem:monotoneremoval}, we have $\Sxa\in \Srobs$ and $\fung{\Axa}{\Sxa}\leq \gamma$.
  
  
  We have proved part of conclusions of the lemma. To complete the proof, We consider the following several cases.
  
  
  
  
  
  \paragraph{Case 1, $v=w$.}
  
  
  Note that $\srx{x_0-v}{x_0+v}{t}-\srx{x_0-v}{x_0+v}{s}=2\gamma$. By Observation \ref{obs:mcloseform}, $\funnum{\Axa}{\gamma}< \funnum{A}{\gamma}$.
  
  
  
  
  
  \paragraph{Case 2, $v=\gamma$.}
  
  In this case, $\max \Axa-\min \Axa \leq \max A-\min A-2\gamma$.
  
  
  \paragraph{Case 3, $v=\ell$, $v<\gamma$ and $v<w$.}
  
  For $A$, $(s+\gamma, x_0)$ is a~\lar~interval, and suppose $[x_0,r]$ is a~\sma~interval.
  
  Since $\funmon{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}=0$, for $A$, $(s+\gamma, x_0)$ is a~\slar~interval. Note that $\ell<w$, so $z=x_0+\ell$. In summary, as $x\in \real$ increasing, $\rho_{\funextr{A}{\gamma}{\Sname}}(x)$ is decreasing when $x\in (s+\gamma, x_0)$, increasing when $x\in [x_0, z]$, and decreasing when $x\in (z, r)$.
  
  For $\Axa$, $[\srx{x_0-v}{x_0+v}{x_0-2\ell}, \srx{x_0-v}{x_0+v}{r}]$ is a~\sma~interval. Since $\ell<w$, $x_0-2\ell$ is inside the~\slar~interval $(s+\gamma,x_0)$ for $A$. Note that $[x_0, z]$, which is the increasing interval of $\rho_{\funextr{A}{\gamma}{\Sname}}(x)$, is removed by space removal, so $[\srx{x_0-v}{x_0+v}{x_0-2\ell}, \srx{x_0-v}{x_0+v}{r}]$ is a~\ssma~interval for $\Axa$. As a result, we have
  \begin{align*}
      \funmonsma{\Axa}{\gamma}{\funextr{A}{\gamma}{\Sxa}}< \funmonsma{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}.
  \end{align*}
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  \iffalse%%%%%%%%%%%%%%
  \paragraph{Case 3, $\ell< x_0-(s+\gamma)<2\ell$, and $\ell<\gamma$.}
  
  In this case, let
  \begin{align*}
  \Axa&=\sra{x_0-(x_0-(s+\gamma))/2}{x_0+(x_0-(s+\gamma))/2}{A},\\
  \Sxa&=\sr{x_0-(x_0-(s+\gamma))/2}{x_0+(x_0-(s+\gamma))/2}{\Sname}.
  \end{align*}
  
  Then $\max \Axa-\min \Axa \leq \max A-\min A$.
  
  Since $\fung{A}{\Sname}\leq \gamma$, by Equations \ref{eq:rmsym} and Lemma \ref{lem:monotoneremoval}, we have $\Sxa\in \Srobs$ and $\fung{\Axa}{\Sxa}\leq \gamma$.
  
  Note that $\srx{x_0-(x_0-(s+\gamma))/2}{x_0+(x_0-(s+\gamma))/2}{s}=s$ and $\srx{x_0-(x_0-(s+\gamma))/2}{x_0+(x_0-(s+\gamma))/2}{t}=t-(x_0-(s+\gamma))=s+\gamma$. 
  
  
  
  If $A=\{x_1,x_2,\dots,x_{\K}\}$ where $x_1\leq x_2\leq \dots\leq x_{\K}$, then there exists $1\leq i_0<\K$ so that $x_{i_0}=s$ and $x_{i_0+1}=t$. By Lemma \label{lem:mvalremoval}, we have
  \begin{align*}
    & \funnum{A}{\gamma} - \funnum{\Axa}{\gamma}    \\
    =& \sum_{i=1}^{\K -1}\I{\srx{a}{b}{x_{i+1}}-\srx{a}{b}{x_{i}}\leq 2\gamma \text{~and~} x_{i+1}-x_{i}>2\gamma}\\
    \geq & \I{\srx{a}{b}{x_{i_0+1}}-\srx{a}{b}{x_{i_0}}\leq 2\gamma \text{~and~} x_{i_0+1}-x_{i_0}>2\gamma}\\
    = & \I{\srx{a}{b}{t}-\srx{a}{b}{s}\leq 2\gamma \text{~and~} x_{t}-x_{s}>2\gamma}\\
    = & 1,
  \end{align*}
  which implies $\funnum{A}{\gamma} > \funnum{\Axa}{\gamma}$.
  
  
  
  
  
  
  \paragraph{Case 4, $x_0-(s+\gamma)\geq 2\ell$, and $\ell<\gamma$.}
  
  In this case, let
  \begin{align*}
  \Axa&=\sra{x_0-\ell}{x_0+\ell}{A},\\
  \Sxa&=\sr{x_0-\ell}{x_0+\ell}{\Sname}.
  \end{align*}
  
  Then $\max \Axa-\min \Axa \leq \max A-\min A$. By Corollary \ref{cor:mvalremoval}, we also have $\funnum{\Axa}{\gamma}\leq \funnum{A}{\gamma}$.
  
  Since $\fung{A}{\Sname}\leq \gamma$, by Equations \ref{eq:rmsym} and Lemma \ref{lem:monotoneremoval}, we have $\Sxa\in \Srobs$ and $\fung{\Axa}{\Sxa}\leq \gamma$.
  
  
  
  
  
  
  
  
  
  
  
  
  
  According to Definition \ref{def:larsma}, for $A$, suppose $-\infty=w_0<w_1<\dots<w_{2m+1}<+\infty$ satisfies $(w_{2i},w_{2i+1})$ is a~\lar~interval for $0\leq i\leq m$, and $[w_{2i-1},w_{2i}]$ is a~\sma~interval for $1\leq i\leq m$. Then for $\Axa$, $(\srx{x_0-\ell}{x_0-\ell}{w_{2i}},\srx{x_0-\ell}{x_0-\ell}{w_{2i+1}})$ is a~\lar~interval for $0\leq i\leq m$, and $[\srx{x_0-\ell}{x_0-\ell}{w_{2i-1}},\srx{x_0-\ell}{x_0-\ell}{w_{2i}}]$ is a~\sma~interval for $1\leq i\leq m$.
  
  Suppose $w_{2i_0}=s+\gamma$ and $w_{2 i_0 +1}=x_0$. Then $\srx{x_0-\ell}{x_0+\ell}{s+\gamma}=s+\gamma$ and $\srx{x_0-\ell}{x_0+\ell}{x_0}=x_0-2\ell$. Besides, we use $q$ to denote $\srx{x_0-\ell}{x_0+\ell}{w_{2i_0 +2}}$, which equals to $(w_{2i_0 +2}-2\ell)$. Then with respect to $\Axa$, $(s+\gamma,x_0-2\ell)$ is a~\lar~interval, and $[x_0-2\ell,q]$ is a~\sma~interval. 
  
  By Corollary \ref{cor:extrexp}, for any $x\in [x_0-\ell,q]$, we have
  \begin{align}
      &\rho_{\Sxa}(x) \label{eq:explfixs} \\
      =&\rho_{\funextr{A}{\gamma}{\Sname}}(x+2\ell)\\
      =&e^{\epsilon(w_{2i_0 +2}-(x+2\ell))}\rho_{\funextr{A}{\gamma}{\Sname}}(w_{2i_0 +2})    \label{eq:expsmalfix}  \\
      =& e^{\epsilon(q-x)}\rho_{\Sxa}(q) ,
  \end{align}
  where Equation \ref{eq:expsmalfix} holds because $\ell$ should be larger if it does not hold.
  
  At the same time, for any $x\in [x-2\ell,x_0-\ell]$, we have
  \begin{align}
      &\rho_{\Sxa}(x)\\
      =&\rho_{\funextr{A}{\gamma}{\Sname}}(x)\\
      =& e^{\epsilon(x_0-\ell-x)} \rho_{\funextr{A}{\gamma}{\Sname}}(x_0-\ell)\label{eq:explarlfix1}  \\
      =& e^{\epsilon(x_0-\ell-x)} \rho_{\funextr{A}{\gamma}{\Sname}}(x_0+\ell) \\
      =& e^{\epsilon(x_0-\ell-x)} \rho_{\Sxa}(x_0-\ell) \\
      =& e^{\epsilon(q-x)} \rho_{\Sxa}(q), \label{eq:explfixt}
  \end{align}
  where Equation \ref{eq:explarlfix1} holds because $(s+\gamma,x_0)$ is a~\lar~interval with respect to $A$, and $x_0$ is a minimal point of $\rho_{\funextr{A}{\gamma}{\Sname}}(x)$.
  
  By Equations \ref{eq:explfixs} to \ref{eq:explfixt}, $\Sxa$ and $\funextr{\Axa}{\gamma}{\Sxa}$ have the same probability density in $[x-2\ell,q]$, and  $[x-2\ell,q]$ is a~\ssma~interval with respect to $(\Axa,\funextr{\Axa}{\gamma}{\Sxa})$. In contrast, $[x-\ell,w_{2i_0 +2}]$ is not a~\ssma~interval with respect to $(A,\Sname)$, otherwise $\ell$ should be larger.
  
  
  Besides, for $1\leq i\leq m$, where $i\neq i_0+1$, one of the following holds
  \begin{enumerate}
      \item For any $x\in [w_{2i-1},w_{2i}]$,
      \begin{align}
          \srx{a}{c+\ell}{x}=x,~~\text{and}~~\rho_{\Sxa}(x)=\alpha\rho_{\funextr{A}{\gamma}{\Sname}}(x) \label{eq:remvshitc3}
      \end{align}
      \item For any $x\in [w_{2i-1},w_{2i}]$,
      \begin{align}
          \srx{a}{c+\ell}{x}=x-2\ell,~~\text{and}~~\rho_{\Sxa}(x-2\ell)=\alpha\rho_{\funextr{A}{\gamma}{\Sname}}(x) \label{eq:remvshitc4}
      \end{align}
  \end{enumerate}
  where $\alpha=(1-\int_{x_0-\ell}^{x_0+\ell}\rho_{\Sname}(x)dx)^{-1}$, which is the same as the definition of $\alpha$ in the proof of Lemma \ref{lem:monotoneremoval}.
  
  So $[\srx{x_0-\ell}{x_0+\ell}{w_{2i-1}},\srx{x_0-\ell}{x_0+\ell}{w_{2i}}]$ is a~\ssma~interval with respect to $(\Axa,\funextr{\Axa}{\gamma}{\Sxa})$ if and only if $[w_{2i-1},w_{2i}]$ is a~\ssma~interval with respect to $(A,\funextr{A}{\gamma}{\Sname})$. As a result, 
  \begin{align*}
      \funmonsma{\Axa}{\gamma}{\funextr{\Axa}{\gamma}{\Sxa}}< \funmonsma{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}. 
  \end{align*}
  
  \fi%%%%%%%%%%%%%%%%%%%%
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  
  \end{proof}
  
  
  
  
  
  
  \begin{lemma}\label{lem:tolaps3}
  
  For $A\in \Kads, \gamma\geq 0, \Sname\in \Srobs$, if $\fung{A}{\Sname}\leq \gamma$ and $\rho_{\funextr{A}{\gamma}{\Sname}}(x)$ does not have a minimal point with respect to $x\in \real$, then there exists $\Axa$ so that $\fung{\Axa}{\Lap}\leq \gamma$.
  
  \end{lemma}

  
  \begin{proof}
  
  According Corollary \ref{cor:extrexp}, if $\rho_{\funextr{A}{\gamma}{\Sname}}(x)$ does not have a minimal point with respect to $x\in \real$, then
  \begin{align*}
      \rho_{\funextr{A}{\gamma}{\Sname}}(x)=e^{-\epsilon\cdot \disr{x}{c}}\rho_{\funextr{A}{\gamma}{\Sname}}(c)
  \end{align*}
  for a certain $c\in \real$.

  Then $\rho_{\funextr{A}{\gamma}{\Sname}}(x+c)=\rho_{\Lap}(x)$. Let $\Axa=A-c$, and we have
  \begin{align*}
  \fung{\Axa}{\Lap}
  =& \int_{x\in \real} \rho_{\Lap}(x) \fung{\Axa}{x} dx  \\
  =& \int_{x\in \real} \rho_{\funextr{A}{\gamma}{\Sname}}(x+c) \fung{\Axa+c}{x+c} dx  \\
  =& \fung{A}{\funextr{A}{\gamma}{\Sname}}  \\
  \leq & \fung{A}{\Sname},
  \end{align*}
  which implies the lemma.
  
  \end{proof}
  
  \begin{lemma} \label{lem:lapoptx}
  
  For any $A\in \Kads$, $\Sname\in \Srobs$, there exists $\Axa\in \Kads$ so that $\fung{\Axa}{\Lap}\leq \fung{A}{\Sname}$.
  
  \end{lemma}



\begin{algorithm}
\caption{Adjust distribution}\label{alg:cap}
\begin{algorithmic}[1]
\State Input: $A\in \Kads$, $\Sname\in \Srobs$.
\State $\Axb\gets A, \Sxb\gets \Sname$.
\While{$\Sxb \neq \Lap$}
\If{$\funmon{A}{\gamma}{\funextr{A}{\gamma}{\Sname}}>0$}
    \State Apply Lemma \ref{lem:tolaps1} on $\Axb,\Sxb$.
\ElsIf{$\rho_{\funextr{A}{\gamma}{\Sname}}(x)$ has a minimal point with respect to $x\in \real$}
    \State Apply Lemma \ref{lem:tolaps2} on $\Axb,\Sxb$.
\Else
    \State Apply Lemma \ref{lem:tolaps3} on $\Axb,\Sxb$.
\EndIf
\EndWhile
    \Comment{When leaving the while loop, $\Sxb=\Lap$.}
\State $\Axa\gets \Axb$.
    \Comment{$\Axa$ satisfies $\fung{\Axa}{\Lap}\leq \fung{A}{\Sname}$, which is stated in the lemma.}
\end{algorithmic}
\end{algorithm}
  
  
  \begin{proof}

  We can adjust $(A,\Sname)$ to be $(\Axa,\Lap)$ without increasing $\fung{A}{\Sname}$ by Algorithm \ref{alg:cap}.
  
  Let $\gamma=\fung{A}{\Sname}$. We define a potential function $\phi(\Axb,\Sxb)$ to be the tuple
  \begin{align*}
      ( \lfloor  (\max \Axb - \min \Axb)/(2\gamma) \rfloor , \funnum{A}{\gamma}, \funmonsma{\Axb}{\gamma}{\funextr{\Axb}{\gamma}{\Sxb}}, \funmon{\Axb}{\gamma}{\funextr{\Axb}{\gamma}{\Sxb}} ).
  \end{align*} For two tuple $X=(x_1,x_2,x_3,x_4)$ and $Y=(y_1,y_2,y_3,y_4)$, we compare them according to lexicographical order. That is, $X=Y$ if $x_i=y_i$ for any $1\leq i\leq 4$. And $X<Y$ if $x_j<y_j$ for a certain $1\leq j\leq 4$ and $x_i=y_i$ for any $1\leq i< j$.
  
  Initially, let $\Axb=A,\Sxb=\Sname$. Then we keep $\fung{\Axb}{\Sname}\leq \gamma$ holding and decrease $\phi(\Axb,\Sxb)$ until $\Sxb=\Lap$. Note that $(\Axb,\Sxb)$ satisfies the precondition of one of Lemmas \ref{lem:tolaps1}, \ref{lem:tolaps2} and \ref{lem:tolaps3} (as $(A,\Sname)$ in those lemmas), so we can update $(\Axb,\Sxb)$ using the lemma (updated value is $(\Axa,\Sxa)$ in those lemmas). After calling Lemma \ref{lem:tolaps3}, $\Sxb$ becomes $\Lap$, which implies have $\fung{\Axb}{\Lap}\leq \fung{A}{\Sname}$, so we can let $\Axa=\Axb$. When calling Lemmas \ref{lem:tolaps1} or \ref{lem:tolaps2}, $\phi(\Axb,\Sxb)$ strictly decrease.
  
  Since $\lfloor  (\max A - \min A)/(2\gamma) \rfloor$ is finite, $\funnum{\Axb}{\gamma}\leq \K$ for any $\Axb\in \Kads$, $\funmonsma{\Axb}{\gamma}{\funextr{\Axb}{\gamma}{\Sxb}}\leq \funnum{\Axb}{\gamma}\leq \K$ for any $\Axb\in \Kads, \Sxb\in \Srobs$, and $\funmon{\Axb}{\gamma}{\funextr{\Axb}{\gamma}{\Sxb}}\leq \funnum{\Axb}{\gamma}+1\leq \K +1$, after finite times of calling Lemmas \ref{lem:tolaps1} or \ref{lem:tolaps2}, Lemma \ref{lem:tolaps3} is called, which means we can finally get $\Axa$ satisfying $\fung{\Axa}{\Lap}\leq \fung{A}{\Sname}$.
  
  
  \end{proof}



  
  
  
  Equation \ref{eq:suff:lapopt} is a corollary of Lemma \ref{lem:lapoptx}, so Theorem \ref{thm:lapopt} is proved.









==> intro.tex <==
\section{Introduction}
Consider a user who wants to issue a query to an online server (e.g. to retrieve a search result or an advertisement), but the query itself reveals private information. Hence, the user might add noise to the query to get some privacy protection; and for a rigorous privacy guarantee, the noise should satisfy differential privacy under the local trust model~ \cite{bebensee2019local}. There is a large and growing literature in differential privacy that analyzes the privacy guarantees provided by various noise mechanisms, and the resultant decrease in the quality of the computed result (see \cite{Xiong2020} for a survey). In particular, for personalized individual queries, such as search, the poor privacy-utility trade-offs of the current state-of-the-art local differentially private mechanisms prevent their practical use.

% often studied as \textit{list learning} \cite{10.1145/3564246.3585190,10.1007/3-540-60454-5_42} in \textit{Probably Approximately Correct} (PAC) framework

We observe that in many situations such as search results or ad delivery, the server is free to return many results, and the user can choose the one that is the most appropriate. In fact, if the server also returns a model for evaluating the quality of these results for the user, then this choice can be made by a software intermediary such as a client running on the user's device. This software intermediary can also be the one that adds the noise to the query, and hence acts as the user's privacy delegate. In applications where the server does not need to know which of the returned results was ultimately chosen by the privacy delegate\footnote{E.g. in search when the goal is only to provide a good search experience, without trying to improve the ranking models based on user activity or in advertising charged per impression, not click.}, any improvement in search or ad quality obtained thanks to the server returning multiple results comes without any privacy trade-off, at least in the stylized model described above.

We call this, new for the differential privacy literature system architecture, the ``Multi-Selection'' approach to privacy, and the key question we ask is: {\em What is the precise trade-off between the number of returned results and quality, and how can this trade-off be achieved?} Of course, had the server simply returned all possible results, there is no loss in quality since the client can choose the optimal result. However, this is infeasible for several reasons -- first, the client's device could be constrained by battery or memory; second, the server also needs to send its model for evaluating the quality of the results and this can be large; and finally, returning all results (such as ads) could compromise proprietary information. We therefore restrict the server to return $k$ results for small $k$, and ask for the tradeoff between $k$ and the quality when the client adds noise to its query that is privacy preserving.

Although variants of this approach have been suggested (particularly in cryptographic contexts~\cite{toubiana2010adnostic}), to the best of our knowledge, no formal results are known on whether this approach does well in terms of reducing the ``price of \textbf{differential} privacy'', or how to obtain the optimal privacy-quality trade-offs. Given the dramatic increase in network bandwidth and on-device compute capabilities of the last several decades, this approach has the potential to offer an attractive pathway to reducing the ``cost of privacy'', and making local differentially privacy practical for personalized individual queries.

\input{relatedak}

\subsection{Multi-Selection Architecture and Model}
In this work, we ask whether we can overcome the above challenges not by relaxing the privacy definition, but by introducing a conceptually different system architecture design. Our ``multi-selection" approach relies on the server returning a small set of results in response to the privatized user input, with the on-device software intermediary deciding, unbeknownst to the server, which of these server responses to use.  This new system architecture, shown in \cref{fig:arch1} is made possible by advances in the reduction of communication costs and power of on-device computation.  In a stylized model, we show theoretically that this new system design enables  new algorithms whose privacy cost on utility is lower than in the traditional local model of DP.

\definecolor{usr}{rgb}{0.7,0.85,1.0}
\definecolor{usrl}{rgb}{0.9,0.95,1.0}
\definecolor{usrline}{rgb}{0.8,0.9,1.0}
\definecolor{sev}{rgb}{1.0,0.85,0.7}
\definecolor{sevl}{rgb}{1.0,0.95,0.9}
\definecolor{sevline}{rgb}{1.0,0.9,0.8}

  \begin{figure}[htbp]
      \centering
      \tikzset{global scale/.style={
            scale=#1,
            every node/.append style={scale=#1}
          }
        }
        \begin{tikzpicture}[global scale = 0.8]

        
         \node[fill=usrl,draw=usrline,rounded corners, minimum width=10cm, minimum height=3cm] at (2.5,2) {};
         
         \node at (2.5,3.8) {Client};
        
         \node[fill=usr,draw,rounded corners, minimum width=3cm, minimum height=1.5cm] at (0,2) {\bf User};
         
         \node[fill=usr,draw,rounded corners, minimum width=3cm, minimum height=1.5cm,align=center] at (5,2) {\bf User Agent \\ e.g. browser};

         
         \node[fill=sevl,draw=sevline,rounded corners, minimum width=5cm, minimum height=3cm] at (11.5,2) {};
         
         \node at (11.5,3.8) {Server};
         \node[fill=sev,draw,rounded corners, minimum width=4cm, minimum height=1.5cm] at (11.5,2) {\bf Result Computation};

         
         \draw[->] (1.5,2.25) -- (3.5,2.25);         \draw[<-] (1.5,1.75) -- (3.5,1.75);         \draw[->] (6.5,2.25) -- (9.5,2.25);         \draw[<-] (6.5,1.75) -- (9.5,1.75);

         \node at (2.5,2.5) {features};
         \node at (2.5,1.5) {best result};
         \node at (8,2.5) {signal with noise};
         \node at (8,1.5) {a set of $k$ results};

         
        \end{tikzpicture}
      \caption{Overall architecture for multi-selection.}    \label{fig:arch1}
  \end{figure}

Concretely, we will analyze the privacy-accuracy trade-off in the simplest scenario -- when the user's query as well as the search results are one-dimensional, every point is a valid query and a valid search result (or an advertisement), and the ``cost" of a search result is measured by the distance between the original query and the result. We will assume that the server has no distributional information on the original query beyond what it can infer from the noisy version. We will further assume the user can send an arbitrary signal to the server, and the server returns a set of $k$ results to the user. As mentioned before, for practical considerations like device memory and battery life, we want the number of returned results, $k$, to be as small as possible.   

The central question we study can now be phrased as:
\begin{quote}
\noindent \textit{What should the user's privacy-preserving signal be, and what is the optimal set of $k$ results to send given this signal so that the client's accuracy for its true query is maximized when it chooses the best of the returned results. }
\end{quote}

Our model is quite stylized in two senses: First, we are assuming the client shares a common model with the server and can easily infer which of the $k$ returned results is optimal. Second, we are assuming the model itself is a one-dimensional line.  However, this stylized setting captures the {\em essence} of the trade-off between $k$ and accuracy we seek to study. Indeed, even here, the multi-selection problem is non-trivial since we need to provide both the privacy-preserving noise mechanism for the client and the server's response. The latter has dimension $k$, the number of returned results. This makes even writing the privacy-accuracy trade-off as a linear program non-trivial. As we show below, there are settings where the optimal mechanism for given $k$ can be non-intuitive. %At the same time, the new system architecture is an opportunity to improve utility as we can design both the noise mechanism and the response.
%\ak{At the same time, the new system architecture is an opportunity to improve utility as we can design both the noise mechanism and the response.}



%\todo{Is this text ok?}
%We note that though the one-dimensional setting is somewhat stylized, the server could reduce multi-dimensional features to a small collection of independent one-dimensional features via dimensionality reduction methods like PCA, which can be common knowledge between the server and the client. Assuming a cost function such as the squared Euclidean norm that is separable across dimensions, with such a reduction, the mechanism can be run separately for each dimension.

%We study the privacy-accuracy trade-off under two canonical models for differential privacy: the ``geographic differential privacy'', where the privacy parameter decays as $\epsilon/R$ for two users separated by distance $R$, and the ``local differential privacy'', where the privacy parameter $\epsilon$ is independent of the distance between users. In the geographic model, we assume users lie on an infinite dimensional line. In the local model, we consider users on a ring. The doubly infinite line is natural for geographic DP, since its canonical example is location. However, local DP only makes sense in a bounded domain, hence the ring is the natural example to analyze in that model.


We study the privacy-accuracy trade-off under ``geographic differential privacy`` model where the privacy parameter decays as $\epsilon/R$ for two users separated by $R$. In our geographic model of differential privacy, we assume users lie on an infinite dimensional line.  




==> intro_modified.tex <==
\section{Introduction}
Consider a user who wants to issue a query to an online server (e.g. to retrieve a search result or an advertisement), but the query itself reveals private information. One commonly studied approach is to send noisy queries satisfying local differential privacy under the local trust model~ \cite{bebensee2019local}. There is a large and growing literature in differential privacy that analyzes the privacy guarantees provided by various noise mechanisms, and the resultant decrease in the quality of the computed result (see \cite{Xiong2020} for a survey). However, the strong privacy constraints in state-of-the-art local differential privacy mechanisms often imply poor privacy utility trade-offs limiting their practical use.% for personalized queries.


%In particular, for personalized individual queries, such as search, the poor privacy-utility trade-offs of the current state-of-the-art local differentially private mechanisms prevent their practical use.


%Hence, the user might add noise to the query to get some privacy protection; and for a rigorous privacy guarantee, the noise should satisfy differential privacy under the local trust model~ \cite{bebensee2019local}. There is a large and growing literature in differential privacy that analyzes the privacy guarantees provided by various noise mechanisms, and the resultant decrease in the quality of the computed result (see \cite{Xiong2020} for a survey). In particular, for personalized individual queries, such as search, the poor privacy-utility trade-offs of the current state-of-the-art local differentially private mechanisms prevent their practical use.

% often studied as \textit{list learning} \cite{10.1145/3564246.3585190,10.1007/3-540-60454-5_42} in \textit{Probably Approximately Correct} (PAC) framework

Our key observation in many situations such as search results or ad delivery, the server is free to return many results, and the user can choose the one that is the most appropriate. In fact, if the server also returns a model for evaluating the quality of these results for the user, then this choice can be made by a software intermediary such as a client running on the user's device. This software intermediary can also be the one that adds the noise to the query and hence acts as the user's privacy delegate. In applications where the server does not need to know which of the returned results was ultimately chosen by the privacy delegate\footnote{E.g. in search when the goal is only to provide a good search experience, without trying to improve the ranking models based on user activity or in advertising charged per group, not click.}, any improvement in search or ad quality obtained thanks to the server returning multiple results comes without any privacy trade-off, at least in the stylized model described above. 

We call this, new for the differential privacy literature system architecture, the ``Multi-Selection'' approach to privacy, and the key question we ask is: {\em What is the precise trade-off that can be achieved between the number of returned results and quality}? Of course, had the server simply returned all possible results, there would have been no loss in quality since the client could choose the optimal result. However, this is infeasible for several reasons -- first, the client's device could be constrained by battery or memory; second, the server also needs to send its model for evaluating the quality of the results and this can be large; and finally, returning all results (such as ads) could compromise proprietary information. We therefore restrict the server to return $k$ results for small $k$, and ask for the tradeoff between $k$ and the quality when the client sends privacy-preserving noisy queries.

Although variants of this approach have been suggested (particularly in cryptographic contexts~\cite{toubiana2010adnostic}), to the best of our knowledge, no formal results are known on whether this approach does well in terms of reducing the ``price of \textbf{differential} privacy'', or how to obtain the optimal privacy-quality trade-offs. Given the dramatic increase in network bandwidth and on-device compute capabilities of the last several decades, this approach has the potential to offer an attractive pathway to reducing the ``cost of privacy'', and making local differential privacy practical for personalized individual queries.

\input{relatedak}

\subsection{Multi-Selection Architecture and Model}

In this work, we ask whether we can overcome the above challenges not by relaxing the privacy definition, but by introducing a conceptually different system architecture design. Our ``multi-selection" approach relies on the server returning a small set of results in response to the privatized user input, with the on-device software intermediary deciding, unbeknownst to the server, which of these server responses to use.  This new system architecture, shown in \cref{fig:arch1} is made possible by advances in the reduction of communication costs and power of on-device computation.  In a stylized model, we show theoretically that this new system design enables new algorithms whose privacy cost on utility is lower than in the traditional local trust model. %model of DP

\definecolor{usr}{rgb}{0.7,0.85,1.0}
\definecolor{usrl}{rgb}{0.9,0.95,1.0}
\definecolor{usrline}{rgb}{0.8,0.9,1.0}
\definecolor{sev}{rgb}{1.0,0.85,0.7}
\definecolor{sevl}{rgb}{1.0,0.95,0.9}
\definecolor{sevline}{rgb}{1.0,0.9,0.8}

  \begin{figure}[htbp]
      \centering
      \tikzset{global scale/.style={
            scale=#1,
            every node/.append style={scale=#1}
          }
        }
        \begin{tikzpicture}[global scale = 0.8]

        
         \node[fill=usrl,draw=usrline,rounded corners, minimum width=10cm, minimum height=3cm] at (2.5,2) {};
         
         \node at (2.5,3.8) {Client};
        
         \node[fill=usr,draw,rounded corners, minimum width=3cm, minimum height=1.5cm] at (0,2) {\bf User};
         
         \node[fill=usr,draw,rounded corners, minimum width=3cm, minimum height=1.5cm,align=center] at (5,2) {\bf User Agent \\ e.g. browser};

         
         \node[fill=sevl,draw=sevline,rounded corners, minimum width=5cm, minimum height=3cm] at (11.5,2) {};
         
         \node at (11.5,3.8) {Server};
         \node[fill=sev,draw,rounded corners, minimum width=4cm, minimum height=1.5cm] at (11.5,2) {\bf Result Computation};

         
         \draw[->] (1.5,2.25) -- (3.5,2.25);         \draw[<-] (1.5,1.75) -- (3.5,1.75);         \draw[->] (6.5,2.25) -- (9.5,2.25);         \draw[<-] (6.5,1.75) -- (9.5,1.75);

         \node at (2.5,2.5) {features};
         \node at (2.5,1.5) {best result};
         \node at (8,2.5) {signal with noise};
         \node at (8,1.5) {a set of $k$ results};

         
        \end{tikzpicture}
      \caption{Overall architecture for multi-selection.}    \label{fig:arch1}
  \end{figure}

%Concretely, we will analyze the privacy-accuracy trade-off in the simplest scenario -- when the user's query, as well as the search results, are one-dimensional, every point is a valid query and a valid search result (or an advertisement), and the ``cost" of a search result is measured by the distance between the original query and the result. 
Concretely, we will analyze the privacy-accuracy trade-off in the simplest scenario -- when the user's query is one-dimensional, every point is a valid search query and the ``cost''(disutility) of a search result $s$ for an user $u$ is given by the minimum distance to an user $u'$ such that search result $s$ is the optimum for user $u'$. \remove{measured by the minimum distance an user needs to move to make the search result $s$ its optimum. }\ak{This is not clear}
We will assume that the server has no distributional information on the original query beyond what it can infer from the noisy query. 
We will further assume the user can send an arbitrary signal to the server, and the server returns a set of $k$ results to the user. As mentioned before, for practical considerations like device memory and battery life, as well as the server's desire to not reveal proprietary information, we want the number of returned results, $k$, to be as small as possible.   

The central question we study can now be phrased as:
\begin{quote}
\noindent \textit{What should the user's privacy-preserving signal be, and what is the optimal set of $k$ results to send given this signal so that the client's accuracy for its true query is maximized when it chooses the best of the returned results. }
\end{quote}

Our model is quite stylized in two ways: First, we are assuming the client shares a common model with the server and can easily infer which of the $k$ returned results is optimal. Second, we are assuming that the users and queries \ak{->queries?} lie on a one-dimensional line. To relax the one-dimensional assumption, one can refer to Appendix \ref{sec-appendix:high-dim-space}. However, this stylized setting captures the {\em essence} of the trade-off between $k$ and accuracy we seek to study. Indeed, even here, the multi-selection problem is non-trivial since we need to provide both the privacy-preserving noise mechanism for the client and the server's response. The latter has dimension $k$, the number of returned results. 
This makes even writing the privacy-accuracy trade-off as an optimization program non-trivial as we may need to optimize over a distribution and the set of $k$ results. \ak{We got to the need to write it as an LP with no context... Need to first write about a typical solution as an LP}
As we show below, there are settings where the optimal mechanism for a given $k$ can be non-intuitive. %At the same time, the new system architecture is an opportunity to improve utility as we can design both the noise mechanism and the response.
%\ak{At the same time, the new system architecture is an opportunity to improve utility as we can design both the noise mechanism and the response.}



%\todo{Is this text ok?}
%We note that though the one-dimensional setting is somewhat stylized, the server could reduce multi-dimensional features to a small collection of independent one-dimensional features via dimensionality reduction methods like PCA, which can be common knowledge between the server and the client. Assuming a cost function such as the squared Euclidean norm that is separable across dimensions, with such a reduction, the mechanism can be run separately for each dimension.

%We study the privacy-accuracy trade-off under two canonical models for differential privacy: the ``geographic differential privacy'', where the privacy parameter decays as $\epsilon/R$ for two users separated by distance $R$, and the ``local differential privacy'', where the privacy parameter $\epsilon$ is independent of the distance between users. In the geographic model, we assume users lie on an infinite dimensional line. In the local model, we consider users on a ring. The doubly infinite line is natural for geographic DP, since its canonical example is location. However, local DP only makes sense in a bounded domain, hence the ring is the natural example to analyze in that model.


While the multi-selection approach is broadly applicable, we study the privacy-accuracy trade-off under the ``geographic differential privacy'' model where the privacy parameter increases as $\epsilon R$ for two users separated by $R$. In appendix \ref{sec:diff-privacy-gen}, we also study a model where the privacy parameter decays as $\epsilon \mathfrak{f}(R)$ for some convex increasing non-negative function $\mathfrak{f}(.)$. In our geographic model of differential privacy, we assume users lie on an infinite dimensional line and the dis-utility of a user from a result is measured with respect to a monotonically increasing non-negative function $\mathfrak{h}(.)$




==> intro_modified_focs.tex <==
\section{Introduction}{\label{sec:introduction_setup}}
Consider a user who wants to issue a query to an online server (e.g. to retrieve a search result or an advertisement), but the query itself reveals private information about the use. One commonly studied approach to protect user privacy from the server in this context is for the user to send a perturbed query, satisfying differential privacy under the local trust model~ \cite{bebensee2019local}. However, since the query itself is changed from the original, the server may not be able to return a result that is very accurate for the original query. 
Our key observation is that in many situations such as search or content recommendations, the server is free to return many results, and the user can choose the one that is the most appropriate, without revealing the choice to the server. 
In fact, if the server also returns a model for evaluating the quality of these results for the user, then this choice can be made by a software intermediary such as a client running on the user's device. This software intermediary can also be the one that acts as the user's privacy delegate and is the one ensuring the local differential privacy protection.  


%There is a large and growing literature in differential privacy that analyzes the privacy guarantees provided by various noise mechanisms, and the resultant decrease in the quality of the computed result (see \cite{Xiong2020} for a survey). However, the strong privacy constraints in state-of-the-art local differential privacy mechanisms often imply poor privacy utility trade-offs limiting their practical use.% for personalized queries.

%Our key observation in many situations such as search results or ad delivery, the server is free to return many results, and the user can choose the one that is the most appropriate. In fact, if the server also returns a model for evaluating the quality of these results for the user, then this choice can be made by a software intermediary such as a client running on the user's device. This software intermediary can also be the one that adds the noise to the query and hence acts as the user's privacy delegate. In applications where the server does not need to know which of the returned results was ultimately chosen by the privacy delegate\footnote{E.g. in search when the goal is only to provide a good search experience, without trying to improve the ranking models based on user activity or in advertising charged per group, not click.}, any improvement in search or ad quality obtained thanks to the server returning multiple results comes without any privacy trade-off, at least in the stylized model described above. 

We call this, new for the differential privacy (DP) literature system architecture, the ``Multi-Selection'' approach to privacy, and the key question we ask is: {\em What is the precise trade-off that can be achieved between the number of returned results and quality under a fixed privacy goal}? Of course, had the server simply returned all possible results, there would have been no loss in quality since the client could choose the optimal result. However, this approach is infeasible due to computation and communication costs, as well as due to potential server interest in not revealing proprietary information. 
We therefore restrict the server to return $k$ results for small $k$, and study the trade-off between $k$ and the quality when the client sends privacy-preserving  queries. Our algorithmic design space consists of choosing the client's algorithm and the server's algorithm, as well as the space of signals they'll be sending.

We now introduce some notation. We denote the set of users by $\mathbb{R}$ and when we refer to an user $u \in \mathbb{R}$, we mean an user with a value $u \in \mathbb{R}$. Let $M$ denote the set of results and $\text{OPT}: \mathbb{R} \rightarrow M$ denotes the function
which maps users to optimal results. This function $\text{OPT}$ is available (known) to the server but is unknown to the users.  

\ak{I think it's still more elegant to talk about users having values, and not to introduce the ad.}
% We now introduce some notation. Let us denote the set of users by $U$ which is embedded in a metric space given by $(d,U)$ and let $M$ denote the set of results. $\text{OPT}: U \rightarrow M$ denotes the function which maps users to the optimal result. This function $\text{OPT}$ is available (known) to the server but is unknown to the users.  \ak{I think it's still more elegant to talk about users having values, and not to introduce the ad.}

 %The second condition is required for mathematical analysis. \sss{Look into it later}

\ak{Need motivation for why disutility is defined this way? It doesn't correspond to "let's see how the returned search result differs from the optimal search result"... Also, why call it disutility and not error? Finally, under what assumptions does $u': OPT(u')=m$ always exist?}

\sss{Gave two examples where such a definition of dis-utility maybe useful.}

\sss{If $u': OPT(u')=m$ does not exist, the set is a null set and the infimum of a null set is $+\infty$}

We now define the dis-utility of an user $u \in \mathbb{R}$ from a result $m \in M$ in Definition \ref{def:disutility_user_result}. Observe that though there is a notion of distance between the users, there may not be a notion of distance between elements in $M$ and thus we may not always be able to define the dis-utility as some function of distance between $\text{OPT}(u)$ and $m$. Further, we present examples  \ref{example:definition_first} and \ref{example:definition_second} to  justify this definition of dis-utility.

\begin{definition}{\label{def:disutility_user_result}}
    Dis-utility of user $u \in \mathbb{R}$ from result $m \in M$: The dis-utility of a user $u\in \mathbb{R}$ from a result $m\in M$ w.r.t some continuously increasing function $\mathfrak{h}(.)$ is given by \footnote{If no such $u'$ exists then the dis-utility is $\infty$ as infimum of a null set is $\infty$.}
    \begin{equation}{\label{eqn:disutil_user_result}}
        \Disutility^{\mathfrak{h}(.)}(u,m) := \inf\limits_{u'\in \mathbb{R}: OPT(u')=m} \mathfrak{h}(|u-u'|)
        %
    \end{equation}%\footnote{If no such $u'$ exists then the disutility is defined to be $\infty$.}
\end{definition}

We now give conditions on a monotonically function $\mathfrak{h}(.)$ that we use to measure the disutility of a user $u \in \mathbb{R}$ from a result $m \in M$. Observe that the first condition \eqref{item:first-propertyh} captures the intuition that dis-utility for the optimal result is zero. The second condition \eqref{item:second-property-h} which bounds the growth of $\mathfrak{h}(.)$ by an exponential function is required for our mathematical analysis but is not very restrictive. Observe that ratios of polynomials and exponential functions like $\sqrt{z},z^2, e^{z}-1$ satisfy the second criterion, however functions like $e^{z^2}-1$ do not.

\ak{Move the reasons for why we need the conditions here: first condition captures the intuitive notion that disutility for the optimal result should be zero, and the second condition is required for our mathematical analyses (but is not very restrictive...?}
\sss{Done}
\begin{align}
     \text{ $\mathfrak{h}(.)$ is a continuously increasing function satisfying $\mathfrak{h}(0)=0$. }\label{item:first-propertyh}\\
    \text{ There exists $\mathcal{B} \in \real^{+}$ s.t. $\log \mathfrak{h}(.)$ is Lipschitz continuous in $[\mathcal{B},\infty)$} \label{item:second-property-h} 
\end{align}
%\zhihao{Do we need the labels above?} \sss{We use it now.}

We now give two examples below where such a definition of dis-utility maybe helpful.

\begin{example}{\label{example:definition_first}}
    Consider a setup where user $u \in \mathbb{R}$ is physically located at position $u$ in the real line. One may relate this to different geographic locations. An user queries a server to get information about its location, for example an user may ask for information about nearby tourist places or restaurants at its location $u$. Thus, one may interpret the function $\text{OPT}$ as the function which maps a location $u$ to information about location $u$. 

    Suppose an user $u \in \mathbb{R}$ receives information from the server about location $u'$. In this case, one may interpret the dis-utility of user $u$ as $\mathfrak{h}(|u-u'|)$ where $\mathfrak{h}(.)$ captures how the dis-utility of an user scales with the distance which is in line with the Definition \ref{def:disutility_user_result}. $\mathfrak{h}(t) = t \text{ or } \sqrt{t}$ could be some examples how the dis-utility of an user scales with the distance. 
    \sss{Read once}
\end{example}


\begin{example}{\label{example:definition_second}}
    We now consider a setup where the results are embedded in some higher dimension space with dimension $\hat{d}$ i.e. $M \subseteq \mathbb{R}^{\hat{d}}$ and consider the case where $\mathfrak{h}(t)=t$. Suppose, the function $\text{OPT}$ is bi-Lipschitz continuous i.e. $|\text{OPT}(u) - \text{OPT}(u')|_1 \leq k^{(1)}|u-u'|$ and $|\text{OPT}(u) - \text{OPT}(u')|_1 \geq k^{(2)}|u-u'|$. 

    Thus, one may argue that $\Disutility^{\mathfrak{h}(.)}(u,\text{OPT}(u')) \leq \frac{1}{k^{(2)}} |\text{OPT}(u)-\text{OPT}(u')|_1$ \newline and $\Disutility^{\mathfrak{h}(.)}(u,\text{OPT}(u')) \geq \frac{1}{k^{(1)}} |\text{OPT}(u)-\text{OPT}(u')|_1$. Thus, in this setup we may argue that our definition \ref{def:disutility_user_result} approximates $|\text{OPT}(u)-m|_1$ upto a constant factor. 

    
\end{example}


% Observe that the first condition is required to ensure that the dis-utility on receiving the optimal result is zero. The second condition implies that the growth of $\mathfrak{h}(.)$ is bounded by some exponential function. Observe that ratios of polynomials and exponential functions like $\sqrt{z},z^2, e^{z}-1$ satisfy the second criterion, however functions like $e^{z^2}-1$ do not. The second condition is required in our mathematical analysis which would be useful in the construction of our optimization problem $\mathcal{O}$ in Section \ref{subsec-comb:primal-feasible}. 

% \begin{enumerate}[label= \arabic*]
%     \item \label{item:first-propertyh} $\mathfrak{h}(.)$ is a continuously increasing function satisfying $\mathfrak{h}(0)=0$.
%     \item \label{item:second-property-h} There exists $\mathcal{B} \in \real^{+}$ s.t. $\log \mathfrak{h}(.)$ is Lipschitz continuous in $[\mathcal{B},\infty)$
% \end{enumerate}


In the next subsection, we shall argue why it is sufficient to study a simplified setup restricting the users and results to the same set $\real$. 

\subsection{Restricting users and results to the same set} {\label{subsec:user_results_restricted}} 

%\zhihao{Shall we use subsection or paragraph here?}
\ak{This comes out of nowwhere and also should not take such prominent space -- if this is a technique for simplifying proofs, then it should appear way later; e.g. after the "our results".}
\ak{This also begs the question of whether disutility was defined in the unusual manner simply to use this trick later?}

\sss{Tried to give two examples why such a definition maybe dis-utility maybe useful. Also, the whole mathematical setup is defined in this setup where users and results lie in $\real$ and optimal result for user $u$ is result $u$ with the dis-utility defined as $\mathfrak{h}(|u-a|)$}

Since $\Disutility^{\mathfrak{h}(.)}(u,\text{OPT}(u')) \leq \mathfrak{h}(|u-u'|)$, we can argue that it is sufficient to study a more simplified setup restricting the users and results to the same set $\real$ with the optimal response for the user $u$ being the result $u$ itself. Thus, the dis-utility of user $u \in \real$ from a result $a \in \real$ is defined as $\mathfrak{h}(|u-a|)$ in the simplified setup. A detailed treatment bounding the cost in the original setup (where results and users lie in different sets) by the cost in the simplified setup is provided in Appendix \ref{appendix-sec:restricted_unrestricted_setup} for our multi-selection model. While one may argue that in such a simplified setup the server may not be necessary at all, we study this simplified setup for ease of exposition and our results would also generalise to the more general case of users and results lying in different sets. %As we shall see in the upcoming below, we study this ``multi-selection'' model for the case where the user set is given by a (doubly infinite) real number line i.e. $U = \mathbb{R}$ and $d(x,y) = |x-y|$. \ak{Why is this preview neeed?}

\subsection{Model of privacy along with system architecture}

A well studied notion of privacy under the local trust model is local differential privacy \cite{bebensee2019local} which requires a privacy guarantee of $\epsilon$ for any two potential values of an individual's data. We redefine it formally below adapted from \cite{6686179,koufogiannis2015optimality}.

\begin{definition}[adapted from \cite{6686179,koufogiannis2015optimality}]
    Let $\epsilon>0$ be a desired level of privacy and let $\mathcal{U}$ be a set of input data and $\mathcal{Y}$ be the set of all possible responses and $\Delta(\mathcal{Y})$ be the set of all probability distributions (over a sufficiently rich $\sigma$-algebra of $\mathcal{Y}$ given by $\sigma(\mathcal{Y})$). A mechanism $Q: u \rightarrow \Delta(\mathcal{Y})$ is $\epsilon$-differentially private if 

    $$ \mathbb{P}(Qu_1 \in S) \leq e^\epsilon \mathbb{P}(Qu_2\in S)$$

    for all $S \in \sigma(\mathcal{Y})$ and $u_1,u_2 \in \mathcal{U}$.
\end{definition}




\ak{poor description of DP b/c it is self-referential -- "local DP requires a privacy guarantee"... better to skip altogether or write a more precise version}
Geographic differential privacy (Geo-DP) \ak{abbreviation of DP should be introduced near differential privacy, not near geographic differential privacy}\cite{andres2013geo} relaxes/generalizes this requirement to consider the distance between the two values, allowing the privacy guarantee to decay linearly with the distance. Geographic DP is a relaxed privacy guarantee, and therefore, allows for achieving better utility. It is appropriate in scenarios such as search, and, therefore, we use it as our privacy notion for the rest of the work. We restate the formal definition from \cite{koufogiannis2015optimality} below. 


\begin{definition}[adapted from \cite{koufogiannis2015optimality}]{\label{def:geo_DP}}
        Let $\epsilon>0$ be a desired level of privacy and let $\mathcal{U}$ be a set of input data and $\mathcal{Y}$ be the set of all possible responses and $\Delta(\mathcal{Y})$ be the set of all probability distributions (over a sufficiently rich $\sigma$-algebra of $\mathcal{Y}$ given by $\sigma(\mathcal{Y})$). A mechanism $Q: u \rightarrow \Delta(\mathcal{Y})$ is $\epsilon$-geographic differentially private if 

    $$ \mathbb{P}(Qu_1 \in S) \leq e^{\epsilon|u_1-u_2|} \mathbb{P}(Qu_2\in S)$$

    for all $S \in \sigma(\mathcal{Y})$ and $u_1,u_2 \in \mathcal{U}$.
\end{definition}




% would enable the noisy query sent by the user to reveal  more information about the user leading to better privacy accuracy tradeoff and thus, we study this model of geographic DP in this work. 


\ak{Poorly phrased -- we study it because it reveals more information about the user? Should be: geographic DP is a relaxed privacy guarantee, and therefore, allows for achieving better utility. It is appropriate in scenarios such as search, and, therefore, we use it as our privacy notion for the rest of the work.}
\sss{Addressed}

% Let us now introduce some notation. 
% \ak{Need to explain why introducting notation! E.g. we now define geographic DP formally.}
% Given a set $S$, if we use $K(\cdot)$ to denote a distribution on $S$, then $K(H)$ is the probability mass of $H\subseteq S$. For distributions $K$ and $K'$ on $S$, we define their distance to be $\ddis{K}{K'} \defeq \sup\limits_{H\subseteq S; K(H) \neq 0 \ak{should this not be K'(H)?}} \frac{K(H)}{K'(H)}$.\footnote{We treat $\frac{a}{0}$ to be $+\infty$ for $a>0$ \ak{if som then why is $K(H) \neq 0$ needed?} \sss{It is needed to avoid 0/0 case which is not covered by our definition.}}. \ak{I am not convinced it has to hold only for $H\subseteq S$}
% \ak{Need to define geographic DP formally in terms of sets; then instantiate it in terms of queries to the server...}
% Suppose $\textbf{P} = \{\dsig{u}\}_{u \in \real}$ characterises the distribution of queries to the server for every $u \in \real$, \ak{$u, \real, P_u$ were not defined! so can't use them like this} then to satisfy $\epsilon$- geographic DP, we must have $\ddis{\dsig{u_1}}{\dsig{u_2}} \leq \epsilon |u_1-u_2|$ for any pair of users $u_1,u_2 \in \real$.  \ak{$d$ was not defined}

\ak{Why not place the formal definition of GDP in our context in the mathematical model description rather than here?}

\subsubsection{System Architecture}

In this work, we do not relax the privacy definition, but consider a conceptually different system architecture design. Our ``multi-selection" approach relies on the server returning a small set of results in response to the privatized user input, with the on-device software intermediary deciding, unbeknownst to the server, which of these server responses to use.  This new system architecture, shown in \cref{fig:arch1} is made possible by advances in the reduction of communication costs and power of on-device computation.  In a stylized model, we show theoretically that this new system design enables new algorithms with lower worst case dis-utility for an user for the same privacy guarantee than in the traditional local trust model. We study the $\epsilon$-geographic model of differential privacy. 


%whose privacy cost on utility 



\ak{need consistency: accuracy, utility, disutility...} is lower than in the traditional local trust model. %model of DP
\ak{Need to say here whether results will be for local GDP, for local DP, for something else...}

\definecolor{usr}{rgb}{0.7,0.85,1.0}
\definecolor{usrl}{rgb}{0.9,0.95,1.0}
\definecolor{usrline}{rgb}{0.8,0.9,1.0}
\definecolor{sev}{rgb}{1.0,0.85,0.7}
\definecolor{sevl}{rgb}{1.0,0.95,0.9}
\definecolor{sevline}{rgb}{1.0,0.9,0.8}

\input{multi-arch-figure}

  % \begin{figure}[htbp]
  %     \centering
  %     \tikzset{global scale/.style={
  %           scale=#1,
  %           every node/.append style={scale=#1}
  %         }
  %       }
  %       \begin{tikzpicture}[global scale = 0.8]

        
  %        \node[fill=usrl,draw=usrline,rounded corners, minimum width=10cm, minimum height=3cm] at (2.5,2) {};
         
  %        \node at (2.5,3.8) {Client};
        
  %        \node[fill=usr,draw,rounded corners, minimum width=3cm, minimum height=1.5cm] at (0,2) {\bf User};
         
  %        \node[fill=usr,draw,rounded corners, minimum width=3cm, minimum height=1.5cm,align=center] at (5,2) {\bf User Agent \\ e.g. browser};

         
  %        \node[fill=sevl,draw=sevline,rounded corners, minimum width=5cm, minimum height=3cm] at (11.5,2) {};
         
  %        \node at (11.5,3.8) {Server};
  %        \node[fill=sev,draw,rounded corners, minimum width=4cm, minimum height=1.5cm] at (11.5,2) {\bf Result Computation};

         
  %        \draw[->] (1.5,2.25) -- (3.5,2.25);         \draw[<-] (1.5,1.75) -- (3.5,1.75);         \draw[->] (6.5,2.25) -- (9.5,2.25);         \draw[<-] (6.5,1.75) -- (9.5,1.75);

  %        \node at (2.5,2.5) {features};
  %        \node at (2.5,1.5) {best result};
  %        \node at (8,2.5) {signal with noise};
  %        \node at (8,1.5) {a set of $k$ results};

         
  %       \end{tikzpicture}
  %     \caption{Overall architecture for multi-selection.}    \label{fig:arch1}
  % \end{figure}

The central question we study can now be phrased as:
\begin{quote}
\noindent \textit{What should the user's privacy-preserving signal be, and what is the optimal set of $k$ results to send given this signal so that the client's dis-utility is minimized when it chooses the best of the returned results.}
\end{quote}

\ak{and here comes the disconnect -- we never spoke about accuracy so far, only about disutility... so either need to postpone the definition of accuracy/ disutility for after this central question formulation, or need to define both and their relationship} 

\sss{Removed those terms and rewrote the sentence.}


\subsection{Mathematically defining the action space of the mechanism \ak{Shorter title:}} \label{sec:simmodel}
\ak{Bigger picture: the space of algorithms we consider in this new architecture consists of a triple -- user's choices to privatize their data, server choices, ...}

\sss{Addresed}

The space of mechanisms we consider in this new architecture consists of a tuple a) set of signals $Z$ b) users' choices to privatise their data denoted by $\Pname$ c) Server's response to an user's signal denoted by $\Qname$. We now formally define the tuple $(Z,\Pname, \Qname)$ below

% To look at this problem, we now start with the following definition to characterise the mechanism which consists of three items: set of signals $Z$, action of an user $u$ and the response of the server on receiving signal $s \in Z$.

\begin{itemize}
    \item A set of signals $Z$.
    \item  The action of users, which involves sampling a signal from a distribution over signals. We use $\dsig{u}$ for $u\in \mathbb{R}$ to denote the distribution of the signals sent by user $u$ which is supported on $Z$. The set of actions over all such users is given by $\Pname = \{\dsig{u}\}_{u \in \real}$.
    \item The distribution over actions of the server, $\dsigq{s}$ when it receives $s\in \Signals$ which characterises the distribution of the $k$ results (ad) that the server sends and thus, it is supported in $\mathbb{R}^k$. We denote the set of all such server actions by $\Qname = \{\dsigq{s}\}_{s \in Z}$. \footnote{We treat this distribution to supported on $\real^k$ instead of $k$-sized set in $\real$ for ease of mathematical typesetting.} 
\end{itemize}


Observe that to find the optimal distribution, we need to jointly optimize over $(Z,\Pname,\Qname)$ with $\epsilon$-geographic differential privacy constraints on $\Pname$ as discussed above. Also, we use $\texttt{Set}(\vect{a})$ to convert a vector $\vect{a} = (a_1,a_2,\ldots,a_k)^T\in \real^k$ to a set of at most $k$ elements, formally $\texttt{Set}(\vect{a}) = \{a_i: i \in [k]\}$. 

\subsubsection{Definition of the cost function}

% We define the cost of the mechanism $(Z,\Pname,\Qname)$ by supremizing \footnote{We write supremum instead of maximum as the maximum over an infinite set may not always be defined.} over the dis-utility of all users in the set $\real$. 
% Note that since we do not make any distributional assumption over users in the set $\real$, this could be natural metric to consider. 

Recall that the dis-utility of an user $u \in \real$ from a result $a \in \real$ was defined by $\mathfrak{h}(|u-a|)$ in Section \ref{subsec:user_results_restricted} for the simplified setup. We now discuss the dis-utility of an user $u$ from the user' action $P_u$ and the server's response $Q_s$ on receiving signal $s$. Since each of these actions could be randomised, we take the expectation over the randomness in the action of the user and the server. Thus, the cost of an user $u$ from the mechanism $(Z,\Pname,\Qname)$ is given by 

\begin{equation}{\label{eqn:cost_user_tuple_mechanism}}
    \text{cost}^{\mathfrak{h}(.)} (u, (Z,\Pname,\Qname)) = \Exxlimits{s\sim \dsig{u}}{\Exxlimits{\vect{a}\sim \dsigq{s}}{ \min_{a \in \texttt{Set}(\vect{a})} \mathfrak{h} (|u-a|)}}
\end{equation}


We now define the cost of a mechanism by supremizing \footnote{We write supremum instead of maximum as the maximum over an infinite set may not always be defined.} over all users $u \in \real$. Since, we refrain from making any distributional assumptions over the users, we cannot choose common metrics like mean or average over the users.



%We study this supremum metric over other metrics like mean/average since we refrain from making any distributional assumption over the users $u \in \real$.  

\begin{equation}{\label{eqn:cost_tuple_mechanism}}
    \text{cost}^{\mathfrak{h}(.)}(Z,\Pname,\Qname) := \sup_{u \in \mathbb{R}} \Exxlimits{s\sim \dsig{u}}{\Exxlimits{\vect{a}\sim \dsigq{s}}{ \min_{a \in \texttt{Set}(\vect{a})} \mathfrak{h} (|u-a|)}}
\end{equation}

% Observe that the this expectation has randomness in the server's action and 


\ak{Need more on why this is natural -- e.g. that this is a worst-case utility aligned with traditional algorithms literature?}
\ak{Move the definition of dis-utility here and gradually build up to the cost formula}
\sss{Done}
\ak{This requires proof; also, mathematical model was in terms of triplet, Z is part of that triplet, so here, need to first define everything in terms of triplet, then explain why OK to get rid of Z later.}
\sss{We still have $Z$ in this section. We get rid of $Z$ in Section 2.1}


% \begin{equation}{\label{eqn:cost_tuple_mechanism}}
%     \text{cost}^{\mathfrak{h}(.)}(Z,\Pname,\Qname) := \sup_{u \in \mathbb{R}} \Exxlimits{s\sim \dsig{u}}{\Exxlimits{\vect{a}\sim \dsigq{s}}{ \min_{a \in \texttt{Set}(\vect{a})} \mathfrak{h} (|u-a|)}}
% \end{equation}
\ak{What is the randomness taken over in these formulas? Need to say so explicitly}
\ak{Why taking expectations if just above claimed that the cost will be worst-case?}

\zhihao{maybe we can say something like, worst-case means the max dis-utility (or other terms such as accuracy) among all users, and dis-utility of a user is defined to be the expected dis-utility w.r.t random signal and random ad sets. }

We now move to define the cost function $\funfgeo{(d,U)}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ by infimizing over the tuple  $(Z,\Pname,\Qname)$ subject to differential privacy constraints on $\Pname$ i.e., user's action ($\Pname$) satisfies $\epsilon$-geographic differential privacy (defined formally in Definition~\ref{def:geo_DP}[adapted from \cite{koufogiannis2015optimality}]). Thus, we define function $\funfgeo{(d,U)}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ as the following optimization problem. 
\ak{This doesn't follow traditional convention -- it's common to define the privacy constraints on the relevant functions, P and Z in this case, not on the cost function. So, you should first define the privacy constraint and then say -- well, our problem is to find the triple so subject to privacy constraints and minimizing cost, therefore, we will be interested in the following optimization problem, and we will denote its minimum possible value by xxx (significantly, the main parameter for the multi-selection is $k$). Also, why is $f$ parameterized by ${\mathfrak{h}(.)}$ but cost isn't, even though they should be parameterized by the same thing?}
\ak{Wouldn't the most natural thing to consider not be the ratio of the optimal solution when $k=1$ to when $k>1$? Is that what is expressed in our results?}

% \[  \funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
% \defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}\\ \Qname\in \Qrobs_{\text{unrestricted},\Signals}}} \sup_{\Dist \in \probm{U}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\left(\Disutility^{\mathfrak{h}(.)}(u,a)\right) }, \]

\begin{align}{\label{eqn:cost_function_defn}}
    \funfgeo{(d,U)}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
\defeq & \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}}} \inf_{\Qname\in \Qrobs_{ \Signals}} \left(\text{cost}^{\mathfrak{h}(.)}(Z,\Pname,\Qname)\right)\nonumber \\
        = & \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}}} \inf_{\Qname\in \Qrobs_{ \Signals}} \left(\sup_{u \in \real} \Exxlimits{s\sim \dsig{u}}{\Exxlimits{\vect{a} \sim \dsigq{s}}{ \min_{a \in \texttt{Set}(\vect{a})} \mathfrak{h} (|u-a|)}} \right) \text{where}
\end{align}

%\ak{This formula needs better typesetting as it is unclear which subscripts belong to which of inf, sup...}

$\Probsgeo{\Signals}:=\{ \Pname | \forall u\in \real, \dsig{u}\text{~is a distribution on $\Signals$,} 
    \text{~and $\Pname$ satisfies $\epsilon$-geographic differential privacy.} \}$.
    %\ak{Inconsistent notation -- why is $u\in \real$ here whereas it was $u \in U$ before? $\Pname_u$ was already defined, etc}

$\Qrobs_{\Signals}:= \{ \Qname | \forall s\in \Signals, \dsigq{s}\text{~is a distribution on $\real^{\K}$} \}$. 


Our aim is to characterise this function and find the tuple $(Z,\Pname,\Qname)$ which infimises this cost function.  

\subsection{Our results and key techical contributions}
\ak{Given that so many of the results are a function of $\mathfrak{h}.$ The significance of what $\mathfrak{h}$ means, what are the natural choices, why it matters, why one would care about changes depending on it needs to be motivated.}

%\zhihao{one baseless thought: for a certain user $u$, if $d(u,a)$ is small, e.g. $d(u,a)=1$, then the user will clearly prefer $a'$ if $d(u,a')=0$. However, if $d(u,a)$ is large, e.g. $d(u,a)=10001$, the user will not clearly prefer $a'$ if $d(u,a')=10000$. In this situation, we want $h(10001)-h(10000)<h(1)-h(0)$}

% We study this problem for the case when the user set is given by a (doubly infinite) real number line, i.e. $U = \mathbb{R}$ and $d(x,y) = |x-y|$. 

Recall that the function $\mathfrak{h}(.)$ characterises how the dis-utility of an user grows with distance. For example, if the user has the diminishing marginal dis-utility with distance, the function $\mathfrak{h}(t)$ could be concave like $\mathfrak{h}(t) = \sqrt{t}$. Otherwise, it could be convex like $\mathfrak{h}(t)=t^2$ or it may also be linear like $\mathfrak{h}(t)=t$. Our main results are:
\begin{itemize}
    \item We show that the Laplace noise addition mechanism (user adding Laplace noise of parameter $\epsilon$ and sending to server) is one of the optimal actions for an user for any $\mathfrak{h}(.)$ satisfying the constraints in equations \eqref{item:first-propertyh} and \eqref{item:second-property-h}.

    \item Although the Laplace noise addition mechanism is optimal for every $\mathfrak{h}(.)$ satisfying constraints in equations \eqref{item:first-propertyh} and \eqref{item:second-property-h}, the optimal \ak{optimal?}\sss{addressed} server actions could be different based on different $\mathfrak{h}$. We give a recursive construction of the optimal server response for a general $\mathfrak{h}$ satisfying equations \eqref{item:first-propertyh} and \eqref{item:second-property-h}.

    \item However, when $\mathfrak{h}(t)=t$, we give an exact construction of the server response and show that $\funfgeo{(\ell_1,\real)}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)} = O(\frac{1}{\epsilon k})$. We further show in Appendix \ref{sec-appendix:mhr} that a cost \ak{was not defined} of $O(\frac{\log k}{k\epsilon})$ is achieved for a noise addition mechanism when the noise distribution satisfies log-concave property which satisfies by most natural distributions like Exponential and Gaussian.

    \ak{comes out of nowhere. is this a new definition of geographic DP? need to use a different notation as funfgeo and $\mathfrak{f}$ look almost identical.} 
    \sss{Yes, it is a new definition and changed the notation.}

    \item In appendix \ref{sec:diff-privacy-gen}, we study a more generalized definition of $\epsilon$-geographic DP (we call it $\mathfrak{g}(.)$-geographic differential privacy) and show that Laplace noise still continues to remain an optimal action choice for an user. This captures scenarios as discussed in \cite{geng2015optimal} where the privacy guarantees exist only in a neighbourhood.

    
    % Further, we generalize our results to the case of $\mathfrak{f}(.)$-geographic differential privacy for a convex increasing function $\mathfrak{g}(.)$ in Appendix \ref{sec:diff-privacy-gen} and show that Laplace noise addition mechanism continues to remain an optimal action choice for an user. This captures scenarios as discussed in \cite{geng2015optimal} where the privacy guarantees exist only in a neighbourhood.
\end{itemize}

We now move to state our main theorem below. 

\begin{restatable}[corresponds to Theorem \ref{thm:optimality-laplace-sim} and Corollary \ref{cor:geofinal}]{theorem}{simrstepe} \label{thm:lap:sim}
For $\epsilon$-geographic differential privacy \ak{where is the $d$ of the geographic?}\sss{$d(.)$ is defined to be the $\ell_1$ norm at the start of the section}, adding Laplace noise, whose density function is $\rho(x)=\frac{\epsilon}{2} \cdot e^{-\epsilon \disrzero{x}} $, is one of the optimal choices of $\Probs{\Signals}$ for users. Further, when $\mathfrak{h}(t)=t$, we have $\funfgeo{(\ell_1,\real)}{\Ads}{\epsilon}{\K} {\mathfrak{h}(.)} = O(\frac{1}{\epsilon k})$ and the optimal mechanism (choice of actions of users and server) itself can be computed in closed form. For a generic $\mathfrak{h}(.)$, the optimal server action $\Qname$ may be computed recursively.
\end{restatable}  

Our key technical contributions in the proof may be summarised below.

\begin{itemize}
    \item We formulate this optimization problem in equation \eqref{eqn:cost_function_defn} as a linear program over function spaces with linear constraints on both derivatives and integrals, we call it Differential integral linear program (DILP). 

    \item Next, we extend the weak duality theorem to the case of DILPs. To the best of our knowledge, the weak duality result for infinite dimensional function spaces exist for linear programs with only integral constraints (check \cite{anderson1987linear}). We believe our extension is novel and has broader implications beyond differential privacy (check Appendix \ref{sec-appendix:weak_duality_application} for two such applications). The proof of this result is technical and involves a careful application of integration by parts to translate the derivative constraint on the primal variable to a derivative constraint on the dual variable.

    \item Finally, we conclude the proof via dual-fitting. We give a solution in the dual DILP with the same objective value as the cost of the Laplace noise addition mechanism. For a generic $\mathfrak{h}(.)$, we show that it is possible to recursively construct the optimal server response and give a closed form expression when $\mathfrak{h}$ is linear.
\end{itemize}





We denote $\funfgeo{(d,U)}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ by $f(\epsilon,k)$ whenever the context is clear.


\subsection{Proof Roadmap and key ideas}{\label{sec:main_technical_contributions}}

\sss{For FOCS, maybe we need to clearly articulate our technical novelty better and how it extends to other problems, maybe}

We first show that the following Laplace noise addition mechanism is natural: the user(client) adds Laplace noise of parameter $\epsilon$ to query (call it signal $s$), the server on receiving signal $s$ responds back with a vector $A \in \real^k$ to minimise the minimum distance of $s$ to a component in $A$ ($\min\limits_{a \in \texttt{Set}(A)} (\mathfrak{h}(|s-a|))$). Our main result shows that this natural mechanism is optimal. This proof is non-trivial and does not follows from the optimality of such noise when $k=1$ as shown in \cite{koufogiannis2015optimality}.

To prove this result, we study a stronger setup where the user has full information and is directly choosing a set $S$ of size $k$ to minimize the expected dis-utility from its query while ensuring that the set $S$ satisfies geographic differential privacy in Section \ref{subsec-comb:proof-step1}.\footnote{This setup is stronger since a user query satisfying differential privacy implies the response set $S$ from the server also satisfies differential privacy from the post-processing theorem in differential privacy.} Observe that this setup involves optimizing over all possible distribution with support in $\real^k$, thus an optimization in a infinite dimensional vector space. Since geographic differential privacy requires the distribution of the response set $S$ to change only slightly as we change the value of user $u$, this naturally translates to a derivative constraint on the distribution of $S$. Observe that, since we also need the distribution to be a valid distribution, we require the probability distribution to integrate to 1. We thus formulate our problem as a Differential Integral Linear Program (DILP) in Section \ref{subsec-comb:primal-feasible}. We formally define DILP with an example in equation \eqref{eq:example_DILP} below. 

\begin{definition}{\label{def:DILP}}
    Differential-integral linear programs (DILP): Differential-integral linear program is a linear program over Riemann integrable function spaces involving constraints on both derivatives and integrals. A simple example may be given in Equation \eqref{eq:example_DILP}. Observe that in equation \eqref{eq:example_DILP}, we define $\mathcal{C}_1$ to be a continuously differentiable function.
\end{definition}

\begin{equation}{\label{eq:example_DILP}}
        \text{\Large{$\tilde{\mathcal{O}}=$} }
        \left\{
        \begin{aligned}
            \inf_{g(.): \mathcal{C}^1(\mathbb{R} \rightarrow \mathbb{R}^{+})} & \int_{\mathbb{R}} |v| g(v) dv\\
            \textrm{s.t.} \quad & \int_{\mathbb{R}} g(v) dv =1\\
            & -\epsilon g(v) \leq g'(v) \leq \epsilon g(v) \text{ }\forall v \in \mathbb{R}
        \end{aligned}
        \right.
\end{equation}

%\zhihao{define $\mathcal{C}^1$ here}



Next, we show that the two stage natural mechanism we described above is optimal via dual-fitting i.e. construction of a feasible solution to a dual infinite dimensional linear program attaining the same objective value in Section \ref{subsec-comb:dual-soln-construction}. However, since the duality theory to the best of our knowledge exists for infinite dimensional linear programs only for integral constraints, we reprove the weak-duality theorem for our setup in Theorem \ref{theorem:weak_duality_result}. However, since DILPs arise in many other problems apart from differential privacy, we believe our weak-duality theorem may be useful in other areas as well. We discuss two such problems (one in control theory \cite{evans1983introduction} and one in job scheduling \cite{anderson1981new}) in Appendix \ref{sec-appendix:weak_duality_application}. The proof for the weak-duality is novel since it requires ideas from integration by parts to translate the derivative constraint on the primal variable to a derivative constraint on the dual variable. Further since our problem requires exchange of limits and integrals, we require a careful application of Fatou's lemma and monotone convergence theorem to exchange limits and integral, a detailed proof is given in Appendix \ref{sec:weak_duality}.



For the case of $\mathfrak{h}(t)=t$, we show that the server response can be explicitly (and easily) calculated using a simple recurrence (Section \ref{subsec-comb:step4}), and when $k$ is odd, it cuts down the cost function decreases by a factor of $(k+1)/2$, comparing to the cost when $k=1$. \ak{-> comparing to the cost when only one result is returned.} Figure \ref{fig:intro1} is an instance of the optimal mechanism.
For general $\mathfrak{h}(.)$, the recurrence still holds but a closed-form solution may not exist. Our main result shows that this natural mechanism is optimal. 

\begin{figure}
      \centering
        \begin{tikzpicture}
        \coordinate (right) at (8,0);
        \coordinate (left) at (0,0);
        \coordinate (o) at (4,0);
        \coordinate (up) at (4,3);
        \coordinate (x0) at (4.5,0);
        \coordinate (s) at (2,0);
        \coordinate (t) at (5.5,0);
        \coordinate (cone) at (4,2.5);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[->](o)--(up);
        \draw[<->](left)--(right);
        \draw[-](cone)--(4.1,2.5);
        \draw node at (3.65,2.5) {$0.5$};
        \draw node at (4.0,-0.3) {$O$};
        \draw node at (4.45,3.1) {$\rho(t)$};
        \draw node at (7.9,-0.2) {$t$};
        % here, eps=0.55
        \draw[blue,domain=0:4] plot(\x,{2.5*exp((\x-4))} );
        \draw[blue,domain=4:8] plot(\x,{2.5*exp(-(\x-4))} );
        \coordinate (r0) at (4,0);
        \coordinate (r3) at ([xshift = 1.3862943611198906188344642429164*2.5 cm] r0);
        \coordinate (r2) at ([xshift = -0.69314718055994530941723212145818*2.5 cm] r3);
        \coordinate (r1) at ([xshift = -1.0986122886681096913952452369225*2.5 cm] r3);
        \coordinate (r-3) at ([xshift = -1.3862943611198906188344642429164*2.5 cm] r0);
        \coordinate (r-2) at ([xshift = 0.69314718055994530941723212145818*2.5 cm] r-3);
        \coordinate (r-1) at ([xshift = 1.0986122886681096913952452369225*2.5 cm] r-3);
        \fill (r0) circle (2pt);
        \fill (r1) circle (2pt);
        \fill (r2) circle (2pt);
        \fill (r3) circle (2pt);
        \fill (r-1) circle (2pt);
        \fill (r-2) circle (2pt);
        \fill (r-3) circle (2pt);
        \coordinate (rowone) at ([xshift=2.5cm] o);
        \coordinate (row-one) at ([xshift=-2.5cm] o);
        \coordinate (rowonec) at ([yshift=-0.3cm] rowone);
        \coordinate (row-onec) at ([yshift=-0.3cm] row-one);
        \coordinate (rowonel) at ([yshift=0.1cm] rowone);
        \coordinate (row-onel) at ([yshift=0.1cm] row-one);
        \draw node at (rowonec) {$1$};
        \draw node at (row-onec) {$-1$};
        \draw[-](rowone)--(rowonel);
        \draw[-](row-one)--(row-onel);
        \end{tikzpicture}
      \caption{Optimal mechanism in geographic differential privacy setting when $\K=7$ and $\epsilon=1$. Suppose the user has a private value $v$. Then the user sends $v+x$ to the server, where $x$ is drawn from Laplace distribution with density $\rho(t)$. \ak{ Also, the distribution should contain $\epsilon$ in its definition!}
      \sss{We fix $\epsilon=1$ for this case.}
      \ak{I know you do, but that's not rigorous, the distribution should be defined in terms of $epsilon$}
      Suppose the server receives $s$. Then the server responds $s+a_1,...,s+a_7$, where the values of $a_1,a_2,...,a_7$ are denoted by black dots on the $x$-axis.
      \ak{For the illustration to be clear, also needs the response dots for discrete Laplace, i.e. if we were to discretize Laplace and truncate to only 7 values, what would they be?}
      }    \label{fig:intro1}
  \end{figure}

% This proof is non-trivial and does not follow from the optimality of such noise when $k=1$ as shown in \cite{koufogiannis2015optimality}. 


We also generalize our results by showing the optimality of Laplace noise addition in $\mathfrak{g}(.)$-geographic differential privacy where the privacy guarantees between two users $u_1$ and $u_2$ does not scale linearly with distance $|u_1-u_2|$ but is given by $\mathfrak{g}(|u_1-u_2|)$ in Appendix \ref{sec:diff-privacy-gen} for some increasing convex function $\mathfrak{g}(.)$. This notion is useful when users have little or no privacy requirements from users far away from it but have higher requirements in the vicinity. Further, we emphasize that the optimality of adding Laplace noise is far from obvious\footnote{In fact, only a few optimal mechanisms are known~\cite{Ghosh2012privacy, gupte2010universally, kairouz2014extremal, ding2017collecting}, and it is known that for certain scenarios, universally optimal mechanisms don't exist~\cite{brenner2014impossibility}.}. For instance, when users and results are located on a ring, Laplace noise is {\em not optimal}, analysed for the case of $k=2$ in Appendix \ref{appendix-sec:non-opt-ex}. While we have not been able to analyze the ring in complete generality for geographic DP, we have been able to explicitly solve it for some specific simple cases using our optimization framework in Section \ref{sec-appendix:primal-feasible}.


% Next, we show that when an user chooses the set $S$ by simulating the action of the server i.e. user  



% Observe it \ak{Need the intuition for why set $S$ satisfying DP is equivalent to the user query satisfying DP; is it??}
% This involves optimizing over all possible $k$-dimensional distributions for $S$ for which we construct a linear program over infinite dimensional spaces \ak{why does it need to be infinite dimensional?} \sss{This is because we are optimizing over all possible distributions which is a function space}involving both integrals and derivatives. 
% We next show that a two-stage mechanism, where the user sends a single noisy value and the server chooses $k$ results by adding $k$ {\em fixed increments} to the chosen value is optimal via dual-fitting,  
% \ak{It's unclear whether the two-stage mechanism arises from the solution to the optimization problem or from our problem set-up -- user sends noisy value and receives k results.}
% Since to the best of our knowledge, duality theory for infinite dimensional linear programs exists only for programs involving integrals, we prove the weak duality theorem for our linear programs.
    




%a) the set of signals $Z$ an user can send b) actions of user $u$ (denoted by distribution $\dsig{u}$) and a server response (denoted by distribution $\dsigq{s}$) on receiving signal $s \in Z$.








%We now move to characterise a mechanism which 




%We now send  



%Of course, had the server simply returned all possible results, there would have been no loss in quality since the client could choose the optimal result. However, this is infeasible for several reasons -- first, the client's device could be constrained by battery or memory; second, the server also needs to send its model for evaluating the quality of the results and this can be large; and finally, returning all results (such as ads) could compromise proprietary information. We therefore restrict the server to return $k$ results for small $k$, and ask for the tradeoff between $k$ and the quality when the client sends privacy-preserving noisy queries.


==> local.tex <==

\newcommand{\rotation}{\mathcal{V}}

\section{Local differential privacy on $d$-dimentional sphere}  \label{sec:localfull}
Let $\sphere\defeq \{x\in \real^{\Dim}| \diszero{x}=1\}$. In this section, $\Users=\Ads=\sphere$, $\disg{x}{y}=\disbb{x}{y}$, and $\defdis{u_1}{u_2}=1$. To be convenient, we use $\disb{x}{y}$ to denote $\disbb{x}{y}$.



\subsection{Optimality of symmetric mechanism}

We show symmetric mechanism in this section. To define what is symmetry, we introduction the group of rotation matrix.

\begin{definition}

Let $\rotation$ be the set of rotation matrices in $\Dim$-dimensional space.
\[ \rotation \defeq \left\{ M\in \real^{\Dim \times \Dim} | M M^{T}=I_{\Dim \times \Dim}, det(M)=1 \right\}, \]
where $I_{\Dim \times \Dim}$ is the identical matrix.

\end{definition}



Note that $(\rotation,\cdot)$ forms a group, where $\cdot$ is matrix multiplication.

\begin{definition}[rotation on sets]

For $A\subset \sphere$ and $M\in \rotation$, define
\begin{align*}
    MA\defeq  \{ Mx | x\in A \}  
    ~~\text{and}~~
    AM\defeq  \{ xM | x\in A \}.
\end{align*}

\end{definition}

\begin{lemma}[Haar distribution / uniform distribution \cite{haar1933massbegriff, bourbaki2004integration}]

There is a probability measure $\mu$ on $\rotation$, such that for any $\C \subset \Rname$,
\[ \mu(\Gamma \C) =  \mu(\C), \forall \Gamma\in \Rname. \]

\end{lemma}


\begin{definition}[symmetry of the system]


For $\Pname\in \Probs{\Kads}$, if for any $u\in \Users, \C\in \measure{\Kads}, M\in \rotation$,
\begin{align*}
    \Pxx{u}{\C}=\Pxx{uM}{\C M},
\end{align*}
then we say $\Pname$ is a symmetric mechanism.

Let $\Psym$ be the set of symmetric mechanisms.


\end{definition}

\begin{theorem}


\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname\in \Probs{\Kads}} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disb{u}{a} }
=
\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disb{u}{a} }.
\end{align*}

\end{theorem}

\begin{proof}

The first equation follows from Theorem \ref{thm:singpoint}. We focus on the second equation.

For $\Pname\in \Probs{\Kads}$, we construct $\Ppname_u\in \Psym$. For any $\C\in \measure{\Kads}$, let
\[ \Ppxx{u}{\C}=\int_{M\in \rotation} \Pxx{uM}{\C M} \mu(dM). \]


For any $u_1,u_2\in \Users$ and $\C\in \measure{\Kads}$, we have
\begin{align*}
\Ppxx{u_1}{\C}
=\int_{M\in \rotation} \Pxx{ u_1 M}{\C M } \mu(dM)
\leq \int_{M\in \rotation} e^{\epsilon} \Pxx{ u_2 M}{\C M }\mu(dM)
%= e^{\epsilon} \int_{M\in \rotation}\Pxx{ u_2 M}{\C M } \mu(dM)
= e^{\epsilon} \Ppxx{u_2}{\C},
\end{align*}
so $\Ppname\in \Probs{\Kads}$.

For any $M_0\in \rotation$ and $\C\in \measure{\Kads}$,
\begin{align*}
\Ppxx{ uM_0}{\C M_0 }
=\int_{M\in \rotation} \Pxx{ uM_0 M}{ \C M_0 M} \mu(dM)
=\int_{M\in \rotation} \Pxx{ uM_0 M}{ \C M_0 M} \mu(d M_0 M)
=\Ppxx{u}{\C},
\end{align*}
so $\Ppname\in \Psym$.

$\Ppname$ is as good as $\Pname$ because for any $u_0\in \Users$,
\begin{align*}
&\Exx{A\sim \Ppname_{u_0}}{ \min_{a\in A}\disb{u_0}{a} } \\
=& \int_{A\in \Kads} \left( \Ppxx{u_0}{d A}\cdot \min_{a\in A}\disb{u_0}{a} \right)  \\
=& \int_{A\in \Kads} \left( \int_{M\in \rotation} \Pxx{u_0 M}{dA \cdot M} \mu(dM)\cdot \min_{a\in A}\disb{u_0}{a} \right)  \\
=& \int_{M\in \rotation}\mu(dM) \left( \int_{A\in \Kads} \Pxx{u_0 M}{dA \cdot M} \cdot \min_{a\in AM}\disb{u_0 M}{a} \right)  \\
=& \int_{M\in \rotation}\mu(dM) \cdot  \Exx{A\sim \Pname_{u_0 M}}{ \min_{a\in A}\disb{u_0}{a} }  \\
\leq & \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disb{u}{a} },
\end{align*}
which implies
\begin{align*}
    \sup_{u\in \Users} \Exx{A\sim \Ppname_u}{ \min_{a\in A}\disb{u}{a} }
    \leq
    \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disb{u}{a} }.
\end{align*}

Since we can construct such $\Ppname\in \Psym \subset \Probs{\Kads}$ for any $\Pname\in \Probs{\Kads}$, we have
\begin{align*}
    \inf_{\Pname\in \Probs{\Kads}} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disb{u}{a} }
    =
    \inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disb{u}{a} }.
\end{align*}



\end{proof}


\begin{corollary}

For any $u_0\in \Users$,
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname\in \Psym} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disb{u}{a} }
=
\inf_{\Pname\in \Psym} \Exx{A\sim \Pname_{u_0}}{ \min_{a\in A}\disb{u_0}{a} }.
\end{align*}

\end{corollary}

\begin{proof}

For any $\Pname\in \Psym$, for any $u_1,u_2\in \Users$, there exists $M\in \rotation$ so that $u_2=u_1 M$, so
\begin{align*}
& \Exx{A\sim \Pname_{u_1}}{ \min_{a\in A}\disb{u_1}{a} }   \\
=& \Exx{A\sim \Pname_{u_1}}{ \min_{a\in A}\disb{u_2}{a M} }   \\
=& \Exx{A\sim \Pname_{u_1}}{ \min_{a\in A M}\disb{u_2}{a} }   \\
=& \Exx{A\sim \Pname_{u_2}}{ \min_{a\in A}\disb{u_2}{a} },
\end{align*}
which implies for any $\Pname\in \Psym$ and $u_0\in \Users$,
\begin{align*}
\sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disb{u}{a} }
=
\Exx{A\sim \Pname_{u_0}}{ \min_{a\in A}\disb{u_0}{a} }.
\end{align*}

\end{proof}

Let $\zerob \defeq (1,0,\dots,0)^{T}\in \sphere$. Similar to Lemma \ref{lem:symtor}, we have the following result.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\zhihao{write proofs?}


\begin{lemma} 

\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname\in \Psym} \Exx{A\sim \Pname_{\zerob}}{ \min_{a\in A}\diszerob{a} }
=
\inf_{\Rname \in \Rrobs} \Exx{A\sim \Rname}{ \min_{a\in A}\diszerob{a} },
\end{align*}
where
\begin{align*}
\Rrobs = \{ \Rname | \R{\cdot}\in \probm{\Kads}; \text{~and~} \forall \C\in \measure{\Kads}, \forall M\in \rotation, \R{\C}\leq e^{\epsilon} \R{\C M} \}.
\end{align*}

\end{lemma}

\begin{lemma}

\begin{align}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszerob{a} }, \label{eq:assepa}
\end{align}
where
\begin{align*}
\Srobs = \{ \Sname | \S{\cdot}\in \probm{\Ads}; \text{~and~} \forall x,y\in \Ads, \rho_{\Sname}(x)\leq e^{\epsilon }\rho_{\Sname}(y) \} .
\end{align*}

\end{lemma}

\zhihao{write the proof, or modify the lemma}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{lemma} [corresponds to Theorem \ref{thm:main2:sim}]  \label{lem:ringbeforedetcal}

\begin{align}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszerob{a} }, \label{eq:assepa}
\end{align}
where
\begin{align*}
\Srobs = \{ \Sname | \S{\cdot}\in \probm{\Ads}; \text{~and~} \forall x,y\in \Ads, \rho_{\Sname}(x)\leq e^{\epsilon }\rho_{\Sname}(y) \} .
\end{align*}

\end{lemma}















\subsection{Results for $\Dim=2$}   \label{sec:unitring}



\zhihaohalfcomment{double check distance is $\disb{\cdot}{\cdot}$}

In this subsection, $\Dim=2$. That is, $\Users$ is a unit circle on $\real^{2}$. For $0\leq x<2\pi$, we use $\dg{x}$ to denote the point $(\cos x, \sin x)^{T}$. Then we have $\disb{\dg{x}}{\dg{y}}=\min\{|x-y|,2\pi-|x-y|\}$. In this case, $\Users=\{w(x)|0\leq x<2\pi\}$, and we have
\begin{align*}
    \funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{A\in \Kads} \inf_{\Tname \in \Trobs} \Exx{x\sim \Tname}{ \min_{a\in A}\disb{\dg{x}}{\dg{a}} },
%=
%\inf_{A\subset [0,2\pi),|A|=\K} \inf_{\Tname \in \Trobs} \Exx{x\sim \Tname}{ \min_{a\in A}\min\{|x-a|,2\pi-|x-a|\} },
\end{align*}
where
\begin{align*}
\Trobs = \{ \Tname | \T{\cdot}\in \probm{[0,2\pi)}; \text{~and~} \forall x,y\in [0,2\pi), \rho_{\Tname}(x)\leq e^{\epsilon }\rho_{\Tname}(y) \} .
\end{align*}


\begin{theorem} [corresponds to Theorem \ref{thm:main2:sim}] \label{thm:localfinal}

Let $t=2\pi / \K$ and $\beta=\frac{1}{2(e^{\epsilon/2}+1)}$. Then we have
\begin{align}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
%\inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\disrzero{a-x} }
\inf_{A\subset [0,2\pi),|A|=\K} \inf_{\Tname \in \Trobs} \Exx{x\sim \Tname}{ \min_{a\in A} \disb{\dg{x}}{\dg{a}} }
=
\beta t.
\label{eq:axsepaballthm}
\end{align}

Furthermore, one of the minimizers of the infimum in Equation \ref{eq:axsepaballthm} is
\begin{align*}
    & A^{*}=\{0,t,2t,\dots,2t(\K-1)\}, \\
    & \rho_{\Tname^{*}}(x)=
    \begin{cases}
    \alpha e^{\epsilon}, & \min_{a\in A^{*}}\disb{\dg{x}}{\dg{a}}\leq \beta t, \\
    \alpha , & \text{otherwise},
    \end{cases}
\end{align*}
where $\alpha$ is the normalizer.


\end{theorem}

\newcommand{\uc}{Uni}


\begin{proof}

    %For $A\in \Kads, \Sname \in \Srobs$, suppose $\Exx{x\sim \Sname}{ \min_{a\in A}\disrzero{a-x} }$.
    
    Let $\gamma=\min_{x\in [0,2\pi)}\rho_{\Tname}(x)$. Then $\max_{x\in [0,2\pi)}\rho_{\Tname}(x)\leq \gamma e^{\epsilon}$. Let $\uc$ denote the uniform distribution on $[0,2\pi)$. For any $A\subset [0,2\pi)$ of size $\K$, and $\Tname \in \Trobs$, we have
    \begin{align*}
        & \Exx{x\sim \Tname}{ \min_{a\in A} \disb{\dg{x}}{\dg{a}} \} } -\beta t    \\
        =& \int_{0}^{2\pi} \rho_{\Tname}(x) \left( \min_{a\in A} \disb{\dg{x}}{\dg{a}}-\beta t\right) dx  \\
        \geq & \int_{0}^{2\pi} \left( 
        \gamma \left(\min_{a\in A}\disb{\dg{x}}{\dg{a}}-\beta t\right) \I{\min_{a\in A}\disb{\dg{x}}{\dg{a}}\geq \beta t}  \right.  \\
        & ~~~~~~~~~~~~~~~~ \left. +  
        \gamma e^{\epsilon} \left(\min_{a\in A}\disb{\dg{x}}{\dg{a}}-\beta t\right) \I{\min_{a\in A}\disb{\dg{x}}{\dg{a}}< \beta t}
        \right) dx  \\
        =& 2\pi \gamma \left(  \int_{\beta t}^{+\infty}\Prxx{x\sim \uc}{\min_{a\in A}\disb{\dg{x}}{\dg{a}}>y} dy  -  e^{\epsilon} \int_{0}^{\beta t}\Prxx{x\sim \uc}{\min_{a\in A}\disb{\dg{x}}{\dg{a}}<y}dy  \right)    \\
        \geq & 2\pi \gamma \left( \int_{\beta t}^{+\infty} \max\{ 1-\frac{2\K y}{2\pi},0\}  dy  -  e^{\epsilon}  \int_{0}^{\beta t} \frac{2\K y}{2\pi} dy  \right)    \\
        =& 0,
    \end{align*}
    which implies Equation \ref{eq:axsepaballthm}.

    By computation, we can verify $\Exx{x\sim \Tname^{*}}{ \min_{a\in A^{*}} \disb{\dg{x}}{\dg{a}} }=\beta t$.

\end{proof}




==> model.tex <==
\section{Model and Overview}




%We analyze a more general case where the query and the results lie on the line, but the noise mechanism is not fixed, and the agent is free to send any arbitrary signal to the platform. For a geographicly constrained version of the privacy definition, Laplacian noise performs optimally in the worst case, assuming that the platform has no distributional information on the original query.


\subsection{Notations}

\zhihaohalfcomment{maybe write all definitions of symbols here}

We use $[m]$ to denote the set $\{1,2,\dots,m\}$, for any non-negative integer $m$. $\natr$ is the set of positive integers, $\ratn$ is the set of rational real numbers, and $\real$ is the set of real numbers.



For any vector $A\subset \Kads$, vector $v\in \rd$, and real number $c\in \real$, define addition and multiplication on sets by 
\begin{align*}
A+v & \defeq \{ a+v | a\in A \}, \\
c\cdot A & \defeq \{ c\cdot a | a\in A \}.
\end{align*}

Similarly, for any set $A\subset \sphere$, for any rotation matrix $M\in \real^{d\times d}$, define
\begin{align*}
    A M \defeq  \{aM|a\in A\},\quad
    \text{and} \quad
    M A \defeq  \{Ma|a\in A\}
\end{align*}

$\E{V}$ denotes the expectation of real random variable $V$. $\Pr{E}$ denotes the probability of an event $E$. $\I{E}$ is the indicator, which has value 1 when the event $E$ happens and has value 0 when $E$ does not happen, and thus we have $\Pr{E}=\E{\I{E}}$.

For any set $S$, $\probm{S}$ is defined as the set of probability measures on $S$.

We sometimes have integral operations. Since we are optimizing the objective over all possible mechanisms, some functions may not be continuous, and some distributions may not have density functions, so we use the Lebesgue integral.%, where the integral value is the same as Riemann integral when the functions are Riemann integrable, but it can work in more general cases.


We use $\Exx{x\sim \mu}{V(x)}$ to denote the expectation of $V(x)$ when the probability measure of $x$ is $\mu$, so
\begin{align*}
    \Exx{x\sim \mu}{V(x)} \defeq \int_{x} V(x)\mu(dx).
\end{align*}

Similarly, we use $\Prxx{x\sim \mu}{E(x)}$ to denote the probability that event $E(x)$ happens when the probability measure of $x$ is $\mu$, so
\begin{align*}
    \Prxx{x\sim \mu}{E(x)} \defeq \Exx{x\sim \mu}{\I{E(x)}} = \int_{x} \I{E(x)}\mu(dx).
\end{align*}

When a probability measure $\mu$ has a probability density, we use $\rho_{\mu}(x)$ to denote its probability density at $x$.



\subsection{Problem setting}

Users are drawn from a distribution $\Dist$, whose support is $\Users$. The set of results is also $\Ads$.

Users send a signal to the server, and the server sends back a set of $k$ results $A$, which is a subset of $\Ads$. Let $\Kads$ be the set of all possible $A$. That is,
\[ \Kads \defeq \{ A\subset \Ads: |A|=\K \}. \]

\zhihaohalfcomment{Why don't we simply assume $A \in \real^{d \times k}$ upfront, and redefine the min operator? Why do we need sets at all? }

%\zhihao{We should assume upfront that the set of signals = vector of k-ads, the user's and platform's strategy has a density, the objective is the max over the users of the error, and this error function is continuous in $\epsilon$. This will allow us to get rid of the measure-based notation and replace it with the standard notation in DP that works with density functions. Further, these are reasonable assumptions that no one will question anyway.
%In the interest of formalism, we should have an appendix where we justify the above assumptions as wlog. Have the measure-based notation and put in the argument from  pages 15-16, the lemmas from Section 5 and from the beginning of Section 6. The former is a standard way to make functions differentiable, so there should be a citation.}

We determine
\begin{enumerate}
\item A set of signals $\Signals$.  \zhihaohalfcomment{countable infinite?}
\item Action of users $\sig{u}{\C}$, denoting the probability that user $u$ sends signal $s\in \C$, for $u\in \Users$ and $\C\in \measure{\Signals}$, where $\measure{\Signals}$ is all the measurable subset of $\Signals$. 
\item Action of server $\sigq{s}{\C}$, denoting the probability that server sends back results $A\in \C$ when receiving signal $s$, for $s\in \Signals$ and $\C\in \measure{\Kads}$, where $\measure{\Signals}$ is all the measurable subset of $\Signals$. 
\end{enumerate}

The system should have differential privacy. We consider two definitions of privacy.
\begin{enumerate}
    \item Geographic differential privacy. For any $\C\in \measure{\Signals}$, for any $u_1,u_2\in \Users$, $\sig{u_1}{\C}\leq e^{\epsilon\cdot \dis{u_1}{u_2}} \sig{u_2}{\C}$, where $\dis{u_1}{u_2}$ is a distance between $u_1$ and $u_2$.
    \item Local differential privacy. For any $\C\in \measure{\Signals}$, for any $u_1,u_2\in \Users$, $\sig{u_1}{\C}\leq e^{\epsilon} \sig{u_2}{\C}$.
\end{enumerate}

\iffalse%
\begin{enumerate}
  \item geographicly differential privacy. For any $\C\in \Signals$, for any $u_1,u_2\in \Users$, $\sig{u_1}{\C}\leq e^{\epsilon \cdot \dis{u_1}{u_2}} \sig{u_2}{\C}$, where $\dis{u_1}{u_2}$ is the distance between $u_1$ and $u_2$.
  \item Local differential privacy. For any $\C\in \Signals$, for any $u_1,u_2\in \Users$, $\sig{u_1}{\C}\leq e^{\epsilon} \sig{u_2}{\C}$.
\end{enumerate}
\fi%

We want to minimize the distance between the user and the closest ad that the user receives, in the worst case with respect to the distribution of users. Formally, we want to compute
\[  \funf{\Users}{\Ads}{\epsilon}{\K} \defeq  \inf_{\Signals}\inf_{\Pname\in \Probs{\Signals},\Qname\in \Qrobs_{\Signals}} \sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\disg{u}{a} }, \]
where
\begin{enumerate}
    \item $\Signals$ can be any set.
    \item $\disg{u}{a}$ is the distance between $u$ and $a$. When we are interested in geographic differential privacy on $\rd$, $\disg{u}{a}=\dis{u}{a}$. When we are interested in local differential privacy on $\sphere$, $\disg{u}{a}=\disbb{u}{a}$, which is the angle difference between $u$ and $a$. We call $\Exx{s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\disg{u}{a} }$ the error of user $u$.
    %\item $\Probs{\Signals}:=\{ \Pname | \forall u\in \Users, \sig{u}{\cdot}\in \probm{\Signals}; \text{~and~} \forall u_1,u_2\in \Users, \forall \C\in \measure{\Signals}, \sig{u_1}{\C}\leq e^{\epsilon\cdot \defdis{u_1}{u_2}} \sig{u_2}{\C}; \\ ~~~~~~~~~~~~~~~~~~~~~~\text{~and~} \text{~$\Pname_{u}(\C)$ is jointly measurable in $u$ and $\C$} \}$,
    
    %where $\defdis{u_1}{u_2}=\dis{u_1}{u_2}$ when we are interested in geographic differential privacy, and $\defdis{u_1}{u_2}=1$ when we are interested in local differential privacy.

    \item $\Probs{\Signals}$ is the set of mechanism satisfying (geographic or local) differential privacy.
    
    \item $\Qrobs_{\Signals}:=\{ \Qname | \forall s\in \Signals, \sigq{s}{\cdot}\in \probm{\Kads} \}$, which is the set of available actions of the server.
\end{enumerate}


\zhihaohalfcomment{need assumption, e.g. $P_{x}(y)$ is measurable w.r.t. $(x,y)$. Otherwise the construction of new mechanism is not well defined}


\subsection{Summary of Results}

We study both the geographic differential privacy model and the local differential privacy model.

In either model, one of the optimal mechanisms satisfies $H=\Kads$, which means the signals sent by users and servers can be drawn from the same set. In fact, the server will directly return the signal it receives. Furthermore, we do not need to consider all the distribution over users, we only care about the user that has the largest error. 

\begin{theorem} \label{thm:main0}

\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname\in \Probs{\Kads}} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }.
\end{align*}

\end{theorem}

\paragraph{Geographic differential privacy}

Before presenting our theorem, we define symmetry of mechanism. If all users add i.i.d. (independent and identically distributed) noises upon their private values, then we say the mechanism is symmetric.

\begin{definition}[symmetric mechanism when $\Users=\rd$] \label{def:symmetric:pre}

For $\Pname\in \Probs{\Kads}$, if for any $u\in \Users, \C\in \measure{\Kads}, c\in \rd$,
\begin{align*}
    \Pxx{u}{\C}=\Pxx{u+c}{\C+c},
\end{align*}
then we say $\Pname$ is a symmetric mechanism.

%Let $\Psym$ be the set of symmetric mechanisms.

\end{definition}



We will show, in geographic differential privacy model, if users and results are drawn from $\real^{\Dim}$, symmetric mechanism one of the optimal choices for users. Specially, when $\Dim=1$, Laplace noise is one of the optimal choices for users.

\begin{theorem}\label{thm:main1}

For geographic differential privacy, if $\Users=\real^{\Dim}$, it is sufficient to only consider symmetric mechanisms. If $\Dim=1$, adding Laplace noise, whose density function is $\rho(x)=e^{-\epsilon \disrzero{u}{x}}/\epsilon$, is one of the optimal choices for users, and in this case $\funf{\Users}{\Ads}{\epsilon}{\K}$ is $O(1/(\epsilon \K))$. Furthermore, when $d=1$, the optimal mechanism can be computed in closed form (Corollary \ref{cor:geofinal}).


\iffalse%%%%%%%%%%%%%%%%
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\begin{cases}
\frac{4}{\epsilon(\K +1)} , & \text{$\K$ is odd},  \\
\frac{2}{\epsilon} \log\left( 1+\frac{2}{\K} \right) , & \text{$\K$ is even},  \\
\end{cases}
\end{align*}
which is $O(1/(\epsilon \K))$. Moreover, in one of the optimal mechanisms, user $u\in \real$ sends signal $u+\eta$, where $\eta$ is drawn from the distribution with density function $\rho(x)=e^{-\epsilon \disrzero{u}{x}}/\epsilon$, and when the server receives signal $s\in \real$, it sends back $\{s+a_1, s+a_2, \dots, s+a_{\K}\}$, where
\begin{enumerate}
    \item If $\K$ is odd, let $t=(\K -1)/2$, and
    \begin{align*}
        \{a_1,\dots,a_{\K}\}=\left\{
        0, \pm \frac{2\log\left(\frac{t+1}{t}\right)}{\epsilon},
        \pm \frac{2\log\left(\frac{t+1}{t-1}\right)}{\epsilon},
        \dots,
        \pm \frac{2\log\left(\frac{t+1}{2}\right)}{\epsilon},
        \pm \frac{2\log\left(t+1\right)}{\epsilon}
        \right\}.
    \end{align*}
    \item If $\K$ is even, let $t=\K/2$, and
    \begin{align*}
        \{a_1,\dots,a_{\K}\}=\left\{
         \pm \frac{\log\left(\frac{t+1}{t}\right)}{\epsilon},
        \pm \frac{\log\left(\frac{t(t+1)}{(t-1)^2}\right)}{\epsilon},
        \pm \frac{\log\left(\frac{t(t+1)}{(t-2)^2}\right)}{\epsilon},
        \dots,
        \pm \frac{\log\left(\frac{t(t+1)}{2^2}\right)}{\epsilon},
        \pm \frac{\log\left(t(t+1)\right)}{\epsilon}
        \right\}.
    \end{align*}
\end{enumerate}
\fi%%%%%%%%%%%%%%%%%%%%%%%%



\end{theorem}



\paragraph{Local differential privacy}


Before presenting our theorem, we define symmetry of mechanism. If all users add i.i.d. (independent and identically distributed) \emph{rotation} noises upon their private values, then we say the mechanism is symmetric.

\begin{definition}[symmetric mechanism when $\Users=\sphere$]


For $\Pname\in \Probs{\Kads}$, if for any $u\in \Users, \C\in \measure{\Kads}$, for any rotation matrix $M\in \real^{d\times d}$,
\begin{align*}
    \Pxx{u}{\C}=\Pxx{uM}{\C M},
\end{align*}
then we say $\Pname$ is a symmetric mechanism.

%Let $\Psym$ be the set of symmetric mechanisms.


\end{definition}


\begin{theorem}\label{thm:main2}




For local differential privacy, if $\Users=\sphere \defeq \{x\in \real^{\Dim}| \diszero{x}=1\}$, it is sufficient to only consider symmetric mechanisms. If $\Dim=2$, when $\sphere$ is a ring, adding a noise with $\K$ equidistant peaks is one of the optimal mechanisms, and in this case, $\funf{\Users}{\Ads}{\epsilon}{\K}$ is $O(1/\K)$. Furthermore, when $d=2$, the optimal mechanism can be computed in closed form (Theorem \ref{thm:localfinal}).




\iffalse%%%%%%%%%%%%%

If $\Dim=2$, when $\sphere$ is a ring, adding a noise with $\K$ equidistant peaks is one of the optimal mechanisms, and in this case, let $t=2\pi / \K$ and $\beta=\frac{e^{\epsilon/2}-1}{2(e^{\epsilon}-1)}$, and we have
\[ \funf{\Users}{\Ads}{\epsilon}{\K}=\beta t = \frac{\pi(e^{\epsilon/2}-1)}{\K(e^{\epsilon}-1)}, \]
which is $O(1/\K)$. Moreover, if we use real number $x\in [0,2\pi)$ to denote the point $(\cos x,\sin x)^{T}$ on $\spherex{2}$ (and if a real number $x$ is not in $[0,2\pi)$, it means $(x~\text{mod}~2\pi)$), in one of the optimal mechanisms, user $u\in \real$ sends signal $u+\eta$, where $\eta\in [0,2\pi)$ is drawn from the distribution with density function
\begin{align*}
    \rho_{\Sname}(\eta)=
    \begin{cases} 
    \alpha , & \beta t< (\eta~\text{mod}~t)< (1-\beta)t,\\
    \alpha e^{\epsilon}, & \text{otherwise},
    \end{cases}
\end{align*}
where $\alpha$ is the normalizer, and when the server receives signal $s\in \real$, it sends back $\{s, s+t, \dots, s+(\K-1)t\}$.

\fi%%%%%%%%%%%%%%%





\end{theorem}







==> non-opt-ex.tex <==
\section{Calculation of Figure \ref{fig:intro3}}    \label{sec:non-opt-ex}

%Given two ads, the unit ring is divided into two half rings, such that the users on one half ring will choose one ad because it is closer, and the users on the other half ring will choose the other ad. As a result, we consider the two half rings independently. The problem becomes, given a half of a unit ring, design a distribution on it, and choose an ad on it. The objective is to minimize the distance between the ad and a user drawn from the distribution.

We calculate the optimal mechanism in geographic differential privacy setting, on a unit ring, when $\epsilon=3/8$, and the number of results is $\K=2$.


Using similar notations as Section \ref{sec:unitring}, we use real numbers in $[0,2\pi)$ to denote users and results on a unit ring, and the original problem is to optimize
\begin{align*}
    \min_{a_1\in [0,2\pi), a_2\in [0,2\pi), \rho(x)} \int_{0}^{2\pi} \min\{\disb{x}{a_1},\disb{x}{a_2}\} \rho(x) dx,
\end{align*}
where $\rho(x)$ is a density function on $[0,2\pi)$ that satisfies differential privacy. That is, for any $x_1,x_2\in [0,2\pi)$, $\rho(x_1)\leq e^{\epsilon \disb{x_1}{x_2}}  \rho(x_2)$.

W.l.o.g., assume $a_1\leq a_2$ and $a_1+a_2=2\pi$. In this case, users in $[0,\pi)$ will choose ad $a_1$ because it is closer, and similarly, users in $[\pi,2\pi)$ will choose $a_2$. Then the problem becomes
\begin{align*}
    \min_{a_1\in [0,\pi), \rho(x)} \left( \int_{0}^{\pi} \disb{x}{a_1} \rho(x) dx + \int_{\pi}^{2\pi} \disb{x}{2\pi-a_1} \rho(x) dx \right),
\end{align*}
where $\rho(x)$ is a density function on $[0,2\pi)$ that satisfies differential privacy.

Since we can consider $[0,\pi)$ and $[\pi,2\pi)$ independently, it is sufficient to optimize
\begin{align*}
    \min_{a\in [0,\pi), \rho(x)} \int_{0}^{\pi} |x-a| \rho(x) dx ,
\end{align*}
where $\rho(x)$ is a density function on $[0,\pi)$ that satisfies differential privacy. Note that $\disb{x}{a}=|x-a|$ when $x,a\in [0,\pi)$.

Using similar arguments as Lemma \ref{lem:h}, the optimal solution satisfies $\rho(x)=c_1 e^{\epsilon x}$ on $[0,t)$ for a certain $c_1\in (0,+\infty)$ and a certain $t\in [0,\pi)$. And it holds that $\rho(x)=c_2 e^{\epsilon x}$ on $[t,\pi)$ for a certain $c_2\in (0,+\infty)$. Since $\rho(x)$ is continuous, and $\int_{0}^{\pi}\rho(x)dx=1$, the density function $\rho(x)$ is determined given $t$. Note that the optimal $a$ is the median of the distribution $\rho(x)$, so $a$ is also determined given $t$. As a result, the only decision is $t$, and the objective function can be written as a function of $t$. Based on calculation on computer, the optimal $t$ is $\pi/2$, which corresponds to the optimal mechanism in Figure \ref{fig:intro3}.



==> ourresult-modified.tex <==
%\subsection{Our results}

%\todo{Provide more context about geographic vs local differential privacy. Explain why we use the line in one case and the ring in the other. }
%\todo{Explain that we need to both provide the noise mechanism and the server's algorithm.}

%\todo{We use server and server interchangably. Mention this somewhere or use server throughout. Similarly for client and user.}


% \subsection{Summary of Results}
% Our main result is to derive optimal mechanisms for the case of geographic DP on an infinite line. The results show an excellent benefit of the new system architecture for the privacy / utility trade-offs.

%In particular, we show that that an user's optimal response may be to add 
%The results are in alignment with the strength of the privacy guarantees of the model --- better utility gain / lower cost of privacy for the weaker privacy definition of geographic DP than local DP. 
%The results show an excellent benefit of the new system architecture for the privacy / utility trade-offs.
%\ak{Comment here or somewhere that results are in alignment with the strength of the privacy guarantees of the model -- better utility gain / lower cost of privacy for the weaker privacy definition of geographic DP than local DP. At the same time, results show an excellent benefit of the new system architecture for the privacy / utility trade-offs.}
 
 
% \todo{The introduction does not map to how the paper is actually organized. It's better to drop the paragraph below and instead use the first paragraph of related work here.} 

% \todo{We don't actually do this first.} We will analyze the quality improvement obtained in the simplest scenario -- when the user's query as well as the search results lie on the line, every point is a valid query and a valid search result,  the noise added is Laplace noise with parameter $\epsilon$, and the ``cost" of a search result is measured by the distance between the original query and the result. We will assume that the server has no distributional information on the original query beyond what it can infer from the noisy version. We will show that with $2k-1$ results, the cost goes down by a factor of $k$. Given the dramatic increase in network bandwidth and server capabilities of the last several decades, this approach offers an attractive pathway to reducing the ``cost of privacy".

%We will then analyze the more general case where the query and the results still lie on the line and the quality measure is the same, but the noise mechanism is not fixed, and the user is free to send any arbitrary signal to the server. For both the local Differential Privacy guarantees which are considered the theoretical gold standard, and a geographically constrained version, which is more pragmatic and perhaps more relevant in some practical settings, we show that the simple approach outlined earlier (i.e. the privacy user adds a Laplace noise to the query and then relies on the server to return the optimum solution to the ``Multi-Selection" problem) is optimum.





\subsection{Geographic DP} 
In the geographic differential privacy setting, we study the case where users and results (ads) are located on a (doubly infinite) line and thus, the optimum result for an user $u$ is the result $u$ itself. We employ this model for clarity in presentation, yet our results extend well beyond this setup. In particular, we relax this assumption in Appendix \ref{appendix-sec:restricted_unrestricted_setup} letting the results and users lie in different sets. In this case, the following mechanism is natural: the client adds Laplace noise to the query, \ak{need to say how the Laplace noise is calibrated wrt sensitivity}
and the server returns the set of values $S$ of size $k$ which minimizes the expected dis-utility of the original query from the closest value in $S$. \ak{the dis-utility and notation for it was only defined in passing; need a formal definition.}
\ak{Cost of privacy, about to be used next, was also not formally defined.}
For the case of $\mathfrak{h}(t)=t$, we show that this set of values can be explicitly (and easily) calculated using a simple recurrence (Section \ref{subsec-comb:step4}), and when $k$ is odd, it cuts down the cost of privacy by a factor of $(k+1)/2$, comparing to the cost when $k=1$. \ak{-> comparing to the cost when only one result is returned.}
For general $\mathfrak{h}(.)$, the recurrence still holds but a closed-form solution may not exist. Our main result shows that this natural mechanism is optimal. This proof is non-trivial and does not follow from the optimality of such noise when $k=1$ as shown in \cite{koufogiannis2015optimality}. %which is significantly more involved (we can not simply assume that adding Laplace noise is optimum, given that the server could have an arbitrarily complex algorithm). 
%  \todo{Maybe put an informal problem definition and theorem statement here?}
Figure \ref{fig:intro1} is an instance of the optimal mechanism.


  \begin{figure}
      \centering
        \begin{tikzpicture}
        \coordinate (right) at (8,0);
        \coordinate (left) at (0,0);
        \coordinate (o) at (4,0);
        \coordinate (up) at (4,3);
        \coordinate (x0) at (4.5,0);
        \coordinate (s) at (2,0);
        \coordinate (t) at (5.5,0);
        \coordinate (cone) at (4,2.5);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[->](o)--(up);
        \draw[<->](left)--(right);
        \draw[-](cone)--(4.1,2.5);
        \draw node at (3.65,2.5) {$0.5$};
        \draw node at (4.0,-0.3) {$O$};
        \draw node at (4.45,3.1) {$\rho(t)$};
        \draw node at (7.9,-0.2) {$t$};
        % here, eps=0.55
        \draw[blue,domain=0:4] plot(\x,{2.5*exp((\x-4))} );
        \draw[blue,domain=4:8] plot(\x,{2.5*exp(-(\x-4))} );
        \coordinate (r0) at (4,0);
        \coordinate (r3) at ([xshift = 1.3862943611198906188344642429164*2.5 cm] r0);
        \coordinate (r2) at ([xshift = -0.69314718055994530941723212145818*2.5 cm] r3);
        \coordinate (r1) at ([xshift = -1.0986122886681096913952452369225*2.5 cm] r3);
        \coordinate (r-3) at ([xshift = -1.3862943611198906188344642429164*2.5 cm] r0);
        \coordinate (r-2) at ([xshift = 0.69314718055994530941723212145818*2.5 cm] r-3);
        \coordinate (r-1) at ([xshift = 1.0986122886681096913952452369225*2.5 cm] r-3);
        \fill (r0) circle (2pt);
        \fill (r1) circle (2pt);
        \fill (r2) circle (2pt);
        \fill (r3) circle (2pt);
        \fill (r-1) circle (2pt);
        \fill (r-2) circle (2pt);
        \fill (r-3) circle (2pt);
        \coordinate (rowone) at ([xshift=2.5cm] o);
        \coordinate (row-one) at ([xshift=-2.5cm] o);
        \coordinate (rowonec) at ([yshift=-0.3cm] rowone);
        \coordinate (row-onec) at ([yshift=-0.3cm] row-one);
        \coordinate (rowonel) at ([yshift=0.1cm] rowone);
        \coordinate (row-onel) at ([yshift=0.1cm] row-one);
        \draw node at (rowonec) {$1$};
        \draw node at (row-onec) {$-1$};
        \draw[-](rowone)--(rowonel);
        \draw[-](row-one)--(row-onel);
        \end{tikzpicture}
      \caption{Optimal mechanism in geographic differential privacy setting when $\K=7$ and $\epsilon=1$. Suppose the user has a private value $v$. Then the user sends $v+x$ to the server, where $x$ is drawn from Laplace distribution with density $\rho(t)$. \ak{ Also, the distribution should contain $\epsilon$ in its definition!}
      \sss{We fix $\epsilon=1$ for this case.}
      \ak{I know you do, but that's not rigorous, the distribution should be defined in terms of $epsilon$}
      Suppose the server receives $s$. Then the server responds $s+a_1,...,s+a_7$, where the values of $a_1,a_2,...,a_7$ are denoted by black dots on the $x$-axis.
      \ak{For the illustration to be clear, also needs the response dots for discrete Laplace, i.e. if we were to discretize Laplace and truncate to only 7 values, what would they be?}
      }    \label{fig:intro1}
  \end{figure}

\ak{This is the most important paragraph in the section so it needs to convey both the result and the intuition behind the result impeccably.}  
To prove this result, we pretend that the user has full information and is directly choosing a set $S$ of size $k$ to minimize the expected dis-utility from its query while ensuring that the set $S$ satisfies geographic differential privacy. \ak{Need the intuition for why set $S$ satisfying DP is equivalent to the user query satisfying DP; is it??}
This involves optimizing over all possible $k$-dimensional distributions for $S$ for which we construct a linear program over infinite dimensional spaces \ak{why does it need to be infinite dimensional?} \sss{This is because we are optimizing over all possible distributions which is a function space}involving both integrals and derivatives. 
We next show that a two-stage mechanism, where the user sends a single noisy value and the server chooses $k$ results by adding $k$ {\em fixed increments} to the chosen value is optimal via dual-fitting, i.e. construction of a feasible solution to a dual infinite dimensional linear program attaining the same objective value. 
\ak{It's unclear whether the two-stage mechanism arises from the solution to the optimization problem or from our problem set-up -- user sends noisy value and receives k results.}
Since to the best of our knowledge, duality theory for infinite dimensional linear programs exists only for programs involving integrals, we prove the weak duality theorem for our linear programs.

%We first show that there exists an optimal mechanism that is symmetric, i.e. shifting the query along the line translates the entire distribution by the same amount. We then show that a two-stage mechanism, where the user sends a single noisy value and the server chooses $k$ results by adding $k$ {\em fixed increments} to the chosen value, is optimal for symmetric distributions. Finally, we show that for such mechanisms, adding Laplace noise is optimal. 

We emphasize that the optimality of adding Laplace noise is far from obvious\footnote{In fact, only a few optimal mechanisms are known~\cite{Ghosh2012privacy, gupte2010universally, kairouz2014extremal, ding2017collecting}, and it is known that for certain scenarios, universally optimal mechanisms don't exist~\cite{brenner2014impossibility}.}. For instance, when users and results are located on a ring, Laplace noise is {\em not optimal}. 
While we have not been able to analyze the ring in complete generality for geographic DP, we have been able to explicitly solve it for some specific simple cases. 
Figure \ref{fig:intro3} illustrates the optimal mechanism under geographic DP for $k=2$. This mechanism uses noise that is a piece-wise composition of Laplace noises; we obtain a cost of 0.72 \remove{n improvement of a factor of 0.558 with this optimal mechanism}whereas Laplace noise gives a cost of 0.75. \remove{ an improvement of only 0.585.} \ak{Very difficult to put these numbers in context, especially that the dependence on $\epsilon$ is hidden and how ``improvement" is measured is not defined.}
We sketch the calculation in Appendix~\ref{sec:non-opt-ex}.
\ak{Would it be possible to numerically solve for a few more cases and make a table of improvements for various values of $\epsilon$ and various values of $k$?}

%\sss{Is Figure 3 optimal or just a factor improvement over Laplace?}
  
  \begin{figure}
      \centering
        \begin{tikzpicture}
        \coordinate (right) at (7.5,0);
        \coordinate (o) at (0,0);
        \coordinate (up) at (0,3);
        \coordinate (x0) at (4.5,0);
        \coordinate (s) at (2,0);
        \coordinate (t) at (5.5,0);
        %
        \coordinate (key1) at (8,2.5);
        \coordinate (key2) at (8.7,2.5);
        \draw[blue,dashed] (key1)--([xshift=0.5cm]key1);
        \fill[blue] ([xshift = -0.070292 cm, yshift = -0.070292 cm]key2) rectangle ([xshift = 0.070292 cm, yshift = 0.070292 cm]key2);
        \draw node at ([xshift = 1.5 cm] key2) {\footnotesize Laplace mechanism};
        \coordinate (key3) at (8,2);
        \coordinate (key4) at (8.7,2);
        \draw[red] (key3)--([xshift=0.5cm]key3);
        \fill[red] (key4) circle (2pt);
        \draw node at ([xshift = 1.5 cm] key4) {\footnotesize Better mechanism};
        %
        \draw (7.7,1.7) rectangle (11.7,2.8);
        %
        \coordinate (cone1) at (0,1);
        \coordinate (cone2) at (0,2);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[->](o)--(up);
        \draw[->](o)--(right);
        \draw[-](cone1)--([xshift = 0.1 cm]cone1);
        \draw[-](cone2)--([xshift = 0.1 cm]cone2);
        \draw node at ([xshift = -0.3 cm] cone1) {$0.1$};
        \draw node at ([xshift = -0.3 cm] cone2) {$0.2$};
        \coordinate (piv) at (3.5,0);
        \draw[-](piv)--([yshift = 0.1 cm] piv);
        \coordinate (2piv) at (7,0);
        \draw[-](2piv)--([yshift = 0.1 cm] 2piv);
        \draw node at ([yshift = -0.3 cm] piv) {$\pi$};
        \draw node at ([yshift = -0.3 cm] 2piv) {$2\pi$};
        \draw node at ([xshift = -0.05 cm, yshift = -0.3 cm] o) {$O$};
        \draw node at (0.45,3.1) {$\rho(x)$};
        \draw node at ([xshift = -0.05 cm, yshift = -0.2 cm] right) {$x$};
        % here, eps=0.55
        \draw[blue,dashed,domain=0:3.5] plot(\x,{0.834005054395031*exp(-(\x-3.5)*pi*3/28)} );
        \draw[blue,dashed,domain=3.5:7] plot(\x,{0.834005054395031*exp((\x-3.5)*pi*3/28)} );
        \draw[red,domain=0:1.75] plot(\x,{1.168554905236987*exp(-(\x-1.75)*pi*3/28)} );
        \draw[red,domain=1.75:3.5] plot(\x,{1.168554905236987*exp((\x-1.75)*pi*3/28)} );
        \draw[red,domain=3.5:5.25] plot(\x,{1.168554905236987*exp(-(\x-5.25)*pi*3/28)} );
        \draw[red,domain=5.25:7] plot(\x,{1.168554905236987*exp((\x-5.25)*pi*3/28)} );
        %\draw[blue,domain=:] plot(\x,{2.6240214001267626006468162172726} );
        %\draw[blue,domain=:] plot(\x,{0.9653235263005390754197259800987} );
        
        \coordinate (r0) at (1.261892227103695,0);
        \coordinate (r1) at (5.738107772896305,0);
        \fill[red] (o) circle (2pt);
        \fill[red] (piv) circle (2pt);
        \fill[blue] ([xshift = -0.070292 cm, yshift = -0.070292 cm]r0) rectangle ([xshift = 0.070292 cm, yshift = 0.070292 cm]r0);
        \fill[blue] ([xshift = -0.070292 cm, yshift = -0.070292 cm]r1) rectangle ([xshift = 0.070292 cm, yshift = 0.070292 cm]r1);
        \end{tikzpicture}
      \caption{Geographic differential privacy setting when users and results are located on a unit ring, for $\K=2$ and $\epsilon=3/8$, showing the stark difference between Laplace noise and the optimal noise. Suppose the user has a private value $v$. Then the user sends $v+x$ to the server, where $x$ is drawn from a noise distribution with density $\rho(x)$, depicted here for both Laplace noise and the optimal noise. Suppose the server receives $s$. Then the server's optimal response is $s+a_1$ and $s+a_2$, where the values of $a_1,a_2$ are denoted by dots on the $x$-axis, again assuming both Laplace noise and the optimal noise. \ak{The figure has similar challenges as the previous one (e.g. lack of dependence on $\epsilon$). \ak{The picture for Laplace doesn't look like a traditional Laplace, why?}}
      \sss{The laplace does not look like traditional Laplace as we should interpret 0 and $2\pi$ to be identical points since they lie on a ring. Thus, we should interpret the region from $[\pi,2\pi]$ as $(-\pi,0)$. \ak{Needs to be explained in the caption for the reader. Also, even on the (0, $\pi$) it doesn't look like half the Laplace, maybe because $\epsilon is 3/8$ and so it's hard to see the curviness... }}
      }%\todo{Can we not rely on color to state which noise is which? Use different colors as well as different type, e.g. dotted vs not for line, and x vs triangle for points, and add a key to the image itself stating which curve corresponds to what. Then reduce the description in the text.}   
      \label{fig:intro3}
  \end{figure}



% {Local DP.} We next consider local differential privacy, when users and results are located on a ring. We will use the angle in $[0,2\pi)$ to denote the position. One optimal mechanism is the following. Users add one type of piece-wise constant noise to the private value before sending it. The server responds $\K$ results by adding the received signal by an angle $2\pi i/\K$ for $0\leq i<\K$. Figure \ref{fig:intro2} is an instance of the optimal mechanism. As with geographic DP, the accuracy of this mechanism is $O(1/k)$. The analysis builds on that for geographic DP: the result described earlier for symmetric distribution holds for this case as well, and only the final step of the analysis is different (and more straightforward).
  
%   \begin{figure}
%       \centering
%         \begin{tikzpicture}
%         \coordinate (right) at (7.6,0);
%         \coordinate (o) at (0,0);
%         \coordinate (up) at (0,3);
%         \coordinate (x0) at (4.5,0);
%         \coordinate (s) at (2,0);
%         \coordinate (t) at (5.5,0);
%         \coordinate (cone1) at (0,1);
%         \coordinate (cone2) at (0,2);
%         %\draw node at ([yshift=-0.3cm]y) {$y$};
%         %\draw node at ([yshift=-0.3cm]z) {$z$};
%         %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
%         %\draw node at ([yshift=-0.3cm]s) {$s$};
%         %\draw node at ([yshift=-0.3cm]t) {$t$};
%         \draw[->](o)--(up);
%         \draw[->](o)--(right);
%         \draw[-](cone1)--([xshift = 0.1 cm]cone1);
%         \draw[-](cone2)--([xshift = 0.1 cm]cone2);
%         \draw node at ([xshift = -0.3 cm] cone1) {$0.1$};
%         \draw node at ([xshift = -0.3 cm] cone2) {$0.2$};
%         \coordinate (piv) at (3.5,0);
%         \draw[-](piv)--([yshift = 0.1 cm] piv);
%         \coordinate (2piv) at (7,0);
%         \draw[-](2piv)--([yshift = 0.1 cm] 2piv);
%         \draw node at ([yshift = -0.3 cm] piv) {$\pi$};
%         \draw node at ([yshift = -0.3 cm] 2piv) {$2\pi$};
%         \draw node at ([xshift = -0.05 cm, yshift = -0.3 cm] o) {$O$};
%         \draw node at (0.45,3.1) {$\rho(x)$};
%         \draw node at ([xshift = -0.05 cm, yshift = -0.2 cm] right) {$x$};
%         % here, eps=0.55
%         \draw[blue,domain=0:0.26427846815870180475276960397815] plot(\x,{2.6240214001267626006468162172726} );
%         \draw[blue,domain=0.26427846815870180475276960397815:1.1357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
%         %\draw[blue,domain=:] plot(\x,{2.6240214001267626006468162172726} );
%         %\draw[blue,domain=:] plot(\x,{0.9653235263005390754197259800987} );
%         \draw[blue,domain=1.1357215318412981952472303960219:1.6642784681587018047527696039782] plot(\x,{2.6240214001267626006468162172726} );
%         \draw[blue,domain=1.6642784681587018047527696039782:2.5357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
%         \draw[blue,domain=2.5357215318412981952472303960219:3.0642784681587018047527696039782] plot(\x,{2.6240214001267626006468162172726} );
%         \draw[blue,domain=3.0642784681587018047527696039782:3.9357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
%         \draw[blue,domain=3.9357215318412981952472303960219:4.4642784681587018047527696039782] plot(\x,{2.6240214001267626006468162172726} );
%         \draw[blue,domain=4.4642784681587018047527696039782:5.3357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
%         \draw[blue,domain=5.3357215318412981952472303960219:5.8642784681587018047527696039782] plot(\x,{2.6240214001267626006468162172726} );
%         \draw[blue,domain=5.8642784681587018047527696039782:6.7357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
%         \draw[blue,domain=6.7357215318412981952472303960219:7] plot(\x,{2.6240214001267626006468162172726} );
% %%
% %0.26427846815870180475276960397815
% %1.1357215318412981952472303960219
% %1.6642784681587018047527696039782
% %2.5357215318412981952472303960219
% %3.0642784681587018047527696039782
% %3.9357215318412981952472303960219
% %4.4642784681587018047527696039782
% %5.3357215318412981952472303960219
% %5.8642784681587018047527696039782
% %6.7357215318412981952472303960219
% %7
% %%
%         \coordinate (r0) at (o);
%         \coordinate (r1) at ([xshift = 1.4 cm] r0);
%         \coordinate (r2) at ([xshift = 1.4 cm] r1);
%         \coordinate (r3) at ([xshift = 1.4 cm] r2);
%         \coordinate (r4) at ([xshift = 1.4 cm] r3);
%         \fill (r0) circle (2pt);
%         \fill (r1) circle (2pt);
%         \fill (r2) circle (2pt);
%         \fill (r3) circle (2pt);
%         \fill (r4) circle (2pt);
%         \end{tikzpicture}
%       \caption{Optimal mechanism in local differential privacy setting when $\K=5$ and $\epsilon=1$. Suppose the user has a private value $v$. Then the user sends $v+x$ to the server, where $x$ is drawn from a noise distribution with density $\rho(x)$. Suppose the server receives $s$. Then the server responds $s+a_1,...,s+a_5$, where the values of $a_1,a_2,...,a_5$ are denoted by black dots on the $x$-axis.}  %\todo{I do not understand this figure. Is the distribution discontinuous? Reply: The distribution is continuous, but the density of the distribution is piece-wise, which means the density function is not continuous}  
%       \label{fig:intro2}
%   \end{figure}

\subsection{Other Noise Models \ak{Situate this appropriately either in 1.2 or in the proof; is this one of the main results listed in 1.2 bullet points? If yes, move to Section 2; if not, add a bullet point at the level of abstraction like in 1.2}} In the analysis above, we assumed that we are given a desired geographic privacy guarantee, and we find the optimal noise as well as the optimal server response to minimize the cost of privacy. In practical situations, it is likely that the noise that is added is not under our control. We show that for the one-dimensional case, as long as the noise that is added by the client satisfies the Monotone Hazard Rate property (which both Laplace noise as well as the commonly used Gaussian noise do), the cost function \ak{before we talked about the cost of privacy, now we are talking about accuracy guarantee; both and the way improvement is measured need to be rigorously defined.} improves as $\tilde{O}\left(\frac{1}{k}\right)$, comparing to the case $k=1$; further, this improvement can be obtained by sampling from the posterior distribution of the noise. The proof is deferred to Appendix~\ref{sec-appendix:mhr}.

We finally note that though the one-dimensional case is somewhat stylized, our main contribution is to show that even this case requires non-trivial ideas. In practice, a server could employ dimension reduction techniques such as Principal Component Analysis (PCA) to create a small number $d$ of dimensions. \ak{Unclear why the server would benefit by creating a small number of dimensions?}
In this case, techniques similar to what we have presented show that the accuracy improves as $\Theta\left(\frac{1}{k^{1/d}}\right)$, and it is conceivable the improvement is even better in the wild. We discuss this in detail with some assumptions in Appendix~\ref{sec-appendix:high-dim-space} under the case where the user disutility does not increase in every dimension but increases in some $d'$ dimensions. \ak{Unclear what this means}


==> ourresult.tex <==
%\subsection{Our results}

%\todo{Provide more context about geographic vs local differential privacy. Explain why we use the line in one case and the ring in the other. }
%\todo{Explain that we need to both provide the noise mechanism and the server's algorithm.}

%\todo{We use server and server interchangably. Mention this somewhere or use server throughout. Similarly for client and user.}


\subsection{Summary of Results}
Our main result is to derive closed-form optimal mechanisms for the two canonical cases of geographic DP on an infinite line and local DP on a ring.
%The results are in alignment with the strength of the privacy guarantees of the model --- better utility gain / lower cost of privacy for the weaker privacy definition of geographic DP than local DP. 
The results show an excellent benefit of the new system architecture for the privacy / utility trade-offs.
%\ak{Comment here or somewhere that results are in alignment with the strength of the privacy guarantees of the model -- better utility gain / lower cost of privacy for the weaker privacy definition of geographic DP than local DP. At the same time, results show an excellent benefit of the new system architecture for the privacy / utility trade-offs.}
 
 
% \todo{The introduction does not map to how the paper is actually organized. It's better to drop the paragraph below and instead use the first paragraph of related work here.} 

% \todo{We don't actually do this first.} We will analyze the quality improvement obtained in the simplest scenario -- when the user's query as well as the search results lie on the line, every point is a valid query and a valid search result,  the noise added is Laplace noise with parameter $\epsilon$, and the ``cost" of a search result is measured by the distance between the original query and the result. We will assume that the server has no distributional information on the original query beyond what it can infer from the noisy version. We will show that with $2k-1$ results, the cost goes down by a factor of $k$. Given the dramatic increase in network bandwidth and server capabilities of the last several decades, this approach offers an attractive pathway to reducing the ``cost of privacy".

%We will then analyze the more general case where the query and the results still lie on the line and the quality measure is the same, but the noise mechanism is not fixed, and the user is free to send any arbitrary signal to the server. For both the local Differential Privacy guarantees which are considered the theoretical gold standard, and a geographically constrained version, which is more pragmatic and perhaps more relevant in some practical settings, we show that the simple approach outlined earlier (i.e. the privacy user adds a Laplace noise to the query and then relies on the server to return the optimum solution to the ``Multi-Selection" problem) is optimum.

\paragraph{Geographic DP.} 
In the geographic differential privacy setting, we study the case where users and results (ads) are located on a (doubly infinite) line. In this case, the following mechanism is natural: the client adds Laplace noise to the query, and the server returns the set of values $S$ of size $k$ which minimizes the expected distance of the original query from the closest value in $S$. We show that this set of values can be explicitly (and easily) calculated using a simple recurrence (Section \ref{sec:simres}), and when $k$ is odd, it cuts down the cost of privacy by a factor of $(k+1)/2$, comparing to the cost when $k=1$.  Our main result shows that this natural mechanism is optimal. This proof is non-trivial and does not follow from the optimality of such noise when $k=1$. %which is significantly more involved (we can not simply assume that adding Laplace noise is optimum, given that the server could have an arbitrarily complex algorithm). 
%  \todo{Maybe put an informal problem definition and theorem statement here?}
Figure \ref{fig:intro1} is an instance of the optimal mechanism.


  \begin{figure}
      \centering
        \begin{tikzpicture}
        \coordinate (right) at (8,0);
        \coordinate (left) at (0,0);
        \coordinate (o) at (4,0);
        \coordinate (up) at (4,3);
        \coordinate (x0) at (4.5,0);
        \coordinate (s) at (2,0);
        \coordinate (t) at (5.5,0);
        \coordinate (cone) at (4,2.5);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[->](o)--(up);
        \draw[<->](left)--(right);
        \draw[-](cone)--(4.1,2.5);
        \draw node at (3.65,2.5) {$0.5$};
        \draw node at (4.0,-0.3) {$O$};
        \draw node at (4.45,3.1) {$\rho(x)$};
        \draw node at (7.9,-0.2) {$x$};
        % here, eps=0.55
        \draw[blue,domain=0:4] plot(\x,{2.5*exp((\x-4))} );
        \draw[blue,domain=4:8] plot(\x,{2.5*exp(-(\x-4))} );
        \coordinate (r0) at (4,0);
        \coordinate (r3) at ([xshift = 1.3862943611198906188344642429164*2.5 cm] r0);
        \coordinate (r2) at ([xshift = -0.69314718055994530941723212145818*2.5 cm] r3);
        \coordinate (r1) at ([xshift = -1.0986122886681096913952452369225*2.5 cm] r3);
        \coordinate (r-3) at ([xshift = -1.3862943611198906188344642429164*2.5 cm] r0);
        \coordinate (r-2) at ([xshift = 0.69314718055994530941723212145818*2.5 cm] r-3);
        \coordinate (r-1) at ([xshift = 1.0986122886681096913952452369225*2.5 cm] r-3);
        \fill (r0) circle (2pt);
        \fill (r1) circle (2pt);
        \fill (r2) circle (2pt);
        \fill (r3) circle (2pt);
        \fill (r-1) circle (2pt);
        \fill (r-2) circle (2pt);
        \fill (r-3) circle (2pt);
        \coordinate (rowone) at ([xshift=2.5cm] o);
        \coordinate (row-one) at ([xshift=-2.5cm] o);
        \coordinate (rowonec) at ([yshift=-0.3cm] rowone);
        \coordinate (row-onec) at ([yshift=-0.3cm] row-one);
        \coordinate (rowonel) at ([yshift=0.1cm] rowone);
        \coordinate (row-onel) at ([yshift=0.1cm] row-one);
        \draw node at (rowonec) {$1$};
        \draw node at (row-onec) {$-1$};
        \draw[-](rowone)--(rowonel);
        \draw[-](row-one)--(row-onel);
        \end{tikzpicture}
      \caption{Optimal mechanism in geographic differential privacy setting when $\K=7$ and $\epsilon=1$. Suppose the user has a private value $v$. Then the user sends $v+x$ to the server, where $x$ is drawn from Laplace distribution with density $\rho(x)$. Suppose the server receives $s$. Then the server responds $s+a_1,...,s+a_7$, where the values of $a_1,a_2,...,a_7$ are denoted by black dots on the $x$-axis.}    \label{fig:intro1}
  \end{figure}
  
To prove this result, we pretend that the user has full information and is directly choosing a set $S$ of size $k$ to minimize the expected distance from its query, while ensuring that the set $S$ satisfies geographic differential privacy.  This involves optimizing over all possible $k$-dimensional distributions for $S$. We first show that there exists an optimal mechanism that is symmetric, i.e. shifting the query along the line translates the entire distribution by the same amount. We then show that a two stage mechanism, where the user sends a single noisy value and the server chooses $k$ results by adding $k$ {\em fixed increments} to the chosen value, is optimal for symmetric distributions. Finally, we show that for such mechanisms, adding Laplace noise is optimal. 

We emphasize that the optimality of adding Laplace noise is far from obvious\footnote{In fact, only a few optimal mechanisms are known~\cite{Ghosh2012privacy, gupte2010universally, kairouz2014extremal, ding2017collecting}, and it is known that for certain scenarios, universally optimal mechanisms don't exist~\cite{brenner2014impossibility}.}. For instance, when users and results are located on a ring, Laplace noise is {\em not optimal}. While we have not been able to analyze the ring in complete generality for geographic DP, we have been able to explicitly solve if for some specific simple cases. Figure \ref{fig:intro3} illustrates the optimal mechanism under geographic DP for $k=2$. This mechanism uses noise that is a piece-wise composition of Laplace noises; we obtain an improvement of a factor of 0.558 with this optimal mechanism whereas Laplace noise gives an improvement of only 0.585. We sketch the calculation in appendix~\ref{sec:non-opt-ex}.


  
  \begin{figure}
      \centering
        \begin{tikzpicture}
        \coordinate (right) at (7.5,0);
        \coordinate (o) at (0,0);
        \coordinate (up) at (0,3);
        \coordinate (x0) at (4.5,0);
        \coordinate (s) at (2,0);
        \coordinate (t) at (5.5,0);
        %
        \coordinate (key1) at (8,2.5);
        \coordinate (key2) at (8.7,2.5);
        \draw[blue,dashed] (key1)--([xshift=0.5cm]key1);
        \fill[blue] ([xshift = -0.070292 cm, yshift = -0.070292 cm]key2) rectangle ([xshift = 0.070292 cm, yshift = 0.070292 cm]key2);
        \draw node at ([xshift = 1.5 cm] key2) {\footnotesize Laplace mechanism};
        \coordinate (key3) at (8,2);
        \coordinate (key4) at (8.7,2);
        \draw[red] (key3)--([xshift=0.5cm]key3);
        \fill[red] (key4) circle (2pt);
        \draw node at ([xshift = 1.5 cm] key4) {\footnotesize Better mechanism};
        %
        \draw (7.7,1.7) rectangle (11.7,2.8);
        %
        \coordinate (cone1) at (0,1);
        \coordinate (cone2) at (0,2);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[->](o)--(up);
        \draw[->](o)--(right);
        \draw[-](cone1)--([xshift = 0.1 cm]cone1);
        \draw[-](cone2)--([xshift = 0.1 cm]cone2);
        \draw node at ([xshift = -0.3 cm] cone1) {$0.1$};
        \draw node at ([xshift = -0.3 cm] cone2) {$0.2$};
        \coordinate (piv) at (3.5,0);
        \draw[-](piv)--([yshift = 0.1 cm] piv);
        \coordinate (2piv) at (7,0);
        \draw[-](2piv)--([yshift = 0.1 cm] 2piv);
        \draw node at ([yshift = -0.3 cm] piv) {$\pi$};
        \draw node at ([yshift = -0.3 cm] 2piv) {$2\pi$};
        \draw node at ([xshift = -0.05 cm, yshift = -0.3 cm] o) {$O$};
        \draw node at (0.45,3.1) {$\rho(x)$};
        \draw node at ([xshift = -0.05 cm, yshift = -0.2 cm] right) {$x$};
        % here, eps=0.55
        \draw[blue,dashed,domain=0:3.5] plot(\x,{0.834005054395031*exp(-(\x-3.5)*pi*3/28)} );
        \draw[blue,dashed,domain=3.5:7] plot(\x,{0.834005054395031*exp((\x-3.5)*pi*3/28)} );
        \draw[red,domain=0:1.75] plot(\x,{1.168554905236987*exp(-(\x-1.75)*pi*3/28)} );
        \draw[red,domain=1.75:3.5] plot(\x,{1.168554905236987*exp((\x-1.75)*pi*3/28)} );
        \draw[red,domain=3.5:5.25] plot(\x,{1.168554905236987*exp(-(\x-5.25)*pi*3/28)} );
        \draw[red,domain=5.25:7] plot(\x,{1.168554905236987*exp((\x-5.25)*pi*3/28)} );
        %\draw[blue,domain=:] plot(\x,{2.6240214001267626006468162172726} );
        %\draw[blue,domain=:] plot(\x,{0.9653235263005390754197259800987} );
        
        \coordinate (r0) at (1.261892227103695,0);
        \coordinate (r1) at (5.738107772896305,0);
        \fill[red] (o) circle (2pt);
        \fill[red] (piv) circle (2pt);
        \fill[blue] ([xshift = -0.070292 cm, yshift = -0.070292 cm]r0) rectangle ([xshift = 0.070292 cm, yshift = 0.070292 cm]r0);
        \fill[blue] ([xshift = -0.070292 cm, yshift = -0.070292 cm]r1) rectangle ([xshift = 0.070292 cm, yshift = 0.070292 cm]r1);
        \end{tikzpicture}
      \caption{Geographic differential privacy setting when users and results are located on a unit ring, for $\K=2$ and $\epsilon=3/8$, showing the stark difference between Laplace noise and the optimal noise. Suppose the user has a private value $v$. Then the user sends $v+x$ to the server, where $x$ is drawn from a noise distribution with density $\rho(x)$, depicted here for both Laplace noise and the optimal noise. Suppose the server receives $s$. Then the server's optimal response is $s+a_1$ and $s+a_2$, where the values of $a_1,a_2$ are denoted by dots on the $x$-axis, again assuming both Laplace noise and the optimal noise.}%\todo{Can we not rely on color to state which noise is which? Use different colors as well as different type, e.g. dotted vs not for line, and x vs triangle for points, and add a key to the image itself stating which curve corresponds to what. Then reduce the description in the text.}   
      \label{fig:intro3}
  \end{figure}



\paragraph{Local DP.} We next consider local differential privacy, when users and results are located on a ring. We will use the angle in $[0,2\pi)$ to denote the position. One optimal mechanism is the following. Users add one type of piece-wise constant noise to the private value before sending it. The server responds $\K$ results by adding the received signal by an angle $2\pi i/\K$ for $0\leq i<\K$. Figure \ref{fig:intro2} is an instance of the optimal mechanism. As with geographic DP, the accuracy of this mechanism is $O(1/k)$. The analysis builds on that for geographic DP: the result described earlier for symmetric distribution holds for this case as well, and only the final step of the analysis is different (and more straightforward).
  
  \begin{figure}
      \centering
        \begin{tikzpicture}
        \coordinate (right) at (7.6,0);
        \coordinate (o) at (0,0);
        \coordinate (up) at (0,3);
        \coordinate (x0) at (4.5,0);
        \coordinate (s) at (2,0);
        \coordinate (t) at (5.5,0);
        \coordinate (cone1) at (0,1);
        \coordinate (cone2) at (0,2);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[->](o)--(up);
        \draw[->](o)--(right);
        \draw[-](cone1)--([xshift = 0.1 cm]cone1);
        \draw[-](cone2)--([xshift = 0.1 cm]cone2);
        \draw node at ([xshift = -0.3 cm] cone1) {$0.1$};
        \draw node at ([xshift = -0.3 cm] cone2) {$0.2$};
        \coordinate (piv) at (3.5,0);
        \draw[-](piv)--([yshift = 0.1 cm] piv);
        \coordinate (2piv) at (7,0);
        \draw[-](2piv)--([yshift = 0.1 cm] 2piv);
        \draw node at ([yshift = -0.3 cm] piv) {$\pi$};
        \draw node at ([yshift = -0.3 cm] 2piv) {$2\pi$};
        \draw node at ([xshift = -0.05 cm, yshift = -0.3 cm] o) {$O$};
        \draw node at (0.45,3.1) {$\rho(x)$};
        \draw node at ([xshift = -0.05 cm, yshift = -0.2 cm] right) {$x$};
        % here, eps=0.55
        \draw[blue,domain=0:0.26427846815870180475276960397815] plot(\x,{2.6240214001267626006468162172726} );
        \draw[blue,domain=0.26427846815870180475276960397815:1.1357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
        %\draw[blue,domain=:] plot(\x,{2.6240214001267626006468162172726} );
        %\draw[blue,domain=:] plot(\x,{0.9653235263005390754197259800987} );
        \draw[blue,domain=1.1357215318412981952472303960219:1.6642784681587018047527696039782] plot(\x,{2.6240214001267626006468162172726} );
        \draw[blue,domain=1.6642784681587018047527696039782:2.5357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
        \draw[blue,domain=2.5357215318412981952472303960219:3.0642784681587018047527696039782] plot(\x,{2.6240214001267626006468162172726} );
        \draw[blue,domain=3.0642784681587018047527696039782:3.9357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
        \draw[blue,domain=3.9357215318412981952472303960219:4.4642784681587018047527696039782] plot(\x,{2.6240214001267626006468162172726} );
        \draw[blue,domain=4.4642784681587018047527696039782:5.3357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
        \draw[blue,domain=5.3357215318412981952472303960219:5.8642784681587018047527696039782] plot(\x,{2.6240214001267626006468162172726} );
        \draw[blue,domain=5.8642784681587018047527696039782:6.7357215318412981952472303960219] plot(\x,{0.9653235263005390754197259800987} );
        \draw[blue,domain=6.7357215318412981952472303960219:7] plot(\x,{2.6240214001267626006468162172726} );
%%
%0.26427846815870180475276960397815
%1.1357215318412981952472303960219
%1.6642784681587018047527696039782
%2.5357215318412981952472303960219
%3.0642784681587018047527696039782
%3.9357215318412981952472303960219
%4.4642784681587018047527696039782
%5.3357215318412981952472303960219
%5.8642784681587018047527696039782
%6.7357215318412981952472303960219
%7
%%
        \coordinate (r0) at (o);
        \coordinate (r1) at ([xshift = 1.4 cm] r0);
        \coordinate (r2) at ([xshift = 1.4 cm] r1);
        \coordinate (r3) at ([xshift = 1.4 cm] r2);
        \coordinate (r4) at ([xshift = 1.4 cm] r3);
        \fill (r0) circle (2pt);
        \fill (r1) circle (2pt);
        \fill (r2) circle (2pt);
        \fill (r3) circle (2pt);
        \fill (r4) circle (2pt);
        \end{tikzpicture}
      \caption{Optimal mechanism in local differential privacy setting when $\K=5$ and $\epsilon=1$. Suppose the user has a private value $v$. Then the user sends $v+x$ to the server, where $x$ is drawn from a noise distribution with density $\rho(x)$. Suppose the server receives $s$. Then the server responds $s+a_1,...,s+a_5$, where the values of $a_1,a_2,...,a_5$ are denoted by black dots on the $x$-axis.}  %\todo{I do not understand this figure. Is the distribution discontinuous? Reply: The distribution is continuous, but the density of the distribution is piece-wise, which means the density function is not continuous}  
      \label{fig:intro2}
  \end{figure}

\paragraph{Other Noise Models.} In the analysis above, we assumed that we are given a desired (local or geographic) privacy guarantee, and we find the optimal noise as well as the optimal server response to minimize the cost of privacy. In practical situations, it is likely that the noise that is added is not under our control. We show that for the one-dimensional case, as long as the noise that is added by the client satisfies the Monotone Hazard Rate property (which both Laplace noise as well as the commonly used Gaussian noise do), the accuracy guarantee improves as $\tilde{O}\left(\frac{1}{k}\right)$,  comparing to the case $k=1$; further, this improvement can be obtained by sampling from the posterior distribution of the noise. The proof is deferred to Appendix~\ref{sec:mhr}.

We finally note that though the one-dimensional case is somewhat stylized, our main contribution is to show that even this case requires non-trivial ideas. In practice, a server could employ dimension reduction techniques such as PCA to create a small number $d$ of dimensions. In this case, techniques similar to what we have presented show that the accuracy improves as $\Theta\left(\frac{1}{k^{1/d}}\right)$, and it is conceivable the improvement is even better in the wild. We discuss this in detail in Appendix~\ref{sec:high_dim}.


==> preliminary.tex <==



\section{Preliminaries}



%\subsection{Preliminary results}



In this section, we show it is sufficient to consider \emph{symmetric} mechanisms, which is formally defined later.

We first show it is sufficient to consider mechanisms in which servers directly return the received signal from the user.

Recall that $\Probs{\Signals}$ is the set of differential private mechanisms that adopt signal set $\Signals$. Then $\Probs{\Kads}$ is the set of differential private mechanisms in which users pick signals from $\Kads$.


\begin{lemma}[corresponds to Theorem \ref{thm:singpoint:sim}]   \label{lem:onlyuserstr}

We have
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K} &= \inf_{\Pname\in \Probs{\Kads}} \sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}F(u,a) } \\& = \inf_{\Pname\in \Probs{\Kads}} \sup_{u \in \Users} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}F(u,a) }
\end{align*}

\end{lemma}

\begin{proof}

Fix $\Signals,\Pname\in \Probs{\Signals},\Qname\in \Qrobs_{\Signals}$. For any $\C\in \measure{\Kads}$, let
\begin{align*}
    \Ppxx{u}{\C}=\Prxx{ s\sim \Pname_u, A\sim \Qname_s}{A\in \C},
\end{align*}
which is the probability that user $u$ receives a result set in $\C$.

Then for any $u_1,u_2\in \Users, \C\in \measure{\Kads}$, we have
\begin{align*}
    \Ppxx{u_1}{\C}
    =&\Prxx{ s\sim \Pname_{u_1}, A\sim \Qname_s}{A\in \C}    \\
    =&\Exx{s\sim \Pname_{u_1}}{\Prxx{ A\sim \Qname_s}{A\in \C}}    \\
    =& \int_{s\in \Signals}{\left(\Prxx{ A\sim \Qname_s}{A\in \C}\cdot \Pxx{u_1}{ds} \right)}    \\
    \leq & e^{\epsilon\cdot \defdis{u_1}{u_2}}\int_{s\in \Signals}{\left(\Prxx{ A\sim \Qname_s}{A\in \C}\cdot \Pxx{u_2}{ds} \right)}    \\
    = & e^{\epsilon\cdot \defdis{u_1}{u_2}}\Exx{s\sim \Pname_{u_2}}{\Prxx{ A\sim \Qname_s}{A\in \C} }    \\
    = & e^{\epsilon\cdot \defdis{u_1}{u_2}}\Exx{s\sim \Pname_{u_2},A\sim \Qname_s}{\I{A\in \C} }    \\
    = & e^{\epsilon\cdot \defdis{u_1}{u_2}} \Ppxx{u_2}{\C},
\end{align*}
so $\Ppname\in \Probs{\Kads}$ because $\Ppxx{u}{\cdot}\in \probm{\Kads}$ for any $u\in \Users$.

At the same time,
\begin{align*}
\Exx{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\disg{u}{a} }
=\Exx{u\sim \Dist, A\sim \Ppname_u}{ \min_{a\in A}\disg{u}{a} },
\end{align*}
so we have
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K} = \inf_{\Pname\in \Probs{\Kads}} \sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }.
\end{align*}

\end{proof}

Fixing a mechanism, we are interested in it performance in the worst case among all possible distributions of users. The worst distribution is in fact an one-point distribution. By linearity of expectation, for any $\Pname\in \Probs{\Kads}$, we have
\begin{align}   \label{eq:userdissingle}
\sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
=
\sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
\end{align}


\iffalse%%%%%%%
\begin{lemma}   \label{lem:onepointdis}

For any $\Pname\in \Probs{\Kads}$, we have
\begin{align*}
\sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
=
\sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
\end{align*}

\end{lemma}

\begin{proof}
First, if $\forall \C\subset \Users, \Dist(\C)=\I{u\in \C}$, then $\Dist\in \probm{\Users}$ and
\begin{align*}
\Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} } = \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} },
\end{align*}
so we have
\begin{align}\label{disToPoint:geq}
\sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
\geq
\sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }.
\end{align}

On the other hand, note that for any $u'\in \Users$,
\begin{align*}
\Exx{A\sim \Pname_{u'}}{ \min_{a\in A}\disg{u}{a} }\leq \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} },
\end{align*}
so for any $\Dist\in \probm{\Users}$,
\begin{align*}
\Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
\leq \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} },
\end{align*}
which implies
\begin{align}\label{disToPoint:leq}
\sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
\leq
\sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }.
\end{align}

Combining Inequality \ref{disToPoint:geq} and Inequality \ref{disToPoint:leq}, we have
\begin{align*}
\sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
=
\sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
\end{align*}

\end{proof}


\fi%%%%%%%%%%%%





Combining Lemma \ref{lem:onlyuserstr} and Equation \ref{eq:userdissingle}, we have the following theorem.


\begin{restatable}{theorem}{rstepa}\label{thm:singpoint}


\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
%=
%\inf_{\Pname\in \Probs{\Kads}} \sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }
=
\inf_{\Pname\in \Probs{\Kads}} \sup_{u\in \Users} \Exx{A\sim \Pname_u}{ \min_{a\in A}\disg{u}{a} }.
\end{align*}

\end{restatable}

    
%\rstepa*
    

It is sufficient to assume the server directly sends back the received signal, and we care the user with largest error.







==> proof-outline.tex <==
\section{Proof Outline}\label{sec:proof-outline}


We first show that the signal set $Z$ can be the $k$-result set $\mathbb{R}^k$ in Section \ref{subsec:proof-step1}. We next formulate an infinite-dimensional infimization linear program denoted as $\mathcal{O}$ and construct an infinite-dimensional supremization linear program denoted as $\mathcal{E}$ in Section \ref{subsec:proof-step2}. Our proof methodology shares similarities with the approach presented in \cite{koufogiannis2015optimality}, but our linear program is notably more intricate and complex due to the involvement of minimization over a set of returned results in the cost function. 

In our problem, we formally establish a weak duality framework between programs $\mathcal{O}$ and $\mathcal{E}$. This proof is imperative since the existing duality framework exists for infinite dimensional linear programs for cases only involving integrals but not for scenarios involving both of them. This proof is further complicated by the fact that we have linear constraints on upper and lower derivatives, since not every probability distribution is differentiable. Since the weak duality proof involves some exchange of limits and integrals, we require a meticulous application of Fatou's lemma and the monotone convergence theorem to prove weak duality.

Finally, we show the optimality of the Laplace noise addition mechanism by dual -fitting i.e. constructing a feasible solution to DILP $\mathcal{E}$ with an objective identical to that of the Laplace noise addition mechanism in Section \ref{subsec:proof-step3}. Finally for the case of $\mathfrak{h}(z)=z$, we show how to compute the server response in a closed form in Section \ref{subsec:proof-step4}.


\subsection{Step 1. Optimal to restrict $\Signals$ in $k$-result set $\Kads$.}\label{subsec:proof-step1} 


Given the behavior of the server, users can themselves compute the distribution of the result set that they will receive. Therefore a user can draw a result set directly from the distribution over the server's action and send the set as the signal. The server returns the received signal, hence removing it from the picture. In other words, it is sufficient to consider mechanisms in $\Probs{\Kads}$, which are in the following form (corresponding to Theorem \ref{thm:singpoint:sim}).

\begin{enumerate}
    \item User located at $v\in \real$ reports $s$ that is drawn from a distribution $\Pname_{v}$ over $\real^{\K}$.
    \item The server receives $s$ and returns $s$.
\end{enumerate}

Observe that this mechanism is only used for the purpose of analysis and the final mechanism will not remove the server and will actually split the computation between the user and the server. 

%%%%%

%In this case, the signal set $\Signals$ is $\Kads$, and we do not need to decide the behavior of the server. We will prove
    

%\begin{restatable}{theorem}{simrstepa}\label{thm:singpoint:sim}
%\begin{align*}
%\funf{\Users}{\Ads}{\epsilon}{\K} = \inf_{\Pname\in \Probs{\real^{\K}}} \sup_{\Dist} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}|u-a| }.
%\end{align*}
%\end{restatable}
    

\subsection{Step 2: Differential-integral linear programs (DILP) to represent cost $\funf{\real}{}{\epsilon}{k}$}{\label{subsec:proof-step2}}

% A DILP denotes is a linear program over function space involving constraints on both derivatives and integrals, a formal definition is given in Definition \ref{eq:example_DILP}. 
We first give the definition of a DILP below.
\begin{definition}{\label{def:DILP}}
    Differential-integral linear programs(DILP): Differential-integral linear program is a linear program over Riemann integrable function spaces involving constraints on both derivatives and integrals. 
    %A simple example may be given in Equation \eqref{eq:example_DILP}.
\end{definition}
We now construct an infimizing DILP $\mathcal{O}$ representing $\funfgeo{U}{}{\epsilon}{k}{\mathfrak{h}(.)}$ using two key ideas.

\begin{itemize}
    \item We approximate every probability distribution $\textbf{P}_u$ by a continuous distribution $g(u,.)$ over $\mathbb{R}^k$ using ideas from mollifier theory.
    \item We show that $\epsilon$-geographic differential privacy implies that $\log g(u,\vect{v})$ is Lipschitz continuous in $u$ with Lipschitz constant $\epsilon$.\footnote{The case when $g(u,\vect{v})$ equals zero is handled separately.}
\end{itemize}

% Further, we prove that the Laplace noise addition mechanism attains a cost of $\hatfunf{\real}{\Ads}{\epsilon}{\K}$ in Lemma \ref{lemma:bounding_f}. We construct a supremizing DILP $\mathcal{E}$ whose objective value is bounded by objective value of $\mathcal{O}$, proven in Theorme \ref{theorem:weak_duality_result}. The proof technique uses similar ideas to that of the proof of weak duality in linear programs. However, since to the best of our knowledge weak duality theory does not exist for DILPs, they exist for infinite dimensional LPs with only integral constraints, we cannot use the existing duality framework to directly construct the dual of DILP $\mathcal{O}$. In the rest of this paper, we shall refer to $\mathcal{E}$ as the dual DILP $\mathcal{E}$.

We construct a supremizing DILP $\mathcal{E}$ whose objective value is bounded by objective value of $\mathcal{O}$, proven in Theorem \ref{theorem:weak_duality_result}. This is one of the most important results in this section and requires a careful analysis. The proof technique uses similar ideas to that of the proof of weak duality in linear programs. However, since to the best of our knowledge weak duality theory exist for infinite dimensional LPs with only integral constraints but not for DILPs, we cannot use the existing duality framework to directly construct the dual of DILP $\mathcal{O}$. In the rest of this paper, we shall refer to $\mathcal{E}$ as the dual DILP $\mathcal{E}$.



\iffalse %%%%%

\begin{restatable}{theorem}{simrstepb} \label{thm:symopt:sim}
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname_{ave}\in \Psym}  \Exx{A\sim \Pname_{ave}}{ \min_{a\in A}|a| },
\end{align*}
where $\Psym$ is the set of symmetric mechanisms that are $\epsilon$-geographicly DP.
\end{restatable}

\fi %%%%%

\subsection{Step 3: Dual fitting to show optimality of the Laplace noise addition mechanism}{\label{subsec:proof-step3}} %the cost function $\funf{\real}{\Ads}{\epsilon}{\K}$ }

We prove that the Laplace noise addition mechanism satisfies geographic differential privacy constraints and attains a cost of $\hatfunf{\real}{\Ads}{\epsilon}{\K}$ in Lemma \ref{lemma:bounding_f}. We next construct a feasible solution to dual DILP $\mathcal{E}$ with an objective arbitrarily close to that of $\hatfunf{\real}{\Ads}{\epsilon}{\K}$. The proof involves carefully choosing a feasible solution and solving an ordinary differential equation (ODE) with a carefully chosen initial value point so that the solution satisfies the constraints of the DILP $\mathcal{E}$. 

    
\subsection{Step 4. Server response given Laplace noise addition.} {\label{subsec:proof-step4}}
With the results in the previous steps, we prove that $\funf{\real}{\Ads}{\epsilon}{\K}$ equals $\hatfunf{\real}{\Ads}{\epsilon}{\K}$ and show that Laplace noise addition mechanism is optimal. 
\begin{enumerate}
    \item User located at $v\in \real$ reports $s=v+x$, where $x$ is drawn from Laplace distribution with density $\rho(x)=\frac{\epsilon}{2} \cdot e^{-\epsilon \disrzero{x}} $.
    \item The server receives $s$ and respond $(s+a_1,\dots,s+a_{\K})$, where $a_1,\dots,a_{\K}$ are fixed real values.
\end{enumerate}

For the case of $\mathfrak{h}(z)=z$, the optimal mechanism is simple enough that the values $a_1, a_2, \ldots, a_k$ can be computed by dynamic programming, as we show in Section~\ref{sec:simres}, and this concludes the proof of Theorem~\ref{thm:lap:sim}. For other general increasing functions, the optimal solution for $\{a_i\}_{i=1}^{k}$ may not always be written in closed form, however we can always write a recursive expression to compute the points. 
\zhihao{Are we sure it is not closed form, or it is saying we don't know the closed form?}
\sss{No, I think till now we could not compute closed form (but not sure) but we can always write it as a recursion. }


%%%%%

%We will prove


%\begin{restatable}{theorem}{simrstepe} \label{thm:lap:sim}
%For geographic differential privacy, it is sufficient to only consider symmetric mechanisms. Adding Laplace noise, whose density function is $\rho(x)=\frac{1}{2\epsilon} \cdot e^{-\epsilon \disrzero{u}{x}} $, is one of the optimal choices for users, and in this case $\funf{\Users}{\Ads}{\epsilon}{\K}$ is $O(1/(\epsilon \K))$. Further, the optimal mechanism itself can be computed in closed form.
%\end{restatable}    
    
    
%\end{itemize}


%\input{ashishproof}




==> proofs_remaining_claims_bak.tex <==
\section{A generalization of $\epsilon$-geographic DP: Proof of claim \ref{claim:diff-privacy-condition_gen} }


%Observe that in this section we define 

\subsection{Proof of Claim \ref{claim:diff-privacy-condition_gen}}\label{sec:diff-privacy-condition-gen-proof}

In this subsection we prove a claim for a necessary and sufficient condition for $\mathfrak{f}(.)$ geographic differential privacy. Recall that $\mathfrak{f}(.)$ is convex increasing function as defined in Assumption \ref{assn:f_defn}.


We now restate and prove Claim \ref{claim:diff-privacy-condition_gen}.

\begin{claim*}
    Suppose, $P_u$ has a probability density function given by $g(u,.): \mathbb{R}^k \rightarrow \mathbb{R}$ for every $u \in \mathbb{R}$. Then, $P$ satisfies $\mathfrak{f}(.)$-geographic differential privacy iff $\max(|\overline{g}_u(u,\vect{x})|, |\underline{g}_u(u,\vect{x})|) \leq \mathfrak{f}'(0) g(u,\vect{x}) \text{ } \forall u \in \mathbb{R};\forall x \in \mathbb{R}^k$ \footnote{$\underline{g}_u(u,\vect{x})$, $\overline{g}_u(u,\vect{x})$ denote the lower and upper partial derivative w.r.t. $u$} for any convex function $\mathfrak{f}(.)$.  
\end{claim*} 


\begin{proof}

\textbf{We first prove the only if statement.}

Assuming $\mathfrak{f}(.)$ geographic differential privacy we prove the desired constraint on $g(u,.)$. 

    Observe that since, $\{P_u\}_{u \in \mathbb{R}}$ satisfies $\mathfrak{f}(.)$ geographic-differential privacy, we must have $g(u_1, \vect{x}) < e^{\mathfrak{f}(|u_1-u_2|)} g(u_2, \vect{x})$.


  Thus, applying $\log$ on both sides we get, 

  \begin{align*}
      & \log g(u + \delta u, \vect{x}) - \log g(u, \vect{x}) \leq \mathfrak{f}(|\delta u|)\\
      \implies & \frac{\max(|\overline{g}_u(u,\vect{x})|, |\underline{g}_u(u,\vect{x})|)} {g(u,\vect{x})} \leq \mathfrak{f}'(0)
  \end{align*}
The last implication follows on limiting $\delta u$ towards zero and $\mathfrak{f}(0)=0$ thus, applying the lower and upper limits respectively and thus we prove the only if statement.


\textbf{We now prove the if statement.}

Here assuming $\max(|\overline{g}_u(u,\vect{x})|, |\underline{g}_u(u,\vect{x})|) \leq \mathfrak{f}'(0) g(u,\vect{x})$, we prove $\mathfrak{f}(.)$-geographic differential privacy.

Now consider $u_1 >u_2$ for some $u_1,u_2 \in \mathbb{R}$.\\

\begin{align*}
    \log g(u_1,\vect{x}) - \log g(u_2, \vect{x}) \overset{(a)}{\leq} \int_{u = u_2}^{u_1} \frac{\overline{g}_u(u,\vect{x})}{g(u,\vect{x})} \leq & \mathfrak{f}'(0) (u_1 -u_2) \\
    & \overset{(b)}{\leq} \mathfrak{f}(u_1-u_2)
\end{align*}

The first inequality $(a)$ follows since we use an upper derivative and the inequality $(b)$ follows from the fact that $\mathfrak{f}(.)$ is a convex function and $\mathfrak{f}(0)=0$ as defined in \ref{sec:diff-privacy-gen}.

\begin{align*}
    \log g(u_1,\vect{x}) - \log g(u_2, \vect{x}) \geq \int_{u = u_2}^{u_1} \frac{\underline{g}_u(u,\vect{x})}{g(u,\vect{x})} \geq & -\mathfrak{f}'(0) (u_1 -u_2) \\
    & \overset{(c)}{\geq} - \mathfrak{f}(u_1-u_2)
\end{align*}


Inequality $(c)$ follows from the fact that $\mathfrak{f}(.)$ is a convex function.
Thus, we get $g(u_1, \vect{x}) \leq e^{-\mathfrak{f}(|u_1-u_2|)} g(u_2,\vect{x})$ on taking exponent on both sides.
 


\end{proof}



%The proof of this claim is given in Section \ref{sec:diff_eqn_soln_first_claim}.



\section{Proof of weak duality as stated in Theorem \ref{theorem:weak_duality_result}}{\label{sec:weak_duality}}


\km{The next lemma is a theorem, and is a restatement of Theorem ...}

\begin{lemma*}
    $\text{opt}(\mathcal{O}) \geq \text{opt}(\mathcal{E})$.
\end{lemma*}

To prove this lemma, we now redefine the optimization problems $\mathcal{O}$ in \eqref{orig_primal}. Observe that in the second constraint of primal \ref{orig_primal}, we may relax the equality to an inequality since, we are computing the infimum. 

\zhihao{We optimize the functions to be rieman integrable, is it on any bounded set, or it also works for unbounded set?}

\sss{Observe that since $g(.)$ is non-negative, Reimann integral on a bounded set would imply the existence of integral on an unbounded set too, the integral may go to infinity but is always defined.}

%We first redefine 


%Note that we assume that all functions are Riemann integrable.
 



% \begin{equation}
% \begin{aligned}
% \min_{w,b,\xi} \quad & \frac{1}{2}w^{t}w+C\sum_{i=1}^{N}{\xi_{i}}\\
% \textrm{s.t.} \quad & y_{i}(w\phi(x_{i}+b))+\xi_{i}-1\\
%   &\xi\geq0    \\
% \end{aligned}
% \end{equation}

%We now rewrite the equations  and \eqref{orig_dual} and prove the weak duality i.e. $\text{opt}(\mathcal{O}) \geq \text{opt}(\mathcal{E})$

\begin{equation}%{\label{orig_primal}}
\text{ $\mathcal{O}$ =}
\left\{
\begin{aligned}
    \inf_{g(.,.): \mathcal{I}^B (\mathbb{R} \times \mathbb{R}^k \rightarrow \mathbb{R}^{+}), \kappa \in \mathbb{R}} \quad & \kappa \\
    \textrm{s.t.} \quad & \kappa - \int\limits_{\vect{x} \in \mathbb{R}^k} \left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right) \geq 0 \text{ }\forall u\in \mathbb{R}\\
    & \int\limits_{\vect{x} \in \mathbb{R}^k} g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right) = 1 \text{ } \forall u\in \mathbb{R}\\
    &  \epsilon g(u,\vect{x}) + \underline{g}_{u}(u,\vect{x}) \geq 0; \text{ }\forall u\in \mathbb{R}; \vect{x} \in \mathbb{R}^k\\
    &  \epsilon g(u,\vect{x}) - \overline{g}_{u}(u,\vect{x}) \geq 0; \text{ }\forall u\in \mathbb{R}; \vect{x} \in \mathbb{R}^k
\end{aligned}
\right.
\end{equation}


\begin{equation}
\text{ {$\mathcal{E}^{int}$ =}}
\left\{
\begin{aligned}
    \sup_{\substack{\delta(.): \mathcal{C}^0 (\mathbb{R} \rightarrow \mathbb{R}^{+}) ,{\nu^{(1)}}(.,.): \mathcal{C}^1 (\mathbb{R} \times \mathbb{R}^k \rightarrow \mathbb{R}^{+}) \\ 
    {\nu^{(2)}}(.,.): \mathcal{C}^1 (\mathbb{R} \times \mathbb{R}^k \rightarrow \mathbb{R}^{+}), 
    \lambda(.): \mathcal{C}^0(\mathbb{R} \rightarrow \mathbb{R}^{+})}} & \int_{u\in \mathbb{R} } {\lambda}(u) \\
    \textrm{ s.t. } \quad & \int_{u\in \mathbb{R}} {\delta}(u) \leq 1\\
    & \hspace{-2 em} - \left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] {\delta}(u) + {\lambda}(u) + \epsilon \left(-{\nu}^{(1)}(u,\vect{x}) +{\nu}^{(2)}(u,\vect{x})\right)\\ 
    & \hspace{5em} + {\nu}^{(1)}_u(u,\vect{x}) +{\nu}^{(2)}_u(u,\vect{x}) \leq 0 \text{    } \forall u\in \mathbb{R}, \forall \vect{x} \in \mathbb{R}^k \\
    & \hspace{-2 em}\exists U: \mathcal{C}^0(\mathbb{R}^k \rightarrow \mathbb{R})  \textrm { s.t. }-\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x}) \geq 0 \text{ }\forall u\geq U(\vect{x}) \text{ } \forall \vect{x} \in (\mathbb{R})^k \\
    & \hspace{-2 em}\exists L: \mathcal{C}^0(\mathbb{R}^k \rightarrow \mathbb{R}) \textrm { s.t. } -\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x}) \leq 0 \text{ } \forall u\leq L(\vect{x}) \text{ } \forall \vect{x} \in (\mathbb{R})^k
    % & \exists U_{\vect{v}} \in \mathbb{R} \textrm { s.t. }-\nu^{(1)}(u,\vect{v}) + \nu^{(2)}(u,\vect{v}) \geq 0 \text{ }\forall u> U_{\vect{v}} \text{ } \forall \vect{v} \in (\mathbb{R})^k\\
    % & \exists L_{\vect{v}} \in \mathbb{R} \textrm { s.t. }-\nu^{(1)}(u,\vect{v}) + \nu^{(2)}(u,\vect{v}) \leq 0 \text{ }\forall u< L_{\vect{v}} \text{ } \forall \vect{v} \in (\mathbb{R})^k\\
   %  & \liminf_{M \to \infty} -{\nu^{(1)}}(M,\vect{x}) + {\nu^{(2)}}(M,\vect{x}) \geq 0 \text{ } \forall \vect{x} \in \mathbb{R}^k\\
   % & \limsup_{M \to \infty}-{\nu^{(1)}}(-M,\vect{x}) + {\nu^{(2)}}(-M,\vect{x})\leq 0 \text{ } \forall \vect{x} \in \mathbb{R}^k\\
\end{aligned}
\right.    
\end{equation}


\begin{equation}
\text{ {$\mathcal{E}$ =}}
\left\{
\begin{aligned}
    \sup_{\substack{{\nu}(.,.): \mathcal{C}^1 (\mathbb{R} \times \mathbb{R}^k \rightarrow \mathbb{R}) \\ 
    \lambda(.): \mathcal{C}^0(\mathbb{R} \rightarrow \mathbb{R}^{+})\\
    \delta(.): \mathcal{C}^0(\mathbb{R} \rightarrow \mathbb{R}^{+})}} & \int_{u\in \mathbb{R} } {\lambda}(u) \\
    \textrm{ s.t. } \quad & \int_{u\in \mathbb{R}} {\delta}(u) \leq 1\\
    & \hspace{-3 em} - \left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] {\delta}(u) + {\lambda}(u) + \epsilon |{\nu}(u,\vect{x})| + {\nu}_u(u,\vect{x})   \leq 0 \text{ } \forall u\in \mathbb{R}, \forall \vect{x} \in \mathbb{R}^k \\
     & \exists U: \mathcal{C}^0(\mathbb{R}^k \rightarrow \mathbb{R})  \textrm { s.t. }\nu(u,\vect{x}) \geq 0 \text{ }\forall u\geq U(\vect{x}) \text{ } \forall \vect{x} \in (\mathbb{R})^k \\
    & \exists L: \mathcal{C}^0(\mathbb{R}^k \rightarrow \mathbb{R}) \textrm { s.t. } \nu(u,\vect{x}) \leq 0 \text{ } \forall u\leq L(\vect{x}) \text{ } \forall \vect{x} \in (\mathbb{R})^k \\    % & \exists U_{\vect{v}} \in \mathbb{R} \textrm { s.t. }\nu(u,\vect{v}) \geq 0 \text{ }\forall u> U_{\vect{v}} \text{ } \forall \vect{v} \in (\mathbb{R})^k\\
    % & \exists L_{\vect{v}} \in \mathbb{R} \textrm { s.t. }\nu(u,\vect{v}) \leq 0 \text{ }\forall u< L_{\vect{v}} \text{ } \forall \vect{v} \in (\mathbb{R})^k\\
\end{aligned}
\right.    
\end{equation}

We now prove the following set of lemmas and denote the optimal value of DILP given by $\mathcal{O}$ as $\text{opt}(\mathcal{O})$

\begin{claim}{\label{claim1}}
    $\text{opt}(\mathcal{E}^{int}) \geq \text{opt}(\mathcal{E})$
\end{claim}

\begin{proof}
    This proof follows by restricting exactly one of the values $\nu^{(1)}(u,\vect{x})$ or $\nu^{(2)}(u,\vect{x})$ = 0. In this case, we may define $\nu(u,\vect{x}) = -\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})$ and thus, $|\nu(u,\vect{x})| = \nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})$. Since, we restrict the optimization variables i.e. add an extra constraint, we get $\text{opt}(\mathcal{E}^{int}) \geq \text{opt}(\mathcal{E})$
\end{proof}

\begin{claim}{\label{claim2}}
    $\text{opt}(\mathcal{O}) \geq \text{opt}(\mathcal{E}^{int})$.
\end{claim}

\textit{Observe that the proof presented below is a slight variation of the proof for weak duality for LPs.}
\begin{proof}
    Now consider, any feasible solution $g(.,.)$ and $\kappa$ in the primal DILP $\mathcal{O}$ and feasible solution $\nu^{(1)}(.,.), \nu^{(2)}(.,.)$ in the dual DILP $\mathcal{E}^{int}$

    Now pre-multiply the first constraint in DILP $\mathcal{O}$ by $\delta(u)$ second constraint in DILP by $\lambda(u)$, the third constraint in DILP by $\nu^{(1)}(u,\vect{x})$ and fourth constraint in DILP $\mathcal{O}$ by $\nu^{(2)}(u,\vect{x})$ and take the \textit{lower Riemann-Darboux integrals} for the last term as $\underline{g}_u$ and $\overline{g}_u$ may not be Riemann integrable, however the first and second terms are integrable.\footnote{$\lowint f(x) dx$ and $\upint f(x) dx$ denotes the lower and upper integral respectively. Since $g(.)$ and $\mathfrak{h}(.)$, $\delta(.)$ and $\lambda(.)$ is Riemann integrable, the product of these functions is also integrable. } Also observe that some limits may take values in the extended reals i.e. $\mathbbm{R} \cup \{-\infty,\infty\}$ and thus, we do this algebra in this space.
    
    

   
    %\footnote{Since distribution $g(.,.)$ and $\nu(.,.)$ is \textit{Reinamann integrable} and product of \textit{integrable} functions is also \textit{integrable}. Also, since $\underline{g}_u(u,.)$ may not be \textit{Riemann integrable}, we take the lower integral which is always defined given the lower bound in third and fourth constraint of LP $\mathcal{O}$}. Thus, we get
    \zhihao{Is $\underline{g}_u$ \textit{Reinamann integrable}?}
    \sss{New proof does not require it as we use lower \textit{Reinamann integral} which is always defined}. 
    
    Observe that $d^l,d^u \in \mathbb{R}$,$\vect{c}^l,\vect{c}^u \in \mathbb{R}^k$ and $c^l_i,c^u_i$ refers to its $i^{th}$ component of $\vect{c}^l$ and $\vect{c}^u \in \mathbb{R}^k$ respectively.


Thus, we get
    %\footnote{}

    \begin{align}
        & \hspace{-1.5 em}\lim_{\substack{d^l \to -\infty \\ d^u \to \infty}} \int\limits_{u = d^l}^{d^u} \delta(u) \left[\kappa - \int\limits_{\vect{x} \in \mathbb{R}^k} \left(\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right) g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right) \right]du \\
        & \hspace{18 em}+ \lim_{\substack{d^l \to -\infty \\ d^u \to \infty}} \int\limits_{u = d^l}^{d^u} \left(\int\limits_{\vect{x} \in \mathbb{R}^k } g(u,\vect{x})  d\left(\prod_{i=1}^{k} x_i\right) \right)\lambda(u) du\nonumber\\
        & \hspace{-3 em}+ \liminf_{d, \vect{c} \to \infty}\lowint_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left((\epsilon g(u,\vect{x}) + \underline{g}_u(u,\vect{x})) \nu^{(1)}(u,\vect{x}) + (\epsilon g(u,\vect{x}) -\overline{g}_u(u,\vect{x})) \nu^{(2)}(u,\vect{x}) \right)d\left(\prod_{i=1}^{k} x_i\right) du \geq \int\limits_{u \in \mathbb{R}} \lambda(u) du\\
        & \hspace{-5 em} \text{ }\implies \lim_{\substack{d^l \to -\infty \\ d^u \to \infty}} \int\limits_{u =d^l}^{d^u} \delta(u) \lim_{\substack{\vect{c}^u \to \infty\\ \vect{c}^l \to -\infty}} \left[\kappa - \int\limits_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left(\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right) g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)\right]du \nonumber\\
        & \hspace{20 em} + \lim_{\substack{d^l \to -\infty \\ d^u \to \infty}} \int\limits_{u =d^l}^{d^u} \lim_{\substack{\vect{c}^u \to \infty\\ \vect{c}^l \to -\infty}} \left[\int\limits_{\vect{x} \in  \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} g(u,\vect{x}) \lambda(u) d\left(\prod_{i=1}^{k} x_i\right) \right] du \nonumber\\
        & \hspace{-3 em}+ \liminf_{d, \vect{c} \to \infty}\lowint_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left((\epsilon g(u,\vect{x}) + \underline{g}_u(u,\vect{x})) \nu^{(1)}(u,\vect{x}) + (\epsilon g(u,\vect{x}) -\overline{g}_u(u,\vect{x})) \nu^{(2)}(u,\vect{x}) \right)d\left(\prod_{i=1}^{k} x_i\right) du \geq \int\limits_{u \in \mathbb{R}} \lambda(u) du\\
        & \hspace{-1 em} \text{ }\overset{(c)}{\implies} \lim_{d\to \infty} \lim_{\vect{c}\to \infty} \int\limits_{u =d^l}^{d^u} \kappa \delta(u) + \left(\int\limits_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left(\left(-\delta(u)  \min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) + \lambda(u)\right)g(u,\vect{x}) \right)d\left(\prod_{i=1}^{k} x_i\right)\right) du \nonumber\\ 
        & \hspace{4 em} + \liminf_{d,\vect{c} \to \infty}\Biggl( \int_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left(\epsilon g(u,\vect{x}) \left(\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})\right)\right) d\left(\prod_{i=1}^{k} x_i\right) du\nonumber\\
        & \hspace{6 em}+ \lowint_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left(\underline{g}_u(u,\vect{x}) \nu^{(1)}(u,\vect{x}) -\overline{g}_u(u,\vect{x}) \nu^{(2)}(u,\vect{x}) \right)d\left(\prod_{i=1}^{k} x_i\right) du\Biggr) \geq \int\limits_{u \in \mathbb{R}} \lambda(u) du\\
        % & \hspace{-1 em} \text{ }\overset{(d)}{\implies} \limsup_{d,\vect{c} \to \infty} \int\limits_{u =d^l}^{d^u} \delta(u)  \left[\kappa + \int\limits_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} -\left(\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right) g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right) \right]du \nonumber\\ 
        % & \hspace{20 em} \text{ } + \limsup_{d,\vect{c} \to \infty} \int\limits_{u =d^l}^{d^u} \delta(u) \left[\int\limits_{\vect{x} \in  \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} g(u,\vect{x}) \lambda(u) d\left(\prod_{i=1}^{k} x_i\right)\right] du \nonumber\\
        % & + \liminf_{d,\vect{c} \to \infty }\lowint_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left((\epsilon g(u,\vect{x}) + \underline{g}_u(u,\vect{x})) \nu^{(1)}(u,\vect{x}) + (\epsilon g(u,\vect{x}) -\overline{g}_u(u,\vect{x})) \nu^{(2)}(u,\vect{x}) \right)d\left(\prod_{i=1}^{k} x_i\right) du \geq \int\limits_{u \in \mathbb{R}} \lambda(u) du\\
        & \hspace{-4.5 em}\overset{(d)}{\implies}   \kappa  + \limsup_{{d},\vect{c} \to \infty}\Biggl(\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left[\int\limits_{u = d^l}^{d^u} \left(-\left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] \delta(u) + \lambda(u) \right)du \right] g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)\Biggr) \nonumber\\
        & + \liminf_{d,\vect{c} \to \infty} \Biggl(\lowint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left[\lowint_{u = d^l}^{d^u} \left(\nu^{(1)}(u,\vect{x}) \underline{g}_u(u,\vect{x}) - \nu^{(2)}(u,\vect{x}) \overline{g}_u(u,\vect{x})\right)  du \right] d\left(\prod_{i=1}^{k} x_i\right)  \nonumber\\ 
        &\hspace{4.5 em} +  \int_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left(\epsilon g(u,\vect{x}) \left(\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})\right)\right) d\left(\prod_{i=1}^{k} x_i\right) du\Biggr) \geq \int\limits_{u \in \mathbb{R}} \lambda(u) du \label{first_part_step}
    \end{align}

\zhihao{In (71), is $\kappa$ has a factor $\delta(u)$?}
\sss{Was a typo addressed now}

$(c)$ \footnote{$d, \to \infty$ is a shorthand notation for $d^u \to \infty$, $d^l \to -\infty$ and $\vect{c} \to \infty$ is a shorthand for $\vect{c}^u \to \infty$ and $\vect{c}^l \to -\infty$ } follows from the following facts.

\begin{itemize}
    \item It follows from monotone convergence theorem (MCT) for the first two integrals which allows us to exchange limit and integral since the expression in $[.]$ is non-decreasing as $\vect{c}^u \to \infty$ and $\vect{c}^l \to -\infty$ due to first constraint of DILP $\mathcal{O}$ and the fact that the $g(.,.)$ is non-negative.
    \item While splitting the integral in the previous step, we replace lower integral by an integral for the second integral in $(c)$ as it is \textit{Riemann integrable}.
\end{itemize}

% $(c)$ \footnote{$d, \to \infty$ is a shorthand notation for $d^u \to \infty$, $d^l \to -\infty$ and $\vect{c} \to \infty$ is a shorthand for $\vect{c}^u \to \infty$ and $\vect{c}^l \to -\infty$ } follows from monotone convergence theorem (MCT) for the first two integrals which allows us to exchange limit and integral since the expression in $[.]$ is non-decreasing as $\vect{c}^u \to \infty$ and $\vect{c}^l \to -\infty$ due to first constraint of LP $\mathcal{O}$ and the fact that the $g(.,.)$ is non-negative. We use the fact that $\liminf_n a_n + \liminf_n b_n \leq \liminf_n (a_n+b_n)$ to combine the first two terms in the previous step 


%Also, we use the fact that $\int_{u} \delta(u)\leq 1$. We also split the last integral in the previous step to obtain two integrals in $(c)$. 

% $(d)$ follows from the fact that $\liminf_m (\liminf_n g(m,n)) \leq \limsup_{m,n} g(m,m)$

\zhihao{For limit exchange, $g(.,.)$ is non-negative, but the expression in [.] may not be non-negative}

\sss{No, it is non-negative check condition 1 and condition 2 of DILP $\mathcal{O}$ and use the fact that g(.) and $\mathfrak{h}(.)$ is non-negative.}


$(d)$ follows from the following steps.

\begin{itemize}
    \item Apply \textit{interated integral} inequality \cite[Proposition 3.9]{integral} that $\lowint_{A \times B} g(A,B) dA dB \leq \lowint_{A} \left[\lowint_{B} g(A,B) dB\right]dA$ for the last integral.

    \item For the first integral, observe that $$\int_{u\in \mathbbm{R}; \vect{x} \in \mathbbm{R}} \left(\kappa + \left(-\delta(u)  \min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) + \lambda(u)\right)g(u,\vect{x}) \right)d\left(\prod_{i=1}^{k} x_i\right) du$$ is defined as the functions are \textit{integrable}. Thus, the joint limit of $d,\vect{c} \to \infty$ is defined and equals to the iterated limit from the \textit{iterated limit theorem}.
    \item We combine the first two integrals in previous step after using the fact that $\lim_n a_n + \limsup_n b_n = \limsup_n (a_n+b_n)$ and exchange integrals using \textit{Fubini's theorem} \cite[Theorem 3.10]{integral} as the functions are \textit{Riemann integrable}.
    \item Also use the fact that $\int_{u \in \mathbbm{R}} \delta(u) \leq 1$.
\end{itemize}

% $(d)$ follows on applying \textit{interated integral} inequality \cite[Proposition 3.9]{integral} that $\lowint_{A \times B} g(A,B) dA dB \leq \lowint_{A} \left[\lowint_{B} g(A,B) dB\right]dA$ for the last integral. We combine the first two integrals in previous step after using the fact $\liminf_m \liminf_n g(m,n) \leq \limsup_{m,n} g(m,n)$ and $\liminf_n a_n + \limsup_n b_n \leq \limsup_n (a_n+b_n)$ and exchange integrals using Fubini's theorem \cite[Theorem 3.10]{integral} as the functions are Riemann integrable.


% $(e)$  follows from \textit{Interated integral} \cite[Proposition 3.9]{integral} (thus bounding lower integral by upper integral and exchanging the integration order) on the first two integrals and the constraint$\int_{u} \delta(u) \leq 1$ in DILP $\mathcal{E}$. Also, we use the fact that integrals (when exist) is always equal to its lower and upper integral. Also, for the last two integrals, we use \textit{interated integral} inequality \cite[Proposition 3.9]{integral} that $\lowint_{A \times B} g(A,B) dA dB \leq \lowint_{A} \left[\lowint_{B} g(A,B) dB\right]dA$. 



% Montononce \textit{interated integral} \cite[Proposition 3.9]{integral} (thus bounding lower integral by upper integral and exchanging the integration order) on the first two integrals and the constraint$\int_{u} \delta(u) \leq 1$ in DILP $\mathcal{E}$. Also, we use the fact that integrals (when exist) is always equal to its lower and upper integral. Also, for the last two integrals, we use \textit{interated integral} inequality \cite[Proposition 3.9]{integral} that $\lowint_{A \times B} g(A,B) dA dB \leq \lowint_{A} \left[\lowint_{B} g(A,B) dB\right]dA$

\zhihao{It seems like, Proposition 3.9 only works for integral on bounded set. On the top of Page 19 in \cite{integral}, it says \emph{Let A' be a bounded subset of $R^m$ and A'' be a bounded subset of $R^n$}}

\sss{Addressed it I put limits outside and used Monotone Convergence Theorem and Fatou's lemma to exchange integrals and limits when needed.}

Now, we bound the term $\lowint_{u \in [d^l,d^u]} \left[\nu^{(1)}(u,\vect{x}) \underline{g}_u(u,\vect{x}) du- \nu^{(2)}(u,\vect{x}) \overline{g}_u(u,\vect{x})\right] du$.\footnote{Note that the second integral is defined as the product of \textit{Riemann integrable} functions is also \textit{integrable}}. Observe that,

\begin{align}
    & \lowint_{u \in  [d^l,d^u]} \left[\nu^{(1)}(u,\vect{x}) \underline{g}_u(u,\vect{x}) du- \nu^{(2)}(u,\vect{x}) \overline{g}_u(u,\vect{x})\right] du +  \int_{u \in [d^l,d^u]} \left(\nu^{(1)}_u(u,\vect{x}) - \nu^{(2)}_u(u,\vect{x})\right) {g}(u,\vect{x}) du\nonumber\\
    \overset{(f)}{\leq} & \left[\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} \label{integral_by_parts}
\end{align}

\zhihao{why is (\ref{integral_by_parts})? And is the right side always zero? (It is $\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x})$ minus itself)}

\sss{Sorry it was a major typo addressed now}

$(f)$ follows from the chain rule of differentiation and the inequality from the fact that we take lower derivative of $-g(.)$ is upper derivative of $g(.)$

\zhihao{Is limsup/liminf sufficient for this argument?} 

\sss{Addressed it now}

% Now, we first show that the following inequality \eqref{ineqtemp1}.

% \begin{align}
% \liminf_{\substack{d^{u} \to \infty \\ d^l \to -\infty}} 
% & \liminf_{\substack{d^{u} \to \infty \\ d^l \to -\infty}} \left[-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x}) + \nu^{(1)}(d^l,\vect{x}) - \nu^{(2)}(d^l,\vect{x})  \right]\nonumber\\
% \overset{(i)}{=} & -\limsup_{d^{u} \to \infty } \left[\left(\nu^{(1)}(d^u,\vect{x}) - \nu^{(2)}(d^u,\vect{x})\right) \right] + \liminf_{d^{l} \to -\infty} \left[\left(\nu^{(1)}(d^l,\vect{x}) - \nu^{(2)}(d^l,\vect{x})\right) \right] \geq 0\label{ineqtemp1}
% \end{align}

% $(i)$ follows from from linearity of the limits and the fact that $\limsup_n A_n = - \liminf_n A_n$ and the last inequality follows from the third and fourth inequality of DILP $\mathcal{E}^{int}$.

Now consider (observe we take the -ve of the last term in Equation \eqref{integral_by_parts}). Note that since it is Riemann integrable, we may replace the lower integral by an integral. %and denote $M(\vect{x})$ as follows.

% $$M^u(\vect{x}) := \text{inf}\left\{\left(-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x})\right) g(d^u,\vect{x}) |  d^u \in \mathbb{R} \right\}$$

% $$M^l(\vect{x}) := \text{inf}\left\{\left(\nu^{(1)}(d^l,\vect{x}) - \nu^{(2)}(d^l,\vect{x})\right) g(d^l,\vect{x}) |  d^l \in \mathbb{R} \right\}$$


% Observe that $M^u(\vect{x})$ is a positive real number as 


% $M_{\vect{c}}$ as the supremum of $\left[\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u = d^l}^{d^u}$ over $\vect{x} \in \prod_{i=1}^{k} [c^l_i,c^u_i]$, observe that it exists as sumpreum of a function over any bounded interval is always defined.


% Now observe that, 

% \begin{align}\label{temp_split}
%     & \limsup_{d,\vect{c} \to \infty} \left[\upint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}-\left[\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} d\left(\prod_{i=1}^{k} x_i\right)\right]\\
%     = & \limsup_{d,\vect{c} \to \infty} \left[\upint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left(-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x})\right) g(d^u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)\right] \\
%     & \hspace{2 em} + \limsup_{d,\vect{c} \to \infty} \left[\upint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left(\nu^{(1)}(d^l,\vect{x}) - \nu^{(2)}(d^l,\vect{x})\right) g(d^l,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)\right]
% \end{align}


% Now let us define the function $\alpha(u,\vect{x}):=  \left(-\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x})$ and observe that $\alpha(u,\vect{x})$ is monotonic in $u$ for $u>M_{\vect{x}}$ [follows from Assumption on DILP $\mathcal{E}^{int}$ and the fact that $g(.)$ is bounded.] 

% Now, consider all $\vect{x} \in \prod_{i=1}^{k} [c^l_i,c^u_i]$ and we can say that $\alpha(u,\vect{x})$ is monotonic in $u$ for $u>U_{\vect{c}} := \sup_{\vect{x} \in \prod_{i=1}^{k} [c^l_i,c^u_i]} M_{\vect{x}}$ for every $x \in \prod_{i=1}^{k} [c^l_i,c^u_i]$ i.e. $\alpha(u,\vect{x}) $.\footnote{Observe that supremum is always finite as supreum of finite elements over a compact set is finite.} 




% Now, we show that first term in Equation \eqref{temp_split} in bounded below by 0.

% \begin{align}{\label{eq_lower_upper_limit_init}}
%     \hspace{-5 em}& \limsup_{d,\vect{c} \to \infty} \left[\upint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\left[\left(-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x})\right) g(d^u,\vect{x}) \right] d\left(\prod_{i=1}^{k} x_i\right)\right]\nonumber\\
%     & \hspace{-4 em} \geq  \limsup_{\vect{c} \to \infty } \liminf_{d \to \infty}\left[\upint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\left(\left(-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x})\right) g(d^u,\vect{x}) \right) d\left(\prod_{i=1}^{k} x_i\right) \right] \nonumber\\
%     & \hspace{-4 em} \geq  \limsup_{\vect{c} \to \infty } \left[\upint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\liminf_{d \to \infty} \left(-\left[\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} +M_{\vect{c},d}\right) d\left(\prod_{i=1}^{k} x_i\right)\right]\nonumber\\ 
%    \overset{(g)}{\geq} & \limsup_{\vect{c} \to \infty} \upint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \liminf_{\substack{d^{u} \to \infty \\ d^l \to -\infty}} \left[-\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} d\left(\prod_{i=1}^{k} x_i\right)\nonumber \\
%     \hspace{-3 em} \overset{(h)}{=} &  \limsup_{\vect{c} \to \infty} \upint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left(\liminf_{d^{u} \to \infty } \left[\left(-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x})\right) g(d^u,\vect{x})\right] + \liminf_{d^l \to -\infty} \left[\left(\nu^{(1)}(d^l,\vect{x}) - \nu^{(2)}(d^l,\vect{x})\right) g(d^l,\vect{x}) \right] \right) \nonumber \\& \hspace{40 em}d\left(\prod_{i=1}^{k} x_i\right) \nonumber\\
%     & \geq 0
% \end{align}




\begin{align}{\label{eq_lower_upper_limit_init}}
    \hspace{-5 em}& \limsup_{d,\vect{c} \to \infty} \left[\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}-\left[\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} d\left(\prod_{i=1}^{k} x_i\right)\right]\nonumber\\
    \overset{(i)}{\geq} &  \limsup_{\vect{c} \to \infty } \liminf_{d \to \infty}\left[\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\left(-\left[\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} \right) d\left(\prod_{i=1}^{k} x_i\right) \right]\nonumber\\
    % & \hspace{-4 em} \geq  \limsup_{\vect{c} \to \infty } \left[\upint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\liminf_{d \to \infty} \left(-\left[\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} \right) d\left(\prod_{i=1}^{k} x_i\right)\right]\nonumber\\
    \overset{(g)}{\geq} & \limsup_{\vect{c} \to \infty} \int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \liminf_{\substack{d^{u} \to \infty \\ d^l \to -\infty}} \left[-\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} d\left(\prod_{i=1}^{k} x_i\right)\nonumber \\
    \hspace{-3 em} \overset{(h)}{\geq} &  \limsup_{\vect{c} \to \infty} \int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \Bigl(\liminf_{d^{u} \to \infty } \left[\left(-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x})\right) g(d^u,\vect{x})\right]  \\
    & \hspace{12 em}+ \liminf_{d^l \to -\infty} \left[\left(\nu^{(1)}(d^l,\vect{x}) - \nu^{(2)}(d^l,\vect{x})\right) g(d^l,\vect{x}) \right] \Bigr) d\left(\prod_{i=1}^{k} x_i\right) \nonumber\\
    & \overset{(m)}{\geq} 0
\end{align}

\zhihao{Fatou's Lemma only works for non-negative functions}

\sss{Addressed check it now, showed that it is positive for sufficiently large $d^u$ and sufficiently small $d^l$.}

% \sss{A generalization of it also allows for bounded functions, we can use that to prove it check \url{https://math.stackexchange.com/questions/521179/generalization-of-fatous-lemma-for-nonpositive-but-bounded-measurable-functions}}

\zhihao{For formulas (46)-(51), we may need to explicitly distinguish $\lim_{d\rightarrow \infty}\lim_{c\rightarrow \infty}$, $\lim_{c\rightarrow \infty}\lim_{d\rightarrow \infty}$, and $\lim_{(d,c)\rightarrow (\infty,\infty)}$, and specify conditions when changing the limit type. There is $\lim_{d\rightarrow \infty}\lim_{c\rightarrow \infty}$ in (46), and there is $\lim_{c\rightarrow \infty}\lim_{d\rightarrow \infty}$ in (51), but it seems like we didn't provide reason for exchanging limit. (We are using $\lim_{(d,c)\rightarrow (\infty,\infty)}$ in the middle, without justification) }

\sss{Provided a reason for the limit exchange in $(i)$ This directly follows from standard limit-exchange theorem as stated. In (46), we used the fact that $\limsup_{m,n} f(m,n) \geq \liminf_{m} \lim_{n} f(m,n)$}

\zhihao{(I'm not confident to say this) In (51), right side of inequality (h), the integral may not be well defined. For example, is it possible that $\liminf_{d^{u} \to \infty } \left[\left(-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x})\right) g(d^u,\vect{x})\right] = +\infty$, while $\liminf_{d^l \to -\infty} \left[\left(\nu^{(1)}(d^l,\vect{x}) - \nu^{(2)}(d^l,\vect{x})\right) g(d^l,\vect{x}) \right] = +\infty$, meaning the integral is not absolutely convergent   }

%\sss{}

\sss{You are absolutely right, however the limits could go to $\infty$ and integral may not be absolutely convergent but still the limit is always defined over extended reals where limits can take value from $\mathbbm{R}\cup \{\infty,-\infty\}$ check out this wiki link \url{https://en.wikipedia.org/wiki/Extended_real_number_line}. For example read up on this how limits are defined for divergent sequences here \url{https://connect.gonzaga.edu/asset/file/1502/ch02_3_infinite_limits_v00.html}. To conclude even if both limits go to $+\infty$, as per extended real system $\infty+ \infty>0$.}

\zhihao{Follow up: in (56), is it possible that the left side is $\kappa - \infty + \infty$?}

\sss{Made some changes in the structuring of the proof. Now both terms in (58) are lower bounded. First limit in (58) + $\kappa$ is lower bounded by the sum of first integral in (48) which is postive from the first constraint in DILP $\mathcal{O}$. Second limit in (58) is positive as lower bounded by second limit of (46) which is further non-negative due to constraint of DILP $\mathcal{O}$.}

%\sss{The second term in (56) + $\kappa$ is lower bounded by the sum of first two terms in (48). Observe that first integral is positive from constraint in DILP $\mathcal{O}$ and second integral is also positive as $\nu^{(1)}$ and $\nu^{(2)}$ is positive and thus, left side in (56) is always lower bounded. Also the third term in (56) is always positive since it is lower bounded by third term in (48).}
%\sss{ We can do this as long as both the integr}

% Read on extended defintion of limits where limits can take value from $\mathbbm{R}\cup \{\infty,-\infty\}$ check out this wiki link \url{https://en.wikipedia.org/wiki/Extended_real_number_line}. For example read up on this how limits are defined for divergent sequences here \url{https://connect.gonzaga.edu/asset/file/1502/ch02_3_infinite_limits_v00.html#:~:text=Extended%20real%20numbers,-Extended%20real%20numbers&text=We%20can%20create%20an%20extension,the%20extended%20real%20number%20system.}. Thus, we can }

$(i)$ follows from the fact that $\limsup_{m,n} f(m,n) \geq \limsup_m \limsup_n f(m,n) \geq \limsup_m \liminf_n f(m,n)$.

$(g)$ follows from the following arguments.

\begin{itemize}
    \item Observe that $\left[-\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u}$ is non-negative for every $\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]$ whenever, $d_u > \sup\{U(\vect{x})| \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]\}$ and $d_l < \inf\{L({\vect{x}})| \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]\}$  from third and fourth constraint of DILP $\mathcal{E}^{int}$. Note that value is finite as supremeum and infimum of \textit{continuous functions} is finite over a \textit{compact set} \zhihao{why it is compact?}\sss{$\prod\limits_{i=1}^{k}[c^l_i,c^u_i]$ is compact as it is closed and bounded subset. $\{c_i\}$ is a finite real number inside the limit.}
    \item Now apply \textit{Fatou's lemma} to conclude $(g)$.
\end{itemize}


$(h)$ follows from the fact that $\liminf_n (A_n+B_n) \geq \liminf_n A_n + \liminf_n B_n$ and the last inequality $(m)$ follows from the following 2 statements.


\begin{itemize}
    \item $\liminf_{d^u \to \infty} \left(-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x})\right) \geq 0$ and $\liminf_{d^l \to -\infty} \left(\nu^{(1)}(d^l,\vect{x}) - \nu^{(2)}(d^l,\vect{x})\right) \geq 0$ follows from third and fourth constraint of DILP $\mathcal{E}^{int}$.

    \item $g(.,.)$ is a bounded function follows from the constraint in DILP $\mathcal{O}$. 

    % \item $0 \leq \limsup_{d^u \to \infty} g(d^u,\vect{x}) \leq \upint_u \overline{g}_u(u, \vect{x}) du \leq \upint_u \epsilon {g}(u, \vect{x}) du = \epsilon$
    
    % which follows from third constraint of DILP $\mathcal{O}$ and also similarly, $\limsup_{d^l \to -\infty} g(d^u,\vect{x}) \leq \epsilon$ from the fourth constraint of DILP $\mathcal{O}$.
\end{itemize}


\zhihao{For the last equation, we don't have $\int_u g(u,x)du = 1$}
\sss{Fixed it by just putting a constraint in DILP  that $g(.)$ is bounded.}

% from third and fourth constraint of DILP $\mathcal{E}^{int}$ and the fact that $g(.,.)$ is non-negative. Observe that the third constraint of DILP $\mathcal{E}^{int}$ implies $\liminf_{d^u \to \infty} \left(-\nu^{(1)}(d^u,\vect{x}) + \nu^{(2)}(d^u,\vect{x})\right) \geq 0$.




Observe that \eqref{eq_lower_upper_limit_init} implies (follows from $\limsup_n A_n = - \liminf_n -A_n$) that 

\begin{equation}{\label{eq_lower_upper_limit_final}}
    \liminf_{d,\vect{c} \to \infty} \left[\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\left[\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} d\left(\prod_{i=1}^{k} x_i\right)\right] \leq 0
\end{equation}


%The third and fourth constraint in the DILP $\mathcal{E}^{int}$ imply that 




%$(b)$ follows from the third and fourth constraints in the DILP $\mathcal{E}^{int}$ on $\nu^{(1)} (u,\vect{x}) - \nu^{(2)} (u,\vect{x})$ as $u \to \infty$ or $u \to -\infty$.

Using inequality in \eqref{integral_by_parts}  and the fact that $\liminf_n (a_n+b_n) \leq \liminf a_n + \limsup_n b_n$, we obtain 
\begin{align}
    & \liminf_{d,\vect{c} \to \infty} \Biggl(\lowint_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left[\lowint_{u = d^l}^{d^u} \left(\nu^{(1)}(u,\vect{x}) \underline{g}_u(u,\vect{x}) - \nu^{(2)}(u,\vect{x}) \overline{g}_u(u,\vect{x})\right)  du \right] d\left(\prod_{i=1}^{k} x_i\right) \nonumber \\ 
    & \hspace{6 em} + \int_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left(\epsilon g(u,\vect{x}) \left(\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})\right)\right) d\left(\prod_{i=1}^{k} x_i\right) \Biggr)du \\
    {\leq} & \liminf_{d,\vect{c} \to \infty} \left[\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\left[\left(\nu^{(1)}(u,\vect{x}) - \nu^{(2)}(u,\vect{x})\right) g(u,\vect{x}) \right]_{u=d^l}^{d^u} d\left(\prod_{i=1}^{k} x_i\right)\right] \\
    & \hspace{6 em}+  \limsup_{d, \vect{c} \to \infty}\Biggr(\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\left[-\int_{u \in [d^l,d^u]} \left(\nu^{(1)}_u(u,\vect{x}) - \nu^{(2)}_u(u,\vect{x})\right) {g}(u,\vect{x}) du\right]d\left(\prod_{i=1}^{k} x_i\right) \nonumber\\
    & \hspace{10 em} + \int_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left(\epsilon g(u,\vect{x}) \left(\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})\right)\right) d\left(\prod_{i=1}^{k} x_i\right) du\Biggr)\\
    \overset{(k)}{\leq} &  \limsup_{d, \vect{c} \to \infty}\Biggr(\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\left[-\int_{u \in [d^l,d^u]} \left(\nu^{(1)}_u(u,\vect{x}) - \nu^{(2)}_u(u,\vect{x})\right) {g}(u,\vect{x}) du\right]d\left(\prod_{i=1}^{k} x_i\right) \nonumber\\
    & \hspace{10 em} + \int_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left(\epsilon g(u,\vect{x}) \left(\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})\right)\right) d\left(\prod_{i=1}^{k} x_i\right) du\Biggr)\label{temp_equation1}
\end{align}

$(k)$ follows on applying Equation \eqref{eq_lower_upper_limit_final}


Now combining \eqref{temp_equation1} and \eqref{first_part_step}, we obtain
\begin{align}
    & \hspace{-6 em}  \kappa  + \limsup_{d, \vect{c} \to \infty}\Biggl(\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left[\int_{u \in [d^l,d^u]} \left(-\left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] \delta(u) + \lambda(u) \right)du \right] g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)\Biggr) \nonumber\\
        &  + \limsup_{d, \vect{c} \to \infty}\Biggr(\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\left[-\int_{u \in [d^l,d^u]} \left(\nu^{(1)}_u(u,\vect{x}) - \nu^{(2)}_u(u,\vect{x})\right) {g}(u,\vect{x}) du\right]d\left(\prod_{i=1}^{k} x_i\right) \nonumber\\
        & \hspace{10 em} + \int_{\substack{u \in [d^l,d^u] \\ \vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}} \left(\epsilon g(u,\vect{x}) \left(\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})\right)\right) d\left(\prod_{i=1}^{k} x_i\right) du\Biggr) \geq \int\limits_{u \in \mathbbm{R}} \lambda(u) du \\
    & \hspace{-6 em}  \overset{(i)}{\implies} \kappa  + \lim_{d, \vect{c} \to \infty}\Biggl(\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \left[\int_{u \in [d^l,d^u]} \left(-\left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] \delta(u) + \lambda(u)\right)du \right] g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)\Biggr) \nonumber\\
        &  + \limsup_{d, \vect{c} \to \infty}\Biggr(\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]}\left[-\int_{u \in [d^l,d^u]} \left(\nu^{(1)}_u(u,\vect{x}) - \nu^{(2)}_u(u,\vect{x})\right) {g}(u,\vect{x}) du\right]d\left(\prod_{i=1}^{k} x_i\right) \Biggr)\nonumber \\
        & \hspace{6 em} + \int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \int_{u \in [d^l,d^u]} \left(\epsilon g(u,\vect{x}) \left(\nu^{(1)}(u,\vect{x}) + \nu^{(2)}(u,\vect{x})\right)\right) d\left(\prod_{i=1}^{k} x_i\right) du\Biggr) \geq \int\limits_{u \in \mathbbm{R}} \lambda(u) du \\
    {\implies} & \kappa + \limsup_{d, \vect{c} \to \infty}\Biggl(\int_{\vect{x} \in \prod\limits_{i=1}^{k}[c^l_i,c^u_i]} \Biggl[ \int_{u \in [d^l,d^u]} \Biggl(-\left(\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right) \delta(u) + \lambda(u) + \epsilon \nu^{(2)}(u,\vect{x})  + \epsilon \nu^{(1)}(u,\vect{x})\Biggr) \\
    & \hspace{10 em} -\left(\nu^{(1)}_u(u,\vect{x}) - \nu^{(2)}_u(u,\vect{x})\right)\Biggr) du\Biggr]
    g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)\Biggr) \geq \int\limits_{u \in \mathbb{R}} \lambda(u) du\\
    & \overset{(j)}{\implies} \kappa \geq \int\limits_{u \in \mathbb{R}} \lambda(u) du
\end{align}

\zhihao{as we discussed, (i) need another way to write}

$(i)$ follows from the fact that both the integrals are \textit{Riemann integrable} from $(-\infty,\infty)$, thus limsup may be replaced by a limit.

The limsup in first term of $(i)$ can be replaced by a limit due as the limit exists since the integral is defined over $(-\infty,+\infty)$ which follows from the following reasons.

\begin{itemize}
    % \item Observe that $\int_{\vect{x} \in \mathbb{R}^k} g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)=1$ for every $u \in \mathbb{R}$ and $\int_{u \in \mathbb{R}} \left(-\left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] \delta(u) + \lambda(u) \right)du$ is defined as functions are non-negative and $\int_u \delta(u) \leq 1$.

    \item Observe that $\int_u \delta(u) \leq 1$ and $\int_{\vect{x} \in \mathbb{R}^k} \min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right) \leq \kappa \text{ } \forall u \in \mathbb{R}$ (first constraint of DILP $\mathcal{O}$) implying that $\int_{\vect{x} \in \mathbb{R}^k} \int_{u \in \mathbb{R}} \min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|)\delta(u) \leq \kappa$. 
    \item Thus, we may conclude that the following integral is defined as it lower bounded by $-\kappa$ since $\lambda(.)$ and $g(.,.)$ is a non-negative function.
    $$\Biggl(\int_{\vect{x} \in \mathbb{R}^k} \left[\int_{u \in \mathbb{R}} \left(-\left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] \delta(u) + \lambda(u) \right)du \right] g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)\Biggr)$$.
    
\end{itemize}


% $\Biggl(\int_{\vect{x} \in \mathbb{R}^k} \left[\int_{u \in \mathbb{R}} \left(-\left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] \delta(u) + \lambda(u) \right)du \right] g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right)\Biggr)$ is defined. This follows fromt eh facts


$(j)$ follows from the first and second constraint in DILP $\mathcal{E}^{int}$. Since this inequality is true for every feasible solution in the primal $\mathcal{O}$ and dual $\mathcal{E}^{int}$, we have the proof in the theorem.
\end{proof}

We now prove Theorem \ref{theorem:weak_duality_result}

\begin{proof}
    

Combining Claim \ref{claim1} and \ref{claim2}, we obtain that $\text{opt}(\mathcal{O}) \geq \text{opt}(\mathcal{E})$.



\end{proof}


\section{Claim to prove continuous bounds $U(\vect{v})$ and $L(\vect{v})$}\label{sec:continuous_bounds_claim}
\km{What is this section? There is no context at all. Section heading is wrong English.}

\begin{claim}{\label{claim:continuity_bounds}}
    Consider a  function $\nu(.,.): \mathcal{C}^1(\mathbbm{R} \times \mathbbm{R}^k \rightarrow \mathbbm{R})$ s.t. zeros of $\nu(.,\vect{v})$ i.e. $\{\mathfrak{u}:\nu(\mathfrak{u},\vect{v})=0\}$ is a \textit{countable} set for every $\vect{v} \in \mathbbm{R}^k$. 
    
    It also satisfies the following two conditions for some constant $C$ independent of $\vect{v}$. Note that $v_{\floor{i}}$ denotes the $i^{th}$ largest component of $\vect{v}$ for every $i \in [k]$.
    \begin{itemize}
        \item $\set[\Big]{\mathfrak{u} \in \mathbb{R}: \nu(\mathfrak{u},\vect{v})=0 \text{ and } \nu_u(\mathfrak{u},\vect{v}) < 0 }$ is upper bounded by $C+ v_{\floor{k}}$ for every $\vect{v} \in \mathbbm{R}^k$. \zhihao{what is $v_{\floor{k}}$?}
        \sss{Check the notation subsection. We defined $v_{\floor{k}}$ to be $k^{th}$ largest component (or basically the largest component of $\vect{v}$.)}
        \item $\forall \vect{v} \in \mathbbm{R}^k \text{ } \exists \text{ }\mathcal{U}$ s.t $\nu(u,\vect{v}) \geq 0 \text{ }\forall u >\mathcal{U}$.
    \end{itemize}
Then there exists $U: \mathcal{C}^0(\mathbbm{R}^k \rightarrow \mathbbm{R})$ s.t. $\nu(u,\vect{v}) \geq 0 \text{ }\forall u\geq U(\vect{v}) \text{ }\forall \vect{v} \in \mathbbm{R}^k$.
\end{claim}


\begin{proof}
    We prove this statement as follows. For every $\vect{v} \in \mathbbm{R}^k$, denote the largest zero of $\nu(.,\vect{v})$ by $p(\vect{v})$. Now construct $U(\vect{v}) = \max(p(\vect{v}), C+ v_{\floor{k}})$. Observe that $\nu(u,\vect{v}) \geq 0 \text{ }\forall u\geq U(\vect{v}) \text{ }\forall \vect{v} \in \mathbbm{R}^k$ follows from the second assumption.

    To prove continuity at $\vect{v} \in \mathbbm{R}^k$, we aim to show the following statement. 

    \begin{equation}{\label{eqn:continuity}}
        \forall \epsilon >0 \text{ } \exists \delta >0 \text{ s.t. } \forall \vect{z} \in \mathbbm{R}^k; \text{ }||\vect{z}-\vect{v}||_1 \leq \delta \implies |U(\vect{z}) - U(\vect{v})| \leq \epsilon.
    \end{equation}
    

   We now show $U(\vect{v})$ is continuous for every $\vect{v} \in \mathbbm{R}^k$. We consider two exhaustive cases below.

    \textit{Case 1}: $p(\vect{v}) \geq C+ v_{\floor{k}}$ and thus, $U(\vect{v}) = p(\vect{v})$. Recall from the second assumption that $\nu(u,\vect{v})$ goes from negative to positive at $u=p(\vect{v})$.

     We now discuss the construction of $\delta$ below for a \textit{sufficiently small} $\epsilon$ as follows. 

    For some $\epsilon$ sufficiently small, we now discuss the construction of an interval around $p_{\vect{v}}$ as $[\mathcal{A}_\vect{v},\mathcal{B}_\vect{v}] = [p_{\vect{v}}-\frac{\epsilon}{2}, p_{\vect{v}}+\frac{\epsilon}{2}]$. Since, $\epsilon$ is sufficiently small, observe that $\nu(\mathcal{A}_{\vect{v}},\vect{v}) = -\zeta_1$ and $\nu(\mathcal{B}_{\vect{v}},\vect{v}) = \zeta_2$ for some $\zeta_1,\zeta_2>0$

    Observe that $\nu(\mathcal{A}_{\vect{v}},\vect{v})$ must be continuous in $\vect{v}$ and thus there must exist $\delta_1>0$ s.t. $\forall \vect{z} \in \mathbbm{R}^k; \text{ }||\vect{z}-\vect{v}|| \leq \delta_1 \implies |\nu(\mathcal{A}_{\vect{v}},\vect{v}) - \nu(\mathcal{A}_{\vect{v}},\vect{z})| \leq \frac{\zeta_1}{2}$ and similarly, choose $\delta_2>0$ s.t. $\forall \vect{z} \in \mathbbm{R}^k; \text{ }||\vect{z}-\vect{v}_1|| \leq \delta_2 \implies |\nu(\mathcal{B}_{\vect{v}},\vect{v}) - \nu(\mathcal{B}_{\vect{v}},\vect{z})| \leq \frac{\zeta_2}{2}$.\footnote{Note that we can do this since, the continuity result holds true for every $\epsilon>0$ and we can choose any $\epsilon$ we want. } 

     \textbf{We choose $\delta = \min(\delta_1,\delta_2,\frac{\epsilon}{2})$ and consider any $\vect{z} \in \mathbbm{R}^k$ satisfying $||\vect{z}-\vect{v}||_1< \delta$ and show \eqref{eqn:continuity}}
    
    
    This  implies $\nu(\mathcal{A}_{\vect{v}},\vect{z}) < -\frac{\zeta_1}{2}<0$ and $\nu(\mathcal{B}_{\vect{v}},\vect{z}) > \frac{\zeta_2}{2}>0$ since, $\nu(\mathcal{A}_{\vect{v}},\vect{v}) = -\zeta_1$ and $\nu(\mathcal{B}_{\vect{v}},\vect{v}) = \zeta_2$. Thus, from \textit{intermediate value and LMVT theorem}, there must exist some zero of $\nu(.,\vect{z})$ (call it $u_0$) with $u_0 \in [\mathcal{A}_{\vect{v}},\mathcal{B}_{\vect{v}}]$ with $\nu(.)$ going from negative to positive i.e. $\nu_u(u_0,\vect{z}) \geq 0$ and $\nu(u_0,\vect{z})=0$

    Also observe that, 

    \begin{align}{\label{eqn1:temp}}
        \mathcal{B}_{\vect{v}} & \overset{(a)}{\geq} C+ v_{\floor{k}}  + \frac{\epsilon}{2}\nonumber\\
        & \overset{(b)}{>} C+ z_{\floor{k}} + \frac{\epsilon}{2} - \delta \geq C+ z_{\floor{k}}
    \end{align}
    

    $(a)$ follows from $p(\vect{v}) \geq C+ v_{\floor{k}}$ and the definition of $\mathcal{B}_{\vect{v}}$. $(b)$ follows from the fact $||\vect{v}-\vect{z}||\leq \delta$. Observe that the last inequality follows from  
    the fact that $\delta< \frac{\epsilon}{2}$.

     Equation \eqref{eqn1:temp} and the first condition in Claim \ref{claim:continuity_bounds}implies that $U(u,\vect{z})$ cannot have a zero in $u$ with $U(u,\vect{z})$ going from positive to negative on the right side of interval $[\mathcal{A}_{\vect{v}},\mathcal{B}_{\vect{v}}]$. This implies that the largest zero of $\nu(u,\vect{z})$ in interval $[\mathcal{A}_{\vect{v}},\mathcal{B}_{\vect{v}}]$ must be the largest zero and thus, it must be $p(\vect{z})$. Also, $p(\vect{z}) > \mathcal{A}_{\vect{v}} > C+z_{\floor{k}}$ and thus, $U(\vect{z}) = p(\vect{z})$

    We thus, have $|U(\vect{z})-U(\vect{v})| = |p(\vect{z})-p(\vect{v})| \leq \epsilon$, since $\max(|\mathcal{A}_{\vect{v}} - p(\vect{v})|,|\mathcal{B}_{\vect{v}} - p(\vect{v})|) < \epsilon$ thus proving the desired result in \eqref{eqn:continuity}


    \textit{Case 2}: $p(\vect{v}) < C+ v_{\floor{k}}$, thus $U(\vect{v}) = C+ v_{\floor{k}}$.

    Since, $p(\vect{v})$ was the largest zero of $\nu(.,\vect{v})$ with $\nu_u(p(\vect{v}), \vect{v}) >0$, observe that $\nu(C+ v_{\floor{k}}, \vect{v}) = \zeta >0$. Now since $\nu(u,\vect{v})$ is continuous, there must exist $\delta_1>0$ s.t. $\forall \hat{u} \in \mathbbm{R}$ satisfying $|\hat{u}-(C+v_{\floor{k}})| < \delta_1$, we have  $|\nu(\hat{u},\vect{v})- \nu(\hat{u},\vect{v})| < \frac{\zeta}{4}$. Similarly, there must exist $\delta_2>0$ s.t. $ \forall \vect{z} \in \mathbb{R}$ satisfying $||\vect{v}-\vect{z}||_1 < \delta_2$, we have $|\nu(C+z_{\floor{k}},\vect{v}) - \nu(C+z_{\floor{k}},\vect{z})| \leq \frac{\zeta}{4}$. \footnote{This holds since continuity result holds for every $\epsilon>0$}

    \textbf{Now we choose $\delta = \min(\delta_1,\delta_2,\epsilon)$ and consider any $\vect{z} \in \mathbb{R}^k$ satisfying $||\vect{z}-\vect{v}||_1 \leq \delta$ to show \eqref{eqn:continuity}.}

    
    Observe that, since, $|(C+v_{\floor{k}}) - (C+ {z}_{\floor{k}})| \leq \delta \leq \delta_1$, we must have $\nu(C+z_{\floor{k}},\vect{v}) = \nu(C+v_{\floor{k}},\vect{v}) + (\nu(C+z_{\floor{k}},\vect{v})- \nu(C+ {v}_{\floor{k}},\vect{v})) \geq \zeta -\frac{\zeta}{4} = \frac{3\zeta}{4}$. Similarly, since $||\vect{v}-\vect{z}|| \leq \delta \leq \delta_2$, we must have $\nu(C+z_{\floor{k}},\vect{z}) = \nu(C+z_{\floor{k}},\vect{v}) + (\nu(C+z_{\floor{k}},\vect{v})-\nu(C+z_{\floor{k}},\vect{v})) \geq \frac{3\zeta}{4}-\frac{\zeta}{4} = \frac{\zeta}{2}>0$.


    Since, $\nu(C+z_{\floor{k}},\vect{z})>0$ and since the second condition in claim \ref{claim:continuity_bounds} says that there can be no zero of $\nu(u,\vect{z})$ in $u$ with $\nu(u,\vect{z})$ going from positive to negative beyond $C+z_{\floor{k}}$ we have the largest zero of $\nu(.,\vect{v})$ should be smaller than $C+z_{\floor{k}}$ and thus $U(\vect{z}) = C+z_{\floor{k}}$.

    Now observe that $|U(\vect{z})-U(\vect{y})| = |(C+z_{\floor{k}})-(C+y_{\floor{k}})| \leq \delta \leq \epsilon$, thus proving the desired statement in \eqref{eqn:continuity}.


    
    

    % Observe that $C+z_{\floor{k}} -  (C+ v_{\floor{k}}) \leq \delta \leq \epsilon$

    % First observe that we have $U(\vect{z}) - (C+ v_{\floor{k}}) \geq C+z_{\floor{k}} - (C+v_{\floor{k}}) \geq -\epsilon$ and now consider two exhaustive cases

    % %Now, we give the construction of $\delta$ for every $\epsilon>0$. Choose $\delta = \epsilon$. 

    % \textit{Case 2(a)} $p_{\vect{z}} \leq C+ z_{\floor{k}} + \frac{\epsilon}{2}$ which implies, that 

    % \begin{align}
    %     p_{\vect{z}} - U(\vect{v}) & \overset{(c)}{\leq} (C+ z_{\floor{k}} + \frac{\epsilon}{2}) - v_{\floor{k}} \\
    %     & \overset{(d)}{\leq} \frac{\epsilon}{2} + \delta \leq \epsilon
    % \end{align}

    % We thus prove that $U(\vect{z})-U(\vect{y}) \leq \epsilon$

    % \textit{Case 2(b)} $p_{\vect{z}} \geq C+ z_{\floor{k}} + \frac{\epsilon}{2}$ This implies that 


    

    
    
\end{proof}




==> relatedak.tex <==
\subsection{Context for Introducing the ``Multi-Selection" Architecture}
% Define DP.
% Differential privacy is a gold standard privacy guarantee, because...
Following a series of high-profile de-anonymizations in practice~\cite{narayanan2008robust} and the reconstruction attack of Dinur and Nissim~\cite{ding2017collecting}, differential privacy (DP)~\cite{dwork2006calibrating} has been firmly established as a privacy desiderata.
An algorithm satisfies differential privacy iff any individual user's data has a negligible impact on the algorithm's output.
Two models of trust are popular within the DP literature, the trusted curator model (TCM) and the local model (LM). The TCM model requires an individual's trust in a curator, as the procedure for privacy preservation is applied by the curator after all individuals' data are collected in the clear. 
In contrast, the local model~\cite{warner1965randomized, kasiviswanathan2011can} requires no such trust -- the individual's data is privatized before it leaves the user device. 

Privacy from the perspective of an individual is particularly desirable in personalized applications such as search, advertising, and recommendation systems. This local model of trust also has its use in medical and mental health-related searches where the individual wants to receive individualized, personalized results without revealing to the search engine that they may be ill. Thus, from the perspective of privacy, the guarantees of the local model of DP are more desirable, not only because they do not require trust in anyone but also because they protect from other modes of attack, such as government subpoenas, malicious company employees, and data breaches. In our work, we shall study the LM of trust since it involves clients querying the server.

% At the same time,
% This is the scenario for which algorithms under local DP give notoriously bad privacy/utility trade-offs, ultimately due to the increase in the  dimensionality of the data.

Within the LM model of trust, a well-studied DP model is local differential privacy which requires a privacy guarantee of $\epsilon$ for any two potential values of an individual's data. Geographic differential privacy \cite{andres2013geo} relaxes/generalizes this requirement to consider the distance between the two values, allowing the privacy guarantee to decay in proportion to the distance. Originally introduced in the context of protecting the privacy of one's location, the intuition behind the relaxation is that the user may want to ensure more privacy protection for their precise location (e.g. they may not want the provider to have a high chance of inferring their precise location within the 7th arrondissement of Paris) but cares less about the privacy of their high-level location (e.g. they may be willing to tolerate an increase in the provider's ability to infer that they are located in Paris rather than London). One can observe that geographic differential privacy satisfies composability and is also robust to post-processing. \ak{need to check and put references} %Put differently, in the geo-indistinguishability framework, the privacy guarantee decays as $\epsilon/R$ for two users separated by distance $R$.  

% Within the differential privacy definitions, the standard requirement is for the $\epsilon$-indistinguishability of the algorithm's outputs to hold for any two potential values of an individual's data. % (equivalently, for any two users). 
% The definition of geo-indistinguishability~\cite{andres2013geo} relaxes / generalizes this requirement to consider the distance between the two values, allowing the privacy guarantee to decay in proportion to the distance. 
% Originally introduced in the context of protecting the privacy of one's location, the intuition behind the relaxation is that the user may want to ensure more privacy protection for their precise location (e.g. they may not want the provider to have a high chance of inferring their precise location within the 7th arrondissement of Paris) but cares less about the privacy of their high-level location (e.g. they may be willing to tolerate an increase in the provider's ability to infer that they are located in Paris rather than London). Put differently, in the geo-indistinguishability framework, the privacy guarantee decays as $\epsilon/R$ for two users separated by distance $R$. 
%Within the differential privacy definitions, two distinct ones are common -- the standard one, which ensures negligible privacy impact of participation for any two potential values of an individual's data; and the geographic, which ensures negligible privacy impact for the values that are at most $R$ apart. 
%Originally introduced in the context of location data, the geographic data privacy makes sense also in \cite{sth}.
%In the first model termed ``geographic differential privacy'', the privacy parameter decays as $\epsilon/R$ for two users separated by distance $R$. 
%It is called geographic because the relaxation with $R$ is originally introduces for protecting location data.
% These privacy models have pros and cons. The local differential privacy model is perhaps the gold standard~\cite{citehere}, primarily because it is composable~\cite{andcitehere} \ak{because resilient against very powerful adversaries}. However, it can lead to utility loss that is too large, since every user needs to be roughly indistinguishable from every other user. %\ak{Propose rephrase: lead to utility loss that is too large.}
 There are several other scenarios where a user may be more sensitive to the leakage of the finer-grained information, rather than coarser-grained information, and thus where the ``geographic" version of the guarantee is applicable, including in the search and advertising domains. 
 For example, the user might be more open to sharing that they are searching for wellness-related information rather than beauty-related information, but less open to sharing that, within wellness, they are interested in diabetes prevention rather than abs strengthening.
 Likewise, they may be more open to sharing their overall salary band (as that information can also, potentially, be inferred from the public knowledge of their role within a company), than sharing their precise salary within that band (as that may lead to unfavorable comparisons with the salaries of colleagues in the same role). 
 %in the In many situations (e.g.~\cite{citesomethings}) a user may be more sensitive to finer-grained information leaking, for instance, the exact address or income, as opposed to coarse-grained information. This motivates the geographic model, where the privacy parameter decays with distance from the user's feature. We present results for both models.


Extensive academic literature developing algorithms for achieving differential privacy has led to a number of practical deployments of DP, including by US Census, Facebook, LinkedIn, Google~\cite{Plume}; see~\cite{Ted} for a complete list as of early 2023. However, most of the deployments assume the trusted curator model of trust. 
A few exceptions to this, assuming the local model of trust, are RAPPOR for finding popular malicious websites by Google~\cite{RAPPOR} and emoji frequency estimation and new word discovery by Apple~\cite{Apple}. 
Notably, the broad purpose and utility of these deployments is for the server to build global models that would then be distributed for each individual to use, for relatively simple tasks such as most-frequent-itemsets or next-word prediction, rather than for personalized queries such as search and advertising.
%Moreover, the two deployments in local model (RAPPOR and Apple) are for building large global models, not for any personalized models, such as search and advertising.
The reason for this is that, even for the simplest data science tasks, there are strong separation results in utility achievable in the LM vs in the TCM (see, e.g.~\cite{BeimelNO08, kasiviswanathan2011can, BassilyS15, ShiCRS17} for a formal treatment). To add, algorithms under local DP often give worse privacy/utility trade-offs with the increase in the dimensionality of the data \cite{s20247030,10.14778/3430915.3430927}.


%Algorithms under local DP often give bad privacy/utility tradeoffs with the increase in dimensionality of the data \cite{s20247030,10.14778/3430915.3430927}.

%local model, where it's individual's data and they are trying to retrieve a result personalized to their specific query. 
%At the same time, privacy from the perspective of individual is particularly desirable in personalized applications such as search, advertising, and recommendation systems. In these scenarios, it is the local model that would be a natural fit, as, for say, medical and mental health related searches, the individual wants to receive individualized, personalized results without revealing to the search engine that they may be ill.
%This is the scenario for which algorithms under local DP give notoriously bad privacy/utility trade-offs, ultimately due to the increase in the  dimensionality of the data \cite{s20247030,10.14778/3430915.3430927}.
%Local DP gives very bad utility for that scenario, as in order to receive any sensible privacy guarantee even for one bit of data, need to flip that bit with probability X; which further grows with the dimensionality of the data. \cite{sth} Cite theory results.

The desire for ensuring privacy in the local model, while maintaining utility and applicability to personalized query scenarios, has resulted in an extensive search for relaxations of DP, such as label-DP~\cite{pmlr-v19-chaudhuri11a}, one-sided DP~\cite{kotsogiannis2020one}, context-aware DP~\cite{pmlr-v119-acharya20a}, per-instance DP~\cite{wang2019per}, and others~\cite{desfontaines2019sok}. 
The potential of these DP relaxations is still being explored, with considerations including the extent to which they capture user-desired notions of privacy and their suitability for composition (a property of the original DP definition that is incredibly desirable when there are multiple uses of the underlying data or the uses repeat over time).
Further, in practice, arguments are often made that due to the harsh privacy-utility trade-off, it is justified to give up on DP altogether and go back to the weaker notion of privacy such as k-anonymity (see, e.g. Google's arguments in its high-profile advertising efforts, the Privacy Sandbox for Advertising~\cite{floc}). 


%People have been looking for relaxations of privacy, whereas we propose a new system architecture that perhaps enables more woeful mechanism.



==> roadmap.tex <==
\subsection{Roadmap}
%In the main paper, we show simplified models and corresponding results. In the appendix, we provide the general model and full proofs.
In the main paper, we give simplified models and corresponding results and provide proof sketches in sufficient detail to convey the main technical ideas. Complete versions of the proofs are presented in the Appendix.


We mainly discuss the multi-selection \ak{multi-selection} model in geographic differential privacy formally defined in Section \ref{sec:simmodel}, and we present the proof of our main result in Section~\ref{sec:simproof}. In Section \ref{sec:simproof}, we present a proof sketch that users should report their values \ak{inconsistent terminology} after adding Laplace noise. This proof sketch is fairly detailed. In Section \ref{subsec-comb:proof-step1}, we show the user can simulate the server before reporting their values. In Section \ref{subsec-comb:primal-feasible}, we represent the objective cost function as an infimizing linear program over infinite dimensional vector spaces and also give the construction of a supremizing linear program which we refer to as the dual program in the rest of this paper. Observe that we have to explicitly prove a lemma lower bounding the objective of infimizing linear program by its dual. This is because the existing theory of infinite dimensional linear programs involves constraints on integrals, not derivatives, for example, check \cite{anderson1987linear}. Since, DILPs can be used to model other problems beyond differential privacy, we believe our weak-duality result has broader application. We give some examples in Appendix~\ref{sec-appendix:weak_duality_application}. Finally, in Section \ref{subsec-comb:dual-soln-construction}, we use dual-fitting to show the optimality of the Laplace noise addition mechanism. We also generalize our results by showing the optimality of Laplace noise addition in $\mathfrak{f}(.)$-geographic differential privacy where the privacy guarantees between two users $u_1$ and $u_2$ does not scale linearly with distance $d(u_1,u_2)$ but scales linearly with $\mathfrak{f}(d(u_1,u_2))$ in Appendix \ref{sec:diff-privacy-gen} for some increasing convex function $\mathfrak{f}(.)$. This notion is useful when users have little or no privacy requirements from users far away from it but have higher requirements in the vicinity.
\sss{Made some changes, needs to be read carefully}

\sss{As we discussed, maybe we need to convey better what is novel in our work and results?}



%, and the server only needs to return the received signal. This result is intermediate, and the server will do something in the final mechanism
% In Section \ref{sec:simproof2}, we show the optimal mechanism can be \emph{symmetric}, which means the users' behavior should be independent of the location. In Section \ref{sec:simproof3}, we show that the optimal behavior is for users to add Laplace noise before sending the signal. In Section \ref{sec:simres}, we show how the server responds after receiving signals with Laplace noise. In Section \ref{sec:simlocal}, we discuss the model in the local differential privacy setting, and the ideas are similar to the geographic differential privacy setting.


==> simple-model-modified.tex <==
\section{The Model for Multi-Selection in Differential Privacy}  \label{sec:simmodel}
%\label{sec:subsecsimmodel}

\ak{I suggest to write this section as follows: here's the formal definition / notation of user data, and the actions available to them and the definition of actions available to the server given the user data. Here's local epsilon geographic DP abstractly defined, and this is what it means in our setting of multi-selection, hence the privacy constraint we need to satisfy. Now the goal is to find the triple of mechanisms that will maximize utility subject to this constraint, where utility is defined as xxx. We then take this formal problem statement and solve it for a special case where values / utility function are ..., and thus the problem formulation thus becomes ...}

%\ak{I'd re-order this -- first introduce the e-geographic DP formally, then introduce our new system architecture formally, then state the minimization desiderata. Also change title of the section to: The Model for Multi-Selection in Geographic Differential Privacy }
%\subsection{Model}  

%\paragraph{$\epsilon$-geographic differential privacy: }
We start with some notation. 
\ak{Need context for this notation; what is the set meant to represent, what kind of values does it take?}

Given a set $S$, if we use $K(\cdot)$ to denote a distribution on $S$, then $K(H)$ is the probability mass of $H\subset S$. For distributions $K$ and $K'$ on $S$, we define their distance to be $\ddis{K}{K'} \defeq \sup\limits_{H\subseteq \ak{should this be $\subseteq$?} S; K(H) \neq 0} \frac{K(H)}{K'(H)}$.\footnote{We treat $\frac{a}{0}$ to be $+\infty$ for $a>0$ \ak{missing why?}} For a $\K$-dimensional vector $\vect{a} = (a_1,\dots,a_{\K})\in \real^{\K}$, we use $\texttt{Set}(\vect{a})$ to convert it into a set, more formally $\texttt{Set}(\vect{a}) = \{a_i: i \in [k]\}$. \ak{Not sure what this conversion buys us, also not sure where we use this notation?}

\sss{We use this notation since we choose an element from the component of $\vect{a}$. for example, it does not make sense to write $x \in \vect{a}$.}


% we also regard it as a set of size $\K$ to be convenient. When we say $a\in (a_1,\dots,a_{\K})$, it means $a\in \{a_1,\dots,a_{\K}\}$.

In the {\em geographic DP} model, there is a set of users $U$. \ak{given that we are using the local model version of geographic DP, why do we need "a set of users" rather than defining everything in terms of two possible values for the same user?}
User $u\in U$ draws a signal from distribution $\Pname_u$ and then sends it to the server. 
To satisfy $\epsilon$-geographic differential privacy, for any two users $u_1,u_2 \in U$, it should hold that $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon\cdot d(u_1,u_2)}$, where $d(u_1,u_2)$ is a certain distance between $u_1,u_2\in U$ such that $(U,d)$ is a metric space. 
%Observe that this distance function may also be dependent on the set $U$.

%\in U$. %

% To satisfy $\epsilon$-local differential privacy, for any 2 users $u_1\in U$ and $u_2\in U$, it should hold that $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon}$. 

In this model, the users and the results belong to the same set $U$. To relax this assumption, check Appendix \ref{appendix-sec:restricted_unrestricted_setup}. The dis-utility of  an user $u \in U$ w.r.t a result $m \in U$ is given by $\mathfrak{h}(d(u,m))$.

\ak{Need to explain why it should satisfy such constraints -- b/c that's the function we can prove stuff about, or some other reason?}
%\sss{The first point comes from the fact that disutility }
\begin{enumerate}[label= \arabic*]
    \item \label{item:first-propertyh} $\mathfrak{h}(.)$ is a continuously increasing function satisfying $\mathfrak{h}(0)=0$.
    \item \label{item:second-property-h} There exists $\mathcal{B} \in \real^{+}$ s.t. $\log \mathfrak{h}(.)$ is Lipschitz continuous in $[\mathcal{B},\infty)$
\end{enumerate}

%Ratios of polynomials and exponential functions satisfy the second criterion for example $\sqrt{z},z^2, e^{z}$, however functions like $e^{z^2}$ do not satisfy the same.
Observe that ratios of polynomials and exponential functions like $\sqrt{z},z^2, e^{z}-1$ satisfy the second criterion, however functions like $e^{z^2}-1$ do not. \ak{Why give $e^{power}$ as an example given that it doesn't even satisfy the first criterion?}\sss{Addressed by defining $e^{z^2}-1$} \ak{no because  $e^{z^2}$ still doesn't satisfy the first criterion. also, why do we even care about such functions? }



% \begin{definition}{\label{def:disutility_user_result}}
%     Dis-utility of user $u$ from result $m$: The dis-utility of an user $u$ from a movie $m$ w.r.t some continuously increasing function $\mathfrak{h}(.)$ is given by \footnote{If no such $u'$ exists then the disutility is $\infty$ as infimum of a null set is $\infty$.}
%     \begin{equation}{\label{eqn:disutil_user_result}}
%         \Disutility^{\mathfrak{h}(.)}(u,m) := \inf\limits_{u': OPT(u')=m} \mathfrak{h}(d_U(u,u'))
%         %
%     \end{equation}%\footnote{If no such $u'$ exists then the disutility is defined to be $\infty$.}
% \end{definition}

% \zhihao{what if no $u'$ such that $opt(u')=m$}
% \sss{We will make it go to $\infty$ then. I will put a footer for that}
% \subsubsection{Restricted setup}

% This setup is very similar to the setup described except the fact that users and results(ads) lie on the same set $U$. The dis-utility of an user $u$ from a result $m$ is given by $\mathfrak{h}(d_U(u,m))$ for some function $\mathfrak{h}(.)$ satisfying properties \ref{item:first-propertyh} and \ref{item:second-property-h}. 


\subsection{The space of server/user actions}
The goal is to determine a mechanism that has the following ingredients:
\ak{Shouldn't both $d$ and $\epsilon$ figure in the input to the mechanism?}
\sss{Yes since we assumed that $d$ and $U$ is universally known in our model, we did not explicitly state that.}
\ak{Needs to be stated for a formal problem definition}

% \paragraph{Multi-Selection model} We assume users and results are located on a line, and the location is denoted by a real number. The distribution of users is $\Dist$, which is supported on $\real$. A user sends a signal to the server, and the server returns a set of $\K$ results, each of which maps to a point on the real line. Then the user chooses the closest among those $\K$ results to its own location. Using the notation defined above, we assume the server responds with a vector in $\real^{\K}$. The goal is to determine a mechanism that has the following ingredients:

\begin{enumerate}
\item A set of signals $\Signals$. 
\item The action of users, which involves choosing a signal from a distribution over signals. We use $\dsig{u}$ for $u\in U$ to denote the distribution of the signals sent by user $u$.  \ak{Wasn't $\dsig{u}$ already defined?} \ak{Also, the user isn't actually sending a distribution of signals, they are sending a signal, drawn from a distribution.}
This distribution is supported on $\Signals$.
\item The distribution over actions of the server, $\dsigq{s}$ when it receives $s\in \Signals$. This distribution denoting the distribution of the result (ad) \ak{remove the ad from here?} set returned by the server given signal $s$ is supported on either $U^k$. \ak{Why is this $U^k$ and not $\Signals^k$? Isn't it better to define the problem generally than with the assumption that users and sets belong to the same set?}
\sss{The signal that an user sends to the server belong to a different set $Z$ but the users and results belong to the same set $U$.} \ak{I understand that this is the simplified case we solve, but if this is the general formulation of the problem, then it should be stated in full generality first and then describe the special case. The formulation of users and results belonging to the same set $U$ is also awkward, it should be at least user *values*. }
\end{enumerate}

The optimal mechanism is computed by jointly  optimizing over the tuple $(Z,\dsig{u},\dsigq{s})$.
 %   \item $\Qrobs_{\text{restricted},\Signals}:=\{ \Qname | \forall s\in \Signals, \dsigq{s}\text{~is a distribution on $U^{\K}$} \}$.
%\end{itemize}


In any {\em feasible geographic DP mechanism}, the  user behavior should satisfy $\epsilon$-geographic differential privacy: for any $u_1,u_2\in U$, it should hold that $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon\cdot d(u_1,u_2)}$. 
For any fixed response size $k$, in order to maximize utility while ensuring the specified level of privacy, the goal is to minimize the disutility of the user from the result that  gives the user minimum dis-utility where the minimisation is over the worst case user $u \in U$. %with respect to distribution of users denoted by $\probm{\Users}$. 
\ak{This is poorly explained -- what is the "worst case user"? Whose utlity are we maximizing? }
\ak{This is also poorly motivated -- presumably we could've picked various cost functions, why do we choose this one?}


% and in any {\em local DP mechanism}, the user behaviour should satisfy $\epsilon$-local differential privacy for any $u_1, u_2 \in U$, it should hold that $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon}$.

\subsection{Cost functions}{\label{sec:objective}} 

%For the unrestricted and restricted setups, we define the cost functions $\funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ and $\funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ respectively below. Recall that $Z$ may denote any set. 

Thus, we define the cost function as follows.

% \[  \funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
% \defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}\\ \Qname\in \Qrobs_{\text{unrestricted},\Signals}}} \sup_{\Dist \in \probm{U}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\left(\Disutility^{\mathfrak{h}(.)}(u,a)\right) }, \]

\[  \funfgeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
\defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}; \Qname\in \Qrobs_{ \Signals}}} \sup_{u \in \Users} \Exxlimits{s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}\left(d(u,a)\right) }, \text{ where }\]
\ak{This formula needs better typesetting as it is unclear which subscripts belong to which of inf, sup...}

$\Probsgeo{\Signals}:=\{ \Pname | \forall u\in U, \dsig{u}\text{~is a distribution on $\Signals$,} 
    \text{~and $\epsilon$-geographic differential privacy is satisfied} \}$.
    \ak{Inconsistent notation -- why is $u\in \real$ here whereas it was $u \in U$ before? $\Pname_u$ was already defined, etc}

$\Qrobs_{\Signals}:= \{ \Qname | \forall s\in \Signals, \dsigq{s}\text{~is a distribution on $U^{\K}$} \}$. 
% \subsubsection{Objective in the unrestricted setup}{\label{sec:relaxed-objective}} In this case, we want to compute cost function $\funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ (and its associated mechanism) for the case of geographic differential privacy which is defined as 
% \[  \funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
% \defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}\\ \Qname\in \Qrobs_{\text{unrestricted},\Signals}}} \sup_{\Dist \in \probm{U}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\left(\Disutility^{\mathfrak{h}(.)}(u,a)\right) }, \text{ where }\]
% and for the case of local differential privacy is defined as
% \[  \funforigloc{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
% \defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsloc{\Signals}\\ \Qname\in \Qrobs_{\text{relaxed},\Signals}}} \sup_{\Dist \in \probm{U}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\left(\Disutility^{\mathfrak{h}(.)}(u,a)\right) }, \]

% $\Probsgeo{\Signals}:=\{ \Pname | \forall u\in \real, \dsig{u}\text{~is a distribution on $\Signals$,} 
%     \text{~and $\epsilon$-geographic differential privacy is satisfied} \}$.


% \begin{enumerate}
% %    \item For $A=(a_1,a_2,\dots,a_{\K})\in \real^{\K}$, we say $a\in A$ if $a\in \{a_1,\dots,a_{\K}\}$.
%     \item $\Probsgeo{\Signals}:=\{ \Pname | \forall u\in \real, \dsig{u}\text{~is a distribution on $\Signals$,} 
%     \text{~and $\epsilon$-geographic differential privacy is satisfied} \}$.

%     % \item $\Probsloc{\Signals}:=\{ \Pname | \forall u\in \real, \dsig{u}\text{~is a distribution on $\Signals$,} 
%     % \text{~and $\epsilon$-local differential privacy is satisfied} \}$.
    
%     \item $\Qrobs_{\text{relaxed},\Signals}:=\{ \Qname | \forall s\in \Signals, \dsigq{s}\text{~is a distribution on $M^{\K}$} \}$.
%  %   \item $\Dist$ is a distribution on users, which is on $\real$.
% \end{enumerate}

% However, in this paper, we will study an objective function where we restrict the server to send responses in $U^k$. This is a reasonable quantity cost function to study since, we bound $\funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ by $\funfgeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ and $\funforigloc{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ by $\funfloc{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ in Theorem \ref{thm:upper-bound-relaxation}.

% \subsubsection{Objective in the restricted setup}\label{sec:objective}

% % In this section we constrain the responses of the server to $U^k$, thus assuming users and results lie on the same set $U$. The distribution over actions of the server $\dsigq{s}$ when it receives $s\in \Signals$. This distribution is supported on $U^{\K}$, denoting the distribution of the result (ad) set returned by the server given signal $s$. Towards this, we now define new objective functions for the geographic differential privacy as follows.

% In this case, we want to compute cost function $\funfgeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ (and its associated mechanism) for the case of geographic differential privacy which is defined as 

% \[  \funfgeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
% \defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsgeo{\Signals}\\ \Qname\in \Qrobs_{\Signals}}} \sup_{\Dist \in \probm{\Users}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}\left(d_U(u,a)\right) }, \]
% % and for the case of local differential privacy is defined as
% % \[  \funfloc{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}
% % \defeq \inf_{\Signals}\inf_{\substack{\Pname\in \Probsloc{\Signals}\\ \Qname\in \Qrobs_{\Signals}}} \sup_{\Dist \in \probm{\Users}} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\left(d_U(u,a)\right) }, \], 
% where $\Qrobs_{\Signals}:=\{ \Qname | \forall s\in \Signals, \dsigq{s}\text{~is a distribution on $U^{\K}$} \}$.

%\km{This theorem appears pointless. Also the transition to the next section is abrupt. What setting are we considering? Why did we define two settings and then forget about them completely? }

%\km{Where are property 1 and property 2?}

% We state a theorem upper bounding $\funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ by $\funfnewgeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$.


% \begin{theorem}{\label{thm:upper-bound-relaxation}}
%     For any $\mathfrak{h}(.)$ satisfying property \ref{item:first-propertyh}, we have $\funforiggeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)} \leq \funfnewgeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$.
% \end{theorem}

% We prove this theorem in Appendix \ref{sec:cost-boundinglemma}. For this proof, we use the property that for any user $u,u^{*} \in U$ with $m^{*} =\text{OPT}(u^{*})$, we have $\Disutility^{\mathfrak{h}(.)}(u,m^{*}) \leq \mathfrak{h}(d_U(u,u^{*}))$. 
In the rest of the paper, we shall consider the case of $U=\real$ and $d(u,v)=|u-v|$ and $\funf{U}{\Ads}{\epsilon}{\K}$ refers to  $\funfgeo{U}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ whenever it is clear from the context. %and often, $\Qrobs_{\text{unrestricted},\Signals}$ is simply referred by $\Qrobs_{\Signals}$.
\section{Main Result}
\label{sec:outline}
Our main result is a simple mechanism for the above problem that we show is {\em exactly optimal} when $U=\real$ and $d(.)$ is the $\ell_1$ norm. %and whose cost improves in $k$ as $f^{\mathfrak{h}(.)}(\real,\epsilon,k) = O\left(\frac{1}{\epsilon k}\right)$ where $\mathfrak{h}(z)=z$. This is presented in Theorem~\ref{thm:lap:sim}. 

% Before presenting the main theorem, we define a function $\hatfunfgeo{\real}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)}$ which characterises the optimal placement of $k$ points in $\real$ to minimise the expected minimum dis-utility among these $k$ points measured with respect to some user $u$ sampled from a Laplace distribution. \ak{This is inconsistent with above; why is a user being sampled from a Laplace distribution and not their set of signals? Why some user where before it was worst-case user?}
% \sss{$\hat{f}$ is just some other term defined for the purpose of our mathematical analysis and our main theorem show that $f(\mathbb{R},\epsilon,k) = \hat{f}(\mathbb{R},\epsilon,k)$}


% \begin{equation}{\label{eq:hat_f_defn}}
%     \hatfunfgeo{\real}{\Ads}{\epsilon}{\K}{\mathfrak{h}(.)} = \min_{A \in \mathbb{R}^k} \mathbb{E}_{y \sim \mathcal{L}_{\epsilon}(0)}\left[\min_{a \in \texttt{Set}(A)} \mathfrak{h} (|y -a |)\right]
% \end{equation}

The following theorem states that Laplace noise addition mechanism for an user is exactly optimal for every $\mathfrak{h}(.)$.
\ak{We said we are looking for the tuple $(Z,\dsig{u},\dsigq{s})$, so the result should be in terms of the tuple, and stated in the terms of that tuple, rather than talk about the noise addition mechanism...}
However, the optimal server response would be different for different functions $\mathfrak{h}(.)$. For $\mathfrak{h}(t)=t$, we give the  characterisation of server action in closed form. \ak{Propose change to $\mathfrak{h}(t)=t$ or some other variable as $Z$ is already taken}

\begin{restatable}[corresponds to Theorem \ref{thm:optimality-laplace-sim} and Corollary \ref{cor:geofinal}]{theorem}{simrstepe} \label{thm:lap:sim}
For $\epsilon$-geographic differential privacy \ak{where is the $d$ of the geographic?}\sss{$d(.)$ is defined to be the $\ell_1$ norm at the start of the section}, adding Laplace noise, whose density function is $\rho(x)=\frac{\epsilon}{2} \cdot e^{-\epsilon \disrzero{x}} $, is one of the optimal choices of $\Probs{\Signals}$ for users, and in this case $\funfgeo{(\ell_1,\real)}{\Ads}{\epsilon}{\K} {\mathfrak{h}(.)} = \hatfunfgeo{\real}{\Ads}{\epsilon}{\K} {\mathfrak{h}(.)}$. Further, when $\mathfrak{h}(z)=z$, we have $\funfgeo{(\ell_1,\real)}{\Ads}{\epsilon}{\K} {\mathfrak{h}(.)} = O(\frac{1}{\epsilon k})$ and the optimal mechanism (choice of actions of users and server) itself can be computed in closed form. For a generic $\mathfrak{h}(.)$, the optimal server action $\Qname$ may be computed recursively.
\end{restatable}  


%\begin{restatable} [corresponds to Lemma \ref{lem:ringbeforedetcal} and Theorem \ref{thm:localfinal}]{theorem}{simlocthm} \label{thm:main2:sim}
%For local differential privacy, it is sufficient to only consider symmetric mechanisms. Adding a noise with $\K$ equidistant peaks is one of the optimal mechanisms, and in this case, $\funf{\Users}{\Ads}{\epsilon}{\K}$ is $O(1/\K)$. Furthermore, the optimal mechanism can be computed in closed form.
%\end{restatable}

%\subsection{Proof sketch of Theorem \ref{thm:lap:sim}}
 %Note that the proof sketch for local differential privacy is similar and will be provided later.

%\todo{State the two theorems here!}


%\todo{Sketch of which proof?}
%Recall that we are interested in
%\[  \funf{\Users}{\Ads}{\epsilon}{\K} \defeq  \inf_{\Signals}\inf_{\Pname\in \Probs{\Signals},\Qname\in \Qrobs_{\Signals}} \sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\disg{u}{a} }. \]

We provide a comprehensive overview of the proof for Theorem~\ref{thm:lap:sim} in Section \ref{sec:simproof}. %The proof involves intricate technical details and we give an outline in Section \ref{sec:proof-outline}. 

%We first show that the signal set $Z$ can be the $k$-result set $\mathbb{R}^k$ in Section \ref{subsec:proof-step1}. We next formulate an infinite-dimensional infimization linear program denoted as $\mathcal{O}$ and construct an infinite-dimensional supremization linear program denoted as $\mathcal{E}$ in Section \ref{subsec:proof-step2}. Our proof methodology shares similarities with the approach presented in \cite{koufogiannis2015optimality}, but our linear program is notably more intricate and complex due to the involvement of minimization over a set of returned results in the cost function. 

% In our problem, we formally establish the weak duality framework between programs $\mathcal{O}$ and $\mathcal{E}$. This proof is imperative since the existing duality framework exists for infinite dimensional linear programs for cases only involving integrals but not for scenarios involving both of them. This proof is further complicated by the fact that we have linear constraints on upper and lower derivatives, since not every probability distribution is differentiable. Since the weak duality proof involves some exchange of limits and integrals, we require a meticulous application of Fatou's lemma and the monotone convergence theorem to prove weak duality.

% Finally, we show the optimality of the Laplace noise addition mechanism by dual -fitting i.e. constructing a feasible solution to DILP $\mathcal{E}$ with an objective identical to that of the Laplace noise addition mechanism in Section \ref{subsec:proof-step3}. Finally for the case of $\mathfrak{h}(z)=z$, we show how to compute the server response in a closed form in Section \ref{subsec:proof-step4}.


%Given the heightened complexity of our objective function compared to that in \cite{koufogiannis2015optimality}, it becomes imperative to formally establish the weak duality theorem within our framework for the infinite-dimensional linear programs $\mathcal{O}$ and $\mathcal{E}$. Note that this proof is important since, the existing duality framework exists for infinite dimensional linear programs for cases only involving integrals but not for scenarios involving both of them. This proof is challenging as we refrain from assuming differentiability of the probability distribution. Consequently, the infinite-dimensional linear programs encompass lower and upper derivatives, necessitating a nuanced proof of weak duality. Our approach involves leveraging lower integrals and a meticulous application of Fatou's lemma and the monotone convergence theorem to facilitate the interchange of limits and integrals. Finally, we conclude the proof by using dual fitting to establish optimality of the Laplace noise addition mechanism by finding a feasible solution to infinite dimensional linear program $\mathcal{E}$.


% A detailed proof sketch of Theorem~\ref{thm:lap:sim} is presented in Section \ref{sec:simproof}. The proof is technical and we formulate an infinite dimensional infimization LP $\mathcal{O}$ and we also construct a infinite dimensional supremization LP $\mathcal{E}$. This proof technique is closest to the one in \cite{koufogiannis2015optimality}, however our linear program is quite more involved and complex since the cost function involves minimisation over a set of results returned. Since, our objective function is much more complex to that in \cite{koufogiannis2015optimality}, we need to formally show the weak duality theorem in our setup on infinite dimensional LPs $\mathcal{O}$ and $\mathcal{E}$ which is quite involved. Since, we do not make any assumptions on the differentiability of the probability distribution, the infinite dimensional LPs involve lower and upper derivatives, making the proof of weak duality quite involved leading us to use lower integrals and a careful use of Fatou's lemma and monotone convergence theorem to exchange limits and integrals.

% The entire proof has many technical details and is deferred to the Appendix. We now provide an outline of this proof. The proof contains four main steps. At each step, we narrow the region of feasible mechanisms while retaining at least one optimal mechanism in it.

% In this section and the subsequent sections discussing geographic privacy, we refer $\funfgeo{\real}{\Ads}{\epsilon}{\K} {\mathfrak{h}(.)}$ by $\funf{\real}{\Ads}{\epsilon}{\K}$, $\Probsgeo{\Signals}$ by $\Probs{\Signals}$ and $\hatfunfgeo{\real}{\Ads}{\epsilon}{\K} {\mathfrak{h}(.)}$ by $\hatfunf{\real}{\Ads}{\epsilon}{\K}$, whenever it is clear from context that we are referring to $\epsilon$-geographic differential privacy. We now discuss the four main steps in our proof.
%\begin{itemize}

\km{Again, I think having two outlines is an overkill. Sections 4 and 5 should be merged.} 

\sss{Are you talking of section 4 and 5 or section 3 and 4.}

\km{I'm talking about 4 and 5. The outline in 4 seems redundant and its content should be merged with 5, with a short summary at the beginning of the section.}



==> simplelocal.tex <==
\section{The Model for Multi-Selection in Local Differential Privacy Model}  \label{sec:simlocal}
%\ak{Similarly, would change title of the section to: The Model for Multi-Selection in Local Differential Privacy Model}


%\paragraph{$\epsilon$-local differential privacy:}

We start with some notation. Recall that given a set $S$, we use $K(\cdot)$ to denote a distribution on $S$, so that $K(H)$ is the probability mass of $H\subset S$. For distributions $K$ and $K'$ on $S$, we define their distance to be $\ddis{K}{K'} \defeq \sup_{H\subset S} \frac{K(H)}{K'(H)}$. For a $\K$-dimensional vector $(a_1,\dots,a_{\K})\in \sphere^{\K}$, we also regard it as a set of size $\K$ to be convenient. When we say $a\in (a_1,\dots,a_{\K})$, it means $a\in \{a_1,\dots,a_{\K}\}$. 

As before, user $u$ draws a signal from distribution $\Pname_u$ and then sends it to the server. To satisfy $\epsilon$-local differential privacy, for any two users $u_1,u_2$, it should hold that $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon}$. (In geographic setting, it is $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon\cdot d(u_1,u_2)}$.)

\paragraph{Multi-selection model on a ring.} We assume users and results are located on a unit ring $\sphere \defeq \{x\in \real^{2}: \diszero{x}=1\}$. The distribution of users is $\Dist$, which is supported on $\sphere$. A user sends a signal to the server, and the server returns a set of $\K$ results. Then the user chooses the closest among those $\K$ results. Using the above notation, the server responds with a vector in $\sphere^{\K}$.

Our goal is to determine a  mechansim characterized by:
\begin{enumerate}
\item A set of signals $\Signals$.% and a distribution $\Dist$ of users over $\real$.
\item The action of users, which is a distribution over signals. We use $\dsig{u}$ for $u\in \sphere$ to denote the distribution of the signals sent by user $u$. This distribution is supported on $\Signals$.
\item The action of the server, $\dsigq{s}$ when it receives $s\in \Signals$. This is distribution of the result set returned by the server given $s$ and is supported on $\sphere^{\K}$. 
\end{enumerate}

The mechanism should be feasible, that is it should satisfy $\epsilon$-local differential privacy: for any $u_1,u_2\in \sphere$, it should hold that $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon}$.

\paragraph{Objective.} Given a fixed number $k$ for result set size, our goal is to maximize utility while ensuring the specified level of privacy. This translates to minimizing the expected distance between the user and the closest ad that the user receives in the worst case with respect to the distribution of users. That is, we want to compute $\funf{\Users}{\Ads}{\epsilon}{\K}$ (and its associated mechanism), which is defined as
\[  \funf{\Users}{\Ads}{\epsilon}{\K}
\defeq \inf_{\Signals}\inf_{\Pname\in \Probs{\Signals},\Qname\in \Qrobs_{\Signals}} \sup_{\Dist} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\arccos(u_1\cdot u_2)  }, \]
where
\begin{enumerate}
%    \item For $A=(a_1,a_2,\dots,a_{\K})\in \real^{\K}$, we say $a\in A$ if $a\in \{a_1,\dots,a_{\K}\}$.
    \item $\Probs{\Signals}:=\{ \Pname | \forall u\in \sphere, \dsig{u}\text{~is a distribution on $\Signals$,} 
    \text{~and $\epsilon$-local differential privacy is satisfied} \}$.
    \item $\Qrobs_{\Signals}:=\{ \Qname | \forall s\in \Signals, \dsigq{s}\text{~is a distribution on $\sphere^{\K}$} \}$.
    \item $\arccos(u_1\cdot u_2)$ is the angle difference between $u_1$ and $u_2$, which defines the distance.
 %   \item $\Dist$ is a distribution on users, which is on $\real$.
\end{enumerate}






\iffalse %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Besides the geographic differential privacy setting, we also consider local differential privacy.  In this setting, the users and Ads locate on a unit ring $\sphere \defeq \{x\in \real^{2}: \diszero{x}=1\}$. The distribution of users is $\Dist$, which is on $\sphere$. The distance between two points in $\sphere$ is their angle difference $d(u_1,u_2)\defeq \arccos(u_1\cdot u_2)$.

We still determine
\begin{enumerate}
\item A set of signals $\Signals$.
\item Action of users, $\dsig{u}$ for $u\in \sphere$, which is a distribution on $\sphere$, denoting the distribution of the signal sent by $u$. 
\item Action of server, $\dsigq{s}$ for $s\in \Signals$, which is a distribution on $\sphere^{\K}$, denoting the distribution of the ads set sent back by the server, when the received signal is $s$. 
\end{enumerate}

The system should have differential privacy. For any $u_1,u_2\in \real$, it should hold that $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon}$. (Recall that this was $e^{\epsilon\cdot |u_1-u_2|}$ in geographic differential privacy setting.)

We want to compute $\funf{\Users}{\Ads}{\epsilon}{\K}$ which is defined as
\[    \inf_{\Signals}\inf_{\Pname\in \Probs{\Signals},\Qname\in \Qrobs_{\Signals}} \sup_{\Dist} \Exx{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\arccos(u_1\cdot u_2) }. \]

\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\paragraph{Our results.} As before, we show that the optimal mechanism is {\em symmetric}, defined as:

\begin{definition}[symmetric mechanism in local differential privacy setting]
For $\Pname\in \Probs{\sphere^{\K}}$, if for any $u\in \Users, \C\subset \sphere^{\K}$, for any rotation matrix $M\in \real^{2\times 2}$,
\begin{align*}
    \Pxx{u}{\C}=\Pxx{uM}{\C M},
\end{align*}
then we say $\Pname$ is a symmetric mechanism.
%Let $\Psym$ be the set of symmetric mechanisms.
\end{definition}

Following a similar argument as in the geographic differential privacy setting, we will show the following theorem, whose proof is presented in in Appendix \ref{sec:localfull}.

\begin{restatable} [corresponds to Lemma \ref{lem:ringbeforedetcal} and Theorem \ref{thm:localfinal}]{theorem}{simlocthm} \label{thm:main2:sim}
For local differential privacy, it is sufficient to only consider symmetric mechanisms. Adding noise whose distribution has $\K$ equidistant modes is one of the optimal mechanisms, and in this case, $\funf{\Users}{\Ads}{\epsilon}{\K}$ is $O(1/\K)$. Furthermore, the optimal mechanism can be computed in closed form.
\end{restatable}


%The proof of this theorem is presented in Appendix \ref{sec:localfull}.


==> simplemodel.tex <==
\section{The Model for Multi-Selection in Geographic Differential Privacy}  \label{sec:simmodel}
\label{sec:subsecsimmodel}

%\ak{I'd re-order this -- first introduce the e-geographic DP formally, then introduce our new system architecture formally, then state the minimization desiderata. Also change title of the section to: The Model for Multi-Selection in Geographic Differential Privacy }
%\subsection{Model}  

%\paragraph{$\epsilon$-geographic differential privacy: }
We start with some notation. Given a set $S$, if we use $K(\cdot)$ to denote a distribution on $S$, then $K(H)$ is the probability mass of $H\subset S$. For distributions $K$ and $K'$ on $S$, we define their distance to be $\ddis{K}{K'} \defeq \sup_{H\subset S} \frac{K(H)}{K'(H)}$. For two real numbers $x,x'\in \real$, we define their distance to be the Euclidean distance $|x-x'|$. Finally, for a $\K$-dimensional vector $(a_1,\dots,a_{\K})\in \real^{\K}$, we also regard it as a set of size $\K$ to be convenient. When we say $a\in (a_1,\dots,a_{\K})$, it means $a\in \{a_1,\dots,a_{\K}\}$.

In the {\em geographic DP} model, there is a set of users User $u$ draws a signal from distribution $\Pname_u$ and then sends it to the server. To satisfy $\epsilon$-geographic differential privacy, for any two users $u_1,u_2$, it should hold that $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon\cdot d(u_1,u_2)}$, where $d(u_1,u_2)$ is a certain distance between $u_1$ and $u_2$.


\paragraph{Multi-Selection model on a line.} We assume users and results are located on a line, and the location is denoted by a real number. The distribution of users is $\Dist$, which is supported on $\real$. A user sends a signal to the server, and the server returns a set of $\K$ results, each of which maps to a point on the real line. Then the user chooses the closest among those $\K$ results to its own location. Using the notation defined above, we assume the server responds with a vector in $\real^{\K}$. The goal is to determine a mechanism that has the following ingredients:

\begin{enumerate}
\item A set of signals $\Signals$.% and a distribution $\Dist$ of users over $\real$.
\item The action of users, which involves choosing a signal from a distribution over signals. We use $\dsig{u}$ for $u\in \real$ to denote the distribution of the signals sent by user $u$. This distribution is supported on $\Signals$.
% \item The distribution over actions of the server, $\dsigq{s}$ when it receives $s\in \Signals$. This distribution is supported on $\real^{\K}$, denoting the distribution of the result (ad) set returned by the server given signal $s$. 

\item The distribution over actions of the server, $\dsigq{s}$ when it receives $\s\in \Signals$
\end{enumerate}

In any {\em feasible mechanism}, the  user behavior should satisfy $\epsilon$-geographic differential privacy: for any $u_1,u_2\in \real$, it should hold that $\ddis{\dsig{u_1}}{\dsig{u_2}}\leq e^{\epsilon\cdot |u_1-u_2|}$.

\paragraph{Objective.} For any fixed response size $k$, in order to maximize utility while ensuring the specified level of privacy, the goal is to minimize the expected distance between the user's location and the location of the closest ad that the user receive. This minimization is in the worst case with respect to the distribution of users. That is, we want to compute cost function $\funf{\Users}{\Ads}{\epsilon}{\K}$ (and its associated mechanism) which is defined as
\[  \funf{\Users}{\Ads}{\epsilon}{\K}
\defeq \inf_{\Signals}\inf_{\Pname\in \Probs{\Signals},\Qname\in \Qrobs_{\Signals}} \sup_{\Dist} \Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}|u-a| }, \]
where
\begin{enumerate}
%    \item For $A=(a_1,a_2,\dots,a_{\K})\in \real^{\K}$, we say $a\in A$ if $a\in \{a_1,\dots,a_{\K}\}$.
    \item $\Probs{\Signals}:=\{ \Pname | \forall u\in \real, \dsig{u}\text{~is a distribution on $\Signals$,} 
    \text{~and $\epsilon$-geographic differential privacy is satisfied} \}$.
    \item $\Qrobs_{\Signals}:=\{ \Qname | \forall s\in \Signals, \dsigq{s}\text{~is a distribution on $\real^{\K}$} \}$.
 %   \item $\Dist$ is a distribution on users, which is on $\real$.
\end{enumerate}



\section{Main Result and Proof Outline}
\label{sec:outline}
Our main result is a simple mechanism for the above problem that we show is {\em exactly optimal}, and whose cost improves in $k$ as $f(\epsilon,k) = O\left(\frac{1}{\epsilon k}\right)$. This is presented in Theorem~\ref{thm:lap:sim}.
%The form one has more complicated proof, but the key ideas of those two models are similar.

\begin{restatable}[corresponds to Lemma \ref{lem:computefal} and Corollary \ref{cor:geofinal}]{theorem}{simrstepe} \label{thm:lap:sim}
For geographic differential privacy, it is sufficient to only consider symmetric mechanisms. Adding Laplace noise, whose density function is $\rho(x)=\frac{1}{2\epsilon} \cdot e^{-\epsilon \disrzero{x}} $, is one of the optimal choices of $\Probs{\Signals}$ for users, and in this case $\funf{\Users}{\Ads}{\epsilon}{\K}$ is $O(1/(\epsilon \K))$. Further, the optimal mechanism (choice of actions of users and server) itself can be computed in closed form.
\end{restatable}  


%\begin{restatable} [corresponds to Lemma \ref{lem:ringbeforedetcal} and Theorem \ref{thm:localfinal}]{theorem}{simlocthm} \label{thm:main2:sim}
%For local differential privacy, it is sufficient to only consider symmetric mechanisms. Adding a noise with $\K$ equidistant peaks is one of the optimal mechanisms, and in this case, $\funf{\Users}{\Ads}{\epsilon}{\K}$ is $O(1/\K)$. Furthermore, the optimal mechanism can be computed in closed form.
%\end{restatable}

%\subsection{Proof sketch of Theorem \ref{thm:lap:sim}}
 %Note that the proof sketch for local differential privacy is similar and will be provided later.

%\todo{State the two theorems here!}


%\todo{Sketch of which proof?}
%Recall that we are interested in
%\[  \funf{\Users}{\Ads}{\epsilon}{\K} \defeq  \inf_{\Signals}\inf_{\Pname\in \Probs{\Signals},\Qname\in \Qrobs_{\Signals}} \sup_{\Dist\in \probm{\Users}} \Exx{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}\disg{u}{a} }. \]



A detailed proof sketch of Theorem~\ref{thm:lap:sim} is presented in Section \ref{sec:simproof}. The entire proof has many technical details and is deferred to the Appendix. We now provide an outline of this proof. The proof contains four main steps. At each step, we narrow the region of feasible mechanisms while retaining at least one optimal mechanism in it.
%\begin{itemize}


\paragraph{Step 1. The signal set $\Signals$ can be the $k$-result set $\Kads$.} Given the behavior of the server, users can themselves compute the distribution of the result set that they will receive. Therefore a user can draw a result set directly from the distribution over the server's action and send the set as the signal. The server returns the received signal, hence removing it from the picture. In other words, it is sufficient to consider mechanisms in $\Probs{\Kads}$, which are in the following form (corresponding to Theorem \ref{thm:singpoint:sim}).

\begin{enumerate}
    \item User located at $v\in \real$ reports $s$ that is drawn from a distribution $\Pname_{v}$ over $\real^{\K}$.
    \item The server receives $s$ and returns $s$.
\end{enumerate}

We remark that this mechanism is only used for the purpose of analysis. The final mechanism will not remove the server and will actually split the computation between the user and the server. 

%%%%%

%In this case, the signal set $\Signals$ is $\Kads$, and we do not need to decide the behavior of the server. We will prove
    

%\begin{restatable}{theorem}{simrstepa}\label{thm:singpoint:sim}
%\begin{align*}
%\funf{\Users}{\Ads}{\epsilon}{\K} = \inf_{\Pname\in \Probs{\real^{\K}}} \sup_{\Dist} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}|u-a| }.
%\end{align*}
%\end{restatable}
    
    
\paragraph{Step 2. Optimality of symmetric mechanisms.} The next step shows it is sufficient to only care about symmetric mechanisms. Symmetric is defined as following (corresponding to Theorem \ref{thm:symopt:sim}).
\begin{enumerate}
    \item User located at $v\in \real$ reports $s=(a_1+v,\dots,a_{\K}+v)$, where $(a_1,\dots,a_{\K})$ is drawn from a distribution $\Pname$ over $\real^{\K}$ that is independent to $v$.
    \item The server receives $s$ and returns $s$.
\end{enumerate}

For an arbitrary mechanism in $\Probs{\Kads}$, we construct a symmetric mechanism by averaging the strategies of different users, and the error of the new mechanism is at most as large as that of the original mechanism.

%%%%%

%We will prove

%\zhihao{symmetric not defined}

\iffalse %%%%%

\begin{restatable}{theorem}{simrstepb} \label{thm:symopt:sim}
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname_{ave}\in \Psym}  \Exx{A\sim \Pname_{ave}}{ \min_{a\in A}|a| },
\end{align*}
where $\Psym$ is the set of symmetric mechanisms that are $\epsilon$-geographicly DP.
\end{restatable}

\fi %%%%%
    
    
\paragraph{Step 3. Concentrating probability mass on a line.} In the symmetric mechanism constructed above, $\Pname$ is a distribution on $\real^{\K}$. We can divide $\real^{\K}$ into equivalence classes, so that the differential privacy only constrains the probability densities of elements inside the same equivalence class. We will show it is optimal to concentrate all probability mass in one equivalence class. In other words, it is sufficient to consider the following type of mechanisms (corresponding to Theorem \ref{thm:symfinal:sim}).

\begin{enumerate}
    \item User located at $v\in \real$ reports $s=v+x$, where $x$ is drawn from a distribution $\Sname$ over $\real$ that is independent to $v$.
    \item The server receives $s$ and responds $(s+a_1,\dots,s+a_{\K})$, where $A=(a_1,\dots,a_{\K})$ is a fixed vector in $\real^{\K}$ independent of the signal.
\end{enumerate}



%%%%%

\iffalse %%%%%
\begin{restatable}{theorem}{simrstepc} \label{thm:symfinal:sim}
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{A\in \real^{\K}} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} },
\end{align*}
where
\begin{align*}
\Srobs = \{ \Sname | \Sname \text{~is a distribution on $\real$};&\\
 \text{~and~} \forall x,y\in \real, \rho_{\Sname}(x)\leq& e^{\epsilon \dis{x}{y}}\rho_{\Sname}(y) \} .
\end{align*}
\end{restatable}
    
\fi %%%%%
    
    
\paragraph{Step 4. Structure of optimal mechanism.} Given $A$ and $\Sname$, we simplify $A$ and $\Sname$ step by step so that a suitably defined potential function decreases at each step. The potential function has discrete value, and the process stops after finite number of steps, when $\Sname$ becomes Laplace distribution. It is therefore sufficient to consider the following type of mechanisms (corresponding to Theorem~\ref{thm:lap:sim}).

\begin{enumerate}
    \item User located at $v\in \real$ reports $s=v+x$, where $x$ is drawn from Laplace distribution with density $\rho(x)=\frac{1}{2\epsilon} \cdot e^{-\epsilon \disrzero{x}} $.
    \item The server receives $s$ and respond $(s+a_1,\dots,s+a_{\K})$, where $a_1,\dots,a_{\K}$ are fixed real values.
\end{enumerate}

At this point, the optimal mechanism is simple enough that the values $a_1, a_2, \ldots, a_k$ can be computed by dynamic programming, as we show in Section~\ref{sec:simres}, and this concludes the proof of Theorem~\ref{thm:lap:sim}.


%%%%%

%We will prove


%\begin{restatable}{theorem}{simrstepe} \label{thm:lap:sim}
%For geographic differential privacy, it is sufficient to only consider symmetric mechanisms. Adding Laplace noise, whose density function is $\rho(x)=\frac{1}{2\epsilon} \cdot e^{-\epsilon \disrzero{u}{x}} $, is one of the optimal choices for users, and in this case $\funf{\Users}{\Ads}{\epsilon}{\K}$ is $O(1/(\epsilon \K))$. Further, the optimal mechanism itself can be computed in closed form.
%\end{restatable}    
    
    
%\end{itemize}







==> simpleproof-modified-dual-fitting.tex <==
\subsection{Dual fitting to show the optimality of Laplace noise addition}\label{sec:dual-soln-construction}
%In this section, we construct a feasible solution to DILP $\mathcal{E}$ whose objective is arbitrarily close to $\hat{f}(\mathbb{R},\epsilon,k)$. To do this, we first construct feasible solutions $\delta^{(c)}(u)$ and $\lambda^{(c)}(.)$ which we define for some $\hat{\lambda}>0$ and $0<\zeta<\epsilon$.

In this section, we first define a mechanism in Definition \ref{def:laplace_noise_addition} which simulates the action of the server corresponding to the Laplace noise addition mechanism in Section \ref{subsec:sim_laplace_noise} and show that the cost of Laplace noise addition mechanism is $\hat{f}(\mathbb{R},\epsilon,k)$. We finally show the optimality of Laplace noise addition mechanism via dual fitting i.e. constructing a feasible solution to the dual DILP $\mathcal{E}$ with an objective function $\hat{f}(\mathbb{R},\epsilon,k)$ in Section \ref{subsec:feasible_soln}.

% Finally we prove Lemma \ref{lemma:dual_schievable} showing that the optimum value of DILP $\mathcal{E}$ is lower bounded by $\hat{f}(\mathbb{R},\epsilon,k)$. 

%
% We define functions $\lambda^{(c)}(.)$ and $\delta^{(c)}(.)$ for some $\hat{\lambda}>0$ and $0<\zeta<\epsilon$.

\subsubsection{Bounding cost function $f(\mathbb{R},\epsilon,k)$ by the cost of Laplace noise adding mechanism}{\label{subsec:sim_laplace_noise}}

\begin{definition}{\label{def:laplace_noise_addition}}
The mechanism associated with $\hat{P}^{\mathcal{L}_{\epsilon}}_u$ corresponds to simulating the action of the server on receiving signal $S_u\sim \mathcal{L}_{\epsilon}(u)$ from user $u$.
    \begin{align}{\label{hat_P_defn}}
    \hat{A} \sim \hat{P}^{\mathcal{L}_{\epsilon}}_u  \iff \hat{A} = & \argmin_{A \in \mathbb{R}^k} \mathbb{E}_{y \sim \mathcal{L}_{\epsilon}(S_u)}\left[\min_{a \in \texttt{Set}(A)} \mathfrak{h} (||y -a ||_1)\right] \text{\footnotemark where } S_u \sim \mathcal{L}_{\epsilon}(u)\\
    \overset{(a)}{=} & \argmin_{A \in \mathbb{R}^k} \mathbb{E}_{y \sim \mathcal{L}_{\epsilon}(0)}\left[\min_{a \in \texttt{Set}(A)} \mathfrak{h} (||y -a ||_1)\right] + S_u \text{\footnotemark where } S_u \sim \mathcal{L}_{\epsilon}(u)
\end{align}
\footnotetext{Observe that we choose a deterministic tie-breaking rule amongst all vectors minimising this objective.} 

The server responds with set of points $\texttt{Set}(\vect{A})$ for some $\vect{A} \in \mathbb{R}^k$ so as to minimise the expected cost with respect to some user sampled from a Laplace distribution centred at $S_u$. Equality $(a)$ follows from the fact that $y \sim \mathcal{L}_{\epsilon}(z) \implies y-z\sim \mathcal{L}_{\epsilon}(0)$ for every $z \in \mathbb{R}$.
\end{definition}


%\km{Make each thing you show a subsection? "Now" $-->$ "First"?}

We show that the following lemma which states that $\hat{P}^{\mathcal{L}_{\epsilon}}$ satisfies $\epsilon$-geographic differential privacy constraints and bound $f(\mathbb{R},\epsilon,k)$ by $\hat{f}(\mathbb{R},\epsilon,k)$.

\begin{restatable} 
[detailed proof in Appendix \ref{sec-appendix:primal-feasible}] {lemma}{simrstepa}\label{lemma:bounding_f}
    $\hat{P}^{\mathcal{L}_{\epsilon}}$  satisfies $\epsilon$-geographic differential-privacy constraints i.e. $\hat{P}^{\mathcal{L}_{\epsilon}} \in \mathcal{P}^{(\epsilon)}_{\mathbb{R}^k}$ and thus, we have $f(\mathbb{R},\epsilon,k) \leq \textit{cost}(\hat{{P}}^{\mathcal{L}_{\epsilon}}) = \hat{f}(\mathbb{R},\epsilon,k)$
     
     % $$f(\mathbb{R},\epsilon,k) \leq \sup_{u \in \mathbb{R}} \underset{A \sim \hat{P}^{\mathcal{L}_{\epsilon}}_u}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h}(||u-a||_1) \right] = \hat{f}(\mathbb{R},\epsilon,k)$$.
\end{restatable}


% \begin{lemma}{\label{lemma:bounding_f}}
%     $\hat{P}^{\mathcal{L}_{\epsilon}}$  satisfies $\epsilon$-geographic differential-privacy constraints i.e. $\hat{P}^{\mathcal{L}_{\epsilon}} \in \mathcal{P}^{(\epsilon)}_{\mathbb{R}^k}$ and thus, we have 
     
%      $$f(\mathbb{R},\epsilon,k) \leq \sup_{u \in \mathbb{R}} \underset{A \sim \hat{P}^{\mathcal{L}_{\epsilon}}_u}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h}(||u-a||_1) \right] = \hat{f}(\mathbb{R},\epsilon,k)$$.
% \end{lemma}


\begin{proof}[Proof Sketch]

     Observe that $\hat{P}^{\mathcal{L}_{\epsilon}} \in \mathcal{P}^{(\epsilon)}_{\mathbb{R}^k}$ from the post processing theorem, refer to \cite{diff-privacy-book} since $S_u \sim \mathcal{L}_{\epsilon}(u)$ satisfies $\epsilon$-geographic differential privacy constraints.\footnote{Post processing theorem can be proven even for $\epsilon$-geographic differential privacy similarly}. Thus, we prove $f(\mathbb{R},\epsilon,k) \leq \text{cost}(\hat{{P}}^{\mathcal{L}_{\epsilon}})$. The equality is fully proven in Appendix \ref{sec-appendix:primal-feasible}.
    
    %and observe that $\min_{A \in \mathbb{R}^k} \mathbb{E}_{y \sim \mathcal{L}_{\epsilon}(S_u)} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h} (||y -a ||_1)\right]$ is independent of $S_u$ and thus, we have 


    
    % \begin{align*}
    %     f(\mathbb{R},\epsilon,k) & \overset{(a)}{\leq} \sup_{u \in \mathbb{R}} \underset{A \sim \hat{P}^{\mathcal{L}_{\epsilon}}_u}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h}(||u-a||_1) \right] \\
    %     & \overset{(b)}{=} \sup_{u \in \mathbb{R}} \underset{S_u \sim \mathcal{L}_{\epsilon}(u)}{\mathbb{E}} \left(\left[\min_{a \in \texttt{Set}(\hat{A})} \mathfrak{h}(||u-a||_1) \right]\Biggl\vert_{\hat{A}=\argmin\limits_{A \in \mathbb{R}^k} \mathbb{E}_{y \sim \mathcal{L}_{\epsilon}(0)}\left[\min\limits_{a \in \texttt{Set}(A)} \mathfrak{h} (||y -a ||_1)\right] + S_u}\right)\\
    %     % & = \sup_{u \in \mathbb{R}} \underset{S_u \sim \mathcal{L}_{\epsilon}(u)}{\mathbb{E}} \left(\left[\min_{a \in \texttt{Set}(\hat{A}+S_u)} \mathfrak{h}(||u-a||_1) \right]\Biggl\vert_{\hat{A}=\argmin\limits_{A \in \mathbb{R}^k} \mathbb{E}_{y \sim \mathcal{L}_{\epsilon}(0)}\left[\min\limits_{a \in \texttt{Set}(A)} \mathfrak{h} (||y -a ||_1)\right] }\right)\\
    %     & \overset{(c)}{=} \sup_{u \in \mathbb{R}} \underset{S_u \sim \mathcal{L}_{\epsilon}(u)}{\mathbb{E}} \left(\left[\min_{a \in \texttt{Set}(\hat{B})} \mathfrak{h}(||(u-S_u)-a||_1) \right]\Biggl\vert_{\hat{B}=\argmin\limits_{A \in \mathbb{R}^k} \mathbb{E}_{y \sim \mathcal{L}_{\epsilon}(0)}\left[\min\limits_{a \in \texttt{Set}(A)} \mathfrak{h} (||y -a ||_1)\right] }\right)\\
    %     & \overset{(d)}{=} \sup_{u \in \mathbb{R}} \underset{y \sim \mathcal{L}_{\epsilon}(0)}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(\hat{B})} \mathfrak{h}(||y-a||_1) \right]\Biggl\vert_{\hat{B}=\argmin\limits_{A \in \mathbb{R}^k} \mathbb{E}_{y \sim \mathcal{L}_{\epsilon}(0)}\left[\min\limits_{a \in \texttt{Set}(A)} \mathfrak{h} (||y-a||_1)\right] }\\
    %     & \overset{(e)}{=}  \min_{A \in \mathbb{R}^k} \mathbb{E}_{y \sim \mathcal{L}_{\epsilon}(0)} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h} (||y-a||_1)\right] = \hat{f}(\mathbb{R},\epsilon,k)
    % \end{align*}

%\km{"check" $-->$ "refer to"?}

% $(a)$ follows from the fact that $\hat{P}^{\mathcal{L}_{\epsilon}} \in \mathcal{P}^{(\epsilon)}_{\mathbb{R}^k}$ from the post processing theorem, refer to \cite{diff-privacy-book} since $S_u \sim \mathcal{L}_{\epsilon}(u)$ satisfies $\epsilon$-geographic differential privacy constraints.\footnote{Post processing theorem can be proven even for $\epsilon$-geographic differential privacy similarly}. 
% $(b)$ follows from the definition in Equation \eqref{eq:hat_f_defn} and $(c)$ follows on substituting $\hat{B} = \hat{A}-S_u$ and $(d)$ follows on substituting $u-S_u$ by $y$ and the fact that $\hat{B}$ is independent of $S_u$ and $(e)$ follows since $\hat{B}$ is minimised over the same objective function and independent of $u$.

%$(a)$ follows from Claim \ref{lemma:lp_formulation} and $(b)$ follows from the definition in Equation \eqref{hat_P_defn}.    
\end{proof}


\subsubsection{Obtaining a feasible solution to DILP $\mathcal{E}$}{\label{subsec:feasible_soln}}

We now construct feasible solutions to DILP $\mathcal{E}$. With this, we now define  

\begin{equation}{\label{eqn:nu_delta_defn}}
    \delta^{(c)}(r) = (\zeta/2) e^{-\zeta|r|} \text{ and } \lambda^{(c)}(r) = \hat{\lambda}\cdot (\zeta/2) e^{-\zeta|r|} \text{ } \forall r \in \mathbb{R}
\end{equation}

% Note that we construct these functions to find a feasible solution to DILP $\mathcal{E}$ with as ``large objective'' ($\hat{\lambda}$) as possible since $\int_{r \in \mathbb{R}} \lambda^{(c)}(r) dr = \hat{\lambda}$. 

Now define $v_{med} = \text{Median}(\texttt{Set}(\vect{v}))$ and for every $\vect{v} \in \mathbbm{R}^k$, we consider the following Differential Equation \eqref{eqn:diff_eqn_nu} in $\hat{\nu}(.)$. %with $\lambda^{(c)}(.)$ and $\delta^{(c)}(.)$ defined in Equation \eqref{eqn:nu_delta_defn}  and define $v_{med} = \text{Median}(\texttt{Set}(\vect{v}))$. 

\begin{equation}{\label{eqn:diff_eqn_nu}}
    -\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|r-a|)\right] \delta^{(c)}(r) + \lambda^{(c)}(r) + \hat{\nu}'(r) + \epsilon |\hat{\nu}(r)| = 0 ; \text{ with  $\hat{\nu}(v_{med}) = 0$}  
\end{equation}


Observe that this equation precisely corresponds to the second constraint of DILP $\mathcal{E}$ (inequality replaced by equality) with an initial value. We now show that a solution $\hat{\nu}(.)$ to \eqref{eqn:diff_eqn_nu} exists such that $\hat{\nu}(r)$ is non-negative for sufficiently large $u$ and non-positive for sufficiently small $r$ to satisfy the last two constraints of DILP $\mathcal{E}$ in Lemma \ref{lemma:diff_eqn_soln}.


The high level idea of this proof is similar to the solution in  \cite[Equation 19]{koufogiannis2015optimality}. However, our differential equation has more complexity since we are minimising over a set of points $\vect{v} \in \mathbb{R}^k$ and also our equation has to be solved for every $\vect{v} \in \mathbb{R}^k$ making it more complex.  

\km{No need to say "detailed proof"; just say "Proved in". }
\km{Can we please not use "Claim" and use "Lemma" instead everywhere? It puts Lemma in a different font, which makes reading difficult.}

\begin{restatable} 
[detailed proof in Appendix \ref{subsec-appendix:diff_eqn_soln}] {lemma}{simrstepa}\label{lemma:diff_eqn_soln}
     Choose $\zeta<\epsilon$ and $0< \hat{\lambda} \leq \frac{\epsilon - \zeta}{\epsilon+\zeta} \hat{f}(\mathbb{R},\epsilon+ \zeta,k)$, then equation $\eqref{eqn:diff_eqn_nu}$ has a unique $\mathcal{C}^1$ solution $\nu^{(c)}(.)$ and there exists $U, L \in \mathbb{R}$ satisfying $\nu^{(c)}(r) \geq 0 \text{ }\forall r \geq U$ and $\nu^{(c)}(r) \leq 0 \text{ } \forall r \leq L$.
     
     % $$f(\mathbb{R},\epsilon,k) \leq \sup_{u \in \mathbb{R}} \underset{A \sim \hat{P}^{\mathcal{L}_{\epsilon}}_u}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h}(||u-a||_1) \right] = \hat{f}(\mathbb{R},\epsilon,k)$$.
\end{restatable}

\begin{proof}[Intuitive explanation]
    We just give an intuition for this proof for the case where $\hat{\lambda}$ exceeds $\frac{\epsilon-\zeta}{\epsilon+\zeta} \hat{f}(\mathbb{R},\epsilon,k)$ by showing two plots in Figure \ref{fig:plotlambda40} and \ref{fig:plotlambda46} for the two cases where $\hat{\lambda} < \frac{\epsilon-\zeta}{\epsilon+\zeta} \hat{f}(\mathbb{R},\epsilon,k)$ and $\hat{\lambda} > \frac{\epsilon-\zeta}{\epsilon+\zeta} \hat{f}(\mathbb{R},\epsilon,k)$ respectively. In the first case, $\nu^{(c)}(r)$ is positive for sufficiently large $r$ and in second case goes negative demonstrating the requirement of the bound $\frac{\epsilon-\zeta}{\epsilon+\zeta} \hat{f}(\mathbb{R},\epsilon,k)$ on $\hat{\lambda}$. 

    \km{The plot is impossible to interpret. What are the values $\lambda$? Why is one plot the opposite of what we want to prove? This needs more explanation. }
    
    
    The two plots are for the case when $\epsilon=1$, $\zeta=0.1$, $\mathfrak{h}(z)=z$ and thus $\frac{\epsilon-\zeta}{\epsilon+\zeta}\hat{f}(\mathbb{R},\epsilon,k)$ may be approximately by $\frac{9}{11}\times \frac{1}{2}=0.44$ as shown in Section \ref{sec:simres}. For the purpose of the plots, we choose $\vect{v} = [- \log 4; \text{ }0; \text{ }\log 4]^T$\footnote{We choose this vector since it minimises equation \eqref{eq:hat_f_defn} and a detailed calculation is given in Section \ref{sec:simres}. \zhihao{it minimizes equation (2) when $\epsilon$ goes to zero, but the figure uses a positive $\epsilon$. Do we need to point it out?}}
    \sss{We can just say it minimises when $\zeta= 0$}
    and demonstrate the point in the Lemma. %A detailed treatment and a formal proof is given in Appendix \ref{subsec-appendix:diff_eqn_soln}.

    
            \begin{figure}[!htp]
        \centering
        \begin{subfigure}{.5\textwidth}
          \centering
          \includegraphics[width= 0.85\linewidth]{lambdahat40.png}
          \caption{Solution for $\hat{\lambda} = 0.40$}
          \label{fig:plotlambda40}
        \end{subfigure}%
        \begin{subfigure}{.5\textwidth}
          \centering
          \includegraphics[width= 0.85\linewidth]{lambdahat46.png}
          \caption{Solution for $\hat{\lambda} = 0.46$}
          \label{fig:plotlambda46}
        \end{subfigure}
        \caption{Solutions for ODE \eqref{eqn:diff_eqn_nu} for $\vect{v} = [- \log 4; \text{ }0; \text{ }\log 4]^T$}
        %\label{fig:plotlambda46}
        \end{figure}
These spikes in the solution maybe observed due to the selection of $\vect{v} \in \mathbb{R}^3$.
    
\end{proof}



\begin{restatable} 
[detailed proof in Appendix \ref{subsec-appendix:diff_eqn_soln}] {lemma}{simrstepa}\label{lemma:dual_achievable}
    $\text{opt}(\mathcal{E}) \geq \hat{f}(\mathbb{R},\epsilon,k)$
     % $$f(\mathbb{R},\epsilon,k) \leq \sup_{u \in \mathbb{R}} \underset{A \sim \hat{P}^{\mathcal{L}_{\epsilon}}_u}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h}(||u-a||_1) \right] = \hat{f}(\mathbb{R},\epsilon,k)$$.
\end{restatable}

We present a proof sketch below where we do not explicitly show the continuity of the bounds $U(.)$ and $L(.)$. A detailed treatment is given in Appendix \ref{subsec-appendix:diff_eqn_soln}. 

\begin{proof}[Proof Sketch]
    Recall the functions $\lambda^{(c)}(.), \delta^{(c)}(.)$ defined in \eqref{eqn:nu_delta_defn}. Also for every $\vect{v} \in \mathbb{R}^k$, we obtain a function $\nu^{(c)}(.,\vect{v})$ [solution of Equation \eqref{eqn:diff_eqn_nu}] with bounds $U(\vect{v})$ and $L(\vect{v})$ satisfying $\nu^{(c)}(r,\vect{v}) \geq 0 \text{ }\forall u\geq U(\vect{v})$ and $\nu^{(c)}(r,\vect{v}) \leq 0 \text{ }\forall u\leq L(\vect{v})$ and this solution is feasible.

    
        
        % \zhihao{A typo in my comment: $v=2/\pi$}
        % \sss{Prove it formally in Claim \ref{lemma:continuity_bounds}}
    


    The objective value of this feasible solution is $\hat{\lambda}$ and the constructed solution is feasible for any $\hat{\lambda} \leq \frac{\epsilon-\zeta}{\epsilon+\zeta} \hat{f}(\epsilon+\zeta,k)$ and $\zeta>0$. Now, since $\hat{f}(\mathbb{R},\epsilon,k)$ is continuous in $\epsilon$, choosing $\zeta$ to be arbitrarily small enables us to get obtain the objective value of the solution arbitrarily close to $\hat{f}(\mathbb{R},\epsilon,k)$ and thus, $\text{opt}(\mathcal{E}) \geq \hat{f}(\mathbb{R},\epsilon,k)$.
    
\end{proof}


%Combining the results in Lemmas \ref{lemma:bounding_f},  \ref{lemma:lp_formulation}, \ref{lemma:dual_achievable} and Theorems  \ref{theorem:weak_duality_result} and Theorem \ref{thm:singpoint:sim}, we prove the following theorem.

\begin{theorem}{\label{thm:optimality-laplace-sim}}
    For $\epsilon$-geographic differential privacy, adding Laplace noise, whose density function is $\rho(x)=\frac{\epsilon}{2} \cdot e^{-\epsilon \disrzero{x}} $, is one of the optimal choices of $\Probs{\Signals}$ for users, and in this case $\funfgeo{\real}{\Ads}{\epsilon}{\K} {\mathfrak{h}(.)} = \hatfunfgeo{\real}{\Ads}{\epsilon}{\K} {\mathfrak{h}(.)}$.
\end{theorem}

\begin{proof}
    Combining the results in Lemmas \ref{lemma:bounding_f},  \ref{lemma:lp_formulation}, \ref{lemma:dual_achievable} and Theorems  \ref{theorem:weak_duality_result} and Theorem \ref{thm:singpoint:sim}, we obtain $\hat{f}(\mathbb{R},\epsilon,k) \leq \text{opt}(\mathcal{E}) \leq \text{opt}(\mathcal{O}) \leq \hat{f}(\mathbb{R},\epsilon,k)$ where $\hat{f}(\mathbb{R},\epsilon,k)$ denotes the cost of Laplace noise addition mechanism $\hat{P}^{\mathcal{L}_{\epsilon}}$ i.e. $\textit{cost}(\hat{P}^{\mathcal{L}_{\epsilon}}) = \hat{f}(\mathbb{R},\epsilon,k)$.

\end{proof}

==> simpleproof-modified-primal-dual.tex <==
\subsection{Dual and primal DILPs and a weak duality result}{\label{sec:primal-feasible}}



In this section, we first represent the cost function $f(\mathbb{R},\epsilon,k)$ by a DILP $\mathcal{O}$, give a construction of the dual DILP $\mathcal{E}$ in and further state a lemma on weak duality upper bounding the optimum value of DILP $\mathcal{E}$ by the optimum value of DILP $\mathcal{O}$. Now we define the cost for mechanism $\textbf{P}$ satisfying $\epsilon$-geographic differential privacy ($\textbf{P} \in \mathcal{P}^{(\epsilon)}_{\mathbb{R}^k}$) in Definition \ref{defn:cost}. %and also define the probability distribution $\hat{P}^{\mathcal{L}_{\epsilon}}_u$ for every $u \in \mathbb{R}$ corresponding to the Laplace noise addition mechanism.



%\km{Why is the next sentence in italics? Maybe start a new subsection?}

% \textit{We now analyse Equation \eqref{eqn:new_expr_f} for the case of $U=\mathbb{R}$ and construct linear programs $\mathcal{E}$ and $\mathcal{O}$.}

\subsubsection{Construction of DILP $\mathcal{O}$ to represent cost function  $f(\mathbbm{R},\epsilon,k)$}

\begin{definition}{\label{defn:cost}}
    Cost of mechanism $\textbf{P} \in \mathcal{P}^{(\epsilon)}_{\mathbb{R}^k}$: We define the cost of mechanism $\textbf{P}$ as
    \begin{equation}{\label{eq:cost}}
        \textit{cost}(\textbf{P}) := \sup_{u \in \mathbb{R}} \underset{A \sim \textbf{P}_u}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h}(|u-a|) \right]
    \end{equation}
\end{definition}

We now define the notion of approximation using cost [defined in Definition \ref{defn:cost}] of mechanisms by a sequence of mechanisms which is used in the construction of DILP $\mathcal{O}$.

\begin{definition}{\label{defn:cost-approx}}
    Arbitrary cost approximation: We call mechanisms $\textbf{P}^{(\eta)} \in \mathcal{P}^{(\epsilon)}_{\mathbb{R}^k}$ an arbitrary cost approximation of mechanisms $\textbf{P} \in \mathcal{P}^{(\epsilon)}_{\mathbb{R}^k}$ if $\lim\limits_{\eta \to 0} \textit{cost}(\textbf{P}^{(\eta)}) = \textit{cost}(\textbf{P})$  
\end{definition}


Now we define the DILP $\mathcal{O}$ to characterise ${f}(\mathbb{R},\epsilon,k)$ as defined in Equation \eqref{eq:new_expr_f} where we optimize over the class of bounded \textit{Riemann integrable functions} non-negative functions and a statement to this effect is proven in Lemma \ref{lemma:lp_formulation}. More specifically, $g(.,.) : \mathcal{I}^B (\mathbb{R} \times \mathbb{R}^k \rightarrow \mathbb{R}^{+})$ denotes that $g(.,.)$ is \textit{Riemann integrable} and a bounded function and we shall see later that $g(.,.)$ is a probability density function of mechanisms satisfying differential privacy constraints.

%We shall see later in the proof of Lemma \ref{lemma:lp_formulation} that $g(u,.)$ is the probability density function of $\textbf{P}^{(\eta)}_u$ for every $u \in \mathbb{R}$ where mechanism $\textbf{P}^{(\eta)}$ is an arbitrary cost approximation of $\textbf{P}$. 


However, observe that the DILP $\mathcal{O}$ involves integrals and thus requires mechanisms to have a valid probability density function, however not every distribution is continuous, and, as a result, may not have a density function (e.g. point mass distributions like $\hat{P}^{\mathcal{L}_{\epsilon}}_u$ defined in Definition \ref{def:laplace_noise_addition}). Using ideas from mollifier theory \cite{99c43556-16f5-3ed5-90f5-6c2bbf257ea3} we construct mechanisms $\textbf{P}^{(\eta)}$ with a valid probability density function that are an arbitrary cost approximation of mechanism $\textbf{P}$ in Lemma \ref{lemma:arbitrary_aprroximation}. 


%where $g(u,.)$ is the probability density function of distributions $\textbf{P}^{(\eta)}_u$ for every $u \in U=\mathbb{R}$ where, $\textbf{P}^{(\eta)}$ arbitrarily approximates cost of $\textbf{P}$ (defined in Definition \ref{defn:cost-approx}) whose construction we give in Lemma \ref{lemma:arbitrary_aprroximation}. 

\begin{equation}{\label{orig_primal}}
    \text{ \Large{$\mathcal{O} =$}}
\left\{
\begin{aligned}
    \inf_{g(.,.): \mathcal{I}^B (\mathbb{R} \times \mathbb{R}^k \rightarrow \mathbb{R}^{+}), \kappa \in \mathbb{R}} \quad & \kappa  \\%\label{primal_main}\\
    \textrm{s.t.} \quad &\kappa - \int\limits_{\vect{x} \in (\mathbb{R})^k} \left[\min_{a \in \texttt{Set}(\vect{x})} \mathfrak{h}(|u-a|) \right] g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right) \geq 0 \text{ }\forall u\in \mathbb{R}\\
    & \int\limits_{\vect{x} \in \mathbb{R}^k} g(u,\vect{x}) d\left(\prod_{i=1}^{k} x_i\right) = 1 \text{ } \forall u\in \mathbb{R}\\
    &  \epsilon g(u,\vect{x}) + \underline{g}_{u}(u,\vect{x}) \geq 0; \text{ }\forall u\in \mathbb{R}; \vect{x} \in \mathbb{R}^k\\
    &  \epsilon g(u,\vect{x}) - \overline{g}_{u}(u,\vect{x}) \geq 0; \text{ }\forall u\in \mathbb{R}; \vect{x} \in \mathbb{R}^k
\end{aligned}
\right.
\end{equation}

In DILP $\mathcal{O}$, we define $\underline{g}_u(u,\vect{x})$ and $\overline{g}_u(u,\vect{x})$ to be the lower and upper partial derivative of $g(u,\vect{x})$ at $u$. Now observe that, we use lower and upper derivatives instead of directly using derivatives as the derivatives of a probability density function may not always be defined (for example, the left and right derivatives are unequal in the Laplace distribution at origin).  

We now move to prove the main lemma stating $\text{opt}(\mathcal{O})= f(\mathbb{R},\epsilon, k)$.  

\begin{lemma}{\label{lemma:lp_formulation}}
        Let $\text{opt}(\mathcal{O})$ denote the optimal value of DILP \eqref{orig_primal}, then  
    $f(\mathbb{R},\epsilon,k) = \text{opt}(\mathcal{O})$.
\end{lemma}

To prove this lemma, we first show two Lemmas \ref{lemma:diff-privacy-condition} and Lemmas \ref{lemma:arbitrary_aprroximation} below.


%We now give a summary of that DILP $\mathcal{O}$ correctly represents $f(\mathbb{R},\epsilon,k)$. Assuming, every $P_u$ has a valid probability density function (i.e. continuous) call it $g(u,.)$ we showing  

%\km{Maybe have a lemma stating the LP captures the optimization problem, and use the lemmas to prove the lemma?}

We now state a lemma relating the last 2 constraints of the DILP $\mathcal{O}$ to $\epsilon$-geographic differential privacy. 
\begin{lemma}{\label{lemma:diff-privacy-condition}}
    Let $P_u$ have a probability density function given by $g(u,.): \mathbb{R}^k \rightarrow \mathbb{R}$ for every $u \in \mathbb{R}$. Then, $P$ satisfies $\epsilon$-geographic differential privacy iff $\max(|\overline{g}_u(u,\vect{x})|, |\underline{g}_u(u,\vect{x})|) \leq \epsilon g(u,\vect{x}) \text{ } \forall u \in \mathbb{R};\forall \vect{x} \in \mathbb{R}^k$ \footnote{$\underline{g}_u(u,\vect{x})$, $\overline{g}_u(u,\vect{x})$ denote the lower and upper partial derivative w.r.t. $u$}   
\end{lemma} 

The proof of this lemma is given in Section~\ref{sec:diff-privacy-condition-proof}. We prove this lemma by showing that $\epsilon$-geographic differential privacy is equivalent to Lipschitz continuity of $\log g(u,\vect{x})$ in $u$.\footnote{It may happen that the $\log$ is not defined as the density is zero at some point, we handle this case separately in the proof.}  



% and the key proof idea in this claim is that $\log g(u,\vect{x})$ is Lipschitz continuous in $u$ with Lipschitz constant $\epsilon$.

% applying $\epsilon$-geographic differential privacy conditions on distributions by showing 

% The following claim shows that that optimal value of linear program $\mathcal{O}$ is $f(\epsilon,k)$. Recall that in the linear program $\mathcal{O}$, $g(u,.)$ relates to the probability density of $\textbf{P}^{(\eta)}_u$ where distributions $\textbf{P}^{(\eta)}$ arbitrarily approximate $\textbf{P}$. Note this claim is important as not every distribution $\textbf{P}_u$ may be a continuous probability distribution and thus may not have a density function for example, point mass distributions like $\hat{P}^{\mathcal{L}_{\epsilon}}_u$ don't. We prove Lemma \ref{lemma:lp_formulation} by showing that any distribution maybe \textit{arbitrarily} approximated by a distribution with a probability density function using ideas from mollifier theory \cite{99c43556-16f5-3ed5-90f5-6c2bbf257ea3} and deferred to Section \ref{sec:proof_lp_formulation}.
% The following claim shows that the the optimal value of DILP $\mathcal{O}$ is $f(\mathbb{R},\epsilon,k)$. In $\mathcal{O}$, $g(u,.)$ is the probability density of $\textbf{P}^{(\eta)}_u$ for every $u \in \mathbb{R}$ where $\textbf{P}^{(\eta)}$ is an arbitrary cost approximation of distribution $\textbf{P}$. This claim is crucial because not every distribution $\textbf{P}_u$ may be continuous, and, as a result, may not have a density function (e.g., point mass distributions like $\hat{P}^{\mathcal{L}_{\epsilon}}_u$ don't). We use ideas from mollifier theory \cite{99c43556-16f5-3ed5-90f5-6c2bbf257ea3} to construct distributions $\textbf{P}^{(\eta)}$ and deferred to Section \ref{sec:proof_lp_formulation}. 


We now state a Lemma showing an arbitrary cost approximation of mechanism $\textbf{P}$ can be constructed with valid probability density functions. The proof of the following lemma is deferred to Section \ref{sec:proof_arbitrary_approximation}.
\begin{lemma}{\label{lemma:arbitrary_aprroximation}}
    Given any mechanism $\textbf{P} \in \mathcal{P}^{(\epsilon)}_{\textbf{R}^k}$ (satisfying $\epsilon$-geographic differential privacy), we can construct a sequence of mechanisms $\textbf{P}^{(\eta)}$ with bounded probability density functions such that $\textbf{P}^{(\eta)}$ is an arbitrary cost approximation of mechanism $\textbf{P} \in \mathcal{P}^{(\epsilon)}_{\textbf{R}^k}$.
    \end{lemma}

 We now show that optimum value of DILP $\mathcal{O}$ equals $f(\mathbb{R},\epsilon,k)$.

\begin{proof}[Proof of Lemma \ref{lemma:lp_formulation}]
    Consider any $\zeta>0$. As established in Lemma \ref{lemma:arbitrary_aprroximation}, it follows for every mechanism $\textbf{P} \in \mathcal{P}^{(\epsilon)}_{\textbf{R}^k}$, we can construct another mechanism $\textbf{P}^{(\eta)}$ with bounded probability density functions whose cost is a $\zeta$ approximation of the cost of mechanism $\textbf{P}$.
   Thus, we can use Lemma \ref{lemma:diff-privacy-condition} to conclude that optimum value of DILP $\mathcal{O}$ is precisely $f(\mathbbm{R},\epsilon,k)$ 
\end{proof}


% The proof of this lemma is technical and uses ideas from mollifier theory \cite{99c43556-16f5-3ed5-90f5-6c2bbf257ea3} and deferred to Section \ref{sec:proof_lp_formulation} to arbitrarily approximate any distribution by a distribution with a probability density function. However, we also state a lemma relating how $\epsilon$

%\km{Why is dual in italics? Start a new subsection about the dual here?}

\subsubsection{Dual DILP $\mathcal{E}$ and statement of weak duality theorem}
Now, we write the \textit{dual} of the DILP $\mathcal{O}$ as the DILP $\mathcal{E}$ in Equation \eqref{orig_dual}. Observe that, we have the constraint that $\delta(.)$ and $\lambda(.)$ is continuous and $\nu(.,.)$
is a $\mathcal{C}^{1}$ function i.e. $\nu(r,\vect{v})$ is \textit{continuously differentiable} in $r$ and \textit{continuous} in $\vect{v}$.
Thus, we may rewrite the equations as 
\begin{equation}{\label{orig_dual}}
    \text{\Large{$\mathcal{E}=$} }
    \left\{
    \begin{aligned}
    \sup_{\substack{\delta(.),\lambda(.): \mathcal{C}^{0}(\mathbb{R}\rightarrow \mathbb{R}^+); \\ \nu(.,.): \mathcal{C}^1(\mathbb{R} \times (\mathbb{R})^k\rightarrow \mathbb{R})} } & \int_{r \in \mathbb{R}} \lambda(r) du\\
    \textrm {s.t. } \quad & \int_{u \in \mathbb{R}} \delta(r) du \leq 1\\
     & \hspace{- 3em} -\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|r-a|) \right] \delta(r) + \lambda(r) + \left(\nu_r(r,\vect{v}) + \epsilon|\nu(r,\vect{v})|\right) \leq 0 \text{ }\forall  r \in \mathbb{R}; \vect{v} \in (\mathbb{R})^k\\
    & \exists U: \mathcal{C}^0(\mathbb{R}^k \rightarrow \mathbb{R})  \textrm { s.t. }\nu(r,\vect{v}) \geq 0 \text{ }\forall r\geq U(\vect{v}) \text{ } \forall \vect{v} \in (\mathbb{R})^k \\
    & \exists L: \mathcal{C}^0(\mathbb{R}^k \rightarrow \mathbb{R}) \textrm { s.t. } \nu(r,\vect{v}) \leq 0 \text{ } \forall r\leq L(\vect{v}) \text{ } \forall \vect{v} \in (\mathbb{R})^k 
\end{aligned}
\right.
\end{equation}

%\km{Why is intuition in air quotes? Also, why is each sentence a paragraph? }

To get some intuition behind the construction of our dual DILP $\mathcal{E}$, relate the equations in DILP $\mathcal{O}$ to the dual variables of DILP $\mathcal{E}$ as follows. The first equation denoted by $\{\delta(r)\}_{r \in \mathbb{R}}$, second equation denoted by $\{\lambda(r)\}_{r \in \mathbb{R}}$ and the last two equations are \textit{jointly} denoted by $\{\nu(r,\vect{v})\}_{r \in \mathbb{R}; \vect{v} \in (\mathbb{R})^k}$. 
\footnote{Note that the variable $\nu(u,\vect{v})$ is constructed from the difference of two non-negative variables corresponding to third and fourth equation respectively. Detailed proof is in Appendix \ref{sec:weak_duality}}.\\
% fourth equation
% $\{\nu^{(2)}(u,\vect{v})\}_{u \in \mathbb{R}; \vect{v} \in (\mathbb{R})^k}$. \\


%\km{Why is knowledge in air quotes? If this is our main result, we should make it a theorem and not a lemma, and highlight it more.}

Observe that in our framework, we have to prove the weak-duality result as to the best of our knowledge existing duality of linear programs in infinite dimensional spaces work for cases involving just integrals. %This theorem would imply the generalization of the weak duality theorem to infinite dimensional linear programs over function spaces involving both derivatives and integral. 
The proof of this Theorem \ref{theorem:weak_duality_result} is technical and we defer the details to Appendix \ref{sec:weak_duality}. 

%We show in Sec \ref{sec:weak_duality} that $\text{opt}(\mathcal{O}) \geq \text{opt}(\mathcal{E})$. 

% We prove the weak duality theorem i.e. Theorem \ref{theorem:weak_duality_result}) in Sec \ref{sec:weak_duality}.  Note that this duality needs to be proven in our setup as the linear programs are over infinite dimensional vector spaces and the duality does not follow directly from standard existing results in linear programs.
\begin{theorem}{\label{theorem:weak_duality_result}}
    $\text{opt}(\mathcal{O}) \geq \text{opt}(\mathcal{E})$
\end{theorem}


==> simpleproof-modified.tex <==
\section{Characterizing the Optimal Mechanism: Proof Sketch of Theorem~\ref{thm:lap:sim}}      
\label{sec:simproof}
% In this section, we provide four sets of mechanisms, where the latter mechanisms are simplifications and special cases of the former ones, and the first set satisfies the model in Section~\ref{sec:subsecsimmodel}. As we narrow down the choice of mechanism, the optimal mechanism is not removed from the set, so we finally get the optimal mechanism in a simple form. Along the way, we provide the proof sketch of Theorem~\ref{thm:lap:sim}. The full proof involves many technical details and is presented in the Appendix.

In this section, we provide the four main steps in the proof and thus prove Theorem~\ref{thm:lap:sim} and the full proof involves many technical details and is presented in the Appendix.
\subsection{Simulating the Server} 
\label{sec:simproof1}
In the model in Section~\ref{sec:simmodel}, user $u$ draws signal $s$ following $\dsig{u}$, and sends $s$ to the server. The server draws a result set $A$ following $\dsigq{s}$, and send $A$ back to the user. This entire computation can be simulated by the user. User $u$ draws $s$ following $\dsig{u}$, then draws $A$ following $\dsigq{s}$, and finally returns $A$ to the server. After the server receives $A$, it just sends $A$ back to the user. Now, the signal set $\Signals$ is $\real^{\K}$, and the server simply returns the signal, so we only need to choose $\Pname$ where the distributions are on $\real^{\K}$.

\begin{example}
Fix a user $u$ and let $\Signals=\{s_1,s_2\}$ and $\Kads=\{A_1,A_2\}$ and user $u$ sends $s_1$ and $s_2$ with equal probability. The server returns $A$ on receiving signal $s$, with the following probability.
\begin{align*}
    &\Prxx{u}{A=A_1 | s=s_1}=0.2,\quad
    \Prxx{u}{A=A_2 | s=s_1}=0.8, \\
    &\Prxx{u}{A=A_1 | s=s_2}=0.4,\quad
    \Prxx{u}{A=A_2 | s=s_2}=0.6.
\end{align*}
Then the probability that $u$ receives $A_1$ is 0.3 and it receives $A_2$ is 0.7. Now consider an equivalent mechanism, where $\Signals=\Kads=\{A_1,A_2\}$, with user $u$ sending signal $A_1$ and $A_2$ with probabilities 0.3 and 0.7.
% \begin{align*}
%     &\Prxx{u}{A=A_1}=0.3, \quad \Prxx{u}{A=A_2}=0.7.
% \end{align*}
When the server receives $A\in \Kads$, it returns $A$.
\end{example}

% \begin{align*}
%     &\Prxx{u}{A=A_1}=0.3, \quad \Prxx{u}{A=A_2}=0.7.
% \end{align*}
We show the new mechanism satisfies differential privacy assuming the original mechanism satisfies it. As a result, we can assume $\Signals=\Kads$ when finding the optimal mechanism.

%Besides, given $\Pname$, the worse user distribution $\Dist$ will concentrate all the mass on the user with largest expected distance to the closest ad, so we have


\begin{restatable} 
[detailed proof in Appendix \ref{sec-appendix:simproof}] {theorem}{simrstepa}\label{thm:singpoint:sim}
\begin{align}{\label{eq:new_expr_f}}
\funf{\Users}{\Ads}{\epsilon}{\K} =\inf_{\Pname\in \Probs{\real^{\K}}} \sup_{u \in U} \Exx{A\sim \Pname_u}{ \min_{a\in \texttt{Set} (A)}\mathfrak{h}(d(u,a)) }.
\end{align}
\end{restatable}


%\simrstepa*

\begin{proof}[Proof Sketch]
Fix $\Signals,\Pname\in \Probs{\Signals},\Qname\in \Qrobs_{\Signals}$. For $u\in \real$ and $S\subset \real^{\K}$, let $\Ppxx{u}{S}$ be the probability that the server returns a set in $S$ to $u$. Then for any $u_1,u_2\in \real, S\subset \real^{\K}$, we can show that $\Ppxx{u_1}{S} \leq e^{\epsilon\cdot d(u_1,u_2)} \Ppxx{u_2}{S}$, and thus $\Ppname\in \Probs{\real^{\K}}$ because $\Ppname_{u}$ is a distribution on $\real^{\K}$ for any $u\in \real$. At the same time,
% \begin{align*}
%     \Ppxx{u}{S}=\Prxx{ s\sim \Pname_u, A\sim \Qname_s}{A\in S}.
% \end{align*}


% \begin{align*}
%     \Ppxx{u_1}{S}
%     =\Prxx{ s\sim \Pname_{u_1}, A\sim \Qname_s}{A\in S}  =& \Exx{s\sim \Pname_{u_1}}{\Prxx{ A\sim \Qname_s}{A\in S}}    \\
%     =& \int_{s\in \Signals}{\left(\Prxx{ A\sim \Qname_s}{A\in S}\cdot \Pxx{u_1}{ds} \right)}    \\
%     \leq & e^{\epsilon\cdot \defdis{u_1}{u_2}}\int_{s\in \Signals}{\left(\Prxx{ A\sim \Qname_s}{A\in S}\cdot \Pxx{u_2}{ds} \right)}    \\
%     = & e^{\epsilon\cdot \defdis{u_1}{u_2}}\Exx{s\sim \Pname_{u_2}}{\Prxx{ A\sim \Qname_s}{A\in S} }    \\
%     %= & e^{\epsilon\cdot \defdis{u_1}{u_2}}\Exx{s\sim \Pname_{u_2},A\sim \Qname_s}{A\in S }    \\
%     = & e^{\epsilon\cdot \defdis{u_1}{u_2}} \Ppxx{u_2}{S},
% \end{align*}

\begin{align*}
\Exxlimits{s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}(d(u,a)) }
=\Exxlimits{A\sim \Ppname_u}{ \min_{a\in \texttt{Set}(A)}\mathfrak{h}(d(u,a)) }, \text{ so we have}
\end{align*}
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K} = \inf_{\Pname\in \Probs{\real^{\K}}} \sup_{u \in U} \Exxlimits{A\sim \Pname_u}{ \min_{a\in \texttt{Set} (A)}\mathfrak{h}(d(u,a)) },
\end{align*}

\km{The English in the paragraph below is off. Can we please use a grammar checker software?}

%The last equality $(a)$ follows since fixing a mechanism, we are interested in it performance in the worst case among all possible distributions of users. The worst distribution is in fact an one-point distribution, completing the proof.

\end{proof}

%In the subsequent section, we analyse and construct a DILP $\mathcal{O}$ to represent $\funf{\Users}{\Ads}{\epsilon}{\K}$ 

\input{simpleproof-modified-primal-dual}
\input{simpleproof-modified-dual-fitting}


\input{ashishproof-modified}



\subsection{Main Theorem}
\km{This is repetitive. Can we just write a sentence pointing to Theorem 3 and omit the section?}
Based on the above arguments, we have the main theorem \ref{thm:lap:sim}.


  

%\simrstepe*


%Furthermore, the optimal mechanism can be computed in closed form. Furthermore, the optimal mechanism can be computed in closed form. The optimal mechanism in a simplified setting is computed in the next section.


\iffalse%%%%%%%%%%%%%%%%
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\begin{cases}
\frac{4}{\epsilon(\K +1)} , & \text{$\K$ is odd},  \\
\frac{2}{\epsilon} \log\left( 1+\frac{2}{\K} \right) , & \text{$\K$ is even},  \\
\end{cases}
\end{align*}
which is $O(1/(\epsilon \K))$. Moreover, in one of the optimal mechanisms, user $u\in \real$ sends signal $u+\eta$, where $\eta$ is drawn from the distribution with density function $\rho(x)=e^{-\epsilon \disrzero{u}{x}}/\epsilon$, and when the server receives signal $s\in \real$, it sends back $\{s+a_1, s+a_2, \dots, s+a_{\K}\}$, where
\begin{enumerate}
    \item If $\K$ is odd, let $t=(\K -1)/2$, and
    \begin{align*}
        \{a_1,\dots,a_{\K}\}=\left\{
        0, \pm \frac{2\log\left(\frac{t+1}{t}\right)}{\epsilon},
        \pm \frac{2\log\left(\frac{t+1}{t-1}\right)}{\epsilon},
        \dots,
        \pm \frac{2\log\left(\frac{t+1}{2}\right)}{\epsilon},
        \pm \frac{2\log\left(t+1\right)}{\epsilon}
        \right\}.
    \end{align*}
    \item If $\K$ is even, let $t=\K/2$, and
    \begin{align*}
        \{a_1,\dots,a_{\K}\}=\left\{
         \pm \frac{\log\left(\frac{t+1}{t}\right)}{\epsilon},
        \pm \frac{\log\left(\frac{t(t+1)}{(t-1)^2}\right)}{\epsilon},
        \pm \frac{\log\left(\frac{t(t+1)}{(t-2)^2}\right)}{\epsilon},
        \dots,
        \pm \frac{\log\left(\frac{t(t+1)}{2^2}\right)}{\epsilon},
        \pm \frac{\log\left(t(t+1)\right)}{\epsilon}
        \right\}.
    \end{align*}
\end{enumerate}
\fi%%%%%%%%%%%%%%%%%%%%%%%%

==> simpleproof.tex <==
\section{Characterizing the Optimal Mechanism: Proof Sketch of Theorem~\ref{thm:lap:sim}}      
\label{sec:simproof}
% In this section, we provide four sets of mechanisms, where the latter mechanisms are simplifications and special cases of the former ones, and the first set satisfies the model in Section~\ref{sec:subsecsimmodel}. As we narrow down the choice of mechanism, the optimal mechanism is not removed from the set, so we finally get the optimal mechanism in a simple form. Along the way, we provide the proof sketch of Theorem~\ref{thm:lap:sim}. The full proof involves many technical details and is presented in the Appendix.

In this section, we describe the four steps involved in the proof of Theorem 

\subsection{Simulating the Server} 
\label{sec:simproof1}
In the model in Section~\ref{sec:simmodel}, user $u$ draws signal $s$ following $\dsig{u}$, and sends $s$ to the server. The server draws a result set $A$ following $\dsigq{s}$, and send $A$ back to the user. This entire computation can be simulated by the user. User $u$ draws $s$ following $\dsig{u}$, then draws $A$ following $\dsigq{s}$, and finally returns $A$ to the server. After the server receives $A$, it just sends $A$ back to the user. Now, the signal set $\Signals$ is $\real^{\K}$, and the server simply returns the signal, so we only need to choose $\Pname$ where the distributions are on $\real^{\K}$.

\begin{example}
Fix a user $u$. Suppose $\Signals=\{s_1,s_2\}$ and $\Kads=\{A_1,A_2\}$. User $u$ sends $s_1$ and $s_2$ with equal probability $1/2$. The server returns $A$ when it receives signal $s$, with the following probability.
\begin{align*}
    &\Prxx{u}{A=A_1 | s=s_1}=0.2,\quad
    \Prxx{u}{A=A_2 | s=s_1}=0.8, \\
    &\Prxx{u}{A=A_1 | s=s_2}=0.4,\quad
    \Prxx{u}{A=A_2 | s=s_2}=0.6.
\end{align*}
Then the probability that $u$ receives $A$ is
\begin{align*}
    &\Prxx{u}{A=A_1}=0.3, \quad \Prxx{u}{A=A_2}=0.7.
\end{align*}

There is an equivalent mechanism, where $\Signals=\Kads=\{A_1,A_2\}$, and $u$ sends signal $A$ with the following probabilities.
\begin{align*}
    &\Prxx{u}{A=A_1}=0.3, \quad \Prxx{u}{A=A_2}=0.7.
\end{align*}
When the server receives $A\in \Kads$, it returns $A$.
\end{example}


We show the new mechanism satisfies differential privacy assuming the original mechanism satisfies it. As a result, we can assume $\Signals=\Kads$ when finding the optimal mechanism.

%Besides, given $\Pname$, the worse user distribution $\Dist$ will concentrate all the mass on the user with largest expected distance to the closest ad, so we have


\begin{restatable} 
[corresponds to Lemma \ref{lem:onlyuserstr}] {theorem}{simrstepa}\label{thm:singpoint:sim}
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K} = \inf_{\Pname\in \Probs{\real^{\K}}} \sup_{\Dist} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}|u-a| }.
\end{align*}
\end{restatable}


%\simrstepa*

\begin{proof}
Fix $\Signals,\Pname\in \Probs{\Signals},\Qname\in \Qrobs_{\Signals}$. For $u\in \real$ and $S\subset \real^{\K}$, let $\Ppxx{u}{S}$ be the probability that the server returns a set in $S$ to $u$.
\begin{align*}
    \Ppxx{u}{S}=\Prxx{ s\sim \Pname_u, A\sim \Qname_s}{A\in S}.
\end{align*}

Then for any $u_1,u_2\in \real, S\subset \real^{\K}$, we have
\begin{align*}
    \Ppxx{u_1}{S}
    =&\Prxx{ s\sim \Pname_{u_1}, A\sim \Qname_s}{A\in S}    \\
    =&\Exx{s\sim \Pname_{u_1}}{\Prxx{ A\sim \Qname_s}{A\in S}}    \\
    =& \int_{s\in \Signals}{\left(\Prxx{ A\sim \Qname_s}{A\in S}\cdot \Pxx{u_1}{ds} \right)}    \\
    \leq & e^{\epsilon\cdot \defdis{u_1}{u_2}}\int_{s\in \Signals}{\left(\Prxx{ A\sim \Qname_s}{A\in S}\cdot \Pxx{u_2}{ds} \right)}    \\
    = & e^{\epsilon\cdot \defdis{u_1}{u_2}}\Exx{s\sim \Pname_{u_2}}{\Prxx{ A\sim \Qname_s}{A\in S} }    \\
    %= & e^{\epsilon\cdot \defdis{u_1}{u_2}}\Exx{s\sim \Pname_{u_2},A\sim \Qname_s}{A\in S }    \\
    = & e^{\epsilon\cdot \defdis{u_1}{u_2}} \Ppxx{u_2}{S},
\end{align*}
so $\Ppname\in \Probs{\real^{\K}}$ because $\Ppname_{u}$ is a distribution on $\real^{\K}$ for any $u\in \real$. At the same time,
\begin{align*}
\Exxlimits{u\sim \Dist, s\sim \Pname_u, A\sim \Qname_s}{ \min_{a\in A}|u-a| }
=\Exxlimits{u\sim \Dist, A\sim \Ppname_u}{ \min_{a\in A}|u-a| },
\end{align*}
so we have
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K} = \inf_{\Pname\in \Probs{\real^{\K}}} \sup_{\Dist} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}|u-a| },
\end{align*}
completing the proof.
\end{proof}



\subsection{Symmetric Mechanisms}
\label{sec:simproof2}
For $A\in \real^{\K}$ and $x\in \real$, we define $A+x$ to be $\{a+x:a\in A\}$. We say a mechanism \emph{symmetric}, if there is a distribution $\Pname_{ave}$ on $\real^{\K}$, so that user $u\in \real$ draws $A$ from $\Pname_{ave}$ and sends signal $A+u$. Then the server simply returns the received signal. In symmetric mechanisms, users behave similarly to each other as the relative position of the signal to the user is independent of user location.

We now modify an arbitrary mechanism to be \emph{symmetric} by averaging the strategy of different users. For example, if $\K=1$, if the probability that the user located at $0$ sends a signal in the interval $[5,8]$ does not equal to the probability that the user located at $1$ sends a signal in the interval $[6,9]$, we can change both probabilities to be their average.

\begin{example}[Making a mechanism symmetric]
Let $\K=1$, $\epsilon=2$. User $u\in \Users$ draw signal $s$ from the distribution with density
\begin{align*}
    \rho_{u}(s)= \alpha_u e^{|u-\lfloor s\rfloor|} ,\quad \text{~for any~} s\in \Users,
\end{align*}
where $\alpha_u=(\int_{s\in \real} e^{|u-\lfloor s\rfloor|} ds )^{-1}$ is the normalizer.

For any users $u,v\in \real$, and signal $s\in \real$, we have $e^{|u-\lfloor s\rfloor|}\leq e^{|u-v|}e^{|v-\lfloor s\rfloor|}$, so $\alpha_u\leq e^{|u-v|}\alpha_v$. As a result, $\rho_{u}(s)\leq e^{2|u-v|}\rho_{v}(s)$, which implies the mechanism satisfies 2-geographic differential privacy. We now construct a symmetric mechanism by averaging the strategy over all users. Here, $u\in \Users$ draws $y$ from the distribution with density $\rho(y)$ and sends the signal $u+y$, where
\begin{align*}
    \rho(y)=\limt{x}{+\infty}{\frac{1}{2x}\int_{-x}^{x}\rho_{u}(u+y) du}=\int_{0}^{1}\rho_{u}(u+y) du.
\end{align*}
The second equation holds because $\rho_{u}(u+y)=\rho_{u+1}((u+1)+y)$ for any $u,y\in \real$. Note that the new mechanism is symmetric. Since the new mechanism is averaging the strategy in the original mechanism, it is not hard to see that it also satisfies 2-geographic differential privacy, and does not have a larger expected value of $|u-s|$.
\end{example}

In this example, the limit value exists. In general, this does not have to be the case. To cover more general cases, we construct symmetric mechanisms that satisfy $\epsilon'$-geographic differential privacy for a sequence of $\epsilon'$, whose error goes to $\funf{\Users}{\Ads}{\epsilon}{\K}$ when $\epsilon'$ goes to $\epsilon$.



\begin{claim}[corresponds to Lemma \ref{lem:changeScale}]   \label{cla:1}
    For any $\K$, for any $\epsilon>0$,
    \begin{align}%\label{limtChangeScale}
    \limt{\epsilon'}{\epsilon^{-}}{ \funf{\Users}{\Ads}{\epsilon'}{\K}}  = \funf{\Users}{\Ads}{\epsilon}{\K}.
    \end{align}
\end{claim}


We will prove the claim in the Appendix. In symmetric mechanisms, for any $u\in \real, \C\subset \real^{\K}$, we have $\Pname_{u}(u+\C)=\Pname_{ave}(\C)$, so $\Exx{A\sim \Pname_u}{ \min_{a\in A}|u-a| } = \Exx{A\sim \Pname_{ave}}{ \min_{a\in A} |a| }$, which means the expected value of $u-a$ is independent of $u$. We have
    

\begin{restatable}[corresponds to Lemma \ref{lem:symtor}]{theorem}{simrstepb} \label{thm:symopt:sim}
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{\Pname_{ave}\in \Psym}  \Exx{A\sim \Pname_{ave}}{ \min_{a\in A}|a| },
\end{align*}
where $\Psym$ is the set of symmetric mechanisms that satisfy $\epsilon$-geographic differential privacy.
\end{restatable}


%\simrstepb*

\begin{proof}


For an arbitrary $\epsilon'<\epsilon$ and $\Ppname\in \Probsx{\epsilon'}{\Kads}$, we construct $\Pname_{ave}$ as follows. Suppose there is a user distribution $\Dist$ whose density is
\begin{align*}
\rho_{\nu}(x) = \alpha \cdot e^{-(\epsilon-\epsilon')|x|}
\end{align*}
for $x\in \Users$, where the constant $\alpha$ is the normalizer satisfying
\begin{align*}
\alpha = \left(\int_{x\in \Users}e^{-(\epsilon-\epsilon')|x|} dx \right)^{-1}.
\end{align*}
For any $u\in \Users$ and $\C\subset \Kads$, let $\Pname_{ave}(\C)$ be the probability that $u \sim \Dist$ reports a signal in $u+\C$. That is,
\begin{align*}
    \Pname_{ave}(\C) \defeq \Exx{u\in \Dist}{\Ppxx{u}{u+\C} }.
\end{align*}
We have
\begin{align*}
 \Exx{A\sim \Pname_{ave}}{ \min_{a\in A}|a| }  
=& \Exx{u\sim \Dist, A \sim \Ppname_u }{ \min_{a\in A}|a-u| }  
\leq  \sup_{\Dist} \Exx{u\sim \Dist, A\sim \Pname_u}{ \min_{a\in A}|u-a| }.
\end{align*}
Note that $\epsilon'$ can be arbitrarily close to $\epsilon$. By Theorem \ref{thm:singpoint:sim} and Claim \ref{cla:1}, it is sufficient to show $\Pname_{ave}$ satisfies $\epsilon$-geographic differential privacy. For any $u_1,u_2\in \Users$, $\C\subset \Kads$, $u_1$ sends a signal in $\C$ with probability $\Pname_{ave}(\C-u_1)$, and $u_2$ sends a signal in $\C$ with probability $\Pname_{ave}(\C-u_2)$. We have
\begin{align*}
& \Pname_{ave}(\C-u_1) \\
=&  \int_{x\in \Users} \Ppxx{x}{x+\C-u_1} \rho_{\nu}(x)dx   \\
\leq & e^{\epsilon' \dis{u_1}{u_2}}\cdot 
    \int_{x\in \Users}  \Ppxx{x-u_1+u_2}{(x-u_1+u_2)+\C-u_2} \rho_{\nu}(x)dx   \\
\leq & e^{\epsilon' \dis{u_1}{u_2}}\cdot e^{(\epsilon-\epsilon') \dis{u_1}{u_2}}\cdot 
 %& \int_{(x-u_1+u_2)\in \Users}  \Ppxx{x-u_1+u_2}{(x-u_1+u_2)+\C-u_2} \rho_{\nu}(x-u_1+u_2)dx   \\
  \int\limits_{(x-u_1+u_2)\in \Users}  \Ppxx{x-u_1+u_2}{x-u_1+\C} \rho_{\nu}(x-u_1+u_2)dx   \\
= & e^{\epsilon \dis{u_1}{u_2}} \cdot \Pxx{ave}{\C-u_2},  
\end{align*}
The final inequality holds since
\begin{align*}
    e^{(\epsilon-\epsilon') \dis{u_1}{u_2}}\rho_{\nu}(x-u_1+u_2) 
    =& e^{-(\epsilon-\epsilon')(\diszero{x-u_1+u_2}-\dis{u_1}{u_2})} 
    \geq e^{-(\epsilon-\epsilon')\diszero{x}} = \rho_{\nu}(x)
\end{align*}
so $\Pname_{ave}$ satisfies $\epsilon$-geographic differential privacy.
\end{proof}




\subsection{Real-valued Signals}
\label{sec:simproof3}
At this point, we only need to construct  the distribution $\Pname_{ave}$ over $\real^{\K}$, so that user $u\in \real$ will draw $A$ from the distribution and send the signal $u+A$. Assuming $\Pname_{ave}$ has a density $\rho(\cdot)$, for any $u\in \Users$ and $A\in \real^{\K}$, we need $\rho(A)\leq e^{\epsilon \diszero{u}} \cdot \rho(A+u)$ to ensure differential privacy. Note that for two signals $A_1,A_2\in \real^{\K}$, if we can not shift $A_1$ to be $A_2$, which means there is no $u\in \real$ so that $A_1+u=A_2$, then we do not have any privacy constraint between $A_1$ and $A_2$. As a result, we define equivalence classes where two signals in $A_1, A_2 \in \real^{\K}$ are in the same class if $A_1 + u = A_2$ for some $u \in \real$. For two signals in different equivalence classes, there is no privacy constraint between them. 

By an averaging argument, we can show that the optimal distribution $\Pname_{ave}$ is distributed over just one equivalence class. Suppose this class is $\{ A_0+x | x\in \real \}$ for a certain $A_0$. The differential privacy constraint is now over the real number $x$, and the goal is to find the best $A_0$. This can be viewed as a one-dimensional signal $x$, and we have the following theorem:


\begin{restatable}[corresponds to Theorem \ref{thm:symfinal}] {theorem}{simrstepc} \label{thm:symfinal:sim}
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\inf_{A\in \real^{\K}} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} },
\end{align*}
where
\begin{align*}
\Srobs = \{ \Sname | \Sname \text{~is a distribution on $\real$};&\\
 \text{~and~} \forall x,y\in \real, \rho_{\Sname}(x)\leq& e^{\epsilon \dis{x}{y}}\rho_{\Sname}(y) \} .
\end{align*}
\end{restatable}


%\simrstepc*


\begin{proof}
    By Theorem \ref{thm:symopt:sim}, it is sufficient to show
    \begin{align*}
        \inf_{\Pname_{ave}\in \Psym}  \Exx{A\sim \Pname_{ave}}{ \min_{a\in A}|a| }
        =
        \inf_{A\in \real^{\K}} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }.
    \end{align*}

    Fix $\Pname_{ave}\in \Psym$. Assume its probability density function is $\rho(A)$ for $A\in \real^{\K}$. (This assumption will be removed in the Appendix.) For any $u\in \Users$ and $A\in \real^{\K}$, we have $\rho(A)\leq e^{\epsilon \diszero{u}} \rho(A+u)$.
    
    Let $G=\{A=(a_1,a_2,\dots,a_{\K})\in \real^{\K}: a_{\K}=0\}$. Then we have
    \begin{align*}
        &\Exx{A\sim \Pname_{ave}}{ \min_{a\in A} |a| } \\ 
        =&
        \int_{A\in \real^{\K}} \left( \min_{a\in A}|a| \right) \rho(A) dA\\
        =&
        \int_{A\in G}\int_{c\in \real} \left( \min_{a\in A}\diszero{a-c}  \right) \rho(A-c) ~dc~ dA \\
        =&
        \int_{A\in G} \left(\int_{x\in \real}\rho(A-x) dx\right) \cdot  
         \left( \int_{c\in \real} \min_{a\in A}\diszero{a-c}\frac{\rho(A-c)}{\int_{x\in \real}\rho(A-x) dx} dc\right) dA \\
        \geq &
        \int_{A\in G} \left(\int_{x\in \real}\rho(A-x) dx\right) \cdot  \left(  \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }\right) dA \\
        \geq & \inf_{A\in \real^{\K}} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }.
    \end{align*}

    On the other hand, for any $A\in \Kads, \Sname \in \Srobs$, let $\Pname(\C)=\Exx{x\sim \Sname}{A-x\in \C}$ for any $\C\subset \Kads$. Then $\Pname \in \Psym$, and we have
    \begin{align*}
        \Exx{x\sim \Sname}{ \min_{a\in A}\diszero{a-x} }
        =
        \Exx{x\sim \Sname}{ \min_{a\in (A-x)}\diszero{a} }
        =
        \Exx{A'\sim \Pname}{ \min_{a\in A'} \diszero{a} }   
        \geq 
        \inf_{\Pname_{ave}\in \Psym}  \Exx{A\sim \Pname_{ave}}{ \min_{a\in A}|a| }.
    \end{align*}
This completes the proof.
\end{proof}




\subsection{Laplace Noise is Optimal}
\label{sec:simproof4}
We will finally show that the optimal distribution $\Sname$ in the previous theorem is the Laplace distribution. Given this, $A_0$ will be an easy computation. We will prove


\begin{restatable}[corresponds to Theorem \ref{thm:lapopt}]{theorem}{simrstepd}     \label{thm:lapopt:sim}
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=&
\inf_{A\in \Kads} \inf_{\Sname \in \Srobs} \Exx{x\sim \Sname}{ \min_{a\in A}\disrzero{a-x} }
=
\inf_{A\in \Kads}  \Exx{x\sim \Lap}{ \min_{a\in A}\disrzero{a-x} },
\end{align*}
where $\Lap$ is the distribution on $\Ads$ with density function
\begin{align*}
    \rho_{\Lap}(x)=\frac{1}{2\epsilon} \cdot e^{-\epsilon \disrzero{x}}.
\end{align*}
\end{restatable}

To show this, given $A$ and $\Sname$, we define a potential function, and modify $A$ and $\Sname$ step by step so that the potential function decreases at each step. The potential function has discrete value, and the process stops after finite number of steps, when $\Sname$ becomes the Laplace distribution. The full proof is in the Appendix, and has the following three main steps, each of which only improves the objective while preserving differential privacy:

\begin{enumerate}
    \item We introduce an operation which converts any distribution in $\Srobs$ to a piece-wise exponential distribution.
    \item We also introduce an operation that removes some space from the real line, concentrating the points in $A$ and the mass in $\Sname$ respectively.
    \item We define a potential function based on (i) the number of pieces in the piece-wise exponential distribution and (ii) how concentrated $A$ and $\Sname$ are. We repeatedly use the operations in the first two steps as long as the potential function decreases and the expected value of $\min_{a\in A}\disrzero{a-u}$ does not increase. The procedure stops some time, and at that time, $\Sname$ becomes the Laplace distribution.
\end{enumerate}

We now present  more details for each of these steps.

\subsubsection{Operation 1: Generating Piece-wise Exponential Distributions}
Given Theorem \ref{thm:symfinal:sim}, we want to find $A\subset \real$ of size $\K$, and a distribution in $\Srobs$ whose density is $\rho(x)$, so that the expected error $\Exx{x\sim \rho}{\min_{a\in A} \disrzero{a-x} }$ is minimized. We now show that the optimal $\rho(x)$ should be \emph{piece-wise exponential}, that is, we can partition $\real$ to be several intervals $(a_i,b_i)$ or $[a_i,b_i]$ for $i=1,2,\ldots$, and for each interval, either $\rho(x)=e^{-\epsilon(x-a_i)}\rho(a_i)$ for any $x\in (a_i,b_i)$, or $\rho(x)=e^{-\epsilon(b_i-x)}\rho(b_i)$ for any $x\in (a_i,b_i)$. We have the following lemma.




  \begin{figure}
      \centering
        \begin{tikzpicture}
        \fill[clar] (0,0) rectangle (1,3);
        \fill[csma] (1,0) rectangle (3,3);
        \fill[clar] (3,0) rectangle (4.5,3);
        \fill[csma] (4.5,0) rectangle (6.5,3);
        \fill[clar] (6.5,0) rectangle (7.5,3);
        \coordinate (right) at (7.5,0);
        \coordinate (o) at (0,0);
        \coordinate (up) at (0,3);
        \coordinate (x0) at (4.5,0);
        \coordinate (s) at (2,0);
        \coordinate (t) at (5.5,0);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[<->](right)--(o)--(up);
        % here, eps=0.55
        \draw[red,samples = 1000,smooth,domain=0:7.5] plot(\x,{1.5+0.5*cos((\x-2)*1.5 r)} );
        \draw[blue,domain=0:2] plot(\x,{(1.5+0.5*cos((1-2)*1.5 r))*exp(0.55*(\x-1))} );
        \draw[blue,domain=2:3] plot(\x,{(1.5+0.5*cos((3-2)*1.5 r))*exp(-0.55*(\x-3))} );
        \draw[blue,domain=3:4.061681] plot(\x,{(1.5+0.5*cos((3-2)*1.5 r))*exp(-0.55*(\x-3))} );
        \draw[blue,domain=4.061681:4.5] plot(\x,{(1.5+0.5*cos((4.5-2)*1.5 r))*exp(0.55*(\x-4.5))} );
        \draw[blue,domain=4.5:6.027356] plot(\x,{(1.5+0.5*cos((4.5-2)*1.5 r))*exp(0.55*(\x-4.5))} );
        \draw[blue,domain=6.027356:6.5] plot(\x,{(1.5+0.5*cos((6.5-2)*1.5 r))*exp(-0.55*(\x-6.5))} );
        \draw[blue,domain=6.5:7.5] plot(\x,{(1.5+0.5*cos((6.5-2)*1.5 r))*exp(-0.55*(\x-6.5))} );
        \fill (s) circle (2pt);
        \fill (t) circle (2pt);
        \draw[decorate,decoration={brace,raise=1pt,amplitude=3pt},purple] (x0) -- (t) node[black,midway,yshift=9pt] {$\gamma$};
        \end{tikzpicture}
      \caption{Piece-wise exponential. The black dots represent numbers in $A$. The light yellow parts are~\sma~intervals, while the light blue parts are~\lar~intervals. The red function is an example original density, and the blue function is the piece-wise exponential density after applying Lemma \ref{lem:pieceexp} on the original density.}    \label{fig:pwexp}
  \end{figure}
  





\begin{lemma}   \label{lem:pieceexp}
Fix $A\in \Kads$, for any distribution in $\Srobs$ whose density function is $\rho(x)$, there is a \emph{piece-wise exponential} density function $\rho'(x)$ in $\Srobs$, such that
\begin{align*}
    \Exx{x\sim \rho'}{\min_{a\in A} \disrzero{a-x} } \leq \Exx{x\sim \rho}{\min_{a\in A} \disrzero{a-x} }.
\end{align*}
\end{lemma}
\begin{proof}
    Fix $A=(a_1,a_2,\dots,a_{\K})\in \Kads$. Let $\gamma=\Exx{x\sim \rho}{\min_{a\in A} \disrzero{a-x} }$. Define $F\defeq \cup_{i=1}^{\K}[a_i-\gamma,a_i+\gamma]$. If $x\in F$, $\min_{a\in A} \disrzero{a-x}\leq \gamma$, and  if $x\notin F$, $\min_{a\in A} \disrzero{a-x}> \gamma$. Write $F$ as the union of a finite number of disjoint intervals, so that there exists a sequence of $-\infty=t_0<t_1<\dots<t_{2m+1}=+\infty$, so that
    \begin{enumerate}
        \item $\min_{a\in A}\disrzero{a-t_i}=\gamma$ for any $0<i\leq 2m$.
        \item For any $1\leq i\leq m$ and $x\in [t_{2i-1},t_{2i}]$, $\min_{a\in A}\disrzero{a-x}\leq \gamma$.
        \item For any $0\leq i\leq m$ and $x\in (t_{2i},t_{2i+1})$, $\min_{a\in A}\disrzero{a-x}> \gamma$.
    \end{enumerate}
  
  For each odd $i$, we call $[t_i,t_{i+1}]$ a~\sma~interval since it contains at least one point in $A$. For each even $i$, we call $(t_i,t_{i+1})$ a~\lar~interval since it does not contain a point in $A$. These~\sma~intervals and~\lar~intervals form a partition of $\real$.  For $\rho(x)\in \Srobs$, we construct a function $\tilde{\rho}(x)$ as following.
  \begin{enumerate}
      \item For any~\sma~interval $[a,b]$, for any $x\in [a,b]$, let $\tilde{\rho}(x)=\min \left\{ e^{\epsilon (x-a)}\rho(a), e^{\epsilon (b-x)}\rho(b) \right\}$.
      \item For $x$ in an~\lar~interval $(a,b)$ where $a,b\in \real$, let $\tilde{\rho}(x)=\max \left\{ e^{-\epsilon (x-a)}\rho(a), e^{-\epsilon (b-x)}\rho(b) \right\}$.
      \item For~\lar~interval $(a,+\infty)$, for any $x\in (a,+\infty)$, let $\tilde{\rho}(x)=e^{-\epsilon (x-a)}\rho(a)$.
      \item For~\lar~interval $(-\infty,b)$, for any $x\in (-\infty,b)$, let $\tilde{\rho}(x)=e^{-\epsilon (b-x)}\rho(b)$.
  \end{enumerate}
  
Let $\alpha\defeq \int_{\real}\tilde{\rho}(x)dx$. We normalize by defining:
  \begin{align*}
  \rho'(x)\defeq \frac{1}{\alpha} \tilde{\rho}(x),
  \end{align*}
We can verify that $\rho'(x)\in \Srobs$. We also have
  \begin{align*}
  & \Exx{x\sim \rho'}{\min_{a\in A} \disrzero{a-x} } - \gamma   
  =   \int_{\real} \rho'(x) (\min_{a\in A} \disrzero{a-x}-\gamma) dx \\
  = & \frac{1}{\alpha} \int_{\real} \tilde{\rho}(x) (\min_{a\in A} \disrzero{a-x}-\gamma) dx   \\
  \leq &  \frac{1}{\alpha} \int_{\real} (\tilde{\rho}(x)-\rho(x)) (\min_{a\in A} \disrzero{a-x}-\gamma) dx   
  \leq  0,  
  \end{align*}
  which implies 
    \begin{align*}
        \Exx{x\sim \rho'}{\min_{a\in A} \disrzero{a-x} } \leq \Exx{x\sim \rho}{\min_{a\in A} \disrzero{a-x} }.
    \end{align*}
\end{proof}

Therefore, any $\Sname$ can be converted to a \emph{piece-wise exponential} distribution while preserving the objective and the privacy constraints.

\subsubsection{Operation 2: Space Removal}
The second important operation is removing space from a distribution. We define this as follows:

\begin{definition}[space removal]  %\label{def:removal}
  Fix $A=(x_1,x_2,\dots,x_{\K})$ and $\rho(x)\in \Srobs$. Given $a,b\in \real$ where $a<b$, if $\rho(a)=\rho(b)$, we can remove the space $[a,b)$ and splice $(-\infty,a)$ and $[b,+\infty)$ together. Formally, $\rho(x)$ becomes $\rho'(x)$ where
  \begin{align*}
      \rho'(x)\defeq
      \begin{cases}
        \alpha \cdot \rho(x), & x<a;    \\
        \alpha \cdot \rho(x+(b-a)), & x\geq a,
      \end{cases}
  \end{align*}
  and $\alpha = \left(1-\int_{a}^{b}\rho(x)dx\right)^{-1}$ is the normalizer.  Similarly, $A$ becomes $A'=(x'_1,x'_2,\dots,x'_{\K})$ where
  \begin{align*}
      x'_i\defeq
      \begin{cases}
        x_i, & x_i<a;    \\
        a, & a\leq x_i<b;    \\
        x_i-(b-a), & x_i\geq b.
      \end{cases}
  \end{align*}
  
  \end{definition}


    
  \begin{figure}[htbp]
      \centering
        \begin{tikzpicture}
        \fill[clar] (0,0) rectangle (3.5,3);
        \fill[cano] (3.5,0) rectangle (4.5,3);
        \fill[csma] (4.5,0) rectangle (7.5,3);
        \coordinate (right) at (7.5,0);
        \coordinate (o) at (0,0);
        \coordinate (up) at (0,3);
        \coordinate (s) at (2,0);
        \coordinate (t) at (5,0);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[<->](right)--(o)--(up);
        \draw[blue,domain=0:4] plot(\x,{(4.5-\x)^0.7} );
        \draw[blue,domain=4:7.5] plot(\x,{(\x-3.5)^0.7} );
        \fill (s) circle (2pt);
        \fill (t) circle (2pt);
        \end{tikzpicture}
        \begin{tikzpicture}
        \fill[clar] (0,0) rectangle (3.5,3);
        \fill[csma] (3.5,0) rectangle (6.5,3);
        \coordinate (right) at (7.5,0);
        \coordinate (o) at (0,0);
        \coordinate (up) at (0,3);
        \coordinate (s) at (2,0);
        \coordinate (t) at (4,0);
        %\draw node at ([yshift=-0.3cm]y) {$y$};
        %\draw node at ([yshift=-0.3cm]z) {$z$};
        %\draw node at ([yshift=-0.3cm]x0) {$x_0$};
        %\draw node at ([yshift=-0.3cm]s) {$s$};
        %\draw node at ([yshift=-0.3cm]t) {$t$};
        \draw[<->](right)--(o)--(up);
        \draw[blue,domain=0:3.5] plot(\x,{(4.5-\x)^0.7} );
        \draw[blue,domain=3.5:6.5] plot(\x,{(\x-2.5)^0.7} );
        \fill (s) circle (2pt);
        \fill (t) circle (2pt);
        \end{tikzpicture}
      \caption{Space removal. The blue function is the density function $\rho(x)$, and the two black dots represent numbers in $A$. We apply space removal on the purple part in the first figure, and splice the blue and yellow part. The result is the second figure.}
  \end{figure}



It can be checked that after space removal, the density function $\rho(x)$ is still in $\Srobs$.  For any $A$ and $\rho(x)\in \Srobs$, after making $\rho(x)$ \emph{piece-wise exponential} using the method in Lemma~\ref{lem:pieceexp}, either this function is already the Laplace distribution (and hence we are done) or there is some $x_0\in \real$ that is a (local) minimal point. This $x_0$ is either in a~\lar~interval or on the boundary of a~\sma~interval. So, there exists a small $\delta>0$ so that
\begin{enumerate}
    \item $\rho(x_0-t)=\rho(x_0+t)=e^{\epsilon t}\rho(x_0)$ for any $t<\delta$.
    \item $\int_{x_0-\delta}^{x_0+\delta}\rho(x)\cdot \left( \min_{a\in A} \disrzero{a-x}  -  \gamma \right) dx \geq 0$, where $\gamma\defeq \Exx{x\sim \rho}{\min_{a\in A} \disrzero{a-x} }$.
\end{enumerate}

We then remove the space $(x_0-\delta, x_0+\delta)$. Suppose $A$ and $\rho(x)$ represent the {\em piecewise exponential} signal after using the method in Lemma~\ref{lem:pieceexp}, and $A'$ and $\rho'(x)$ are values after the space removal step above. Let $\alpha \defeq \left(1-\int_{a}^{b}\rho(x)dx\right)^{-1}$. Then we have
\begin{align*}
    & \Exx{x\sim \rho'}{\min_{a\in A'} \disrzero{a-x} } - \Exx{x\sim \rho}{\min_{a\in A} \disrzero{a-x} }    \\
  = &  \int_{-\infty}^{x_0-\delta} \rho'(x) \left(\min_{a\in A'} \disrzero{a-x} - \gamma  \right) dx 
   +  \int_{x_0-\delta}^{+\infty} \rho'(x) \left(\min_{a\in A'} \disrzero{a-x}  -  \gamma  \right) dx  \\
  \leq &  \alpha \int_{-\infty}^{x_0-\delta} \rho(x) \left(\min_{a\in A} \disrzero{a-x}  -  \gamma  \right) dx 
   +  \alpha \int_{x_0+\delta}^{+\infty} \rho(x) \left(\min_{a\in A} \disrzero{a-x}   -  \gamma  \right) dx  \\
  = & - \alpha \int_{x_0-\delta}^{x_0+\delta}\rho(x)\cdot \left( \min_{a\in A} \disrzero{a-x}  -  \gamma \right) dx 
  \leq  0,  
\end{align*}
which implies $\Exx{x\sim \rho'}{\min_{a\in A'} \disrzero{a-x} } \leq \Exx{x\sim \rho}{\min_{a\in A} \disrzero{a-x} }$.

\paragraph{Repeating operations.} We can therefore perform the above two operations while preserving differential privacy and (weakly) improving the objective, as long as $\rho(x)$ has a minimal point. As mentioned above, once $\rho(x)$ has no minimal point, it is a Laplace distribution and we are done.  The only remaining part is showing that the above operations need only be applied a finite number of times before we obtain the Laplace distribution. In the Appendix, we define a discrete bounded-value potential function which strictly decreases after one step of the above process hence showing finite-time termination.  It implies that in an optimal mechanism, the distribution $\Sname$ is the Laplace distribution.


\input{ashishproof}

\subsection{Main Theorem}
Based on the above arguments, we have the main theorem.


  

\simrstepe*


%Furthermore, the optimal mechanism can be computed in closed form. Furthermore, the optimal mechanism can be computed in closed form. The optimal mechanism in a simplified setting is computed in the next section.


\iffalse%%%%%%%%%%%%%%%%
\begin{align*}
\funf{\Users}{\Ads}{\epsilon}{\K}
=
\begin{cases}
\frac{4}{\epsilon(\K +1)} , & \text{$\K$ is odd},  \\
\frac{2}{\epsilon} \log\left( 1+\frac{2}{\K} \right) , & \text{$\K$ is even},  \\
\end{cases}
\end{align*}
which is $O(1/(\epsilon \K))$. Moreover, in one of the optimal mechanisms, user $u\in \real$ sends signal $u+\eta$, where $\eta$ is drawn from the distribution with density function $\rho(x)=e^{-\epsilon \disrzero{u}{x}}/\epsilon$, and when the server receives signal $s\in \real$, it sends back $\{s+a_1, s+a_2, \dots, s+a_{\K}\}$, where
\begin{enumerate}
    \item If $\K$ is odd, let $t=(\K -1)/2$, and
    \begin{align*}
        \{a_1,\dots,a_{\K}\}=\left\{
        0, \pm \frac{2\log\left(\frac{t+1}{t}\right)}{\epsilon},
        \pm \frac{2\log\left(\frac{t+1}{t-1}\right)}{\epsilon},
        \dots,
        \pm \frac{2\log\left(\frac{t+1}{2}\right)}{\epsilon},
        \pm \frac{2\log\left(t+1\right)}{\epsilon}
        \right\}.
    \end{align*}
    \item If $\K$ is even, let $t=\K/2$, and
    \begin{align*}
        \{a_1,\dots,a_{\K}\}=\left\{
         \pm \frac{\log\left(\frac{t+1}{t}\right)}{\epsilon},
        \pm \frac{\log\left(\frac{t(t+1)}{(t-1)^2}\right)}{\epsilon},
        \pm \frac{\log\left(\frac{t(t+1)}{(t-2)^2}\right)}{\epsilon},
        \dots,
        \pm \frac{\log\left(\frac{t(t+1)}{2^2}\right)}{\epsilon},
        \pm \frac{\log\left(t(t+1)\right)}{\epsilon}
        \right\}.
    \end{align*}
\end{enumerate}
\fi%%%%%%%%%%%%%%%%%%%%%%%%

==> test-proof.tex <==
\section{Construction of the dual feasible solution to dual LP $\mathcal{E}$}\label{sec:dual-soln-construction}

In this section, we aim to construct a feasible solution to LP $\mathcal{E}$ whose objective ``arbitrarily'' approximates $\hat{f}(\epsilon,k)$ in Lemma \ref{lemma:dual_schievable}. Towards this, we first prove Claim \ref{diff_eqn_soln_claim} which shows the existence of a feasible solution $\nu(.,\vect{v}): \mathbb{R} \rightarrow \mathbb{R}$ for every $\vect{v} \in \mathbb{R}^k$ for suitably chosen feasible functions $\delta(.)$ and $\lambda(.)$ (defined in equation \eqref{eqn:nu_delta_defn}) and finally we prove Lemma \ref{lemma:dual_schievable} showing that the optimum value of LP $\mathcal{E}$ in lower bounded by $\hat{f}(\epsilon,k)$. 

%
We define functions $\lambda^{(c)}(.)$ and $\delta^{(c)}(.)$ as follows for some $\hat{\lambda}>0$ and $0<\zeta<\epsilon$.
\begin{equation}{\label{eqn:nu_delta_defn}}
    \delta^{(c)}(u) = (\zeta/2) e^{-\zeta|u|} \text{ and } \lambda^{(c)}(u) = \hat{\lambda}\cdot (\zeta/2) e^{-\zeta|u|} \text{ } \forall u \in \mathbb{R}
\end{equation}


Note that we construct these functions to find a feasible solution to LP $\mathcal{E}$ with as ``large objective'' ($\hat{\lambda}$) as possible since $\int_{u \in R} \lambda^{(c)}(u) du = \hat{\lambda}$. Towards this, for every $\vect{v} \in \mathbbm{R}^k$, we now consider the following differential equation \eqref{diff_eqn_nu} in $\hat{\nu}(.)$ with $\lambda^{(c)}(.)$ and $\delta^{(c)}(.)$ defined in equation \eqref{eqn:nu_delta_defn}  and define $v_{med} = \text{Median}(\texttt{Set}(\vect{v}))$ for the equation below. 

\begin{equation}{\label{diff_eqn_nu}}
    -\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|u-a|)\right] \delta^{(c)}(u) + \lambda^{(c)}(u) + \hat{\nu}'(u) + \epsilon |\hat{\nu}(u)| = 0 ; \text{ with  $\hat{\nu}(v_{med}) = 0$}  
\end{equation}

Observe that this equation precisely corresponds to the second constraint of LP $\mathcal{E}$ (inequality replaced by equality) with an initial value. In claim \ref{diff_eqn_soln_claim}, we show that there always exists a solution $\hat{\nu}(.)$ to \eqref{diff_eqn_nu} such that $\hat{\nu}(u)$ is non-negative for sufficiently large $u$ and non-positive for sufficiently small $u$\footnote{We may still need to prove continuity of the bounds $U(.)$ and $L(.)$ which we discuss in Lemma \ref{lemma:dual_schievable}} to satisfy the last two constraints of LP $\mathcal{E}$. 

In the next subsection, we state two technical lemmas whose proofs we defer to Section \ref{sec:proof_hat_f_claim} and \ref{sec:diff_eqn_soln_first_claim} which we use in the proof of Lemma \ref{lemma:dual_schievable} and Claim \ref{diff_eqn_soln_claim}.

% Observe by symmetry that $\mathbb{E}_{y \in \mathcal{L}_{\epsilon}(z)}\left[\min_{a \in \texttt{Set}(A)} \mathfrak{h} (||y -a ||_1)\right]$ is independent of $z$ and let us denote it by $\hat{f}(\epsilon,k)$ and thus, $\sup_{u \in \mathbb{R}} \underset{A \sim \hat{P}^{\mathcal{L}_{\epsilon}}_u}{\mathbb{E}} \left[\min_{a \in \texttt{Set}(A)} \mathfrak{h}(||u-a||_1) \right] = \hat{f}(\epsilon,k)$. 



% Clearly these set of points constructed from $\{\hat{P}^{\mathcal{L}_{\epsilon}}_u\}_{u \in \mathbb{R}}$ satisfy $\epsilon$-geographic DP and thus, $f(\epsilon,k) \leq \hat{f}(\epsilon,k)$. 
% In this section we show that the following distribution $\hat{P}^{\mathcal{L}_{\epsilon}}$ is \textit{optimal} i.e. minimises \eqref{infimization_expr} and satisfies $\epsilon$-geographic DP. We showed in the previous section (using Lemmas \ref{lemma:weak_duality_result} and Claim \ref{lemma:bounding_f}) that $\text{opt}(\mathcal{E}) \leq \text{opt}(\mathcal{O}) \leq \hat{f}(\epsilon,k)$.
% We now show that $\text{opt}(\mathcal{E}) \geq \hat{f}(\epsilon,k)$ in Lemma \ref{lemma:dual_schievable} by using Claim \ref{diff_eqn_soln_claim} to show $\hat{P}^{\mathcal{L}_{\epsilon}}$ is \textit{optimal} i.e. $\text{opt}(\mathcal{O})= {f}(\epsilon,k) = \hat{f}(\epsilon,k)$. 
\subsection{Technical claims used }
% However to prove Claim \ref{diff_eqn_soln_claim}, we require a technical Claim \ref{hat_f_claim} which we also state below and prove in Section \ref{sec:proof_hat_f_claim}.

%This claim shows that we can 

%This claim essentially states that a symmetric 

\sss{A sentence is to be written to describe the lemma}
\begin{claim}{\label{hat_f_claim}}
   Consider any vector $\vect{q} \in \mathbb{R}^k$ and consider any $v_{med} \in \mathbb{R}$ satisfying $v_{med} \geq \text{Median}(\texttt{Set}(\vect{q}))$. Then the following holds true (recall the definition of $\hat{f}(\epsilon,k)$ from equation \eqref{hat_f_defn})

   \begin{equation}
       2 \int_{v_{med}}^{\infty} \left[ \min_{a \in \texttt{Set}(\vect{q})}  \mathfrak{h}(|t-a|)\right] \left(\epsilon/2\right) e^{-\epsilon (t-v_{med})} dt\geq \hat{f}(\epsilon,k).
   \end{equation}
\end{claim}

This claim is proven in section \ref{sec:proof_hat_f_claim}. 

We now state the next claim which say that we says that there exists a solution to equation \eqref{diff_eqn_nu}. This claim states that zeros of the solution to equation \eqref{diff_eqn_nu} with negative derivative is upper bounded and states that zeros with positive derivative is lower bounded. 

\begin{claim}{\label{diff_eqn_soln_first_claim}}
    Choose any $0<\hat{\lambda} \leq \frac{\epsilon - \zeta}{\epsilon+\zeta} \hat{f}(\epsilon+ \zeta,k)$ for some $0<\zeta<\epsilon$. Then for every $\vect{v} \in \mathbbm{R}^k$, a unique $\mathcal{C}^1$ solution $\nu^{(c)}(.)$ exists to differential equation \eqref{diff_eqn_nu} satisfying the following two constraints for some constant $C$ independent of $\vect{v} \in \mathbb{R}^k$. Note that $v_{\floor{i}}$ denotes the $i^{th}$ largest component of $\vect{v}$ for every $i \in [k]$.

    \begin{itemize}
        \item $\set[\Big]{\mathfrak{u} \in \mathbb{R}: \nu^{(c)}(\mathfrak{u})=0 \text{ and } \nu^{(c)'}(\mathfrak{u}) < 0 } \text{ is upper bounded}$ by $C + v_{\floor{k}}$.
        \item $\set[\Big]{\mathfrak{u} \in \mathbb{R}: \nu^{(c)}(\mathfrak{u})=0 \text{ and } \nu^{(c)'}(\mathfrak{u}) > 0 } \text{ is lower bounded}$ by $-C + v_{\floor{1}}$.
    \end{itemize}
    
\end{claim}

The proof of this claim is given in Section \ref{sec:diff_eqn_soln_first_claim}. With these claims, we now prove the following claim \ref{diff_eqn_soln_claim} which shows that $\nu^{(c)}(.)$ is ``positive'' for sufficiently large $u$ and ``negative'' for sufficiently small $u$.
 

\subsection{Obtaining a feasible solution to LP $\mathcal{E}$}

\begin{claim}{\label{diff_eqn_soln_claim}}
        Choose $\zeta<\epsilon$ and $0< \hat{\lambda} \leq \frac{\epsilon - \zeta}{\epsilon+\zeta} \hat{f}(\epsilon+ \zeta,k)$, then equation $\eqref{diff_eqn_nu}$ has a unique $\mathcal{C}^1$ solution $\nu^{(c)}(.)$ and there exists $U, L \in \mathbb{R}$ satisfying $\nu^{(c)}(u) \geq 0 \text{ }\forall u \geq U$ and $\nu^{(c)}(u) \leq 0 \text{ } \forall u \leq L$. 
\end{claim}     

%define functions $\lambda^{(c)}(.)$ and $\delta^{(c)}(.)$ as follows.

%     $$\delta^{(c)}(u) = (\zeta/2) e^{-\zeta|u|} \text{ and } \lambda^{(c)}(u) = \hat{\lambda}\cdot (\zeta/2) e^{-\zeta|u|} \text{ } \forall u \in \mathbb{R}$$. Consider the following differential equation \eqref{diff_eqn_nu} in $\hat{\nu}(.): \mathbb{R} \rightarrow \mathbb{R}$ for every $\vect{v} \in \mathbb{R}^k$ and define $v_{med} = \text{Median}(\texttt{Set}(\vect{v}))$.
%     \begin{equation}{\label{diff_eqn_nu}}
%     -\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|u-a|)\right] \delta^{(c)}(u) + \lambda^{(c)}(u) + \hat{\nu}'(u) + \epsilon |\hat{\nu}(u)| = 0 ; \text{ with initial condition $\hat{\nu}(v_{med}) = 0$}  
% \end{equation}

    
    % Also, there exists a constant $C$ (independent of $\vect{v}$) such that \footnote{$v_{\floor{i}}$ denotes the $i^{th}$ largest element amongst the components of $\vect{v}$ for every $i \in [k]$.}




% \begin{claim}
%     Consider the following differential equation in $y(.)$ where $\lambda(.)$ is a \textit{Reinmann integrable} non-negative function with $\lambda(.)$ being monotonically increasing for sufficently large $u$.

%     \begin{equation}{\label{test_eqn}}
%         y'(x) + |y(x)| = \lambda(x)
%     \end{equation}
% Then equation \eqref{test_eqn} has an unique $\mathcal{C}^1$ solution in $y(.)$ and $\lim_{u \to \infty} y(u)$ and $\lim_{u \to -\infty} y(u)$ exist.
% \end{claim}




% We now use claim \ref{hat_f_claim} to claim \ref{diff_eqn_soln_claim}. 
% Observe that equation \eqref{diff_eqn_nu} is precisely the second constraint (inequality replaced by equality) in LP $\mathcal{E}$ for a given $\vect{v} \in \mathbb{R}^k$ and we show that there exists a solution to \eqref{diff_eqn_nu} with desired bounds $U$ and $L$ in following claim for some feasible $\delta(.)$ and $\lambda(.)$. The last statement says that zeros of the solution to equation \ref{diff_eqn_nu} with positive first derivative is upper bounded and zeros with negative first derivative is lower bounded. The last statement is slightly technical and we need it to prove the existence of continuous bounds $U(\vect{v})$ and $L(\vect{v})$. 
% \begin{claim}{\label{diff_eqn_soln_claim}}
%     For any $\vect{v} \in \mathbb{R}^k; \zeta<\epsilon$ and $0< \hat{\lambda} \leq \frac{\epsilon - \zeta}{\epsilon+\zeta} \hat{f}(\epsilon+ \zeta,k)$, define functions $\lambda^{(c)}(.)$ and $\delta^{(c)}(.)$ as follows.

%     $$\delta^{(c)}(u) = (\zeta/2) e^{-\zeta|u|} \text{ and } \lambda^{(c)}(u) = \hat{\lambda}\cdot (\zeta/2) e^{-\zeta|u|} \text{ } \forall u \in \mathbb{R}$$. Now define the following differential equation \eqref{diff_eqn_nu} in $\hat{\nu}(.): \mathbb{R} \rightarrow \mathbb{R}$ for every $\vect{v} \in \mathbb{R}^k$.
%     \begin{equation}{\label{diff_eqn_nu}}
%     -\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|u-a|)\right] \delta^{(c)}(u) + \lambda^{(c)}(u) + \hat{\nu}'(u) + \epsilon |\hat{\nu}(u)| = 0
% \end{equation}

%     Then equation $\eqref{diff_eqn_nu}$ has a $\mathcal{C}^1$ solution $\nu^{(c)}(.)$ and there exists $U, L \in \mathbb{R}$ satisfying $\nu^{(c)}(u) \geq 0 \text{ }\forall u \geq U$ and $\nu^{(c)}(u) \leq 0 \text{ } \forall u \leq L$. Also, there exists a constant $C$ (independent of $\vect{v}$) such that \footnote{$v_{\floor{i}}$ denotes the $i^{th}$ largest element amongst the components of $\vect{v}$ for every $i \in [k]$.}

    
% \end{claim}


\begin{proof}
    % Let us denote $v_{med} = \text{Median}(\texttt{Set}(\vect{v}))$ and now we construct a solution for this differential equation with the initial value point of $\hat{\nu}^{(c)}(v_{med}) = 0$. From \textit{global uniqueness and existence} condition of \textit{Cauchy-Lipschitz} theorem in \cite[Theorem 2]{existenceode}, we can show that there is a \textit{unique} solution $\hat{\nu}^{(c)}(.)$ of equation \eqref{diff_eqn_nu} satisfying this initial value condition as \textit{Lipschitz} conditions as described in \cite[Theorem 2]{existenceode} is satisfied in equation \eqref{diff_eqn_nu}. Also, observe that this function is \textit{continuously differentiable}.  
    
    
    % From Picard-Lindel Theorem for first degree ODEs in \cite{nagle2004fundamentals}, we have that there must exist some $\hat{\nu}^{(c)}(.)$ satisfying this initial value condition. Now, we show that $\lim_{u \to \infty} \hat{\nu}^{(c)}(u)$ exits and is positive using contradiction. %from the solution constructed with $\hat{\nu}^{(c)}(v_{med}) = 0$.
    
    %We prove this statement by constructing a solution starting from the initial point $u=v_{med}=\text{Median}(\texttt{Set}(\vect{v}))$. Clearly, $\hat{\nu}'(u)<0$ for $u = v_{med}^{+}$. 

    %Suppose, $\lim_{u \to \infty} \hat{\nu}^{(c)}(u) \not \geq 0$. 



    Recall from claim \ref{diff_eqn_soln_first_claim}, that there exists a unique $\mathcal{C}^1$ solution (denoted by $\nu^{(c)}(.)$) to \eqref{diff_eqn_nu}. Uniqueness and existence of the solution can be shown from \textit{global uniqueness and existence} condition of \textit{Cauchy-Lipschitz} theorem in \cite[Theorem 2]{existenceode} as \textit{Lipschitz} conditions as described in \cite[Theorem 2]{existenceode} is satisfied in equation \eqref{diff_eqn_nu}.

    We first prove the following equation \eqref{eqn:non-existence2} which states that there cannot be an open interval in a subset of $[v_{med},\infty)$ where $\nu^{(c)}(.)$ is non-negative in \ref{proof-eqn:non-existence2} and use this statement to prove the main claim in \ref{proof-claim}.

    \begin{equation}{\label{eqn:non-existence2}}
            \set[\Big]{ \mathfrak{u} \in \mathbbm{R}\given \nu^{(c)}(u) \leq 0 \text{ }\forall u>\mathfrak{u}} = \phi
    \end{equation} 

    \begin{pfparts}
        
    \item[\namedlabel{proof-eqn:non-existence2}{Proof of equation \eqref{eqn:non-existence2}}.]
    
    % satisfying 

    % \begin{equation}{\label{eqn:existence1}}
    %         % \set[\Big]{ \mathfrak{u} \in \mathbbm{R}\given \not\exists u_0 \in [\mathfrak{u},\infty) \textrm{ s.t. } \left(\nu^{(c)}(u_0)=0 \text{ and } \nu^{(c)'}(u_0) < 0 \right)} \neq \phi
    %         \set[\Big]{\mathfrak{u} \in \mathbb{R}: \nu^{(c)}(\mathfrak{u})=0 \text{ and } \nu^{(c)'}(\mathfrak{u}) < 0 } \text{ is upper bounded by $C + v_{\floor{k}}$}. 
    % \end{equation}. 

    % We now show that it also satisfies equation \ref{eqn:non-existence2} that we describe below. 


    % We now prove the following 2 statements in equations \eqref{eqn:existence1} and \eqref{eqn:non-existence2} to prove there exists $U$ s.t. $\nu^{(c)}(u) \geq 0 \text{ }\forall u>U$. Informally, equation \eqref{eqn:existence1} says that points $u \in \mathbb{R}$ where $\nu^{(c)}(u)$ crosses from positive to negative is upper bounded. and equation \ref{eqn:non-existence2} says that there there cannot exist an \textit{open interval} where $\nu^{(c)}(.)$ is non-positive.  We prove the equations \eqref{eqn:existence1} and \eqref{eqn:non-existence2} in \ref{proof-eqn:existence1} and \ref{proof-eqn:non-existence2} respectively for some constant $C$ independent of $\vect{v}$.

    % \begin{itemize}
    %     \item \begin{equation}{\label{eqn:existence1}}
    %         % \set[\Big]{ \mathfrak{u} \in \mathbbm{R}\given \not\exists u_0 \in [\mathfrak{u},\infty) \textrm{ s.t. } \left(\nu^{(c)}(u_0)=0 \text{ and } \nu^{(c)'}(u_0) < 0 \right)} \neq \phi
    %         \set[\Big]{\mathfrak{u} \in \mathbb{R}: \nu^{(c)}(\mathfrak{u})=0 \text{ and } \nu^{(c)'}(\mathfrak{u}) < 0 } \text{ is upper bounded by $C + v_{\floor{k}}$}. 
    % \end{equation}
    %     \item \begin{equation}{\label{eqn:non-existence2}}
    %         \set[\Big]{ \mathfrak{u} \in \mathbbm{R}\given \nu^{(c)}(u) \leq 0 \text{ }\forall u>\mathfrak{u}} = \phi
    %     \end{equation} 
    % \end{itemize}

    % We show that these 2 statements imply the existence of $U\in \mathbbm{R}$ s.t. $\nu^{(c)}(u)\geq 0 \text{ }\forall u\geq U$. Suppose $\mathfrak{u}$ satisfies the condition in equation \eqref{eqn:existence1}. Now let us denote the set of all the closed intervals in $[v_{med},\infty)$, where $\nu^{(c)}(.)$ is non-negative by $\mathcal{I}^{pos}$\footnote{We can construct such intervals as $\nu^{(c)}$ is \textit{continuously differentiable} and there does not exist an interval where $\nu^{(c)}$ is zero.}. Now observe, that the equation \eqref{eqn:existence1} implies that \textit{upper bound} of every interval in $\mathcal{I}^{pos}$ must be upper bounded by $\mathfrak{u}$. This implies the existence of an open interval where $\nu^{(c)}(.)$ is non-negative or an open interval where $\nu^{(c)}(.)$ is non-positive. However equation \eqref{eqn:non-existence2} implies that there can not exist an open interval where $\nu^{(c)}(.)$ is non-positive and thus, we show that there exists an open interval where  $\nu^{(c)}(.)$ is non-negative proving the desired statement in Claim \ref{diff_eqn_soln_claim}.


    % \begin{pfparts}
    %         \item[\namedlabel{proof-eqn:existence1}{Proof of equation \eqref{eqn:existence1}}.]
    %         \textit{We first prove that $\lim_{u \to \infty} \mathfrak{h}(u)> \hat{\lambda}$}. First observe from Claim \ref{hat_f_claim}) (substituting $\epsilon$ by $\epsilon+\zeta$) that

    % \begin{align*}
    % & \int_{v_{med}}^{\infty} \left[ \min_{a \in \texttt{Set}(\vect{q})}  \mathfrak{h}(|t-a|)\right] \left(\epsilon+ \zeta\right) e^{-(\epsilon+\zeta) (t-v_{med})} dt\geq \hat{f}(\epsilon+\zeta,k).\\
    % \implies & \int_{v_{med}}^{\infty} \left[ \min_{a \in \texttt{Set}(\vect{q})}  \mathfrak{h}(|t-a|)-\hat{f}(\epsilon+\zeta,k)\right] (\epsilon+\zeta) e^{-(\epsilon+\zeta) (t-v_{med})} dt \geq 0
    % \end{align*}

    % This, implies that for some $t > v_{med}$ s.t. $\left[ \min_{a \in \texttt{Set}(\vect{q})}  \mathfrak{h}(|t-a|)-\hat{f}(\epsilon+\zeta,k)\right]>0$ and since, we know $\mathfrak{h}(.)$ is monotonic, we can argue that $\lim_{u \to \infty} \mathfrak{h}(u)> \hat{f}(\epsilon+\zeta,k)> \hat{\lambda}$. Let us denote the the smallest $u$ s.t. $\mathfrak{h}(u) > \hat{\lambda}$ by $\mathfrak{u}^s$. Now observe for $u>(v_{\floor{k}}+ \mathfrak{u}^s)$, $\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|u-a|)\right]\delta^{(c)}(u) - \lambda^{(c)}(u)$ is non-negative.

    % Suppose there exists $u_0 \in [v_{\floor{k}}+ \mathfrak{u}^s,\infty)$ satisfying, $\nu^{(c)}(u_0)= 0$ and $\nu^{(c)'}(u_0)<0$ thus, $\nu^{(c)'}(u_0)+\nu^{(c)}(u_0)<0$ , thus contradicting the fact that $\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|u-a|)\right]\delta^{(c)}(u) - \lambda^{(c)}(u)>0$ is non-negative in $u \in [v_{\floor{k}}+ \mathfrak{u}^s,\infty)$. Thus, we show that there does not exist $u_0 > v_{\floor{k}}+ \mathfrak{u}^s$ satisfying $\nu^{(c)}(u_0)= 0$ and $\nu^{(c)'}(u_0)<0$ thus proving the desired statement, since $\mathfrak{u}^s$ is a constant independent of $\vect{v}$.

    % \item[\namedlabel{proof-eqn:non-existence2}{Proof of equation \eqref{eqn:non-existence2}}.]

    We now assume the \textit{contradictory} statement that there exists $u^{\max} \in \mathbbm{R}$ s.t. $\hat{\nu}^{(c)}(u)\leq 0$ for all $u>u^{\max}$. We consider the smallest such $u^{\max}$ and clearly, from continuity $\hat{\nu}^{(c)}(u^{\max}) = 0$.  

    % We first show that the limit $\lim_{u \to \infty} \hat{\nu}^{(c)}(u)$ exists. Observe that for sufficiently large $u$,\\ $\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|u-a|)\right] = \mathfrak{h}(|u-v_{\floor{k}}|)$ and thus, $\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|u-a|)\right] \delta^{(c)}(u) - \lambda^{(c)}(u)$ has a fixed sign (positive or negative) for sufficiently large $u$ and thus, $\hat{\nu}^{(c)}(u)$ is monotonic for sufficiently large $u$ and the limit must exist. We first show that $\lim_{u \to \infty} \hat{\nu}^{(c)}(u) \geq 0$. 

   % We now start with the contradictory statement that $\lim_{u \to \infty} \hat{\nu}^{(c)}(u) < 0$. Now, consider the smallest $u^{\max}$ s.t. $\hat{\nu}^{(c)}(u)<0$ for all $u>u^{\max}$ and clearly, from continuity $\hat{\nu}^{(c)}(u^{\max}) = 0$. 

    Thus, the solution to the differential equation in $[u^{\max},\infty)$ may be given by $\hat{\nu}^{(c)}(u) \\ = \left(\int_{u^{\max}}^{u} \left[-\lambda^{(c)}(t) +\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|t-a|) \right]\delta^{(c)}(t) \right] e^{-\epsilon t} dt\right)e^{\epsilon {u}}$

However, since $\hat{\nu}^{(c)}(u)$ is negative in $[u^{\max},\infty)$, we have

\zhihao{In (12), is it possible that the left side equals to 0?}

\sss{No, it is not possible that left side equals zero as it cannot be identically zero for $[u_{max},\infty)$ since the functions are continuous. This would imply that $-\lambda^{(c)}(t) +\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|t-a|) \right]\delta^{(c)}(t)$ is zero in $[u_{max},\infty)$ implying, $\mathfrak{h}(|t-a|)=\hat{\lambda}$ which is a contradiction since, $\lim_{u \to \infty} \mathfrak{h}(u) > \hat{\lambda}$ as shown in proof of Claim \ref{diff_eqn_soln_first_claim}}

\begin{align}
    & \int_{u^{\max}}^{\infty} \left[-\lambda^{(c)}(t) +\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|t-a|) \right]\delta^{(c)}(t) \right] e^{-\epsilon t} dt <0\\
    \implies & \int_{u^{\max}}^{\infty} \left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|t-a|) \right] \left(\frac{{\zeta}}{2}\right) e^{-{\zeta}|t|} (\epsilon/2)e^{-\epsilon t} dt < \int_{u^{\max}}^{\infty} \lambda^{(c)}(t) (\epsilon/2)e^{-\epsilon t}dt \label{curr_eqn}
\end{align}


We now consider two exhaustive cases and treat them separately $u^{max} > 0$ and $u^{max}<0$. We denote $q_i=v_i+v_{med}-u^{max} \forall i \in [k]$ and $\vect{q} = [q_1, q_2, \ldots, q_k]$

\textit{Case a}: Let us first consider the case where $u^{max}>0$. We thus get from equation \eqref{curr_eqn}

\begin{align}
    \overset{(a)}{\implies} & e^{-(\epsilon+{\zeta})(u^{\max}-v_{med})}. \int_{v_{med}}^{\infty} \left[\min_{\substack{a \in \texttt{Set}(\vect{q})}} \mathfrak{h}(|t-a|) \right] \left(\frac{{\zeta}}{2}\right) e^{-{\zeta}t} (\epsilon/2)e^{-\epsilon t} dt < (1/4)\hat{\lambda} e^{-(\epsilon+{\zeta})u^{\max}} \left(\frac{\epsilon{\zeta}}{\epsilon+{\zeta}}\right)\\
    \implies & 2\int_{v_{med}}^{\infty} \left[\min_{\substack{a \in \texttt{Set}(\vect{q}) }}\mathfrak{h}(|t-a|) \right]((\epsilon+{\zeta})/2)e^{-(\epsilon + {\zeta}) t} dt <\hat{\lambda}e^{-(\epsilon+{\zeta})v_{med}} \\
    {\implies} & 2\int_{v_{med}}^{\infty} \left[\min_{\substack{a \in \texttt{Set}(\vect{q}) }}\mathfrak{h}(|t-a|) \right]((\epsilon+{\zeta})/2)e^{-(\epsilon + {\zeta}) (t-v_{med})} dt <\hat{\lambda}\\
    \overset{(b)}{\implies} & \hat{f}(\epsilon+{\zeta},k) < \hat{\lambda}
\end{align}



which is a contradiction.

$(a)$ follows from the fact that $u^{\max}>0$, thus $|t|=t$ and applying change of variables. The argument for $(b)$ follows from Claim \ref{hat_f_claim}.

% Consider $\hat{f}(\epsilon,k)$ as defined in \eqref{hat_f_defn} and the clearly, the points $\vect{x}$ attaining this minimum is symmetric about $z$ and thus $z = x_{med} = \text{Median}(\vect{x})$ Thus,

% $\hat{f}(\epsilon,k) = 2.\min_{\vect{x} \in (\mathbb{R})^k} \int_{t= x_{med}}^{\infty} \left[\min_{a \in \vect{x}} \mathfrak{h}(|y-a|)\right] (\epsilon/2) e^{-\epsilon (t - x_{med})}$ and thus implying, 

% $\hat{f}(\epsilon,k) \leq 2 \int_{t= v_{med}}^{\infty} \left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|y-a|)\right] (\epsilon/2) e^{-\epsilon (t - v_{med})}$ for every $\{v_i\} \in (\mathbb{R})^k$, thus implying $(c)$

\textit{Case b}: Consider the case when $u^{max}<0$. We can thus write equation \eqref{curr_eqn}
\begin{align}
    {\implies} & \int_{u^{max}}^{0} \left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|t-a|) \right] \left(\frac{\epsilon{\zeta}}{4}\right) e^{{\zeta}t} e^{-\epsilon t} dt + \int_{0}^{\infty} \left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|t-a|) \right] \left(\frac{{\zeta}\epsilon}{4}\right) e^{-{\zeta}t} e^{-\epsilon t} dt\\
    & < \int_{u^{max}}^{0} \hat{\lambda} \left( \epsilon{\zeta}/4 \right) e^{{\zeta} t} e^{-{\epsilon} t} dt + \int_{0}^{\infty} \hat{\lambda} \left( \epsilon{\zeta}/4 \right) e^{-{\zeta} t} e^{-{\epsilon} t} dt \\
    \overset{(a)}{\implies} & e^{-(\epsilon-{\zeta}) u^{max}}\int_{v_{med}}^{v_{med}-u^{max}} \left[\min_{a \in \texttt{Set}(\vect{q})} \mathfrak{h}(|t-a|) \right] e^{-(\epsilon-{\zeta})(t-v_{med})}  dt  \\
    + & e^{-(\epsilon+{\zeta}) u^{max}}\int_{v_{med}-u^{max}}^{0} \left[\min_{a \in \texttt{Set}(\vect{q})} \mathfrak{h}(|t-a|) \right] e^{-(\epsilon+{\zeta})(t-v_{med})} dt <  \hat{\lambda}\left[ \frac{1}{(\epsilon+{\zeta})} + \frac{e^{-(\epsilon-{\zeta})u^{max}} -1}{(\epsilon - {\zeta})}\right]\\
    \overset{(b)}{\implies} & e^{-(\epsilon-{\zeta}) u^{max}}\int_{v_{med}}^{\infty} \left[\min_{a \in \texttt{Set}(\vect{q})} \mathfrak{h}(|t-a|) \right] e^{-(\epsilon+{\zeta})(t-v_{med})}  dt  < \hat{\lambda}\left[ \frac{1}{(\epsilon+{\zeta})} + \frac{e^{-(\epsilon-{\zeta})u^{max}} -1}{(\epsilon -{\zeta})}\right]\\
    {\implies} & 2e^{-(\epsilon-{\zeta}) u^{max}}\int_{v_{med}}^{\infty} \left[\min_{a \in \texttt{Set}(\vect{q})} \mathfrak{h}(|t-a|) \right] \left(\frac{\epsilon+{\zeta}}{2}\right)e^{-(\epsilon+{\zeta})(t-v_{med})} dt  < \hat{\lambda}\left[1 + \frac{(\epsilon + {\zeta})}{(\epsilon -{\zeta})} (e^{-(\epsilon-{\zeta})u^{max}} -1)\right]\\
    {\implies} & \frac{e^{-(\epsilon-{\zeta}) u^{max}}2} {\left[1 + \frac{(\epsilon + {\zeta})}{(\epsilon -{\zeta})} (e^{-(\epsilon-{\zeta})u^{max}} -1)\right]}\int_{v_{med}}^{\infty} \left[\min_{a \in \texttt{Set}(\vect{q})} \mathfrak{h}(|t-a|) \right] \left(\frac{\epsilon+{\zeta}}{2}\right)e^{-(\epsilon+{\zeta})(t-v_{med})} dt  < \hat{\lambda}\\
    \overset{(c)}{\implies} & \left(\frac{\epsilon-{\zeta}}{\epsilon+{\zeta}}\right)2\int_{v_{med}}^{\infty} \left[\min_{a \in \texttt{Set}(\vect{q})} \mathfrak{h}(|t-a|) \right] \left(\frac{\epsilon+{\zeta}}{2}\right)e^{-(\epsilon+{\zeta})(t-v_{med})} dt  < \hat{\lambda}\\
    & \overset{(d)}{\implies} \left(\frac{\epsilon-{\zeta}}{\epsilon+{\zeta}}\right) \hat{f}(\epsilon+{\zeta},k)< \hat{\lambda}
\end{align}

which is a contradiction.

$(b)$ follows from the fact that $\epsilon-{\zeta} < \epsilon+{\zeta}$ and thus, $-(\epsilon-{\zeta})u^{max} < -(\epsilon+{\zeta})u^{max}$ since $u^{max} <0$. Also, $-(\epsilon+{\zeta})(t-v_{med}) < -(\epsilon-{\zeta})(t-v_{med})$ for $t>v_{med}$.
$(c)$ follows from by infimising $\frac{e^{-(\epsilon-{\zeta}) u^{max}}} {\left[1 + \frac{(\epsilon + {\zeta})}{(\epsilon -{\zeta})} (e^{-(\epsilon-{\zeta})u^{max}} -1)\right]}$ over all $u^{max}<0$ (happens as $u^{max} \to -\infty$) and $(d)$ follows from Claim \ref{hat_f_claim}.

We thus prove equation \eqref{eqn:non-existence2} by showing contradiction under both cases.

% \begin{equation}{\label{eqn:non-existence2}}
%             \set[\Big]{ \mathfrak{u} \in \mathbbm{R}\given \nu^{(c)}(u) \leq 0 \text{ }\forall u>\mathfrak{u}} = \phi
% \end{equation} 

% Thus, we show that $\lim_{u \to \infty } \hat{\nu}^{(c)}(u) \geq 0$ from contradiction in both cases. However, since $\hat{\nu}^{(c)}(.)$ is monotonic for sufficiently large $u$, we can say that $\exists U \in \mathbb{R}$ s.t. $\hat{\nu}^{(c)}(u) \geq 0 \text{ }\forall u >U$. 



% Using a very similar argument we can also show  that $\exists L \in \mathbb{R}$ s.t. $\hat{\nu}^{(c)}(u) \leq 0 \text{ }\forall u <L$. 



% \textit{We now show the existence of bounds $U$ s.t. $\nu^{(c)}(u)\geq 0 \forall u \geq U$ by using equation \eqref{eqn:existence1} and \eqref{eqn:non-existence2} below.}

\item[\namedlabel{proof-claim}{Proof of claim \ref{diff_eqn_soln_claim}}.]


% \item[\namedlabel{proof-eqn:non-existence2}{Proof of equation \eqref{eqn:existence1}}.]
    

Observe that equation \eqref{eqn:existence1} follows from Claim \ref{diff_eqn_soln_first_claim} and equation \eqref{eqn:non-existence2} (restated below) which has been shown above.

\begin{equation}{\label{eqn:existence1}}
            % \set[\Big]{ \mathfrak{u} \in \mathbbm{R}\given \not\exists u_0 \in [\mathfrak{u},\infty) \textrm{ s.t. } \left(\nu^{(c)}(u_0)=0 \text{ and } \nu^{(c)'}(u_0) < 0 \right)} \neq \phi
            \set[\Big]{\mathfrak{u} \in \mathbb{R}: \nu^{(c)}(\mathfrak{u})=0 \text{ and } \nu^{(c)'}(\mathfrak{u}) < 0 } \text{ is upper bounded by $C + v_{\floor{k}}$}. 
\end{equation}. 

\begin{equation*}
            \set[\Big]{ \mathfrak{u} \in \mathbbm{R}\given \nu^{(c)}(u) \leq 0 \text{ }\forall u>\mathfrak{u}} = \phi
\end{equation*} 


% \begin{equation}{\label{eqn}}
    
% \end{equation}

    % We now show that it also satisfies equation \ref{eqn:non-existence2} that we describe below. 


    % We now use the following statements in equations \eqref{eqn:existence1} and \eqref{eqn:non-existence2} to prove there exists $U$ s.t. $\nu^{(c)}(u) \geq 0 \text{ }\forall u>U$. Informally, equation \eqref{eqn:existence1} says that points $u \in \mathbb{R}$ where $\nu^{(c)}(u)$ crosses from positive to negative is upper bounded. and equation \ref{eqn:non-existence2} says that there there cannot exist an \textit{open interval} where $\nu^{(c)}(.)$ is non-positive.  We prove the equations \eqref{eqn:existence1} and \eqref{eqn:non-existence2} in \ref{proof-eqn:existence1} and \ref{proof-eqn:non-existence2} respectively for some constant $C$ independent of $\vect{v}$.



% Recall that 


Let us denote the set of all the closed intervals in $[v_{med},\infty)$, where $\nu^{(c)}(.)$ is non-negative by $\mathcal{I}^{pos}$\footnote{We can construct such intervals as $\nu^{(c)}$ is \textit{continuously differentiable} and there does not exist an interval where $\nu^{(c)}$ is identically zero.}. Now observe, that the equation \eqref{eqn:existence1} implies that \textit{upper bound} of every interval in $\mathcal{I}^{pos}$ must be upper bounded by $C+ v_{\floor{k}}$. This implies the existence of an open interval where $\nu^{(c)}(.)$ is non-negative or an open interval where $\nu^{(c)}(.)$ is non-positive. However equation \eqref{eqn:non-existence2} implies that there can not exist an open interval where $\nu^{(c)}(.)$ is non-positive and thus, we show that there exists an open interval where  $\nu^{(c)}(.)$ is non-negative proving the statement in Claim \ref{diff_eqn_soln_claim} that there exists $U \in \mathbbm{R}$ s.t. $\nu^{(c)}(u)\geq 0 \forall u \geq U$. 

\end{pfparts}

Using a very similar approach, we can prove that $\nu^{(c)}(u) \leq 0$ for $u\leq L$ for some $L \in \mathbbm{R}$.
    %We first prove equation \eqref{eqn:existence1} below.

    
        

    

%    \sss{Needs to be written better with more clarity}.
    % \textit{We first show that }$\hat{\nu}^{(c)}(u)$ is monotonic for sufficiently large $u$. Observe that for sufficiently large $u$,\\ $\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|u-a|)\right] = \mathfrak{h}(|u-v_{\floor{k}}|)$ and thus, $\left[\min_{a \in \texttt{Set}(\vect{v})} \mathfrak{h}(|u-a|)\right] \delta^{(c)}(u) - \lambda^{(c)}(u)$ is positive and monotonic for sufficiently large $u$ (since $\lim_{u \to \infty}\mathfrak{h}(u) > \lambda$) and thus, $\hat{\nu}^{(c)}(u)$ is monotonic for sufficiently large $u$. 
    
    
    
%$\lim_{u \to -\infty } \hat{\nu}^{(c)}(u) \leq 0$. 

\zhihao{I didn't get the proof for $\lim_{u \to -\infty } \hat{\nu}^{(c)}(u) \leq 0$ in a short time. Maybe need to double check}


\sss{Maybe you can start with the same proof and argue suppose there exists $u^{min}$ s.t. $\hat{\nu}^{(c)}(u)>0 \forall u <u^{min}$ and now use the solution for ODE in in $(-\infty,u^{min}]$ and proceed with 2 cases like $u^{min}<0$ and $u^{min}>0$. Everything stays same just signs are reversed.}
\end{proof}


We now prove the main lemma \ref{lemma:dual_schievable} which shows that the $\hat{f}(\epsilon,k)$ is achievable by some solution in the LP $\mathcal{E}$. Observe that this feasible solution is constructed using $\delta^{(c)}(.), \lambda^{(c)}(.)$ and $\nu^{(c)}(.)$ that we defined to satisfy equation \eqref{diff_eqn_nu} and ensured positivity and negativity of $\nu^{(c)}(.)$ for ``sufficiently'' large and small $u$ respectively for every $\vect{v} \in \mathbb{R}^k$. However, we also require a technical claim \ref{claim:continuity_bounds} to prove the existence of continuous bounds $U(.)$ and $L(.)$. For sake of brevity, we state and prove it in Section \ref{sec:continuous_bounds_claim}. 


\begin{lemma}\label{lemma:dual_schievable}
     % For every $\zeta>0$, we may construct solution feasible solutions $\lambda(.)$ and $\nu(.,.)$ in the continuous LP $D$ s.t. the objective function of LP $D$ in \eqref{orig_dual} is at least $\frac{\epsilon-\zeta}{\epsilon+\zeta} \hat{f}(\epsilon+\zeta,k)$.
     $\text{opt}(\mathcal{E}) \geq \hat{f}(\epsilon,k)$
 \end{lemma}


\begin{proof}
    Recall the functions $\lambda^{(c)}(.), \delta^{(c)}(.)$ defined in \eqref{eqn:nu_delta_defn}. Also for every $\vect{v} \in \mathbb{R}^k$, we obtain a function $\nu^{(c)}(.,\vect{v})$ [solution of equation \eqref{diff_eqn_nu}] with bounds $U(\vect{v})$ and $L(\vect{v})$ satisfying $\nu^{(c)}(u,\vect{v}) \geq 0 \forall u\geq U(\vect{v})$ and $\nu^{(c)}(u,\vect{v}) \leq 0 \forall u\leq L(\vect{v})$. Now, we argue that this solution is feasible attaining an objective value of $\hat{\lambda}$ which we argue below.

    \begin{itemize}
        \item Observe that $\int_{u \in \mathbb{R}} \lambda^{(c)}(u) = \hat{\lambda}$ and $\int_{u \in \mathbb{R}} \delta^{(c)}(u) = 1$
        \item The second constraint is satisfied as $\nu^{(c)}(\vect{v},.)$ is a solution of equation \eqref{diff_eqn_nu}.
        \item Bounds $U(\vect{v})$ and $L(\vect{v})$ exist from statement in Claim \ref{diff_eqn_soln_claim}. However, the proof of continuity of $U(.)$ and $L(.)$ is slightly technical and we formally prove this in Claim \ref{claim:continuity_bounds}. Observe that all the assumptions in Claim \ref{claim:continuity_bounds} is satisfied due to results from Claim \ref{diff_eqn_soln_claim} and Claim \ref{diff_eqn_soln_first_claim}.
        
        % \footnote{This can be proven formally as follows. Denote the largest value of $u \in [\text{Median}(\texttt{Set}(\vect{v})),\infty)$ where $\nu(u,\vect{v}) = 0$ (and crosses from -ve to +ve) by ${p}(\vect{v})$ for every $\vect{v} \in \mathbb{R}^k$ [existence is guaranteed from Claim \ref{diff_eqn_soln_claim}].  Now show that $p(\vect{v})$ is \textit{continuous} in $\vect{v}$ as $\mathfrak{h}(.)$ is continuously increasing. \zhihao{could you prove it with more details? I didn't fully understand it. I am think about something like $\nu(u,v)=sin(u)/u -v$, then $p(v)$ is not continuous at $v=\pi/2$}
        % \sss{Yes, a crucial assumption is that $\nu(u,\vect{v})\geq 0 \forall u \geq U(\vect{v})$. I will prove a lemma below.}}
        \zhihao{A typo in my comment: $v=2/\pi$}
        \sss{Prove it formally in Claim \ref{claim:continuity_bounds}}
    \end{itemize}


    Now observe that the objective value of this feasible solution in $\hat{\lambda}$ and the constructed solution is feasible for any $\hat{\lambda} \leq \frac{\epsilon-\zeta}{\epsilon+\zeta} \hat{f}(\epsilon+\zeta,k)$ and $\zeta>0$. Now, since $\hat{f}(\epsilon,k)$ is continuous in $\epsilon$, choosing $\zeta$ to be ``arbitrarily'' small enables us to get obtain the objective value of the solution arbitrarily close to $\hat{f}(\epsilon,k)$ and thus, $\text{opt}(\mathcal{E}) \geq \hat{f}(\epsilon,k)$.
    
\end{proof}

